ChameleMon: Shifting Measurement Attention as Network State Changes

Flow-level network measurement is critical to many network applications. Among various measurement tasks, packet loss detection and heavy-hitter detection are two most important measurement tasks, which we call the two key tasks. In practice, the two key tasks are often required at the same time, but existing works seldom handle both tasks. In this paper, we design ChameleMon to support the two key tasks simultaneously. One key design/novelty of ChameleMon is to shift measurement attention as network state changes, through two dimensions of dynamics: 1) dynamically allocating memory between the two key tasks; 2) dynamically monitoring the flows of importance. To realize the key design, we propose a key technique, leveraging Fermat's little theorem to devise a flexible data structure, namely FermatSketch. FermatSketch is dividable, additive, and subtractive, supporting the two key tasks. We have fully implemented a ChameleMon prototype on a testbed with a Fat-tree topology. We conduct extensive experiments and the results show ChameleMon supports the two key tasks with low memory/bandwidth overhead, and more importantly, it can automatically shift measurement attention as network state changes.

==> InputFiles/author_format.tex <==
\author{Tong Yang, Gaogang xie, Yanbiao Li, Qiaobin Fu, Alex X. Liu, Qi Li, Laurent Mathy}

\numberofauthors{6}
\author{
\alignauthor
Tong Yang,Gaogang Xie*\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences (CAS), China.}\\
       \affaddr{ICT, CAS, China.}\\
       \email{yangtongemail@gmail.com, *xie@ict.ac.cn}
\alignauthor
YanBiao Li\\
       %\affaddr{College of Computer Science and Electronic Engineering, Hunan University, China}\\
       \affaddr{Hunan University, China}\\
       \email{lybmath\_cs@hnu.edu.cn}
\alignauthor
Qiaobin Fu\\
       \affaddr{ICT, CAS, China}\\
       \email{fuqiaobin@ict.ac.cn}
\and
\alignauthor Alex X. Liu\\
       \affaddr{Department of Computer Science and Engineering, Michigan State University}\\
       \email{alexliu@cse.msu.edu}
\alignauthor Qi Li\\
       \affaddr{ICT, CAS, China}\\
       \email{liqi19872006@gmail.com}
\alignauthor Laurent Mathy\\
       \affaddr{University of Liege, Belgium}\\
       \email{laurent.mathy@ulg.ac.be}
}


\author{\IEEEauthorblockN{Tong Yang\IEEEauthorrefmark{1},
Xiaoming Li\IEEEauthorrefmark{1},
Alex X. Liu\IEEEauthorrefmark{2},
Qiaobin Fu\IEEEauthorrefmark{3},
Gaogang Xie\IEEEauthorrefmark{4}}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science Department, Peking University, Beijing, China}
\IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science and Engineering, Michigan State University}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Computer Science Department, Boston University, USA}
\IEEEauthorblockA{\IEEEauthorrefmark{4}ICT, CAS, China}
}

==> NSDI2022_9/1_Intro.tex <==
\presec 
\section{Introduction} 
\postsec

%网络测量很重要,流级别测量逐渐成为工业界的共识
Network measurement provides critical statistics for various network operations, such as traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, and failure troubleshooting \cite{handigol2014know,netbouncer2019}.
% %


Recently, the emerging programmable switches inject new vitality into network measurement, and designing novel sketches for flow-level measurement capabilities on programmable switches becomes a hot topic \cite{zhang2021cocosketch,beaucoup2020,univmon2016,sketchlearn2018,huang2017sketchvisor,elastic2018}.
%need to improve
%点出硬件平台是潮流
%近来，随着可编程交换机的出现，由于其线速的特点，在可编程交换机上支持流级别测量成为了一个热点话题
%流级别测量主要可以分为两类任务：首先是最重要的丢包检测，可以直接反应应用质量，然后是一些普通任务，侧面的反应网络状态和应用质量。
%Section 2添加一个包含大量网络测量任务的表格，论述丢包是最重要的
%flow-level
%测量分为两类，一类的开销是O（流数），只有丢包和heavy-change是O（difference），这两种的理论是两类，一类容忍误差，一类不容忍误差。都很重要。两类任务往往采取不同数据结构，相比之下，丢包更重要。
%
%第一种需求，兼顾，第二种需求，elastic，正常时少测丢包。
%我们是变色龙，我们设计一个结构
%网络无丢包是heavy hitter（90%）（相关的），一些丢包是heavy hitter+every-loss （）, 疯狂丢包是heavy-loss（90%）丢包严重时只想要重要的丢包，降低代价，应该返回重要的信息，返回太多丢包浪费分析资源，降低管理难度，需要fast response(没有现有算法支持）。
%第二段最重要的网络任务是：heavy-hitter和packet loss。在网络没有丢包时，解释三个状态。随着网络变化在三个状态中灵活的转换。
%
% \ykc{Among all the flow-level measurement tasks, packet loss detection and heavy-hitter detection are considered as the most important.}

%
% This is because packet loss detection can directly characterize the application performance and user experience, while heavy-hitter detection can benefit
% %
% Specifically, when the packet losses are rare in the network, we should allocate most of the resources for heavy-hitter detection, while reserves only a small amount of resources for packet loss detection to handle the potential small burst of packet losses.
%
% \wyh{two priority level?   1) high priority. 2) low priority.}
% Flow-level measurement mainly consists of two kinds of tasks: 
% According to the measurement targets, flow-level measurement tasks can mainly be divided into two kinds: 1) normal tasks focus on normal per-flow statistics, including flow size estimation, heavy-hitter detection, entropy estimation, \etc{}, whose measurement overhead is usually related to the number of flows; 2) anomaly tasks focus on network anomalies, including packet loss detection and heavy-change detection, whose measurement overhead is usually related to the number of anomalies; 
%

%Most existing solutions often focus on either anomaly tasks or normal tasks, and our observation is that 两类
% \wyh{Flow-level measurement tasks can be divided into two kinds according to the priority:}
% 1) the \wyh{high-priority tasks}, \ie, packet loss detection, which directly characterizes application performance and network condition; 2) the \wyh{low-priority tasks} that laterally characterize application performance and network condition through approximate flow-level statistics, including flow size estimation, heavy-hitter detection, entropy estimation, \etc{}.
%自然，我们希望同时支持以上两类任务。


%这样？hao
%In flow-level measurement system, there are two key obstacles:
%
%Naturally, we hope to support both kinds of tasks simultaneously.
%
%Considering packet loss detection can directly characterize application performance and network condition, it is of the most importance in all the tasks, and we should support it first.
%
%
%  [lg;                                                                                                                                                                               ]%Aiming at the above two kinds of tasks, various solutions are proposed.
%
Among all flow-level measurement tasks, packet loss detection and heavy-hitter detection attract the most attention, which we call two \textit{key tasks}.
%
However, the two key tasks are seldom considered and supported simultaneously in one solution.
%
One reason behind is that solutions designed for packet loss detection and solutions designed for heavy-hitter detection usually differ significantly in data structures and operations.
%and therefore most solutions only support \ykc{either one}.
%但是在一个practical的network，两类任务都是要检测的。
%However, both tasks are required in a real-world scenario.

However, in practice, the two key tasks are often required at the same time, and there are only limited resources for measurement in programmable switches.
%我们需要构建一个灵活的/flexible，完备的，高效的/efficicent测量系统，可以调和这两种测量任务.
%
Therefore, the \textit{first requirement} for a practical measurement system is versatile to support the two key tasks with high accuracy using limited resources, where limited resources refer to sub-linear space complexity.
%

Based on the first requirement, the \textit{second requirement} is to pay attention to different key tasks for different network states.
% Based on the first requirement, further, the system should have different measurement attention for different network states.
% Based on the first requirement, a practical system further requires the attention to different tasks as the network state changes.
% %
% Based on the first requirement, a practical system further requires the attention on different tasks to change according to the network state.
% Based on the first requirement, a practical system further requires automatically shifting its attention between the above two tasks as network condition changes.
% Based on the first requirement, a practical system should pay different amount of attention to different tasks under different network conditions.
% Based on the required two tasks, a practical system requires shifting its attention between the above two tasks as network condition changes.
% Based on the first requirement of both tasks, a practical system requires shifting its attention between the two tasks as network condition changes.
%
% The network condition frequently changes, placing different demands on the resources for packet loss detection and heavy-hitter detection over time.
When the network state is healthy and there are only few packet losses in the network, the system should pay more attention (\eg, allocate more memory) to heavy-hitter detection.
%
When the network state is ill and there are lots of packet losses in the network, the system should pay more attention to packet loss detection, especially for those flows which experience a great number of packet losses.

% The network condition frequently changes, placing different resource demands on packet loss detection and heavy-hitter detection.
% %
% Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
% %
% Therefore, the second requirement for a practical measurement system is to self-adapt to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%加变色龙 shift focus attention 关键词。

% Meeting the above two requirement is not enough.
% %
% For example, we use a great amount resource. can meet ...
% Third...
% Besides from above two requirements, our third requirement is the high resource efficiency, \ie, high accuracy under limited resources. 
% leverage the limited resources to provide high accuracy results as much as possible
% The measurement system should leverage the limited resources to provide high accuracy results as much as possible.
% , To avoid occupying the resources for main network functions,
% In summary, it is desired to design a \ykc{comprehensive/universal/generic/versatile/multi-function}, self-adaptive, and efficient measurement system.
In summary, it is desired to design a practical measurement system with the following requirements: \textbf{[R$_{1.1}$]} \textit{versatility requirement}: supporting both packet loss detection and heavy-hitter detection simultaneously; \textbf{[R$_{1.2}$]} \textit{efficiency requirement}: achieving high accuracy with sub-linear space complexity; \textbf{[R$_{2}$]} \textit{attention requirement:} paying attention to different key tasks for different network states.

% %这样的测量系统需要三点：1）支持两类任务；2）运行时自动地调整内存以适应网络状况的变化 3）accurate。
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]

%     \item \textbf{[R1]} \textit{Comprehensiveness requirement.}
    
%     \item \textbf{[R2]} \textit{Self-adaptation requirement:}
%     The network condition inevitably changes as time elapses, placing different demands on the resources required for packet loss detection and heavy-hitter detection at different time.
%     %
%     Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
%     %
%     Therefore, the system is desired to be self-adaptive to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%     % first allocating appropriate resources for the packet loss detection to guarantee its accuracy, and then allocating the remaining resources for \ykc{other tasks}.
    
%     \item \textbf{[R3]} \textit{Efficiency requirement:}
%     \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
%     %
%     Therefore, the system is desired to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.
%     %, so as to avoid limiting the main network functions running on switches.
%     % However, it records all the IDs and frequencies of flows in a zero-error manner, and thus requires unacceptable memory overhead.
%     %
% \end{itemize}
% % Besides the above two requirements, we find the efficiency is also a key requirement of the practical measurement system.
% %
% \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
% %
% Therefore, the third requirement for a practical measurement system is to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.


% %
% In addition, the system should also be self-adaptive, and memory efficient.




% Therefore, it is desired to design a \ykc{comprehensive/universal/generic/versatile/multi-function}, self-adaptive, and efficient measurement system that meets the following three \ykc{corresponding} requirements:
% %
% %这样的测量系统需要三点：1）支持两类任务；2）运行时自动地调整内存以适应网络状况的变化 3）accurate。
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]

%     \item \textbf{[R1]} \textit{Comprehensiveness requirement:}
%     Both packet loss detection and heavy-hitter detection greatly benefit the smooth functioning/running of the network.
%     %
%     For example, packet loss detection benefits diagnosis of network failures \cite{007-2018} and service-level agreement (SLA) delivery \cite{netseer2020};
%     %
%     heavy-hitter detection benefits load balancing \cite{curtis2011devoflow,al2010hedera}, DDoS attack detection \cite{lakhina2004characterization}, and traffic engineering \cite{benson2011microte}. 
%     %
%     Therefore, the system is desired to be comprehensive, supporting both tasks simultaneously.
%     %尽管相比正常任务，异常任务更能反应应用质量以及网络状况，也因此有助于诊断网络故障，正常任务所提供的信息往往也是许多网络功能不可或缺的，例如TE，LB，counting。因此，系统被期望同时支持两类任务
    
%     \item \textbf{[R2]} \textit{Self-adaptation requirement:}
%     The network condition inevitably changes as time elapses, placing different demands on the resources required for packet loss detection and heavy-hitter detection at different time.
%     %
%     Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
%     %
%     Therefore, the system is desired to be self-adaptive to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%     % first allocating appropriate resources for the packet loss detection to guarantee its accuracy, and then allocating the remaining resources for \ykc{other tasks}.
    
%     \item \textbf{[R3]} \textit{Efficiency requirement:}
%     \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
%     %
%     Therefore, the system is desired to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.
%     %, so as to avoid limiting the main network functions running on switches.
%     % However, it records all the IDs and frequencies of flows in a zero-error manner, and thus requires unacceptable memory overhead.
%     %
% \end{itemize}
% The system should meet the following three requirements: \textbf{[R1]}, supports both anomaly and normal tasks; \textbf{[R2]}, automatically adapts to the change real-time network condition; \textbf{[R3]}, consumes only a small amount of memory/bandwidth.
% %
% First, the system should support both anomaly and normal tasks simultaneously, considering that both provide \ykc{critical statistics of interest for different applications}.%表现出应用的需要。
%考虑到交换机极其有限的资源，我们应该尽可能最大化给定的内存的利用率。当网络状况良好，丢包数量少时，我们应该最小化用于检测丢包的资源，将资源尽可能用于支持普通任务。
%Considering the 10MB-level memory in switches, typically there is only a small portion of memory 
%Second, the system should automatically adapt to the real-time network condition, considering that the network condition is changeable and places different demands on the resources/memory required for different measurement tasks at different time.
%the dynamic network condition places different demands on the memory required for the packet loss detection at different time.
%

%
%
% When the network condition is fine and only a few flows experience packet losses, which we call victim flows, the system should minimize the memory for packet loss detection, and allocate the remaining memory for other tasks.
% %
% When the network condition is poor and the given memory cannot capture all the victim flows, the system should first capture the most valuable victim flows with most of the memory, which could be victim flows with large frequency or user-specified \wyh{high-priority} flows, and we call these flows \textit{heavy-losses}.
%

%

%当网络很恶劣的时候，已有资源无法检测all-loss，我们应该主要检测最重要的丢包（heavy-loss），丢包的大流或者用户指定的高优先级流，用最有限的memory记录最有价值的信息。
%
%总而言之，我们想要一个能同时支持两类任务，自适应网络状态，且始终最大化资源利用率和支持最重要任务的测量系统。

%1.2
% 1.1 采样算法
% 1.2 sketch 算法。
% 1.3 measurement system
% 提出了很多sketch，most只能做一类，数据结构上的特点：对sketch，error changes smoothly with memory change， Lossradar直接降为0
% %
% 还有一些versatile sketch UNivmon，Elastic,FLyMon,Beaucoup，LightGuardian支持4-10没有touch丢包的问题，不好直接扩展，唯一一个两类都做的是flowradar，不满足r2，以及r3。
%Although researchers and engineers have proposed various solutions for network measurement, none of them meets the above three requirements simultaneously.
% %
%根据测量目标，我们将现有工作分为三类，我们分别讨论其中的代表工作是否满足上述三个要求。
Existing solutions can be mainly classified into three categories according to supported measurement tasks:
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]


    
    \item \textit{1) Solutions for packet loss detection:}
    Typical solutions including LossRadar \cite{lossradar2016} based on Invertible Bloom filter \cite{eppstein2011s}, NetSight \cite{handigol2014know} based on in-band network telemetry (INT), Netseer \cite{netseer2020} based on the advanced features of programmable switches, and more.
    %
    These solutions fail to meet \textbf{[R$_{1.1}$]} because they do not handle heavy-hitter detection.
    %
    
    \item \textit{2) Solutions for heavy-hitter detection:}
    These solutions are usually based on sketches, including HashPipe \cite{sivaraman2017heavy}, UnivMon \cite{univmon2016}, ElasticSketch \cite{elastic2018}, BeauCoup \cite{beaucoup2020}, and more.
    %
    %
    These solutions fail to meet \textbf{[R$_{1.1}$]} because they do not handle packet loss detection.
    % They can be classified into two kinds.
    % %
    % The first kind of solutions is designed for only heavy-hitter detection, including HashPipe \cite{sivaraman2017heavy}, PRECISION \cite{ben2018efficient}, HeavyKeeper \cite{yang2019heavykeeper}, and more.
    % %
    % Obviously, this kind of solutions fails to meet \textbf{[R$_{1.1}$]}.
    % %
    % The second kind of solutions is designed for many measurement tasks using only one sketch, including UnivMon \cite{univmon2016}, ElasticSketch \cite{elastic2018}, BeauCoup \cite{beaucoup2020}, CocoSketch \cite{zhang2021cocosketch}, FlyMon \cite{zheng2022flymon}, and more.
    % %
    % % To support as many tasks as possible, the second kind of solutions manage to design one sketch for many measurement tasks, 
    % %
    % However, this kind of solutions does not handle packet loss detection, and thus fails to meet \textbf{[R$_{1.1}$]}.
    
    
    
    
    
    
    \item \textit{3) Solutions for both tasks:}
    These solutions support both tasks by recording exact IDs of all flows, including FlowRadar \cite{flowradar2016}, OmniMon \cite{omnimon2020}, Counter Braids \cite{lu2008counter}, and more.
    %
    % The first kind of solutions supports both tasks with low memory/bandwidth overhead through packet sampling, including Everflow \cite{everflow2015}, Netflow \cite{netflow2004}, sFlow \cite{sflow2001}, and more.
    % %
    % However, this kind of solutions only measures sampled packets, and inevitably suffers from poor accuracy in packet loss detection.
    %
    %
    %
    However, recording exact IDs of all flows requires memory/bandwidth overhead linear with the number of flows.
    %
    Therefore, these solutions fail to meet \textbf{[R$_{1.2}$]}.
    %
    % However, it records all the IDs and frequencies of flows in a zero-error manner, and thus requires unacceptable memory overhead.
    %
    %When it cannot record all the flows within the memory constraint, it fails to support any task
    
    
    % However, the data structures for anomaly tasks and those for normal tasks are \ykc{usually} heterogeneous, and thus the combination can hardly reconfigure its memory flexibly to adapt to real-time network condition.
    %
    % \wyh{However, the combination cannot flexibly adapt to real-time network condition, because the data structures of different kinds of solutions are usually heterogeneous, and thus different solutions cannot share the resources at run-time when the resources required for different measurement tasks change.}
    % 这两类solution同时部署时，因为结构不同无法runtime共享，适应实时网络。
    
    % \bbb{Solutions for anomaly tasks:}
    % %不满足both tasks
    
    % \bbb{Solutions for normal tasks:}
    
    
    % \item \textbf{Probing} solutions \cite{?} send tailored probes to measure the status/condition of switches or links, and thus have no visibility to flow-level statistics.
    
    % \item \textbf{Sampling} solutions \cite{?} collect desired statistics from packets or flows selected by random sampling or rule matching, and thus cannot cover all flows in both high-priority and low-priority tasks.
    % %

    
    
    %  \item \textbf{Programmable switch assisted} solutions \cite{?} leverage the advanced features and capabilities of programmable switches to monitor specific network events. 
    %  %
    %  Among them, Netseer is most relevant to our design goal, which achieves full coverage of packet loss detection.
    %  %
    %  However, Netseer is not designed for low-priority tasks.
     
     
    %  \item \textbf{Sketch-based} solutions collect desired flow-level statistics by recording every packet in compact probabilistic data structures, namely \textit{sketches}.
    %  %
    %  Existing sketches could be mainly classified into two kinds: 1) Online and fast sketches that tolerate the error caused by hash collisions and can report queries at any time; 2) Offline and accurate sketches that eliminate the error caused by hash collisions through decoding.
    %  %
    %  The first kind of sketches \cite{?} are typically designed for low-priority tasks that only require approximate flow-level statistics, while the second kind of sketches \cite{?} are typically designed for packet loss detection that require zero-error estimation of flow size change across switches.
    %  %
    %  FlowRadar \cite{?}, the only sketch that supports both high-priority and low-priority tasks, requires unacceptable memory overhead as it records the IDs and sizes of all flows in a zero-error manner.
     
    %  \item \textbf{In-band} solutions carry desired statistics in packet headers, and thus suffer from trade-off between measurement granularity and bandwidth overhead.
    %  %
    %  Among them, LightGuardian makes a good trade-off by compressing packet-level statistics into novel sketches, measuring flow-level statistics with low bandwidth overhead.
    %  %INT
    %  However, LightGuardian does not record flow IDs, and thus can hardly support tasks relying on flow IDs, such as packet loss detection and heavy-hitter detection, without the assistance of end-hosts.

%第一段是总起，overview，claim一遍好处。一段
%key design，key idea，key technique 两段 （变色龙 architecture/framework/philosophy)
%补充段 没提的创新，理论，系统
%主要实验结果（可选）
%key contribution
     
\end{itemize}

%In summary, no existing solution meets the three requirements.%做不了的本质原因是异构性，这导致A+B也不行
%现有算法做不了，除了第三类，前两类不能解决，flowradar这类需要所有的ID和counter，总space的开销超过了完美哈希表所需要的空间，linear space complexity，我们追求sublinear，其中一种是A+B，A+B可以做到sublinear不同构
In summary, the first two categories of solutions cannot meet \textbf{[R$_{1.1}$]} due to their limited measurement capabilities, and the third category of solutions cannot meet \textbf{[R$_{1.2}$]} due to their linear space complexities.
%
A naive solution meeting both \textbf{[R$_{1.1}$]} and \textbf{[R$_{1.2}$]} is to combine the first two categories of solutions: choosing one solution in each category to detect heavy-hitters (HHs for short) and packet losses, respectively.
%
% For example, the solution uses LossRadar for packet loss detection and uses Elastic Sketch for heavy-hitter detection.
%这个问题很challenge
%提r1 r2的全称
However, such a combination fails to achieve \textbf{[R$_{2}$]} on programmable switches. 
%
The reason behind is that the data structures and operations of different categories of solutions usually differ significantly\footnote{For example, LossRadar \cite{lossradar2016} records the IDs and existences of packets using XOR operation and addition, while HashPipe \cite{sivaraman2017heavy} records the IDs and sizes of flows using comparison, substitution, and addition.},
% \footnote{To support packet loss detection that requires zero-error estimation of flow size changes across switches, the first category of sketching algorithms chooses to eliminate hash collisions through decoding.
% %
% In contrast, to support heavy-hitter detection tolerates limited error, the second category of sketching algorithms chooses to embrace hash collisions and select the estimation with least collisions to minimize error.
% %
% Therefore, the data structures of the two categories of sketching algorithms are inherently heterogeneous.
% %
% The first category cannot support query before decoding, while the second category supports direct query;
% %
% As memory increases, the error of the first category sharply decreases around a sharp threshold, while the error of the second category decreases smoothly.}
and therefore the solutions in different categories can only utilize their resources allocated at compile time, which prohibits flexible allocation of memory resources between packet loss detection and heavy-hitter detection.
%
Therefore, the naive solution cannot pay attention to different key tasks for different network states.
%
%一类加法和替换，异或加法，没有替换，误差的角度一类平滑变化，一类有threshold，directly
%第一类拥抱冲突，选择冲突最弱的估计值，第二类通过复杂的解码消除冲突。这第一类支持直接查询，误差平滑变化，第二类不支持直接查询，误差有sharp threshold, sharply changes,这导致他们的数据结构有本质的不同。
%

% and thus different solutions cannot share the resources at run-time when the resources required for different measurement tasks change.

% However, the data structures of the two solutions for combination are \ykc{usually} heterogeneous, and thus they can hardly share memory with each other to adapt to real-time network condition.

% Towards the desired measurement system, a straightforward solution is to combine solutions for packet loss detection and solutions for heavy-hitter detection, so as to meet \textbf{[R1]} and \textbf{[R3]} simultaneously.
% %


%
%\ykc{To address this issue}, we design \systemname{}.%满足三个要求，做其他测量任务，实现了一个testbed，优化精度。
%

%key idea
In this paper, we design \systemname{}, which meets all the above requirements simultaneously.
%
Besides the two key tasks, \ie, packet loss detection and heavy-hitter detection, \systemname{} can support five common measurement tasks. 
%
Compared to the state-of-the-art solutions, for packet loss detection, \systemname{} reduces the memory overhead from proportional to the number of all flows (FlowRadar) or lost packets (LossRadar), to proportional to the number of flows experiencing packet losses, which we call \textit{victim flows}; 
%t
for heavy-hitter detection and the other five tasks, \systemname{} achieves at least comparable accuracy.
%
%We further build a prototype to verify the efficiency and the capability to self-adapt to real-time network condition of \systemname{}.
Our \systemname{} has a key design and a key technique as follows.


%Shift and focus the attention
The key design of \systemname{} is to shift measurement attention as network state changes, which is just like the process of the chameleons changing their skin coloration, through two dimensions of dynamics:
1) dynamically allocating memory between the two key tasks; 2) dynamically monitoring the flows of importance.
%
First, \systemname{} monitors the network state and allocates memory between the two key tasks accordingly.
%
When the network state is healthy and only a few packet losses occur in the network, \systemname{} pays most attention to and allocates most of the memory for heavy-hitter detection.
%
As the network state degrades and packet losses increase, \systemname{} gradually shifts measurement attention to and allocates more and more memory for packet loss detection.
%
Second, \systemname{} ranks the flows according to their importance, and selects those of most importance to monitor.
% For packet loss detection, 
When the network state is ill and there are too many victim flows in the network, \systemname{} selects those flows experiencing many packet losses (called \textit{heavy-losses}, HLs for short) to monitor, instead of monitoring all victim flows.
%

%写一个总结串一下这个过程。
%
Overall, when the network state continuously degrades from the healthy state to the ill state, \systemname{} runs as follows.
%
%
1) As the number of victim flows increases, \systemname{} leverages the first dimension of dynamic: gradually shifting measurement attention to and allocating more and more memory for packet loss detection;
%
2) When the victim flows are too many to monitor, \systemname{} leverages the second dimension of dynamic: focusing measurement attention on HLs while monitoring a small portion of other packet losses (named \textit{light-losses}, LLs for short) through sampling.

% Based on the number of victim flows in the network, we classify the network state into three levels, each of which is represented by one color widely used in traffic lights, \ie, green, yellow and red.
% %
% When the network state is at green level, there are only rare packet losses in network.
% %
% While it is not trivial to identify heavy-losses during monitoring, our observation is that large flows are more likely to become heavy-losses, because they can lose more packets and should lose more packets for the same network state compared to small flows.
% % %
% because small flows cannot lose too many packets due to their limited flow sizes.

% Therefore, \systemname{} selects those large victim flows to monitor to approximate the monitoring of heavy-losses.
%
% 
% For such network state, \systemname{} pays most attention to and allocates most of the memory for heavy-hitter detection, and only reserves a small amount of memory for packet-loss detection to handle the potential small burst of packet losses.
% %
% As the network state degrades and packet losses increase, the network state transitions to yellow level when the reserved memory cannot monitor all the victim flows.
% %
% For such network state, \systemname{} gradually shifts measurement attention to and allocates more and more memory for packet loss detection.
% %
% As the network state further degrades and packet losses further increase, the network state transitions to red level when \systemname{} cannot allocate more memory for packet loss detection and fails to monitor all the victim flows.
% %
% For such network state, \systemname{} gradually pays most measurement attention to and allocates most of the memory for packet loss detection, so as to monitor all the heavy-losses and a portion of light-losses.
%Similarly, for heavy-hitter detection, \systemname{} selects the largest flows to monitor when the allocated memory cannot monitor all the flows.


% %The key technique is our system is to leverage Fermat's Little Theorem theorem to devise a generic and compact data structure to support heavy hitters and packet losses simultaneously.
To realize the key design, \systemname{} incorporates a key technique, leveraging Fermat's little theorem\footnote{Fermat's little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$.} to devise a flexible data structure, namely \textit{\sketchname{}}.
%
The data structure of \sketchname{} is made of many same units.
%
\sketchname{} is dividable, additive, and subtractive, supporting packet loss detection and heavy hitter detection simultaneously.
%
%By partitioning \sketchname{} into three parts, and using each of them to support heavy-loss detection or heavy-hitter detection, \systemname{} can flexibly move the partition points to shift attention and allocate memory between the  two key tasks as network state changes.
%
By dividing \sketchname{} into three parts to detect HLs, LLs, and HHs, \systemname{} can flexibly move the division points to shift attention and allocate memory between the two key tasks as network state changes.
%
%When \systemname{} cannot monitor all victim flows, \systemname{} further partitions the part that supports packet loss detection into two parts, so as to monitor heavy-losses and light-losses separately.
%
For each incoming packet, We further use a flow classifier (TowerSketch \cite{yang2021sketchint}) to determine which of the three parts to insert.
%
For packet loss detection, owing to Fermat's little theorem, \sketchname{} only requires memory proportional to the number of victim flows. 
%
Differently, the state-of-the-art solutions require memory proportional to the number of all flows (FlowRadar) or lost packets (LossRadar).
%
%

Thanks to the visibility to per-flow size provided by Towersketch, \systemname{} can support five other common measurement tasks, including flow size estimation, heavy-change detection, flow size distribution estimation, entropy estimation, and cardinality estimation.
%
We have fully implemented a \systemname{} prototype on a testbed with a Fat-tree topology composed of 10 Tofino switches and 8 end-hosts.
%
We conduct extensive experiments and the results show that \systemname{} supports both kinds of tasks with low memory/bandwidth overhead, and more importantly, it can automatically shift measurement attention as network state changes at run-time.
%
We have released all related source codes at Github\footnote{\url{https://github.com/ChameleMoncode/ChameleMon}}.
%我们用一个分流器去决定每一个数据包应该进入三个部分中的哪一个部分。

%记录频数信息，做common tasks

% To further identify heavy-hitters and heavy-losses that are selected to monitor, \systemname{} deploys a TowerSketch \cite{yang2021sketchint} before \sketchname{}es.
%

% %
% By querying flow sizes, \systemname{} can easily identify selected flows for heavy-hitter detection using a threshold, but still has no visibility to heavy-losses that experience most severe packet losses.
%数据结构 同时支持两个   一套机制数据结构一分为二 切分点来回漂移  可任意切分 灵活切分 一部分做hh，一部分HL，切分点运行时可以自动漂移。
%可切分可合并可组合  可加可减   灵活flexible 
%


%设计一套机制，将数据结构一分为几，支持多种任务

%when the network state is excellent and there is almost no victims flows in the network, the allocated memory cannot measure all the flows and we measure those heavy flows 
%
% \sketchname{} can support both packet loss detection and heavy-hitter detection with homogeneous data structures.
% The homogeneity facilitates \systemname{} to flexibly adjust the memory size of \sketchname{} for supporting each task by simply changing its available range of index, enabling dynamic memory allocation between the two tasks at run-time.
% %
% \sketchname{} significantly reduces the memory overhead for packet loss detection from being proportional to number of flows (FlowRadar) or lost packets (LossRadar) to being proportional to number of victim flows, so as to achieve low memory/bandwidth overhead.
% %

%
% Then, \systemname{} allocates the memory for each task according to its number of selected measurement objects.
%

%
%In practice, \systemname{} always reserves a portion of memory for heavy-hitter detection to maintain minimal support for it.
%系统的key idea是通过两方面的动态调整来自动适应实时网络状态: 1) 动态地为不同地测量任务选择最有价值地测量目标 2)根据选择的目标动态地为不同测量任务分配内存
%
%这两个动态性依次作用以完成自适应
%
%首先，系统感知到需要测量的总目标的数量以及分布，包括全部流的ID以及其进入网络时频数，以及丢包流的ID以及其在网络中丢失的包数。
%
%第二，系统根据目标的重要性排序，对于流内部来说，越大越重要，对于丢包流来说，也是越大越重要，正常来说，所有的丢包流都比正常流重要。其中有一部分大流是特殊的，因为我们想始终维持对一部分大流的可见性。
%
%第三依据排序，系统根据已有的资源，利用阈值选定top-k需要测量的目标。
%第四，依据选定的测量目标向对应的任务分配内存。
%
%
%基于总内存的限制，我们选择
% The key idea of \systemname{} to adapt 
% %在runtime随着网络状态好坏的变化runtime动态自动分配给heavy-hitter和packet loss detection.
% %这个有什么好处，需要什么技术。
% The key idea of \systemname{} is to dynamically allocate memory for each task at run-time as network condition changes, which is just like the process of the chameleons changing their skin coloration.

% first sense the real-time network condition, and then properly allocate the memory for different measurement tasks based on the sensed condition, which is just like the process of the chameleons changing their skin coloration.
% %
% Based on the three \ykc{primary} colors, we coarsely classify the network condition into three states.
% %
% The first state is \textit{green}, that the network condition is excellent and the packet losses are rare\wyh{/nearly-zero}.
% %
% Under green network condition, \systemname{} uses most of the memory to support \ykc{normal} tasks with high accuracy, while reserving a fixed small amount of memory to handle the potential small burst of packet losses.
% %
% As the network condition degrades, when the reserved small memory cannot record all the flows experiencing packet losses, which we call \textit{victim flows}, it transits to the second state, \ie, \textit{yellow}.
% %
% Under yellow network condition, \systemname{} uses more than the reserved small memory to handle packet losses.
% %
% As the network condition further degrades, \systemname{} allocates more and more memory for packet loss detection until there is no more available memory, and then the network condition transits to the third state, \ie, \textit{red}.
% %
% Under red network condition, \systemname{} cannot record all the victim flows even with the maximum available memory, and thus \systemname{} shifts to record the victim flows with high priorities, which could be flows with relatively large frequency or user-specified flows, and we call these flows \textit{heavy-losses}.
%当丢包少的时候，我们用大部分的内存支持高精度的正常测量，保留少量丢包内存来应对突发的少量丢包情况。当丢包部分发现情况恶化，就扩大丢包部分的存储，保证丢包的测量，减少正常测量的资源分配，直到正常测量被压缩到最小。如果网络情况进一步恶化，对丢包部分进行进一步切分，通过阈值筛选重要的丢包流，并采样部分不重要的丢包流进行记录。通过流分布分析丢包流分布，划定heavy loss和light loss，检测出所有的heavy loss，对light loss进行采样汇报。保证测量系统在各种状态下能够用最少量的资源关注最关键的信息。

%上述设计从宏观角度上通过动态资源分配来接近设计目标，但是即使资源分配弹性合理，如果的memory efficiency不够高，仍然无法达成design goal。
%to address the challenge， 我们设计了 一个同构的sketch，他能同时支持两类任务，并且将首要关注的丢包测量开销从O包个数降低成了O丢包流。
%上述设计从宏观角度上通过动态资源分配来接近设计目标，which motivates us to design a data structures that supports both tasks, 但另一个关键问题是数据结构的memory efficiency必须足够令人满意。丢包的理想方案是xxx。。。批判loss radar，说费马 flow level开销小。同时费马还能被用于flow level支持正常任务，适用于前述框架，开销也很小。
%  
% \bbb{\systemname{} meets three technical challenges and addresses each of them.}
%
%key tech 利用费马小定理解决了。。。。
%

%

%
% The key design of \sketchname{} is to leverage Fermat's Little Theorem\footnote{Fermat's little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$.} and modular operations to overcome the counter overflows when Invertible Bloom Lookup Table \cite{goodrich2011invertibleIBLT} (IBLT) is used to recording multiple duplicate keys (\eg, <flow ID, frequency> doublet) while preserving additivity and subtractablity.
%


%
% \sketchname{} supports both tasks with internally homogeneous data structures, so as to enable dynamic memory allocation between them.
%
% \sketchname{} can achieve low memory/bandwidth overhead, because it significantly reduces the overhead for packet loss detection from proportional to number of flows (FlowRadar) or lost packets (LossRadar) to proportional to number of victim flows.
%
% \sketchname{} reduces the memory overhead for packet loss detection from proportional to number of flows (FlowRadar) or lost packets (LossRadar) to proportional to number of victim flows, so as to achieve low memory/bandwidth overhead.
%
%The second key challenge is how to handle red network condition by heavy-losses.
% The second key challenge is to identify heavy-losses under red network condition.
% %
% To address this challenge, \systemname{} deploys a simple and accurate TowerSketch \cite{yang2021sketchint} before \sketchname{}es to support online frequency query, so as to identify heavy-losses.
% %
% Considering IDs of small non-victim flows are redundant statistics for most tasks, \systemname{} uses TowerSketch to identify small flows to further reduce the memory overhead for normal tasks. 
% %

% The \textbf{second} key challenge is to identify the selected measurement objects.
% %
% To address this challenge, we propose a threshold-based identification method.
% %
% \systemname{} deploys a TowerSketch \cite{yang2021sketchint} to support online flow size query.
% %
% By querying flow sizes, \systemname{} can easily identify selected flows for heavy-hitter detection using a threshold, but still has no visibility to heavy-losses that experience most severe packet losses.
% %
% Our observation is that only large flows can become heavy-losses, because they can lose more packets and should lose more packets for the same network state compared to small flows.
% %
% Based on the observation, \systemname{} identifies heavy-losses using another threshold.
% %
% The threshold is zero when all victim flows can be measured, and gradually increases as the network state further degrades and \systemname{} must select victim flows to measure. 
% %
% In addition, with the help of TowerSketch, \systemname{} can support five more typical measurement tasks, including flow size estimation, heavy-change detection, flow size distribution estimation, entropy estimation, and cardinality estimation.
% The challenge is easy to address under green or yellow network condition as \systemname{} can record all the victim flows. 
% However, under red network condition, \systemname{} can only record heavy-losses, and thus loses the crucial visibility to the number and flow size distribution of victim flows.
% %
% Without such visibility, \systemname{} cannot shift to record all the victim flows even if the network condition is already yellow.
% % While it might be easy under green or yellow network condition as \systemname{} can record all the victim flows, under red network condition, \systemname{} can only record heavy-losses, and thus loses visibility to the number and flow size distribution of victim flows.
% %
% Therefore, under red network condition, \systemname{} reserves a small amount of memory to record a portion of low-priority victim flows (called \textit{light-losses}) through sampling, so as to complement the visibility.
% To address this challenge under red network condition, \systemname{} reserves a small amount of memory to record a portion of the victim flows with low priorities through sampling, which we call \textit{light-losses}.
%
% By synthesizing the sampled light-losses and all the heavy-losses, \systemname{} then can still has an unbiased visibility to the number and flow size distribution of victim flows even under red network condition.

%我们需要能够同时支持两类task的solution，两部分的结构需要是同构/相同的，以支持dynamic memory allocation between different measurement tasks
%challenge 2
% 绝对的低开销。 极端情况丢包很多，lossradar等开销和丢包个数正比的方案不可用。
%
%为了实现这个想法，系统需要支持dynamic memory allocation between different measurement tasks。
%为了解决这个issue，我们设计了一个同时支持两类task的solution，两部分的结构需要是同构/相同的
%2.一套精确感知网络状态的方案。
% We split the overall flow-level statistics along two dimensions as illustrated in Figure \ref{?}.
% %
% Among them, the desired statistics for supporting high-priority tasks are the IDs and frequency changes of all victim flows, while that for supporting low-priority tasks are the IDs of large flows and the frequencies of all flows.
% %
% To record the above statistics, the minimum required memory should be the sum of two parts: 1) a frequency part that is sublinear or linear to the number of flows considering that most of the required flow frequencies can be approximate; 2) an ID part that is linear to the number of large flows and victim flows considering that the required flows IDs must be exact. 
% %
% However, existing sketches can hardly support packet loss detection with memory overhead proportional to the number of victim flows.
% %
% To address this issue, we propose \sketchname{}, the key innovation of \systemname{}.
% %
% \sketchname{} leverages Fermat's little theorem and modular operations to overcome the counter overflows when IBLT is used to record duplicate keys, and preserves the additivity and subtractibility of IBLT.
% %
% In this way 
% If unfortunately the network condition degrades to a point where the given memory cannot record all the victim flows, we decide to record at the heavy-losses, while samples and records a small portion of light-losses for comprehensively sensing the real-time network condition.
% %
% In summary, their are at most 
% Towards supporting both kinds of tasks and achieving lightweight, our first design choice is to design a memory-efficient \systemname{} data plane that can record almost only the desired flow statistics at any network condition.

%
%The key innovation of \systemname{}
%
% The key innovation of \systemname{} is a novel sketch of the second kind, namely \sketchname{}.
% %
% \sketchname{} supports both high-priority and low-priority tasks to facilitate the dynamic memory allocation for adaptation to real-time network condition.
% %
% Compared to FlowRadar, \sketchname{} reduces the memory overhead required for packet loss detection from proportional to the number of flows to proportional to the number of victim flows.
% % %
% To further reduce the memory overhead required for low-priority tasks to achieve lightweight, we find the IDs of normal small flows are redundant, and deploys a sketch of the first kind before \sketchname{} to identify large flows.
% %
% \bbb{\sketchname{} design:}

%



%核心思想，设计一个同时支持一类任务和二类任务的sketch，以方便内存的动态共享。
%
% The key innovation of \systemname{} is to design a novel sketch, namely \sketchname{}.
% %
% %和flowradar类似，sketch可以支持两种任务，但相比flowradar在支持高优先级丢包检测时将开销从和流数成正比降低到了和丢包数成正比
% \sketchname{} can be flexibly divided into any number parts, each of which can support both high-priority and low-priority tasks independently, so as to facilitate the dynamic memory allocation for adaptation to real-time network condition.
% %
% Further, we deploy a flow classifier before 
% %

% Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}.
% %
% \ykc{Recently, with the increasing importance of user experience, measuring at flow level gradually becomes industrial consensus.}


% At a high level, flow-level measurement tasks can be classified into two kinds: 1) \sn{} tasks that measure flow statistics in one network node, including flow sizes\footnote{We use the terms flow sizes and flow frequencies interchangeably.}, heavy-hitters, flow size distribution, \etc{}; 2) \cn{} tasks that measure the changes of flow frequnecies across many network nodes, including packet loss detection.
% %自然，我们想要一个能支持两类任务的低开销测量能力。
% Naturally, we want measurement capabilities that supports the above two kinds of tasks simultaneously with minimum memory/bandwidth overhead, so as to avoid limiting the main network functions running on network nodes.
% %

% From the perspective of information volume, the minimum required information for supporting the first kind of tasks consists of the exact flow IDs of large flows and the approximate frequency of each flow, while that for supporting the second kind of tasks consists of the exact IDs and frequencies changes of the flows that experience packet losses, which we call \textit{victim flows} for convenience.
% %
% To record the above information, the minimum required memory should be the sum of two parts: 1) a frequency part that is sublinear or linear to the number of flows considering that most of the required flow frequencies can be approximate; 2) an ID part that is linear to the number of large flows and victim flows considering that the required flows IDs must be exact. 
% %
% We regard the memory overhead that meet the above two criteria as near-optimal, and one of our design goal is to support both kinds of tasks with near-optimal memory overhead.

% %
% With the rapid growth of bandwidth and relative stop growth of memory, while the given memory could be larger than the near-optimal memory overhead in most cases, so as to accurately measure the network, when the network condition quickly degrades and the number of victim flows drastically increases, memory overhead exceeds the limited memory, memory wastage, accuracy drop.
% %
% Therefore, The second design goal is to elastically adapt to network condition, record the most valuable information without memory wastage.
% %
% Achieving all the design goals is challenging: 1) no prior work achieves; 2) ??




==> NSDI2022_9/5_Implementation.tex <==
% \section{Implementation}
% \label{sec:shortimpl}
% We have implemented a \systemname{} prototype on Tofino 32D switches as the edge switches and a server as the central controller, with xx lines of P4 code and xx lines of C/C++ code.
% %
% Figure \ref{?} depicts the implementation logic of the \systemname{} data plane in ASIC.
% %
% In this section, we mainly lay out the parameter settings and resource usage of the \systemname{} data plane.
% %
% \textit{For other implementation details of the \systemname{} data plane and control plane, please refer to Appendix \ref{sec:protoimplementaion}.}
%






==> NSDI2023/2intro.tex <==
\presec 
\section{Introduction} 
\postsec

\begin{comment}


\title{Lightweight Network Flow Measurement over Loss Detection and Flow Sketching}

核心：轻量（低空间开销，包括存储和传输）

1.1 Background and Motivation
    P1：数据中心测量很重要。有两个关键问题需要“轻量”（低存储和传输开销）的测量解决方案：
        A、Loss Detection 丢包检测。发现丢包流ID和对应丢包数量，并且定位丢包位置。
        B、Flow Sketching 全流测量。测量全流特征（包括大流ID、频数等内容）。

1.2 Limitations of Prior Art
    
    P1：
    A、传统丢包检测方案的缺陷——空间（存储+带宽）开销大。
        传统的丢包检测有两种。
        一种是lossradar（开销与丢包个数相关）。其基于单个丢包检测，一个丢包的大流要么导致整个结构无法解码，要么占用大量空间，开销过大。本质原因是其检测粒度过细，冗余信息多（同一个流的丢包被多次重复记录）。
        一种是基于全流统计的flow radar（开销和全流规模相关），开销过大。
        我们希望通过更低量级的空间开销，发现丢包流ID和丢包个数、并定位丢包。
    
    P2：
    B、全流测量（Flow Sketching）方案在实现高准确度时不轻量
        定义高准确性：99.9999\%的流误差小于阈值（比如10 packets）。
        现有可编程交换机可实现的全流测量包括两类。
        一类是轻量但不够准确，需要通过增加哈希和数组个数来达到99.9999\%，包括 Elastic、 univmon、nitro、coco等。
        一类是准确但是不轻量，被称为编码-解码方案。包括Flow radar、黄群老师的Near zero error等。他们不轻量是因为他们对全流信息进行了无差别的压缩。
        我们希望能够同时做到准确和轻量，使用少量（3个）数组和哈希，达到高准确度。
    
1.3 Proposed Approach

    P1：
    针对上述缺陷，我们的核心思路包含两个方面：
    对应上面的问题A
        我们的approach是设计开销和“丢包流”个数相关的轻量丢包检测数据结构。“丢包流”个数远小于“丢的包数”和“全流数”，因此能显著降低开销，没有明显损失（仍然能定位丢包位置，lossradar得到的额外信息（seqnumber）并没有直接作用）。
    
    P2：
    对应上面的问题B
        我们通过大小流过滤器分离大流和小流。对于条数众多的小流，使用极高压缩率（比大流高100倍）“隐式”地编码ID，其ID在丢包发生时可以被还原，其他时间不一定。虽然失去了还原所有小流ID的能力，但是节省了10倍的存储。实现了轻量性。
        对条数较少的大流，使用“显式”的编码-解码方案记录完整ID和频数，其ID与频数任何时候均可还原，总开销可控且轻量。
    
    P3：
    算法设计难点 Technical Challenges and Solutions中的challenge
    我们需要一款数据结构，在可编程交换机上支持：a）“丢包流”个数开销的丢包检测 b）轻量且准确的流信息存储。      （这里感觉没写好，但是没想到更好的说法）
    现有的loss radar和Flow radar的数据结构不可用，其基于XOR操作的编码会导致同flowID的不同数据包相互抵消。而基于加法的IBLT，虽然简单讨论过对“多次插入”的拓展，但是并没有进行对应设计以解决相关实践问题，也没有讨论求“差集”的场景。
    
    
    P4：
    算法设计方案
    我们设计了新型数据结构Fermat IBLT，解决了多个现有技术问题并且进行了更多创新：
        1、解决溢出问题。IBLT需要累加FlowID，这很容易导致counter溢出。我们通过取模操作避免了counter溢出。取模看似损耗了信息，但我们通过费马小定理的逆元操作将FlowID准确地还原。一个64bit计数器最高支持63bit的ID编码。
        2、解决冗余指纹。我们通过无额外存储代价的校验方式：重哈希进行校验。
        3、解决长ID问题。对于13 Byte 乃至更长的 ID，我们设计了ID切片方案，使得P4可实现。
        4、动态压缩特性。数据结构支持快速折叠、合并。根据预估的丢包流数进行折叠，弹性地使用有限的带宽资源。
    
    
2 费马算法  （1页）
  这一章主要介绍单个费马算法。
    P1：总起 概括内容 idea
  2.1 数据结构设计
    P2：数据结构组成
  2.2 基本操作
    P3：插入元素/编码操作    （带例子）
    P4：解码操作
  2.3 扩展操作
    P5：两个数据结构做差
    P6：两个数据结构加和
    P7：数据结构折叠
  
3 全流测量系统（单点）   （1页~1.25页）
 3.1 Overview
    P1：总起，介绍idea大小流分流思想   画一个框图例子
 3.2 插入操作
    P2：插入流程 
        溢出的插入大流部分费马，否则插入小流部分费马
 3.3 查询操作
    P3：解码查询方式
        查询大流ID（解码大流费马）
        大流频数（大流费马+tower部分）
        小流频数（tower部分）
    P4：在线查询方式
        非精确查询：大流费马3个counter取最小+tower部分。
    P5：查询其余测量内容，cardinality、Flow Size Distribution、entropy等
 P6：discussion 讨论优势
 
4 丢包检测系统（全网）  （1页~1.5页）
 4.1 Overview 
    P1：总起 问题定义 画圈  图示画一个示意图
    P2：介绍检测流程
 4.2 部署方式与插入
    P3：sketch部署 画圈 哪些节点布sketch
    P4：插入条件 哪些流进入sketch
 4.3 汇聚
    P5：如何生成单点的数据结构 大小流费马折叠合并
    P6：信息汇聚方式（加和、解码等）
    P7：时钟同步
 4.4 定位
    trace route 定位丢包
5.实验
    
    
    
% 3 系统设计 
%  3.1 Overview
%     P1：总起，介绍idea大小流分流思想   画一个框图例子
%     P2：插入流程 
%         溢出的插入大流部分费马，否则插入小流部分费马
%  3.2 全流测量
%     P1：总起    
%     P2：解码查询方式
%         查询大流ID（解码大流费马）
%         大流频数（大流费马+tower部分）
%         小流频数（tower部分）
%     P3：在线查询方式
%         非精确查询：大流费马3个counter取最小+tower部分。
%     P4：查询其余测量内容，cardinality、Flow Size Distribution、entropy等
%     P5：discussion 讨论优势
%  3.3 丢包检测
%     P1：总起
%     P2：如何生成单点的数据结构 大小流费马折叠合并
%     P3：sketch部署 画圈 哪些节点布sketch
%     P4：插入条件 哪些流进入sketch
%     P5：信息汇聚方式（加和、解码等）
%     P6：trace route 诊断原因
\end{comment}



    
    % 关键技术-1：
    %     a）可求差。整体数据结构可以做差，并且解码。这样可以获得流级别的丢包信息。
    %     为了满足性质a（可求差）和b（高准确），我们对传统的IBLT进行了修改，使其支持多重集合的编码。我们利用了取模操作解决溢出问题，并且通过基于费马小定理的乘法逆元运算还原流ID。传统的IBLT的XOR操作并不支持同个流的多次插入。此时，数据结构支持求差，并且可以被解码。
    
    % 关键技术-2：为了满足性质c（轻量性），我们对大小流进行了分流，以取得最优的存储性价比。小流流数多，只统计频数（平均每流消耗xx Byte），大流流数少，统计ID+频数（平均每流消耗xx Byte）。
    

\subsection{Background and Motivation}
\postsec
%%
As data center networks have grown rapidly in both size and complexity, managing such networks has been a difficult task that involves a great deal of manual effort.
%
Although the concept of self-driving networking has been proposed \cite{feamster2017andJennifer}, industrial grade solutions have not emerged.
%
A self-driving networking solution should consist of three components for performance monitoring, fault diagnosis, and emergency response, respectively.
%
The performance monitoring component measures network metrics that represent the status of a network, such as packet loss, congestion, and link utilization, and detect network anomalies.
%
The monitoring component needs to be both scalable and generally applicable.
%
For scalability, for example, for a packet loss based network monitor, its communication and computation complexity need to be scalable with the number of lost packets.
%
For applicability, a network monitor should work for different types of switches.
%
Given a network anomaly, the fault diagnosis component localizes the root cause.
%
Given a root cause, the emergency response component calculates a remedy solution that can address the detected anomaly, such as changing the routing path for a flow so that an abnormal path can be avoided.

\subsection{Limitations of Prior Art}
%%
Some pioneer work has been done towards the ultimate goal of self-driving networks; however, they are either not scalable or not generally applicable.
%
LossRadar \cite{lossradar2016} captures each packet loss individually in a data center network.
%
Although LossRadar can be deployed on different types of switches, its transmission and computation overhead increases linearly with the number of lost packets, which is not scalable and thus difficult to be deployed in industry as a network anomaly may cause a large number of lost packets.
%
NetSeer \cite{netseer2020} is an in-data-plane monitor that aggregates abnormal flow events in a data plane and locates the root cause of an anomaly.
%
Although NetSeer is scalable with the number of lost packets, it can only be deployed on programmable P4 switches.

\begin{table*} [!ht]
\begin{center}
\caption{Comparison with the state-of-the-arts. In this table, $\Delta F$ refers to the number of flows with packet losses, $\Delta P$ refers to the number of packets with packet losses, $F$ refers to the number of flows, and BM refers to P4 behavior model \cite{p4behaviormodel}.}
\vspace{0.3cm}
\label{table:compare}
\begin{tabular}{|c|c|c|c|c|}
\hline

\textbf{Characteristics}&\textbf{FermatDriver}&\textbf{LossRadar}&\textbf{FlowRadar}&\textbf{NetSeer}\\
\hline
Computation/Communication complexities& $O(\Delta F)$& $O(\Delta P)$& $O(F)$ & $O(\Delta P \sim \Delta F)$\\
\hline
Independence on programmable switch & \checkmark& \checkmark& \checkmark & $\times$\\
\hline
Implementation in Tofino switch& \checkmark& BM& BM & \checkmark\\
\hline
\end{tabular}
\vspace{-0.2in}
\end{center}
\end{table*}



\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.84\linewidth]{figure/algfiggure/FermatIntroArc.jpg}
    \vspace{0.2cm}
    \caption{Design philosophy of \sketchname{}.}
    \label{algopic:insertion}
    \postfig
\end{figure}


\presub \subsection{Proposed Approach} \postsub
%
Towards the ultimate goal of self-driving networking, we build a system called \emph{FermatDriver}, which can fast and accurately monitor packet losses, detect anomalies, pinpoint root causes, and find urgent response solutions.
%
For network anomaly detection, we propose a fast, accurate, and light-weight sketch based algorithm, called \sketchname{}, for monitoring the number of lost packets, and our algorithm works for different types of switches, no matter they are programmable or not.
%
We focus on packet losses because most network anomalies (no matter caused by switch hardware, software, configuration, or protocols) experience packet losses.
%
The key novelty of our packet loss monitoring algorithm is on designing a new sketch data structure based on the Fermat's little theorem for handling register overflows and de-duplicate lost packets.
%
For root cause localization, we propose a fast machine learning scheme that can pinpoint root cause with high accuracy.
%
For emergency response, we propose different response strategies for anomalies with different levels.

%%
Our packet loss monitoring algorithm is both scalable and generally applicable.
%
For scalability, the computation and communication complexities of our algorithm are both $O(\Delta F)$, where $\Delta F$ is the number of flows with packet losses.
%
In contrast, the computation and communication complexities of the state-of-the-art packet loss monitoring algorithm, LossRadar \cite{lossradar2016}, is $O(\Delta P)$, where $\Delta P$ is the number of lost packets.
%
Note that $\Delta F$ is typically orders of magnitude smaller than $\Delta P$ as one flow may have many lost packets.
%
For applicability, our algorithm can be deployed on both programmable and non-programmable switches.

%%
We implemented our packet loss monitoring scheme, root cause localization scheme, and emergency response scheme, and deployed them on a testbed environment with 10 switches and 8 end-hosts connected with 40Gbe links in a FatTree topology.
%
%
Our experimental results show that within tens of milliseconds, the system can accurately monitor packet losses, pinpoint network faults that lead to packet losses, and automatically calculate an emergency response plan for mitigating these network faults.
%
All related codes will be open-sourced anonymously\footnote{\url{https://github.com/FermatDriver/FermatDriver}}.

==> NSDI2023/4Algorithm.tex <==




\newcommand{\classifiername}{TrimmedSketch}


\presec \section{Data Plane Design} \postsec
The key design of \systemname{} is to distinguish each kind of flow information and encode them to corresponding data structures.
%
In this section, we first propose our key algorithm, namely \sketchname{}, which works as a data-plane hash table for encoding flow information.
%
Second, we propose a flow classifier to distinguish between elephant flows and mice flows. 


\wyh{Abstract of this section. 
In the data plane, each packet goes through the classifier first and then inserts to either ElephantSketch or MiceSketch.
We design two key algorithms, \classifiername{} for classifier, and \sketchname{} for both ElephantSketch and MiceSketch.
}
% ElephantSketch and MiceSketch use the same algorithm with different sizes
% Both ElephantSketch and MiceSketch use a same data structure called .
% key algorithms in the data plane, \sketchname{} and \classifiername{}.

% As shown in Figure \ref{algopic:overview}, 
% There are three components in the data plane: 
% \begin{itemize}[itemsep=-1mm]
%     \item Classifier, which identifies the packets of elephant flows\footnote{Elephant flows are flows with sizes more than $L$ (packets).};
%     \item ElephantSketch, which compresses the elephant flows and can be decoded easily and precisely;
%     \item MiceSketch, which compresses the mice flows and can report lost flows;
% \end{itemize}
% 1) a \textbf{Classifier} for identifying the packets of elephant flows, defined as flows with sizes more than $L$ (packets); 2) an \textbf{ElephantSketch} for compressing the elephant flows, which is precise and can be decoded easily; 3) a \textbf{MiceSketch} for compressing the mice flows, which can decode the lost flows in the future.

% \bbb{Workflow:}
% Each incoming packet carries a flow ID (\eg, 5-tuple) and will first go through the flow classifier. Then, according to the classification, \ie, elephant flow or mice flow, the packet will be inserted to the sparse \sketchname{} or dense \sketchname{}, respectively.
% Periodically, the control plane reads the three components from data plane and analyzes the measurement result.
% The sparse \sketchname{} can be fast decoded in linear time, and the decoded elephant flows are all exact with nearly zero failure probability.
% Similarly, the dense \sketchname{} can decode lost flows fast and exactly.





\presub \subsection{The \sketchname{} Algorithm} \postsub

Our \textbf{key design} of \sketchname{} is to leverage Fermat’s little theorem\footnote{Fermat’s little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$.} and modulo operations to address the key bottleneck of the original IBF, \ie, the counter overflows when IBF is used to recording multiple duplicate keys (\eg, <flow ID, frequency> doublet), so as to achieve memory-efficiency and hardware friendliness, while preserving the additivity and subtractability of IBF.
%我们的核心思想是利用费马小定理与取模操作，在解决IBF在用于记录多个重复的key时的counter溢出问题以实现内存高效与硬件友好性的同时，保留IBF自身的可加可减性。
As a result, \sketchname{} can work as an efficient hash table implemented in data plane for recording flow information, and because of its additivity and subtractability, \sketchname{} also supports network-wide flow-level packet loss detection with low memory and transmission overhead (proportional to the number of victim flows).
%

In this section, we first propose the data structure of \sketchname{}, and then describe its encoding operation and decoding operation in sequence.
%如此，fermat既可以作为高效的数据平面哈希表用于记录大流信息，由于其可加可减性，fermat也支持流级别的低开销的丢包检测 (内存开销与丢包的流数成正比)


% \bbb{Key idea:}
% Our key idea is to leverage Fermat’s little theorem for insertion, addressing the problem of overflows of counters to achieve memory-efficiency and hardware friendliness.
% %
% Fermat’s little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$. We use this theorem and the modulo operation to reduce the memory overhead of recording the sum of the flow IDs of the incoming packets.
\subsubsection{Data structure}

As shown in Figure~\ref{algopic:insertion}, \sketchname{} has $d$ equal-sized bucket arrays $\mathcal{B}_1, \cdots, \mathcal{B}_d$, each of which consists of $m$ buckets.
%
Each bucket array $\mathcal{B}_i$ is associated with a pairwise-independent hash function $h_i(\cdot)$ that maps each incoming packet into one bucket in it. 
%modulo operation?
Each bucket $\mathcal{B}_i[j]$ contains two counters: 1) a \textit{count counter} $\mathcal{B}_i^{c}[j]$ recording the number of packets mapped into the bucket; 2) an \textit{ID counter} $\mathcal{B}_i^{ID}[j]$ recording the result of the sum of flow IDs of packets mapped into the bucket modulo a prime $p$.
%
Note that $p$ must be larger than any available flow ID and uniform for all buckets.
%
At initialization, we set all counters of all buckets in \sketchname{} to zero, and set $p$ to a proper value.


\subsubsection{Encoding Operation}
\bbb{Encoding/Insertion:} 
To insert an incoming packet of flow $f$, we first calculate the $d$ hash functions to locate the \textit{$d$ mapped buckets}: $\mathcal{B}_1[h_1(f)], \mathcal{B}_2[h_2(f)], \cdots, \mathcal{B}_d[h_d(f)]$. 
%
For each mapped bucket $\mathcal{B}_i[h_i(f)]$, we update it as follows.
%
First, we increment its \textit{count counter} $\mathcal{B}_i^{c}[h_i(f)]$ by one. 
%
Second, we update its \textit{ID counter} through modular addition: $\mathcal{B}_i^{ID}[h_i(f)] \gets \left(\left( \mathcal{B}_i^{ID}[h_i(f)] + f \right) \mod{p}\right)$. 

%有问题的例子
\bbb{\textit{Example:}}
 As shown in Figure~\ref{algopic:insertion}, to insert an incoming packet of flow $f = 8$, we calculate the two hash functions to get the two mapped buckets of $f$, \ie{}, $\mathcal{B}_1[2]$ and $\mathcal{B}_2[3]$. 
 For each mapped bucket, first, we increment its \textit{count counter}: $\mathcal{B}_1^{c}[2]$ is incremented to 2 and $\mathcal{B}_2^{c}[3]$ is incremented to 1.
% %
 Second, we update its \textit{ID counter}: $\mathcal{B}_1^{ID}[2]$ is updated to $\left( \mathcal{B}_1^{ID}[2] + f \right) \mod{p} = \left( 4 + 8  \right) \mod{11} = 1$, and $\mathcal{B}_2^{ID}[3]$ is updated to $\left( \mathcal{B}_2^{ID}[3] + f \right) \mod{p_2} = \left( 0 + 8 \right) \mod{11} = 8$. 
%???
%Specifically, we update $\mathcal{B}_1^{ID}[2]$ to $\left( \mathcal{B}_1^{ID}[2] + f \right) \mod{p} = \left( 4 + 8  \right) \mod{11} = 1$, and we update $\mathcal{B}_2^{ID}[3]$ to $\left( \mathcal{B}_2^{ID}[3] + f \right) \mod{p_2} = \left( 0 + 8 \right) \mod{11} = 8$. 

\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.84\linewidth]{figure/algfiggure/Fermat-Insertion-crop.pdf}
    \vspace{0.2cm}
    \caption{An encoding/insertion example of \sketchname{}.}
    \label{algopic:insertion}
    \postfig
\end{figure}


\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.95\linewidth]{figure/algfiggure/fermatArtFull.jpg}
    \vspace{0.2cm}
    \caption{\sketchname{}.}
    \label{algopic:insertion}
    \postfig
\end{figure}

\subsubsection{Decoding Operation}


%\bbb{Decoding:}
\wyh{
%decode把什么变成了什么。查询不一定要decode
}
%decoding operation有两个重要的子操作，我们首先介绍调用了这两个子操作的工作流程，然后具体介绍每个操作的细节。
The decoding operation has three important suboperations: 1) \textit{pure bucket verification} that verifies whether a non-zero bucket only records packets of a single flow (pure bucket) with small false positive rate; 2) \textit{pure bucket extraction} that extracts the single flow with certain frequency from a pure bucket; 3) \textit{flow deletion} that deletes a flow with certain frequency from \sketchname{}. 
%
Next, we first describe the workflow of the decoding operation which frequently invokes the three suboperations, and then describe their details.  

\bbb{Workflow:}
The decoding operation consists of two steps.
%
First, we traverse \sketchname{} and push each bucket into a decoding queue.
%
Second, after traversal, we pop buckets one by one from the decoding queue.
%
For each popped bucket, we perform \textit{pure bucket verification} to verify whether it is a pure bucket.
%
If so, we perform \textit{pure bucket extraction} to extract a flow and its frequency from the bucket, and then perform \textit{flow deletion} to delete the flow from \sketchname{}.
%
After \textit{flow deletion}, except the popped pure bucket, we push the other mapped buckets into the decoding queue.
%% 组织语言???
The decoding stops when the decoding queue is empty.
%
After this, if there are still non-zero buckets in \sketchname{}, the decoding is considered as failed; Otherwise, the decoding is considered as successful.
 
% First, we look for buckets that include just one flow (we call these buckets \textit{pure buckets} and call the flows inside them as \textit{pure flows}). 
% Second, for each pure bucket, we delete the flow recorded in it from our \sketchname{}. 
% We repeat these two steps until all buckets are empty (successful decoding) or no bucket is pure (failed decoding). 
% Next, we explain the details of the two steps. 
\bbb{Pure bucket verification:}
Suppose a bucket ${B}_i[j]$ only records a single flow $f^{\prime}$, it should satisfy that $\mathcal{B}_i^{c}[j] \times f^{\prime} \mod p = \mathcal{B}_i^{ID}[j]$.
%
Leveraging Fermat's little theorem, we can get that $f^{\prime} = (\mathcal{B}_i^{ID}[j] \times (\mathcal{B}_i^{c}[j])^{p-2}) \mod p$.
%
Considering that bucket ${B}_i[j]$ should be one of the $d$ mapped buckets of flow $f^{\prime}$, to verify whether ${B}_i[j]$ is a pure bucket, we propose a verification method namely \textit{rehashing verification}: We calculate the $i^{th}$ hash function to get the $i^{th}$ mapped bucket of $f^{\prime}$, \ie{}, we calculate $h_i(f^{\prime})$.
%
Then we check whether $h_i(f^{\prime})$ is equal to $j$. 
If so, we consider $\mathcal{B}_i[j]$ as a pure bucket. 
%
The rehashing verification will inevitably misjudge some impure buckets as pure buckets due to hash collisions, and the false positive rate is $\frac{1}{m}$\footnote{For any impure bucket, we can calculate its flow ID, and the flow ID could be rehashed to the same bucket with probability $\frac{1}{m}$.}.
%
we demonstrate that such false positives has little impact on decoding through discussion ($\S$~\ref{?}) and experiments ($\S$~\ref{?}).

\bbb{Pure bucket extraction:}
For every verified pure bucket ${B}_i[j]$, we calculate the flow ID $f^{\prime}$ of its recorded single flow as $f^{\prime} = (\mathcal{B}_i^{ID}[j] \times (\mathcal{B}_i^{c}[j])^{p-2}) \mod p$, and the corresponding frequency as $\mathcal{B}_i^{c}[j]$.

\bbb{Flow deletion:}
To delete flow $f^{\prime}$ with frequency $n$ from \sketchname{}, first, we locate its $d$ mapped buckets.
%
For every mapped bucket ${B}_i[h_i(f^{\prime})]$, we decrement its count counter ${B}_i^{c}[h_i(f^{\prime})]$ by $n$, and update its ID counter to $({B}_i^{ID}[h_i(f^{\prime})] - n \times f^{\prime}) \mod p$

% \bbb{1) Looking for pure buckets:} 
% We repeatedly check all buckets in \sketchname{}. 
% For each bucket $\mathcal{B}_i[t]$, we propose two methods to check whether it is pure: 
% The first method is called \textbf{ID verification}: 
% We just suppose $\mathcal{B}_i[t]$ is pure and try to get the flow ID recorded in it. 
% Specifically, we calculate $f_1^{\prime} = \left( \mathcal{B}_i^{mod_1}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_1-2} \right) \mod{p_1}$ and $f_2^{\prime} = \left( \mathcal{B}_i^{mod_2}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_2-2} \right) \mod{p_2}$. 
% Then we check whether $f_1^{\prime}$ is equal to $(f_2^{\prime} \mod{} p_1)$. 
% If not, $\mathcal{B}_i[t]$ is definitely not a pure bucket. 
% If so, let $f^{\prime} = f_2^{\prime}$, and we continue to perform the second method.
% The second method is called \textbf{Rehashing verification}: 
% We calculate the $i^{th}$ hash function to get the $i^{th}$ mapped bucket of $f^{\prime}$, \ie{}, we calculate $h_i(f^{\prime})$. 
% Then we check whether $h_i(f^{\prime})$ is equal to $t$. 
% If not, $\mathcal{B}_i[t]$ cannot be pure. 
% If so, we think $\mathcal{B}_i[t]$ is a pure bucket. 
% Note that the checking procedure has false positive error but no false negative error, \ie{}, we may consider some bucket as a pure bucket whereas it is actually not pure. 
% % Our experimental results show that this false positive rate is small and tunable ($\S$~\ref{?}). 

% \bbb{2) Deleting pure flows:} 
% After finding a pure bucket $\mathcal{B}_i[t]$, we insert the flow inside it (\ie{}, flow $f^{\prime}$) and its corresponding size $\mathcal{B}_i^{sum}[t]$ into a list. 
% Then we delete $f^{\prime}$ from our \sketchname{} by repeating the deletion operation $\mathcal{B}_i^{sum}[t]$ times. 
% Specifically, to delete a packet of flow $f$, we first get its $d$ mapped buckets by calculating hash functions. 
% Then, for each mapped bucket $\mathcal{B}_i[h_i(f)]$, we subtract one from its \textit{sum counter} $\mathcal{B}_i^{sum}[h_i(f)]$, and update its two \textit{modulo counter}s as $\mathcal{B}_i^{mod_1}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_1}[h_i(f)] - f \right) \mod{p_1}$ and $\mathcal{B}_i^{mod_2}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_2}[h_i(f)] - f \right) \mod{p_2}$. 

\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.84\linewidth]{lzr/pics/Fermat-Decoding.pdf}
    \vspace{0.2cm}
    \caption{Decoding example of \sketchname{}.}
    \label{algopic:decoding}
    \postfig
\end{figure}

\bbb{\textit{Example:}}
% As shown in Figure~\ref{algopic:decoding}, to decode \sketchname{}, we first check all buckets to look for pure buckets. 
% For bucket $\mathcal{B}_2[1]$, after \textit{ID verification} and \textit{Rehashing verification}, we consider it as a pure bucket. 
% Then we delete the pure flow inside $\mathcal{B}_2[1]$ from our \sketchname{}. 
% Specifically, we first locate the two mapped buckets $\mathcal{B}_1[2]$ and $\mathcal{B}_2[1]$, and then subtract $f^{\prime}$ from the two buckets. 

\subsubsection{Discussion}
\bbb{Memory efficiency:} 
Suppose \sketchname{} is large enough, and the pure bucket verification has negligible false positive rate.
%
The decoding operation is almost the same as that of IBLT, which is exactly the procedure used to find the 2-core of a random
hypergraph \cite{dietzfelbinger2010tight,molloy2004pure}.
%
As a result, \sketchname{} shares similar properties with IBLT, that its memory overhead is linear to the number of inserted flows, and the number of hash functions, \ie, the number of the bucket arrays $d$ is recommended to set to three to achieve the highest memory efficiency \cite{goodrich2011invertibleIBLT}.
%
Although prior work pointed out that better memory efficiency could be achieve through ??? (3 hash, 19hash) \cite{??}, we do not recommend it as it requires much more hardware resources, and thus is unfriendly to hardware.

\bbb{Handling false positives in rehashing verification:}
As discussed above, we will inevitably misjudges some impure buckets as pure buckets, then extract and delete flows that are not inserted into \sketchname{}, and finally could hinder the decoding.
%
From another point of view, such a misjudged impure bucket, or false positive, equals to insert a new flow with a negative frequency to \sketchname{}.
%
In the decoding procedure, this newly inserted flow could also be extracted and deleted from \sketchname{}, and then the impact caused by the false positive disappears.
%
To avoid the pure bucket verification repeatedly misjudge the same impure buckets, once we find that a flow has been extracted twice, whose frequency is the opposite number of each other, we add this flow and its frequency as a doublet to a blocklist.
%
Pure bucket verification will also check whether the calculated flow ID $f^{\prime}$ and its corresponding frequency is in the blocklist.
%
If so, it must not be a pure bucket.
%
In summary, the false positives cannot break the property that the memory overhead of \sketchname{} is linear to the number of inserted flows, but can slightly increase the linear coefficient.

\bbb{Time complexity of decoding:}
Suppose the pure bucket verification has negligible error rate, and the decoding is successful.
%
In the first step, we traverse \sketchname{} and push all non-zero buckets into the decoding queue, and thus the corresponding time complexity is O(dm).
%
In the second step, we perform pure bucket verification for all buckets in the queue, which consists of all the buckets pushed into in the first step, and the other mapped buckets of each extracted flow.
%
Therefore, the corresponding time complexity is O(dm)+O(flow number??).
%
Considering that the memory overhead is linear to the number of inserted flows, the overall time complexity bounded by O(dm).


\bbb{Option: fingerprint verification.}
Similar to IBLT, to reduce the false positive rate in pure bucket verification, we can perform another verification method namely fingerprint verification by adding an additional $w$-bit fingerprint counter in each bucket.
%
For each incoming packet of flow $f$, a new hash function $h_{fp}(\cdot)$ gives it a $(w-1)$ bit fingerprint $h_{fp}(f)$.
%
The fingerprint counter in each bucket records the result of the sum of fingerprints of packets mapped into the bucket modulo a prime $p_{fp}$, where $p_{fp}$ must be $w$-bit.
%
The fingerprint verification works as follows.
%
Suppose a bucket is pure.
%
Leveraging Fermat's litter algorithm, we can calculate the fingerprint of the recorded single flow in a similar way as we calculate its flow ID.
%
If the calculated fingerprint is equal to the fingerprint of the calculated flow ID, we consider the bucket passes the fingerprint verification.
%
Only buckets pass both the rehashing and fingerprint verification will be considered as pure.

\bbb{Variant: different-sized bucket arrays.}
As shown in Figure ~\ref{?}, for \sketchname{} with equal-sized bucket arrays, the linear coefficient between the number of buckets (memory overhead) and the number of inserted flows has a sharp threshold: when the linear coefficient the sharp threshold, the decoding rate sharply increases to 100\%. 
%
This property is annoying when the linear coefficient is just slightly smaller than the sharp threshold, that almost all the memory are wasted as we can hardly decode flows from \sketchname{}.
%
To address this issue, we propose a variant of \sketchname{} whose performance degrades elegantly as the memory shrinks. 
%
The only difference between the variant and the basic \sketchname{} is that the variant has different-sized bucket arrays.
%
The rationale behind is detailed as follows.
%
As shown in Figure ~\ref{?}, although the threshold for the variant to achieve 100\% decoding rate is slightly larger than the sharp threshold for the basic \sketchname{}, its decoding rate decreases much more slower when the linear coefficient decreases.


\subsubsection{Deployment}


\bbb{Motivation:} 
\wyh{A satisfactory monitoring component is with low overhead, including three aspects: 1) Storage complexity: low memory consumption in switches; 2) Communication complexity: low bandwidth overhead in transmission; 3) Computation complexity: fast processing speed in decoding. 
The three complexities of the state-of-the-art LossRadar are linear to the number of lost packets.
To achieve a much lower complexity, it is desired to devise a light algorithm whose complexities are linear to the number of flows suffering packet losses, which are called \textit{victim flows}, rather than the number of lost packets.}

\bbb{Discussion:}
We have two verification methods in decoding, but they are not necessary in some cases. When the storage/transmission/computation overhead is critical and a little higher probability of decoding failure is tolerable, we can omit the second modulo counter and the ID verification. From our strict proof and experimental result in \label{sec:algo:math}, a \sketchname{} with one modulo counter and rehashing verification can achieve a similar small probability of failed decoding as the original \sketchname{}.


\wyh{Mathematical properties. xxx xxx xxx }




\presub \subsection{Classifier} \postsub

\bbb{The Straw-man Solution.} 
To identify elephant flows, \ie, flows with $>L$ packets, a straw-man solution is to use an online flow size estimator, \eg, a Count-Min (CM) sketch, as the classifier through comparing the estimated flow size with $L$. Specifically, when choosing the CM sketch as the classifier, we insert all incoming packets to CM.
After each insertion, CM reports the renewed estimated flow size and we identify the incoming packet as an elephant one only when its new estimated flow size is greater than $L$.

% However, CM and other common flow size estimators are not memory efficient enough as a classifier, because of the following two observations:

\bbb{Weakness of the Straw-man:} The straw-man solution can be $4~16$ times more memory efficient because it consumes most memory to return specific values greater than $L$. The estimate operation of CM is to report the minimum value of multiple counter selected by hashing. If we set all counters greater than $L$ to $L+1$, the CM still report the same classification results. In practice\footnote{160Gb gateway? 98\% flow <10 pps}, $L$ is a small threshold, \eg, 10. The counters of CM and other common flow size estimators can be reduce from $32bit/64bit$ to $8bit/4bit$, which means that the classifier can be $4\sim 16$ times more memory efficient.

\subsubsection{Our Classifier--- \classifiername{}} 

\bbb{Data Structure:}
\classifiername{} consists of two arrays: array $A[\cdot]$ with $w$ x-bit-size counter and array $B[\cdot]$ with $\frac{w}{2}$ y-bit-size counter ($y>x$), \eg, $L=10, x=2, y=4,$ and $w=10000$. 
Two independent hash functions ($H_a(\cdot)$ and $H_b(\cdot)$) map each FlowID to one counter (called mapped counter) in each array, respectively. The two mapped counters of flow $f$ are $C_1=A[H_a(f) \mod{} w]$, and $C_2=B[H_b(f) \mod{} \frac{w}{2}]$. 
When one counter reaches it maximum value (\eg, $C_1=2^x-1$), it is full.

\bbb{Addition Operation:} 
The addition operation is to add the flow size of the given flow $f$ by one.
First, we calculate the hash and find the two mapped counters of flow $f$, denoted as $C_1$ and $C_2$. Then, we add $C_1$ by one if $C_1$ is not full (\ie, $C_1<2^x-1$). Finally, we add $C_2$ by one if it is not full.

\bbb{Query Operation:}
\wyh{
The query operation reports the estimated flow size of the given flow $f$.
We find the two mapped counters, \ie, $C_1$ and $C_2$, and check whether they are full. 
If one mapped counter (\eg,$C_1$) is not full, we know that the flow size of $f$ must be less than it ($C_1$), because every packet of $f$ must increment it ($C_1$) by one.
We report the minimum value as the answer among all none-full mapped counters.
If both mapped counters are full, we report infinity.
% When both $C_1$ and $C_2$ are not full, we report the minimum one among $C_1$ and $C_2$ as the estimated flow size.
% When there is one full counter among $C_1$ and $C_2$, we report the other counter as the answer.
% When both $C_1$ and $C_2$ are full, we report infinity as the answer.
}

\bbb{Processing Incoming Packets.} 
\wyh{For each incoming packet with flowID $f$, we need to classify it and update the flow size.
First we perform the query operation and its estimated flow size $\widehat{f}$. If $\widehat{f}<L$, we classify the packet into a mice one. Otherwise, we classify it into an elephant one. Then we perform the addition operation over $f$ to update the flow size. 
In implementation, the query and addition can be performed simultaneously in a pipeline.
}




% The estimated flow size is the minimum value among the reported sizes. If neither array reports size, the estimation is the maximum full counter value $2^y-1$.
% Finally, we compare the estimated flow size with $L$. If it is greater than $L$, we classify the flow into an elephant one. Otherwise, it is a mice one.

% For each incoming packet with flowID $f$, we first update its flow size and then classify it (into elephant or mice).
% Specifically, if $C_1$ is not full, \ie, $C1<2^x-1$, we increment $C_1$ by one and the first array reports $C_1$, which means that the flow size of $f$ is no greater than $C_1$. Otherwise, when $C_1$ is full, we do nothing. In the same way, we increment $C_2$, and get the reported size from the second array if it reports.
% Specifically, if $C_1$ is not full, \ie, $C1<2^x-1$, we increment $C_1$ by one and the first array reports $C_1$, which means that the flow size of $f$ is no greater than $C_1$. Otherwise, when $C_1$ is full, we do nothing. In the same way, we increment $C_2$, and get the reported size from the second array if it reports.

% \bbb{Query Operation:}
% \wyh{
% The estimated flow size is the minimum value among the reported sizes. If neither array reports size, the estimation is the maximum full counter value $2^y-1$.
% Finally, we compare the estimated flow size with $L$. If it is greater than $L$, we classify the flow into an elephant one. Otherwise, it is a mice one.}


==> NSDI2023/5SingleDevice.tex <==


\presec \section{Control Plane Design} \postsec


\wyh{We introduce how we detect flows with packet loss inside a switch and how we perform various measurement tasks.
We assume that we have read all related parts from the data plane to the control plane.
}

\subsection{Loss detection}


\wyh{What is loss detection. 
Our loss detection aims at finding all flows with lost packets in our monitor range, including their flow IDs and packet loss frequencies.
In this section, we only introduce how we find them in a single switch. We will extend the monitor range to network wide in ...
}

\wyh{Workflow. %resize->Merge->subtraction->decode  xxxx
There are four steps in loss detection:
1) Resize the larger ElephantSketch to the same size as the smaller MiceSketch.
2) Merge the resized ElephantSketch with MiceSketch, which gets a compact representation of all flows.
3) Subtract the egress Sketch from the merged sketch, which gets a representation of lost flows.
4) Finally, we decode the sketch from step 3) and get the lost flowIDs with frequencies.
We introduce the key operations as follows.
}

\bbb{Resize:}
\wyh{
A \sketchname{} with $m$ buckets can be resized to $m'=\frac{m}{k}$ buckets, where $\frac{m}{k}, k \in \mathbb{N}$, and the \sketchname{} after the resize has the same function as the original one.}
For each bucket array, we split it into $k$ segments, each with $m'$ buckets, and merge corresponding buckets. Specifically, we merge $\{\mathcal{B}_i[j], \mathcal{B}_i[j+m'], \dots, \mathcal{B}_i[j+(k-1)m]\} (j\in [0, m') ) $ from the original \sketchname{} into one bucket $\mathcal{B}'_i[j]$. 
When merging multiple buckets to one, we sum up all sum counters to get new sum counter, and sum up each kind of modulo counters respectively, \eg, ${\mathcal{B}^{mod_1}}'_i[j]=\left(\sum_{t=0}^{k-1} \mathcal{B}^{mod_1}_i[j+t\cdot m']\right) \mod{}p_1$.
After the resize, the parameters including $d$, $p_1$, and $p_2$ remain the same. Each new hash function is the original one with modulo operation: $h'_i(f) := h_i(f) \mod m'$.


\bbb{Merge:}
\wyh{
The merge operation takes a pair of \sketchnamees{}, denoted as $A$ and $B$, and reports $C=A+B$.
$A$ and $B$ must use the same parameters including the hash functions, bucket numbers, and primes. 
For each pair of corresponding buckets in the same position of the two sketches, we merge them to one bucket by summing up each field respectively.
}


\bbb{Subtraction:}
The subtraction operation takes a pair of \sketchnamees{}, denoted as $A$ and $B$, and reports $C=A-B$.
$A$ and $B$ must use the same parameters.
We perform the subtraction operation for each pair of sum counters, and perform the modulo subtraction operation for each pair of modulo counters.





\subsection{Flow Sketching}


%得到流量关键信息：大流ID 频数 小流频数

\wyh{Enhanced Decode.} We can directly decode the ElephantSketch to get Flow IDs and corresponding flow sizes as we introduced in Sec. \ref{?}. MiceSketch provides an addition verification method for the decode procedure of ElephantSketch. Specifically, to check a flowID, we can query its flow size in the classifier, and report that the ID is false when the classifier reports a flow size less than $L$. Because a flow cannot be inserted into the ElephantSketch when its estimated
flow size $\widehat{f}$ is less than $L$. In this way, we can decode the ElephantSketch with a higher certainty, and get flow IDs with corresponding flow sizes. We assume that we can successfully decode all flows in the ElephantSketch, because the successful rate is provable high.


\wyh{Flow size estimation (offline).} We perform the enhanced decode to retrieve flow IDs with flow sizes. For these flows, we add each flow size by $L$ and report the flow sizes. When the user query the size of a specific flow, we just report above result if the queried ID appeared. Otherwise, we query the classifier to get an estimated flow size and report the minimum among the estimated one and $L$.

\wyh{Flow size estimation (online).} The user may need the flow size in the data plane without relying on the control plane, in the scenario of ....
When the user query the size of a specific flow, we query the classifier to get an estimated flow size. If the estimated size is not infinity, we report it as the answer. Otherwise, we access the ElephantSketch to perform an online query without decode as follows. We access the $d$ mapped buckets and find the minimum sum counter. We report the addition of the minimum counter and $L$.

\wyh{Heavy hitter detection.} To detect heavy flows whose flow size is greater than $L$, we just perform the enhanced decode to retrieve flow IDs with flow sizes. We are sure that no heavy flows is missed. If the user wants to eliminate the false flow ID of non-heavy flows, we just drop all IDs whose flow sizes is no greater than $L$. 
 

\bbb{Heavy change detection:}
reporting every flow whose size varies more than a pre-defined threshold $\Delta_c$ in two consecutive time windows.
%
For every edge switch, we set \ykc{the filter threshold to $\Delta_c$.}
%
Similarly, we can acquire all heavy hitters in two consecutive time windows.
%
For every heavy hitter, we query its flow sizes in the two windows, and then calculates the difference.
%
if the absolute value of the difference is larger than $\Delta_c$, we report it as a heavy change.


\bbb{Flow size distribution estimation:} 
estimating the distribution of flow sizes in a time window. 
%
After each round of collection, for every edge switch, we first estimate the distribution of the TowerSketch deployed in it by applying the basic MRAC algorithm \cite{kumar2004data} to each counter array of the TowerSketch.
%
Then, we sum it with the distribution of the flows decoded from \ykc{the heavy part of \sketchname{}}.
%
Finally, we sum up the distribution of all edge switches to estimate the flow size distribution of the given network.

\bbb{Entropy estimation:} 
estimating the entropy of flow sizes in a time window.
%
With the estimation of flow size distribution, we can then estimate the entropy as $-\sum \left ( n_i \cdot \frac{i}{N}\log{\frac{i}{N}} \right )$, where $n_i$ is the number of flows with size of $i$, and $N = \sum ( i \cdot N_i)$. 

\bbb{Cardinality estimation:} 
estimating the number of flows in a time window.
%
After each round of collection, for every edge switch, we apply linear counting algorithm to the bottom array of the Towersketch deployed in it to estimate the number of flows, as the bottom array has the most counters.
%
Then, we sum up the number of flows of all edge switches as the result.




==> NSDI2023/6NetworkWide.tex <==
\presec 
\section{\systemname{} Deployment} 
\postsec
There is still a small gap between the designs of data plane and control plane described above and a operational measurement system, as they do not address the key issue: how to support persistent measurement in a endless timeline.
%
In this section, first, we propose the extensions to the designs of data plane and control plane, so that \systemname{} can operate as a measurement system in a single switch.
%
%
Then, we propose a network-wide deployment strategy, applying \systemname{} to a more realistic scenario.
%We first introduce how to collect sketches to suppor persistent measurement, then introduce how to query the collected sketches.

\subsection{Single-switch \systemname{}}
%一个测量系统应该解决以下两个问题：如何支持周期性的测量，以保证测量结果的及时性；如何采集
%
\bbb{Data plane extension:}
Control plane needs to periodically collect sketches from data plane and clean them to support persistent measurement.
%
%
However, both the two operations need time, and thus inevitably collide with the normal packet insertion process.
%
The collision will seriously degrade the performance of loss detection task that requires zero-error statistics.
%
%
To address this issue, we decide to add a periodically flipping 1-bit timestamp in Ingress to split the timeline into consecutive equal-sized measurement windows, and add an additional copy of sketches in data plane for rotation.
%
%
Each value of the 1-bit timestamp (0/1) corresponds to a distinct set of sketches.
%
Every incoming packet will be marked with the value of the timestamp, and then the packet will be inserted to the corresponding set of sketches in the switch pipeline.
%
In this way, sketches in Ingress and Egress can agree on the boundary of measurement windows, avoiding the error caused by the misalignment of windows\footnote{Suppose there are ten packets in every measurement window. If a packet is mistaken for belonging to the next window, this packet will be considered as lost in the measurement results of the current window.}.

\bbb{Control plane extension:}
Every time the timestamp flips, for sketches in Ingress, no packet will be inserted to the set of sketches corresponding to the previous timestamp, and thus control plane can instantly collect and clean them.
%
However, for sketches in Egress, after the timestamp flips, the packets marked with the previous timestamp could still be inserted to that set of sketches.
%
That is because there are buffers between Ingress and Egress, and packets may queue in the buffers.
%
Therefore, before collecting and cleaning sketches in Egress, control plane must wait an additional time longer than the queuing delay.
%
Considering that the buffer sizes of DCN switches are at 10MB-level \cite{zeng2019congestion}, with 40Gb link speed, the queuing delay is at 1ms-level in most cases.
%
To handle the queuing delay, we set the additional time to 2ms, and the length of measurement windows to 10ms in the implementation of single-switch \systemname{} ($\S$~\ref{?}).
%
%考虑到blabla，这个排队时间最长为xxms,那么翻转时间最多为xxxms。

\section{Network-wide \systemname{}} \postsec
Compared to measuring a single switch, measuring a network is a more realistic application scenario.
%
Aiming at this, we propose a generic deployment strategy for networks of any scale and any topology.
%
Our strategy only require edge switches to support data plane deployment, because they can capture all the traffic that enters and leaves the network, which is enough for all measurement tasks.
%
Further, we slightly modify designs of data plane and control to adapt them to network-wide measurement.
%全流
%For tasks A, edge switches can support them as they can capture all traffic enter
%
The corresponding modifications are detailed as follows.
%

\bbb{Data plane modifications:} 
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=0pt,partopsep=0pt]
    
    \item \textit{Inserting specific packets:}
    For network-wide \systemname{}, edge switches are only responsible for packets enters or leave the network.
    %
    Therefore, as shown in Figure \ref{?}, for every edge switch, only the packets entering the network will be inserted into the sketches in Ingress, and the packets leaving the network will be inserted into the sketches in Egress.
    %
    %
    
    \item\textit{Aligning measurement windows:}
    Similar to single-switch \systemname{}, sketches in Ingress and Egress should agree on the boundary of measurement windows to avoid error.
    %
    Therefore, every packet must carry the 1-bit timestamp from the switch where it enters the network to the switch where it leaves the network, so as to indicate which set of sketches it should be inserted to
    %
    To address this issue, for every edge switch, it colors the unused bit\footnote{As pointed by RFC 8321 (AM-PM) \cite{fioccola2018alternate}, the unused bit could be the last reserved bit of the Flag field in IPv4 header.} in the packet header of every packet enters the network with the 1-bit timestamp.
\end{itemize} 


\bbb{Control plane modifications:}

\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=0pt,partopsep=0pt]
\item \textit{Collecting sketches:}
    Similar to single-switch \systemname{}, for every edge switch, once the 1-bit timestamp flips, control plane can instantly collect the set of sketches corresponding to the previous timestamp in Ingress.
    %
    Differently, for sketches in Egress, we cannot collect them until all packets carrying the previous timestamp leave the network.
    %
    Therefore, there must be time synchronization between edge switches, so as to ensure that their timestamps flip at roughly the same time.
    %
    Then, control plane can find opportunities to collect sketches in Egress.
    %
    Further, the length of measurement window must be longer than the longest time that a packet can stay in the network, and much larger than the time synchronization precision.
    %
    We set it to 100ms in the implementation of network-wide \systemname{} implementation ($\S$ ~\ref{?}).
    
    \item\textit{Provide queries:}
    \systemname{} needs to synthesize collected sketches from all edge switches to provide queries.
    %
    For per flow tasks, for any flow, we query the sketches from the switch where it enters the network through the same strategy as described in Section \ref{?}.
    %
    For large flow tasks, we first query the sketches from every edge switch through the same strategy as described in Section \ref{?}, and then sum up the results.
    %
    For loss tasks, .... 
\end{itemize} 

\presec
\subsection{Discussion}
\bbb{Supported number of lost flows:}
% \presub \section{\systemname{} Overview TBR} \postsub
% %
% The overview of our system \systemname{} is shown in Figure \ref{pic:overview}.
% %
% \systemname{} deploys multiple pairs of our \sketchnamees{} inside and between the switches, to monitor the flow-level packet losses in the key forwarding point.
% %
% Each switch in the data center network communicates with the central controller periodically to transmit all the internal \sketchnamees{} to the central controller after each monitoring period.
% %
% The central controller decodes the flow-level packet loss events in key forwarding points according to the corresponding paired \sketchnamees{}, and diagnoses the root cause of packet losses through trained machine learning models.
% %
% Finally, the controller calculates emergent response plans for mitigating the identified network faults.

% \begin{figure}[htbp!]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{0cm}
%     \prefig
%     \centering  
%     \includegraphics[width=0.995\linewidth]{lzr/pics/Fermat_workflow.pdf}
%     \vspace{-0.2cm}
%     \caption{\systemname{} Overview.}
%     \label{pic:overview}
%     \postfig
% \end{figure}

% %%
% \noindent
% \textbf{Monitoring.}
% %
% Our \systemname{} monitors packet loss events in the key forwarding point (such as physical links, and switch queues) by deploying a pair of \sketchnamees{} on the upstream and downstream of this point.
% %
% The sketch on each forwarding point records all the packets that pass through the point.
% %
% Thus, for each packet from a source to a destination, if it is dropped at some point along the way, then this packet must be recorded only at all the upstream points from the source to the dropping point, and must not be recorded at all the downstream points from the dropping point to the destination; if this packet is not dropped, then it must be recorded at all sketches deployed along the path from the source to the destination.
% %
% \systemname{} deployed at the central controller periodically collects all these \sketchnamees{}.
% %
% To identify all the packets that may get lost at a switch or a link, \systemname{} ``subtracts'' the downstream \sketchname{} from the upstream \sketchname{}, and decodes the result to obtain the set of all packets lost at this point.






% \presec
% \subsection{Placing \sketchnamees{}}
% \postsec
% \label{sec:algo:encode}
% Placing a pair of \sketchnamees{} can detect the victim flows in the path between them. With proper placement strategy, the monitoring component can achieve full coverage of the network, capturing victim flows with accurate location information.
 


 
% \presec
% \subsubsection{Where to Place \sketchnamees{}}
% \postsec
% \label{sketchplace}
% A systematic placement strategy of \sketchnamees{} provides the ability to pinpoint where the flows lose their packets, \ie, in which switch or which link the loss happens.
% % An important requirement for the placement of \sketchnamees{} is the ability to pinpoint where the flows lose their packets, \ie, in which device or which link the loss happens.

% \bbb{LossRadar's placement.}
% LossRadar \cite{lossradar2016} divides the network into individual long paths.
% Each path starts just after the stage in the upstream switch that selects the egress port, and ends before the stage in the downstream switch that selects the egress port. 
% % LossRadar \cite{lossradar2016} divides the network into individual paths, each of which starts just after the upstream switch selects the output port and ends where the downstream switch selects the output port. 
% %
% For each path, LossRadar places an upstream meter at its beginning and a downstream meter at its end. 
% For example, in Figure \ref{algopic:placement}, Switch C is an upstream switch and Switch D is a downstream switch. The path starts from the upstream meter to the downstream meter. 

% \bbb{LossRadar's shortcoming.}
% Similar to LossRadar, our monitoring component can also place \sketchnamees{} as LossRadar.
% However, this placement suffers two shortcomings. First, as LossRadar has no visibility to further location information, it can hardly distinguish intra-switch/inter-switch packet losses. 
% %Though LossRadar has root cause analyzer, for example, it can hardly distinguish intra-switch packet loss caused by random drop specific to one port or inter-switch packet loss caused by bent fiber, because these two types of loss show no difference in LossRadar. 
% %
% Second, the paths start at ToR (Top of Rack) switches and end at end-hosts are not well considered. For these paths, because there are only upstream meters, all the victim flows in these paths cannot be detected.

% \bbb{\systemname{}'s placement.}
% We propose our placement strategy that overcomes these shortcomings by placing additional \sketchnamees{} to further divide the long paths in LossRadar. As shown in Figure \ref{algopic:placement}, to avoid these two shortcomings, for each path, our monitoring component further divides each long path into two short intra-switch/inter-switch paths from the position after the egress queue, and additionally places \sketchname{} at the boundary. The additional \sketchname{} is considered as the downstream \sketchname{} of the intra-switch path, and the upstream \sketchname{} of the inter-switch path simultaneously.
% In this way, the victim flows in intra-switch/inter-switch paths can be explicitly located. Besides, the operators can at least detect intra-switch victim flows in the edge paths, and further detect inter-switch victim flows by placing \sketchname{} in end-hosts.
% At a cost, this placement consumes an additional switch resources.
% In the deployment, we choose placement strategies flexibly based on the remaining resources.
% In this paper, we default to this placement strategy.
% \presec
% \subsubsection{AM-PM \sketchname{}}
% \postsec

% To ensure the correctness of detection, for each pair of \sketchnamees{}, they should be collected after the last packet inserted into the upstream \sketchname{} is inserted into the downstream \sketchname{}. 

% \bbb{AM-PM timestamp.}
% To guarantee this, we choose to divide the traffic into continuous monitoring periods.
% %
% We leverage a timestamp flipping method similar to Alternate Marking Performance Measurement (AM-PM) \cite{am-pm}. 
% %
% Each switch maintains and periodically flips a 1-bit AM-PM timestamp just after the ingress ports, and attaches the AM-PM timestamp to each incoming packet.
% With the AM-PM timestamp, each switch \textit{``dominates''} a group of paths that upstream \sketchnamees{} in these paths are in the switch. That is to say, traffic passing through a group of paths is divided into continuous and alternating AM and PM equal-sized monitoring periods by the flipping timestamp in the corresponding switch. 
% %According to when the traffic arrives at ingress ports, the traffic is divided into different monitoring intervals with different upstream timestamps, and the upstream timestamp is assigned to each incoming packet.
% %
% Each \sketchname{} is also equally divided into an AM part (AM \sketchname{}) and a PM part (PM \sketchname{}) for packets in AM periods (with AM timestamps) and PM periods (with PM timestamps), respectively. 

% \begin{figure}[h!]
%     \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{0cm}
%     \prefig
%     \centering  
%     \includegraphics[width=1.0\linewidth]{lzr/pics/Fermat_switch.pdf}
%     \vspace{-0.2cm}
%     \caption{Placement of \sketchnamees{}.}
%     \label{algopic:placement}
%     \postfig
% \end{figure}


% \bbb{Distinguishing monitoring period.}
% To insert each packet into corresponding part of \sketchname{}, we need to correctly distinguish which monitoring period the packet resides in.
% %
% For each intra-switch path, it is easy to distinguish because the AM-PM timestamp can be easily attached to and transmitted with the packet in the same switch.
% %
% However, for each inter-switch path, its downstream \sketchname{} placed in another switch has no visibility to the AM-PM timestamp in the upstream switch. 
% %
% Therefore, we need a communication mechanism for timestamp transmission across switches. Similar to LossRadar, we achieve this by storing the attached AM-PM timestamp in one of the unused bits of IPv4 protocol. 
% %
% In this way, downstream \sketchname{} in inter-switch path can also correctly distinguish the monitoring period of each packet and insert it into the corresponding part. 
% %no priority queue

% \presec
% \subsection{Collecting \sketchnamees{}}
% \postsec
% \label{sec:algo:trans}


% For each path, to detect the victim flows in the latest monitoring period, the corresponding AM/PM \sketchnamees{} should be collected periodically. In this section, we focus on two parts: 1) when to correctly collect \sketchnamees{}; 2) how to quickly collect \sketchnamees{}.

% \presec
% \subsubsection{When to Collect \sketchnamees{}}
% \postsec
% To guarantee the correctness of detection, for each path, each pair of AM/PM \sketchnamees{} should be collected after the traffic with AM/PM timestamps has passed through the path totally, and before the next AM/PM monitoring period starts. 
% %
% Considering the situation that the switch is severely congested, after a monitoring period ends, the additional waiting time for its traffic to totally pass through the path is up to $2ms$ \cite{kannan2019precise}. 
% This requires 1) the predefined waiting time must be longer than $2ms$; 2) the monitoring period must be at least longer than the additional waiting time. Therefore, in order to provide enough time for decoding, diagnosis, and response, we consider 10$\sim$20$ms$ as the most fine-grained scale for monitoring period to achieve both correctness and timeliness. 


% \presec
% \subsubsection{How to Quickly Collect \sketchnamees{}}
% \postsec
% %Take switches with data plane and control plane as example. %Considering a switch $S$ and the paths controlled by its AM-PM timestamp, because the control plane of switch $S$ naturally has visibility to its timestamp, it can easily determine when to start fetching \sketchnamees{} of these intra-switch/inter-switch paths.
% %However, the specific strategy to fetch \sketchnamees{} is architecture-dependent, and we describe strategies for software switches and programmable switches below.
% %
% When a switch $S$ determines to collect \sketchnamees{}, \textit{it only focus on the paths that it dominates.}
% It needs to fetch \sketchnamees{} in the intra-switch paths from its data plane, and downstream \sketchnamees{} in the inter-switch paths from the data planes of its downstream switches.
% %
% Because it is naturally fast to fetch \sketchnamees{} from the data plane of software switch, we focus on how to fetch \sketchnamees{} from the data plane of programmable switch at a fast speed.

% \bbb{Slow strawman solution.}
% With interfaces (\eg, BFRT API in Tofino switch) for communication between control plane and data plane provided by vendors, in the strawman solution, for switch $S$, its control plane directly fetches \sketchnamees{} in the intra-switch paths from the data plane. Note that we just fetch downstream \sketchnamees{} here because their paired upstream \sketchnamees{} are essentially downstream \sketchnamees{} in the intra-switch paths. To further fetch downstream \sketchnamees{} in the inter-switch paths from the data planes of downstream switches, the control plane communicates with downstream switches, and inform their control planes of fetching corresponding \sketchnamees{} from their data planes. 
% However, this solution suffers from the extremely limited rate of accessing registers from the data plane through provided interfaces (about 500K 32-bit entries per second). Therefore, this solution can hardly achieve 10$ms$-level monitoring.
% %

% \bbb{Fast INT-like strategy:}
% To speed up the collection process, we propose another INT-like \cite{kim2015band} strategy to fully utilize programmable data plane.
% %
% For switch $S$, to collect \sketchnamees{} in the intra-switch paths, instead of accessing registers through the provided interface, we use tailored packets to piggyback \sketchnamees{} from the data plane. 
% %
% To save the CPU resources required for packet generation, the control plane just inject one trigger packet into the data plane, and leverage the switch mirror component to generate all needed tailored packets.
% %
% Every time a tailored packet passes through the switch pipeline, it piggybacks and clears a bucket of each array of each \sketchname{}.
% %
% To further minimize the cost of packet receiving, we leverage the recirculate port to recirculate the tailored packets multiple times, so as to pack the piggybacked buckets to jumbo frames.
% %
% Note that the recirculation does not result in any tailored packet loss. That is because the tailored packets only occupy the recirculate port and CPU PCIE port, which are usually at low utilization or idle. 
% %
% To fetch downstream \sketchnamees{} in the inter-switch paths from the data planes of downstream switches, switch $S$ informs each downstream switch, and piggybacks the downstream \sketchnamees{} as described above.
% %
% Leveraging the high-speed data plane, the strategy can support 10-$ms$ level monitoring period.

% \presec
% \subsection{Decoding \sketchnamees{}}
% \postsec
% \label{sec:decode}
% After collecting a pair of \sketchnamees{}, the monitoring component decodes them to detect the victim flows. As there are lots of available compute resources (switch CPUs and central controller) in the network, we focus on where to execute decoding. 

% \bbb{Distributed decoding manner.}
% To minimize the burden on the central controller, we propose a distributed decoding manner. If a switch CPU utilization is less than a predefined threshold, the tailored packets that piggyback \sketchname{}es in its dominated paths will be transmitted to the switch. Otherwise, they will be transmitted to the central controller.
% %
% After receiving the tailored packets, the receiver reconstructs \sketchnamees{} and executes decoding.
% %
% After decoding, no matter where the decoding is executed, the decoding results will be transmitted to the central controller as the input of the diagnosis component. 
% %
% Note that a programmable switch establishes and maintains persistent TCP connections through in-band network with other switches and the central controller. As a result, all \sketchnamees{} and decoding results can be completely and reliably transmitted to the central controller. These connections will be directed to the highest priority queue in switches, so as to achieve the fastest collection.
% %field $\mathbb{Z}_p$, where $p$ is the prime used in \sketchnamees{}, 



% \presec
% \subsection{Mathematical Analysis}
% \postsec
% \label{sec:algo:math}




% \begin{theorem}
% For a given number of loss flows $F$, \aname{} encodes each packet in $O(d)$ time, and finds all $F$ flows with at least $1-O(F^{2-d})$ probability, which consumes $O(F)$ space and communication overhead and $O(d F)$ time overhead.
% \end{theorem}

% \begin{proof}

% Suppose the verification of the pure bucket is correct every time, the decode procedure is the same as finding a 2-core of a random hypergraph. Specifically, each bucket of \aname{} can be regarded as a point, and each flow can be regarded as a super edge connecting $d$ random points. A \aname{} can be considered as a random graph.
% A 2-core of a graph is a sub-graph that all vertices have degree at least 2. If a 2-core exists, \aname{} cannot decode all loss flows completely. Otherwise, suppose all verifications are correct, \aname{} can decode all flows. The probability of a 2-core exists has been well studied. Existing results \cite{molloy2004pure} show that when the graph size (number of buckets) is grater than $(c_d+\epsilon)F$, the 2-core does not exist with probability $1-O(F^{2-d})$, in which condition we can decode all flows. 
% \begin{align}
%     c_d\approx c_d^*=\frac{\ln(d)+\ln(\ln(d))}{d(1-\frac{1}{d\ln(d)})^{d-1}}.
% \end{align}
% When $d=3$ or $4$, we have $c_3^*=1.22, c_4^*=1.29$. The space and communication complexity is $O(F)$.





% When considering the verification with errors, the probability of successful decode keeps in a same level as that of verification without error. The failure probability of rehashing verification is $\frac{1}{m}<\frac{d}{F}$, and that of ID verification is $\frac{1}{min(p_1, p_2)}$. There are at most $2F d$ different values need to be verified. By Chenoff bound, there is no more than $t=4d^2$ error with probability $1-O(e^{-F})$, which probability can be considered as $100\%$.
% $t=4d^2$ is a constant relative to $F$. These $t$ errors can be considered as a case that $d*t$ random buckets are poisoned, which means these buckets cannot be used for decoding. Existing work \cite{molloy2004pure, rink2013mixed, goodrich2011invertibleIBLT} shows that the probability of decode failure incurred by poisoned bucket is of the same order as the probability that all the mapped buckets of a flow are poisoned, which is $F(\frac{dt}{F})^d=o(F^{2-d})$. If we additionally use ID verification, the probability of decode failure is $\frac{o(F^{2-d})}{min(p_1, p_2)}$, which is an ignorable probability.
% Our simulation results (See Figure \ref{math:successpr} and \ref{math:decoderato}) also prof our theory results. Therefore, the probability of finding all $F$ flows is at least $1-O(F^{2-d})$, with $O(F)$ space and communication overhead. As there is only constant number of errors $t$, \aname{} can decode all flows with $O(d F)$ time complexity.
% \end{proof}


% \begin{figure}[h!]
%     \setlength{\abovecaptionskip}{-0.15cm}
%     \setlength{\belowcaptionskip}{0cm}
%     \prefig
%     \centering  
%     \includegraphics[width=0.7\linewidth]{lzr/pics/math/decode_success_rate.pdf}
%     \vspace{0.2cm}
%     \caption{The probability of decoding all loss flows reaches $100\%$ sharply when the total number of buckets is $1.23$ times more than the number of loss flows, where \textit{``ID-V''} means using the technique of ID Verification. ($d=3$)}
%     \label{math:successpr}
%     \postfig
% \end{figure}


% \begin{figure}[h!]
%     \setlength{\abovecaptionskip}{-0.15cm}
%     \setlength{\belowcaptionskip}{0cm}
%     \prefig
%     \centering  
%     \includegraphics[width=0.7\linewidth]{lzr/pics/math/ratio_of_decoded_flows.pdf}
%     \vspace{0.2cm}
%     \caption{The average ratio of the decoded flows among all loss flows reaches $100\%$ sharply, where \textit{``ID-V''} means using the technique of ID Verification. ($d=3$)
%     }
%     \label{math:decoderato}
%     \postfig
%     \vspace{0.3cm}
% \end{figure}

% Compare with the state-of-the-art algorithm of finding the differences, Invertible Bloom Lookup Tables (IBLT) \cite{goodrich2011invertibleIBLT}, we reduce the memory and communication overhead by $m\log_2(m)$ bits, and achieves a new function of aggregating the attributes of the same key.


% \presec
% \section{Diagnosing Root Causes of Packet Losses}\postsec
% After the monitoring component decodes the paired \sketchnamees{} and captures the victim flows in the last period, the diagnosis component pinpoints corresponding root cause of packet losses.
% %
% In this section, we first propose a general ML-based method to identify classes of packet losses without visibility to packet forwarding logic. 
% Second, with the identified class, if we can go deeper into packet forwarding logic, we propose another method based on error codes to further pinpoint the root causes, and improve the accuracy of our ML-based method.
% Third, we discuss the ability of \systemname{} to diagnose packet losses under different settings. 
% %Third, we propose a path tracing method working in \systemname{} to help diagnose the root causes and the following re-configuration.
% % \sout{to diagnose them}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}

% \begin{table*}[]
% \caption{Classes and root causes of packet losses, and the packet losses that \systemname{} can diagnose. LR refers to LossRadar's placement, and FD refers to \systemname{}'s placement in Section \ref{sketchplace}. \checkmark means the root cause can be pinpointed, and $\circ$ means the class can be identified.}
% \vspace{0.3cm}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \label{pkt:loss}
% Class                                                                           & Root cause                & ML (LR)                   & ML (FD)                   & ML+EC (LR)                & ML+EC (FD)                \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Forwarding\\ Blackhole\end{tabular}} & Forwarding table mismatch & $\circ$                   & $\circ$                   & \checkmark & \checkmark \\ \cline{2-6} 
%                                                                                 & ACL rule drop             & $\circ$                   & $\circ$                   & \checkmark & \checkmark \\ \hline
% \multirow{2}{*}{Random Drop}                                                    & Swicth ASIC failure       & $\circ$                   & \checkmark & $\circ$                   & \checkmark \\ \cline{2-6} 
%                                                                                 & Bent Fiber                & $\circ$                   & \checkmark & $\circ$                   & \checkmark \\ \hline
% Forwarding Loop                                                                 & TTL=0                   & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
% Congestion                                                                      & Unexpected traffic volume & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
% \end{tabular}
% \end{table*}

% \presec
% \subsection{Diagnosing using Machine Learning}
% \label{sec:ana:ml}


% \subsubsection{Motivation to Use Machine Learning} \postsec

% %
% As shown in Table \ref{pkt:loss}, there are mainly four classes and six root causes of packet losses. \textit{We exclude link failure from the table because all the packets are lost in the link, which is a significant characteristic for diagnosis.}
% %
% In general, when the monitoring component is deployed in commodity switches and software switches, the packet forwarding logic is usually fixed, and invisible to the deployed monitoring component.
% %
% In this case, it is difficult to pinpoint root causes, because different root causes of the same class may look like the same.
% For example, forwarding table mismatch and ACL rule drop show no difference. 
% %
% Therefore, we focus on identifying classes of packet losses. 
% To achieve this, the state-of-the-art LossRadar analyzes the patterns of the lost packets, such as 5-tuple, IP\_ID, TTL, timestamp, TCP flags, \etc{}
% %
% However, the diagnosis component cannot obtain packet-level information used by LossRadar, it can only obtain the victim flow IDs and the numbers of lost packets after decoding.
% %
% Note that all the sum counters of a \sketchname{} make up a Count-Min sketch \cite{cmsketch}, so the central controller can also get several frequency estimators of each victim flow\footnote{For \sketchnamees{} decoded in switches, the frequency estimators can also be transmitted to the central controller.}.
% %
% After a thorough study of the four classes of packet losses, we find different class will lead to different numerical relationship between the frequency of the flow and the number of the lost packets. Motivated by this, we choose to use machine learning to train a classifier to identify the classes.
% %

% \presec
% \subsubsection{Identifying Loss Classes} \postsec

% In this section, we elaborate on our insights about how the classes of packet losses are identified.

% \bbb{Forwarding blackhole:}
% %
% %The forwarding blackhole caused by forwarding table mismatch or ACL rule will drop all packets belonging to a flow.
% A forwarding blackhole will drop all packets belonging to a flow.
% %
% In this case, each packet sent from the TCP sender will time out, resulting in the TCP congestion window rapidly reduced to 1.
% %
% After that, TCP sender will send one packet after every RTO (Retransmission Timeout).
% %
% Therefore, the packet losses caused by forwarding blackhole has the following characteristics:
% %
% the number of lost packets is almost the same as the frequency estimator, and the number of lost packets in each monitoring period is almost the same (\ie, the ratio of monitoring period to RTO\footnote{In DCTCP, the RTO is set to 10ms by default.}) except for the first period.

% \bbb{Forwarding loop:}
% %
% A forwarding loop will also cause all packets of a flow to be lost, resulting in the TCP congestion window becoming 1.
% %
% Therefore, the number of lost packets in each monitoring period is almost the same.
% %
% There is a significant difference between packet losses caused by loop and packet losses caused by blackhole: each lost packet passes through the switches in the loop many times.
% %
% Therefore, the packet losses caused by loop has the following significant characteristic: 
% %
% the ratio of the frequency estimator to the number of lost packet is similar to the number of times a packet passes through the switch (\ie, the ratio of the initial TTL to the loop length).

% \bbb{Congestion \& Random drop: }
% %
% For the packet losses caused by congestion or random drop, the number of lost packets belonging to one flow in each monitoring period is no longer a fixed value.
% %
% Both of them will cause a portion of packets to be dropped, which makes it difficult to distinguish them from each other in terms of packet losses ratio.
% %
% However, previous work \cite{yang2018empowering} pointed out that larger network traffic will make the difference of several frequency estimators of a flow greater, which makes it possible to identify these classes.


% \presec
% \subsubsection{Classifier Training} \postsec
% In this section, we present the workflow in classifier training: 1) feature selection; 2) training data collection; 3) classifier model decision.

% \bbb{Feature selection.}
% Based on the above insights, we propose to use the following features to represent a flow-level packet loss event:
% %
% The features include data of several consecutive monitoring periods that start from the earliest period in which packet losses are detected.
% %
% The data of each monitoring period includes: 
% %
% 1) the number of lost packets; 
% %
% 2) the estimated proportion of packet loss, \ie, the proportion of the number of lost packets to the smallest frequency estimator;
% %
% 3) the difference of frequency estimator, \ie, the ratio of the second smallest (the third smallest, ..., the largest) frequency estimator to the smallest frequency estimator.
% %
% Using more monitoring periods to generate features can achieve higher accuracy, but the cost is that it takes longer time to obtain the results (\S \ref{sec:exp:ml}).
% %
% Operators of \systemname{} need to make a trade-off between the \textit{accuracy} and \textit{timeliness}.

% \bbb{Training data collection.}
% The diagnosis component needs labeled dataset to train the classifier. With the deployment of our monitoring component, the packet losses are collectable. However, the classes of packet losses are invisible.
% %
% Therefore, we can only collect a large amount of unlabeled data with features described above.
% To label the data, we inject a small number of trigger flows\footnote{the destination IP of these flows are set to 0.0.0.0, so as to avoid any possible conflict with rules in switches.} into the network, and configure the switches to make these flows experience different classes of packet losses. After the packet losses of these trigger flows are detected, we can collect a small amount of pre-labeled data.
% %
% Then, we cluster the unlabeled data into multiple groups using the most widely-used clustering algorithm DBSCAN \cite{ester1996density}. 
% %
% We keep adjusting the parameters of DBSCAN until more than 90\% of the pre-labeled data in each group belong to one class. 
% Finally, for each group, we label all the unlabeled data in it as the major class.
% %If we can configure the switches, an option to improve the accuracy of label is to sample lost packets. We adopt xxx?? as our cluster algorithm. 

% \bbb{Model decision.}
% With the labeled data, we can train the classifier. 
% %
% Making a trade-off between accuracy and computation efficiency, we choose the multi-layer perceptron \cite{pal1992multilayer} with two hidden layers as the classification model, and use cross-entropy as the loss function.
% %
% In order to ensure that the classifier can adapt to the varying network traffic, we collect training data and train the classifier periodically.



% %



% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% \presec
% \subsection{Diagnosing using Programmable Switches}
% \postsec
% \label{sec:p4}
% When the monitoring component is deployed in the programmable data plane, we can dig deeper into the packet forwarding logic, and further pinpoint the root causes. 
% There are three kinds of root causes that are visible to the packet forwarding logic: 1) forwarding table mismatch, which means no rule in the forwarding table matches the packet; 2) ACL rule drop, which means an rule in the ACL table matches the packet; 3) TTL=$0$.
% The first two root causes will lead to forwarding blackholes, and the third one suggests the packet is trapped in a forwarding loop.
% % 
% To record the root causes, we assign a 2-bit error code (EC) to each kind of root cause, and reserve $0$ to indicate that there is no explicit root cause for packet losses. 
% %
% For each incoming packet. we concatenate its 5-tuple and the error code, and insert the result of concatenation into \sketchnamees{}. 
% %
% In this way, we can directly pinpoint the root causes of packet losses after decoding.
% %
% Further, because part of the unlabeled training data can be labeled, the accuracy of the classifier improves.   

% \presec
% \subsection{Diagnosis Ability under Different Settings}
% \postsec
% The ability of \systemname{} is determined by the placement strategy and whether error code is available. As shown in Table \ref{pkt:loss}, \systemname{} with only ML-based method cannot distinguish forwarding table mismatch from ACL rule drop because they show no difference; \systemname{} with LossRadar's placement cannot distinguish switch ASIC failure from bent fiber, because it cannot distinguish intra-switch/inter-switch packet losses.

 


==> NSDI2023/7Handling_extremely_poor_network.tex <==
\presec 
\section{Handling Poor Network} 
\postsec

==> NSDI2023/7Recoverymodule.tex <==
\presec
\section{Responding to Network Anomalies}
\postsec
\label{sec:rec}


To respond to network anomalies, the response component formulates re-configuration strategies according to different root causes of packet losses, and then classify them into different risk-levels. 
%
For strategies of different risk-levels, the response component executes them in different working modes.  
%
In this section, we first describe each risk-level and its corresponding working mode in \systemname{}.
%
Then, we detail the reasons for the classification, and the re-configuration strategies for each root cause.
%
\textit{Note that all the re-configuration strategies are based on a premise that the network topology is known to \systemname{}. The central controller informs the switches of the re-configuration strategies over persistent TCP connections.}

\presec
% \subsection{Low-risk Strategies}
\subsection{Strategies for Low-Risk Anomalies}
\postsec

For low-risk strategies, \systemname{} executes them silently. Low-risk strategies include strategies for forwarding loop, forwarding table mismatch, and congestion caused by uneven ECMP. We consider these strategies as low-risk because they are per-flow response. That is to say, in these strategies, each rule re-configured in the forwarding table only affects a flow.




\presec
\subsubsection{Forwarding Loop}
\postsec
Due to the high packet processing speed of switches, a looped flow usually generates a burst, leading to severe congestion. Not only the flow itself, but also other flows passing through the loop suffer serious packet loss and throughput drop. Therefore, we need to quickly eliminate the loop. 

\bbb{Strategy.}
Leveraging the path tracing method mentioned in Appendix \ref{sec:ana:pt}, for each flow $f$ trapped in forwarding loop, we can quickly locate its path and forwarding loop. Then, we select the switch closest to the destination end-host in the forwarding loop, and re-configure its forwarding table to redirect $f$ to the switch closest to the destination end-host in the network.

\bbb{Rollback.}
We need to rollback because we may misjudge the root cause. We adopt a naive strategy, that if the re-configuration cannot work, we quickly withdraw it and report it to the operator.


\presec
\subsubsection{Forwarding Table Mismatch}
\postsec
When forwarding table mismatch happens on a certain flow, it will be dropped and suffer serious throughput drop. Therefore, we need to quickly direct this flow to its destination end-host.

\bbb{Strategy.}
For each flow $f$ dropped by table lookup miss in a certain switch, we re-configure its forwarding table to redirect $f$ to the switch closest to the destination end-host in the network. 

\bbb{Rollback.}
The same as that in loop.

 
\presec
\subsubsection{Congestion Incurred by Uneven ECMP}
\postsec
ECMP is a widely used routing strategy for load balance in data centers. However, ECMP performs badly when the traffic is extremely skewed to the hash function used in ECMP, leading to load imbalance and serious congestion. Therefore, we need to rearrange the traffic to avoid congestion.

\bbb{Strategy.}
Our strategy is to redirect the flows with packet loss in the latest monitoring period to the idle links. For each optional link, we coarsely estimate the traffic volume directed to it by summing the sum counters of \sketchname{}. For the link with less traffic volume, we re-configure the forwarding table to redirect part of flows to it. In this way, we avoid congestion and reduce the number of packets loss. 

\bbb{Rollback.}
After executing the re-configuration, if traffic becomes more uneven in the following several periods, \systemname{} realizes the packet loss is caused by a sudden burst, and then withdraw the re-configuration.

\presec
\subsection{Strategies for Medium-Risk Anomalies}
\postsec
For medium-risk strategies, \systemname{} requests the permission of operators before execution.
Medium-risk strategies include strategies for link failure, switch ASIC failure, and bent fiber. We consider these strategies as medium-risk because they are per-link response. That is to say, in these strategies, each rule re-configured in the forwarding table affects all the flows directed to a certain link.

\bbb{Common strategy.}
There is a common strategy as it is a per-link anomaly, and all the traffic should be directed away from the abnormal link. To achieve this, we re-configure the forwarding tables of the affected switches to ensure that no flows will be directed to the abnormal link. 


\presec
\subsection{Strategies for High-Risk Anomalies}
\postsec
For high-risk strategies, \systemname{} only notifies the operators of flows suffering packet loss and corresponding root causes.
High-risk strategies include strategies for ACL rule drop. We consider these strategies as high risk because ACL rule is related to network security, even asset safety. Therefore, we consider \systemname{} should have no permission to access ACL rules, let alone re-configure them. 

\presec
\subsection{Discussion}
\postsec
The response component can work well with the diagnosis component which only relies on ML-based method. Although the diagnosis component can hardly distinguish forwarding table mismatch from ACL rule drop, it just needs to regard all blackholes as caused by forwarding table mismatch.
In this way, the blackhole caused by forwarding table mismatch can be re-configured, and the blackhole caused by ACL rule drop is never affected.


%First

%Suppose the remote controller understands the topology of the network well. Once the analysis module determines that there is a link failure, the recovery module sends some packets to the affected switches to reconfigure the flow table to ensure that no flows will be directed to the failed link. For example, as shown in Figure \ref{?}, once link ? is failed, the controller notifies switch ? to redirect its flows. 

%However, the link failure may be recovered after replacing the questioned fiber with a new one, and our system should redirect the traffic to this link at that time. This requires our system to continuously sense the condition of the failed link. Therefore, after a link is regarded as failed, its upstream switch generates and sends a probing flow to the failed link in each measurement epoch. Therefore, once the link failure is recovered, the probing flow will not be dropped. At that time, the 
%controller sends packets to withdraw the reconfiguration of flow table.





%Network operators need to carefully update the forwarding table. However, update error is unavoidable, and the recovery module need to recover them as fast as possible.

%\presec
%\section{Recovery agent}
%After the analyzer module determine the type of packet drops, if the type can be recovered by the recovery agent, then the analyzer module informs the recovery agent 
%\postsec



==> NSDI2023/Overview.tex <==
\presec \section{\systemname{} Overview} \postsec
%
%Given a network, the monitoring goal of \systemname{} is to report flow statistics and frequency changes for all flows enter the network.
%
%For flow statistics, \systemname{} lets every edge switch to encode every packet's information that enters the network.
%
%To further su flow frequency changes, \systemname{} lets every edge switch to encode every packet's information that enters the network. 







In this section, we provide an overview of \systemname{} at a high level. 
%
% \presec \subsection{Overview} \postsec
% We introduce how we leverage our \sketchname{} to construct a flow sketching system in a single switch.
\wyh{Rationale or not ?}

\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{wuyuhan/overview.pdf}
    \vspace{0.2cm}
    \caption{Overview.}
    \label{algopic:overview}
    \postfig
\end{figure}

\presub \subsection{Overview } \postsub

\wyh{
\bbb{Structure:}
As shown in Figure \ref{algopic:overview}, there are four components in the data plane: 1) a \textbf{Classifier} for identifying the packets of elephant flows, defined as flows with sizes more than $L$ (packets); 2) an \textbf{Elephant Sketch} for compressing the elephant flows by \sketchname{}, which is precise and can be decoded easily; 3) a \textbf{Mice Sketch} for compressing the mice flows by \sketchname{}; 4) a \textbf{Loss Sketch} compressing all flows for loss detection by \sketchname{}.

\bbb{Workflow of Insertion:}
Each incoming packet carries a flow ID (\eg, 5-tuple) and will first enter the upstream switch. In the switch, the packet first go through the flow classifier. Then, according to the classification, \ie, elephant flow or mice flow, the packet will be inserted to the Elephant Sketch or Mice Sketch, respectively. Next, the packet leaves the upstream switch, goes through the blackbox network, and enters the downstream switch if the packet is not lost. Finally, the packet will be inserted into the Loss Sketch.


\bbb{Workflow of Query:}
Periodically, the control plane reads the four components from data plane and analyzes the measurement result.
The Elephant Sketch can be fast decoded in linear time, and the decoded elephant flows are all exact with nearly zero failure probability. 
Through the classifier and the Elephant Sketch, we can estimate per-flow sizes and decode the Flow ID of all elephant flows.
Finding flows with packet losses requires the three sketches work together: resize the elephant sketch, merge it with the mice sketch, minus the merged sketch with loss sketch, and decode it.



}



























































% We begin by defining the problem scope ($\S$~\ref{2:scope}), and then briefly describe the end-to-end workflow of \systemname{} to solve the problem ($\S$~\ref{2:workflow}).

% \presec
% \subsection{Problem Scope}
% \postsec
% \label{2:scope}
% Given a measurement object, which could be a single switch or a network consisting of multiple switches and links (\eg, Figure \ref{?}), we assume that it satisfies the following two requirements: 1) no packet will be generated in it; 2) all flows entering it will finally leave it if no packet losses occur, \ie, no packet is destined for any switch in it.
% %
% For such an object, its desired measurement should cover the flow sketching and loss detection defined as follows, and we summarize three key requirements (R1-R3) from them.
% %

% %
% \bbb{Flow sketching:} we should provide flow size estimation for all flows entering the given object (R1), and additionally provide the flow IDs (\eg, 5-tuple, source IP address) of large flows among them (R2);
% %

% \bbb{Loss detection:}
% \systemname{} should provide the flow ID and the number of lost packets for every flow that suffers packet loss in the given object, no matter where packet losses occur (R3).

% %
% \presec
% \subsection{End-to-end Workflow}
% \postsec
% \label{2:workflow}

% %抽象出一个“入探测”和“出探测”

% %The end-to-end workflow of \systemname{} is shown in Figure \ref{pic:overview}.
% In this section, we first describe the workflow when the measurement object is a single switch, then we extend it to support \textbf{a-giant-switch} \cite{???see univmon} abstraction to support the measurement object to be a network.
% %
% \presec
% \subsubsection{Workflow for A Single Switch}
% \postsec
% To better illustrate the workflow, we split the workflow into data plane and control plane designs, and focus on how the design can satisfy the key requirements.
% %
% %

% \bbb{Data plane design:} 
% %
% We take a PISA switch as an example. 
% %
% As shown in Figure \ref{?}, the incoming packets will undergo the following four components in sequence. 
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=0pt,partopsep=0pt]
%     \item \textit{Flow size estimator (Ingress):} 
%     To satisfy R1 and R2, we need a flow size estimator to distinguish between large flows and small flows and provide flow size estimation. 
%     %
%     A kind of promising solutions are sketches, and we select TowerSketch \cite{?}, a lightweight, accurate, and hardware-friendly sketch, as the flow size estimator.
%     %
%     The flow size estimator should be deployed in the Ingress so as to avoid the potential interference of packet losses.
    
%     \item \textit{Large flow recorder (Ingress):}
%     With the output of the flow size estimator, we can then identify large flows.
%     %
%     To satisfy R2, we further need a large flow recorder to record information of large flows.
%     %
%     We devise \sketchname{}, a hardware-friendly flow encoder that can encodes flow IDs and flow sizes without error, as the large flow recorder, which outperforms FlowRadar \cite{flowradar2016} in terms of memory-efficiency.
%     %
%     Moreover, the large flow recorder can be used to optimize the flow size estimation of large flows, and thus better satisfy R1.
%     %
%     Similarly, the large flow recorder also should be deployed in the Ingress.
    
%     \item \textit{Small flow recorder (Ingress):}
%     To satisfy R3, our main methodology is to encode the information of flows upstream and downstream, and mine the packet losses from the difference between upstream and downstream encoders.
%     %
%     Specifically, in a single switch, upstream refers to Ingress, and downstream refers to Egress.
%     %
%     Therefore, we further need a small flow recorder to record information of small flows, and we build another \sketchname{} as the small flow recorder.
%     %
%     The sum of the two flow recorders can work as the upstream encoder.
%     %
%     In PISA switches, the two flow recorders can be paralleled as a packet can only be identified as either small flow or large flow, so as to save hardware resources.
    
%     \item \textit{All flow recorder (Egress):}
%     To satisfy R3, we need an all flow recorder to encode the information of all flows in the Egress.
%     %
%     Similarly, we build a \sketchname{} as the all flow recorder, encoding every incoming packet in the Egress.
% \end{itemize} 

% \bbb{Control plane design:} Control plane periodically collects sketches from data plane, and then leverages the combination of the collected sketches to provide queries.
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=0pt,partopsep=0pt]
    
%     \item \textit{Flow sketching (R1-R2):}
%     %控制面需要收集sketch以支持测量
%     %现在的控制面API太慢了，考虑到交换机的内存极其有限，漫长的收集时间可能会导致测量精度大幅降低甚至不可用
%     %为了解决这个问题，我们利用数据面提高收集性能
%     control plane provides queries with the flow size estimator and the large flow recorder.
%     %
%     %However, existing control plane APIs provided by hardware switches are inefficient, and thus cannot support timely measurement (make measurement useless).
%     %
%     %To address this issue, we speed up the collection by leverage the flexible SALU components in the data plane to carry counters in tailored packets. 
    
%     \item\textit{Loss detection (R3):}
%     control plane provides queries with the small flow recorder, the large flow recorder, and the all flow recorder.
% \end{itemize} 







% %这一章，我们从一个high-level介绍我们的系统。
% %首先，我们介绍我们数据平面的设计，
% %然后，我们介绍我们控制平面的设计

% R1: hierarchical measurement accuracy: for different statistics, we need different accuracy-baseline to support different tasks.
% R2: High volume: data plane of \systemname{} should only record information which benefit the accuracy to measure most volume

% R4: hardware friendliness

==> NSDI2023/Tasks.tex <==
\section{Supported Tasks}
In this section, we first elaborate on how \systemname{} support seven flow sketching tasks ($\S $~\ref{tasks:flow}).
%
Second, we introduce xx?? packet loss tasks supported by \systemname{} ($\S $~\ref{tasks:loss}). 

\subsection{Flow Sketching Tasks}
\label{tasks:flow}

\bbb{Flow Size Estimation:}
estimating the flow size of any flow with ID $f$ in a time window.
%
For every flow, suppose we know its flow ID and the edge switch where it enters the network.
%
%
Then, we can query \ykc{the TowerSketch and the heavy part of \sketchname{}} deployed in that switch for the flow size as described in Section \ref{?}.
%
%

\bbb{Heavy hitter detection:}
reporting every flow whose size is larger than a pre-defined threshold $\Delta_h$ in a time window.
%
For every edge switch, we set \ykc{the filter threshold to $\Delta_h$.}
%
After each round of collection, for every edge switch, we decode \ykc{the heavy part of \sketchname{}} deployed in it to acquire a set of flows with ID $f_j$ and flow size $p_j$.
%
For every decoded flow $f_j$, we report it as a heavy hitter, and its size as $(p_j+\Delta_h)$.
%
%
%Then, for every potential heavy hitter, as described in flow size estimation, we re-query its upper bound of flow size.
%

\subsection{Loss Tasks}
\label{tasks:loss}

==> NSDI2023/intro.tex <==
\presec 
\section{Introduction} 
\postsec
\subsection{Background and Motivation}
%现有频数-based flow-level测量问题分两类：单点测量，流在网络上传输的测量
%correspondingly, 测量方案也分两类做第一类的算法(空间 M1)，做第二类的算法(空间M2)
%针对这两类问题，有对应两类解决方案
%一个完整的测量系统应该全部支持，一个naive solution是A+B,我们的design goal是比min(A,B)小l
%第三类是straight forward,记录所有信息，储存全流信息，和现有比起来消耗太大，放在rw

Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}.
%
Recently, sketch-based solutions, where sketches are a kind of probabilistic sub-linear data structures, have been widely acknowledged as one of the most promising solutions in network measurement \cite{sketchlearn2018,opensketch2013,zhang2021cocosketch,nitrosketch2019,ben2017constant}.
%

%这里应该是对任务分类，而不是对sketch分类。因为后文的内容都是对任务分类。
%标题如果改成Being and Change，现有intro的表达要改吗？
\sout{Different from existing classifications, we classify existing sketches into two categories:}\wyh{Before approaching the problem of existing sketches, we classify the key measurement tasks into two categories:} \textbf{flow statistics} and (flow) \textbf{frequency changes}.
Flow statistics in this paper refer to per-flow statistics in one network node, including flow size, heavy hitter, flow size distribution, entropy, \textit{etc.} 
% Frequency changes 包含的内容好像不太对，讲重复了？per-flow packet loss/increase是不是就包括后面的东西？这里对flow的定义不清晰。
Frequency changes refer to the changes of flow frequency (the number of packets) across many network nodes, 
\sout{including per-flow packet loss, per-flow packet increase, broadcast, multicast, broadcast loss/increase, multicast loss/increase, etc.}
\wyh{including per-flow packet loss, per-flow packet increase, broadcast, multicast, etc.}
%
\sout{From the perspective of information theory, the included information of first kind is very high due to the large number of network flows, while the information of the second kind is small because only a few flows experience changes of packet count.}
\wyh{From the perspective of information theory, the required information for answering the first kind exactly is much higher than that of the second kind, because the first kind covers the large number of all flows while the second kind only focuses on a few flows that experience changes of packet count.}
%
From the network abnormal perspective, most of the first kind is just statistics and normal, while most of the second kind are abnormal \wyh{and more noteworthy}.
Therefore, it is often desired that the solution for the first kind allows small error while the solution for the second kind is error-less.
% 

\wyh{\wyh{Some immoderate solutions} addressing both kinds are to store all $\langle flow~ID, frequency \rangle$ information \wyh{exactly} (\eg, FlowRadar\cite{flowradar2016}, Counter braids \cite{lu2008counter}, OmniMon \cite{omnimon2020}), which either require large memory or need \wyh{ additional }expensive overhead to collect all flow IDs. }
In contrast, practical and memory-efficient works separate the two kinds and design solutions individually.
For examples, sketches of CM \cite{cmsketch}, Count \cite{countsketch}, CU \cite{cusketch}, UnivMon \cite{univmon2016}, Nitro \cite{nitrosketch2019}, and more \cite{elastic2018} focus on the first kind of tasks, while LossRadar \cite{lossradar2016} focuses on the second kind. 
However, this requires building two compact sketches with memory $m_A$ and $m_B$ for each kind of tasks respectively, which is both time and memory consuming.
%
Our design goal is to \textit{quickly handle both kinds of tasks simultaneously using memory size less than} $min\{m_A,m_B\}$.


% 
\wyh{old existing solutions paragraph:}
Therefore, existing works separate them and design solutions individually.
For examples, sketches of CM \cite{cmsketch}, Count \cite{countsketch}, CU \cite{cusketch}, UnivMon \cite{univmon2016}, Nitro \cite{nitrosketch2019}, and more \cite{elastic2018} focus on the first kind of tasks, while LossRadar \cite{lossradar2016} focuses on the second kind. 
%
However, in practise, it is usually that both kinds of tasks are coexistent.
% wyh：这里应该不能说effective？
\sout{One effective solution is to store all $\langle flow~ID, frequency \rangle$ information (\eg, FlowRadar\cite{flowradar2016}, Counter braids \cite{lu2008counter}, OmniMon \cite{omnimon2020}), which either needs large memory or needs expensive overhead to collect all flow IDs. }
%
\wyh{\wyh{One immoderate solution} addressing both kinds is to store all $\langle flow~ID, frequency \rangle$ information \wyh{exactly} (\eg, FlowRadar\cite{flowradar2016}, Counter braids \cite{lu2008counter}, OmniMon \cite{omnimon2020}), which either requires large memory or needs \wyh{ additional }expensive overhead to collect all flow IDs. }
%
Another solution is to build two compact sketches with memory $m_A$ and $m_B$ for each kind of tasks respectively, while is both time and memory consuming.
%
The design goal is to \textit{quickly handle both kinds of tasks simultaneously using memory size less than} $min\{m_A,m_B\}$.







\begin{comment}

Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}.
%
Recently, sketch-based solutions, where sketches are a kind of probabilistic sub-linear data structures, have been widely acknowledged as one of the most promising solutions in network measurement \cite{sketchlearn2018,opensketch2013,zhang2021cocosketch,nitrosketch2019,ben2017constant}.
%


Different from existing classifications, we classify existing sketches into two categories: \textbf{flow statistics} and (flow) \textbf{frequency changes}.
Flow statistics in this paper refer to per-flow statistics in one network node, including flow size, heavy hitter, flow size distribution, entropy, \textit{etc.} 
%
Frequency changes refer to the changes of flow frequency (the number of packets) across many network nodes, including per-flow packet loss, per-flow packet increase, broadcast, multicast, broadcast loss/increase, multicast loss/increase, etc.
%
From the perspective of information theory, the included information of first kind is very high due to the large number of network flows, while the information of the second kind is small because only a few flows experience changes of packet count.
%
From the network abnormal perspective, most of the first kind is just statistics and normal, while most of the second kind are abnormal.
%
Therefore, it is often desired that the solution for the first kind allows small error while the solution for the second kind is error-less.
%
Existing works often separate them and design solutions individually. 
For examples, sketches of CM \cite{cmsketch}, Count \cite{countsketch}, CU \cite{cusketch}, UnivMon \cite{univmon2016}, Nitro \cite{nitrosketch2019}, and more \cite{elastic2018} focus on the first kind of tasks, while LossRadar \cite{lossradar2016} focuses on the second kind. 
%
However, in practise, it is usually both kinds of tasks are coexistent.
%
One effective solution is to store all $<flow~ID, frequency>$ information (\eg, FlowRadar\cite{flowradar2016}, Counter braids \cite{lu2008counter}, OmniMon \cite{omnimon2020}), which either needs large memory or needs expensive overhead to collect all flow IDs. 
%
Another solution is to build two compact sketches with memory $m_A$ and $m_B$ for each kind of tasks respectively, while is both time and memory consuming.
%
The design goal is to \textit{quickly handle both kinds of tasks simultaneously using memory size less than} $min\{m_A,m_B\}$.

\end{comment}


%yt comment
\begin{comment}
Based on the exactness of provided statistics, existing sketches can be divided into two kinds: 1) approximate solutions and 2) exact solutions. 
%
The first kind is approximate solutions, which can provide approximation of desired statistics at a high throughput under tight memory limitations.
%
Typical solutions include CM \cite{cmsketch}, CU \cite{cusketch}, and Count \cite{countsketch}.
%
Due to the high accuracy and versatility of the newly proposed solutions \cite{elastic2018, univmon2016}, approximate solutions have become one of the most promising solutions for error-tolerant measurement tasks that allow limited amount of estimation error, including flow size estimation \cite{ribeiro2006fisher}, heavy hitter detection \cite{bandi2007fast}, entropy estimation \cite{lall2006data,zhao2007data}, and more \cite{kumar2004data}.
%
However, the estimation error of approximate solutions prevent them from supporting tasks that require zero-error measurement. 
%
The primary one is flow size change estimation, which provides basis for loss detection: By comparing the change of exact flow sizes between nearby forwarding nodes \cite{flowradar2016}, loss detection aims at finding the abnormal flows with packet losses, which could be incurred by congestion \cite{dhamdhere2018inferring,fanou2017investigating}, link failures \cite{iannaccone2002analysis}, BGP misconfigurations \cite{mahajan2002understanding,feamster2005detecting}, and more \cite{gill2011understanding}.
%误差容忍的sketch在解决这个问题的时候会表现非常差，因为估计的不准确导致被认为存在丢包
\wyh{This task requires zero-error measurement instead of approximate solutions, because we cannot distinguish whether the change of the estimated flow size is due to the packet loss or the estimation error from the sketch itself.
}
The second kind is exact solutions.
%
Typical solutions include LossRadar \cite{lossradar2016}.
%
\ykc{These solutions provide exact statistics of the change of flow sizes, and thus cannot support error-tolerant tasks requiring flow sizes.}
%
%However, their memory overhead is proportional to the number of flows, which is unpractical considering the great traffic volume and the limited on-board memory (xx MB memory for FlowRadar on P4 supports xx flows, but xx flows required).

%In summary, the state-of-the-art approximate solutions cannot support the primary zero-error task, loss detection, while exact solutions can only support loss detection.
%
% A naive solution is to build two sketches with memory size of A+B, while our design goal is to use one sketch with less memory than min{A, B}.

%Our design goal is to overcome the shortcomings of prior solutions and inherit their strengths: A measurement system that addresses both error-tolerant tasks and the loss detection with high memory efficiency.
\end{comment}


%yt comment
\begin{comment}

% Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}
% %sampling probing
% % probing?? which type?比如pingmesh 感觉一直不是flow level的测量对，probing是linklevel
% Based on the correctness of the statistics, existing flow-level measurement solutions can be classified into two types: 1) approximate solutions, including sketches and sampling, and 2) exact solutions, including FlowRadar and FlowTable. 
% % Recently, sketch-based solutions, where sketches are a kind of probabilistic data structures, have been widely acknowledged in network measurement \cite{sketchlearn2018,opensketch2013,zhang2021cocosketch,nitrosketch2019,ben2017constant}.
% %
% % Based on how to measure the network traffic, existing sketches can be divided into two kinds: 1) approximate solutions and 2) exact solutions. 
% %


% Recently, sketches, which achieve the best accuracy at a high throughput under tight memory limitations, become the most promising approximate solutions for error-tolerant measurement tasks, including flow size estimation \cite{ribeiro2006fisher}, heavy hitter detection \cite{bandi2007fast}, and more \cite{kumar2004data, lall2006data,zhao2007data}.
% %
% However, the estimation error of sketches prevents them from supporting error-sensitive measurement tasks requiring exact statistics.
% The primary one is the loss detection for fault diagnosis: Loss detection aims at finding the abnormal flows with packet losses exactly, which could be incurred by congestion \cite{dhamdhere2018inferring,fanou2017investigating}, link failures \cite{iannaccone2002analysis}, BGP misconfigurations \cite{mahajan2002understanding,feamster2005detecting}, and more \cite{gill2011understanding}.
% Existing loss detection solution relies on comparing the change of exact flow sizes between nearby forwarding nodes \cite{flowradar2016}.
% %误差容忍的sketch在解决这个问题的时候会表现非常差，因为估计的不准确导致被认为存在丢包
% The exact flow sizes are indispensable here because we cannot distinguish whether the change of the estimated flow size is due to the packet loss or the estimation error from the sketch itself.

% % However, the estimation error of sketches prevent them from supporting  tasks requiring exact statistics, \ie, \ykc{flow size change}. 
% % %
% % The primary one is the loss detection for fault diagnosis: loss detection aims at finding the abnormal flows with packet losses, which could be incurred by congestion \cite{dhamdhere2018inferring,fanou2017investigating}, link failures \cite{iannaccone2002analysis}, BGP misconfigurations \cite{mahajan2002understanding,feamster2005detecting}, and more \cite{gill2011understanding}.
% % Existing loss detection solution relies on comparing the change of exact flow sizes between nearby forwarding nodes \cite{flowradar2016},
% % %误差容忍的sketch在解决这个问题的时候会表现非常差，因为估计的不准确导致被认为存在丢包
% % \wyh{This task requires zero-error measurement instead of approximate solutions, because we cannot distinguish whether the change of the estimated flow size is due to the packet loss or the estimation error from the sketch itself.
% % }


% % The first kind is approximate solutions, which can provide approximation of desired statistics at a high throughput under tight memory limitations.
% % %
% % Typical solutions include CM \cite{cmsketch}, CU \cite{cusketch}, and Count \cite{countsketch}.
% % %
% % Due to the high accuracy and versatility of the newly proposed solutions \cite{elastic2018, univmon2016}, approximate solutions have become one of the most promising solutions for error-tolerant measurement tasks that allow limited amount of estimation error, including flow size estimation \cite{ribeiro2006fisher}, heavy hitter detection \cite{bandi2007fast}, entropy estimation \cite{lall2006data,zhao2007data}, and more \cite{kumar2004data}.
% % %
% % However, the estimation error of approximate solutions prevent them from supporting tasks that require zero-error measurement. 
% % %
% % The primary one is flow size change estimation, which provides basis for loss detection: By comparing the change of exact flow sizes between nearby forwarding nodes \cite{flowradar2016}, loss detection aims at finding the abnormal flows with packet losses, which could be incurred by congestion \cite{dhamdhere2018inferring,fanou2017investigating}, link failures \cite{iannaccone2002analysis}, BGP misconfigurations \cite{mahajan2002understanding,feamster2005detecting}, and more \cite{gill2011understanding}.
% % %误差容忍的sketch在解决这个问题的时候会表现非常差，因为估计的不准确导致被认为存在丢包
% % \wyh{This task requires zero-error measurement instead of approximate solutions, because we cannot distinguish whether the change of the estimated flow size is due to the packet loss or the estimation error from the sketch itself.
% % }


% The second type of solutions, exact solutions, including FlowRadar \cite{flowradar2016} and FlowTable \cite{?}, can address both error-tolerant and error-sensitive tasks.
% However, their memory overhead is proportional to the number of flows, which is intolerable considering the great traffic volume and the limited on-board memory (xx MB memory for FlowRadar on P4 supports xx flows, but xx flows required).


% % % The second kind is exact solutions.
% % %
% % Typical solutions include FlowRadar \cite{flowradar2016}, FlowTable \cite{?}.
% % %
% % \ykc{These solutions provide zero-error measurement for both error-tolerant and zero-error tasks.}
% % %
% % However, their memory overhead is proportional to the number of flows, which is unpractical considering the great traffic volume and the limited on-board memory (xx MB memory for FlowRadar on P4 supports xx flows, but xx flows required).

% In summary, the state-of-the-art approximate solutions cannot support the primary error-sensitive task, loss detection, while exact solutions suffer from high memory overhead.
% %
% Our design goal is to overcome the shortcomings of prior solutions and inherit their strengths: A measurement system that addresses both error-tolerant tasks and the loss detection with high memory efficiency.

% Design goal: cover both functions with smaller memory.
% A naive solution is to build two sketches with memory size of A+B, while our design goal is to use one sketch with less memory than min{A, B}.
\end{comment}

\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.98\linewidth]{wuyuhan/intro_graph2.pdf}
    \vspace{0.2cm}
    \caption{Design philosophy of \sketchname{}.}
    \label{intro:philo}
    \postfig
\end{figure}

\subsection{Our Approach}

% \wyh{
% Towards the design goal, we build a system, namely \systemname{}, which breaks the memory cost of each kind of tasks and can often outperform $min\{m_A, m_B\}$ at high speed.
% We introduce our observation and key techniques, followed by how we approach the design goal.
% }


Towards the design goal, we build a system, namely \systemname{}, to measure both kinds of tasks at the same time.
%ykc:好像不能说more
\systemname{} is generic, which addresses more measurement tasks than all existing works.
%
\systemname{} is memory efficient, which is close to the goal of less memory than $min\{m_A, m_B\}$.
%
\systemname{} is accurate, which is much more accurate than existing works using the same size of memory.
%
\systemname{} is fast, \wyh{where} each insertion only needs limited number of hash computations and memory accesses.
%
These advantages is owing to an observation and two key techniques as follows.



\wyh{Tri-hierarchy Observation:}
\bbb{Key observation:} 
We first analyze the information we need to save/store/record and the corresponding overhead.
%Despite the memory overhead, an ideal solution is to save/record all flow IDs and all flow sizes, like FlowRadar.
As shown in Figure \ref{intro:philo}, we divide the information into four parts\footnote{1...2...3..4..} ($\mathit{1},\mathit{2},\mathit{3},\mathit{4}$) according to the flow type (elephant or mice flows).
%
Among them, a few flows may experience flow size change, drawn by a red rectangle with $\mathit{5}$.
%
Below we classify them into three kinds with different priorities.
1) High priority. Elephant flows and flow size changes ($\mathit{1}$, $\mathit{2}$ and $\mathit{5}$) are the most important.
Fortunately in practice, the number of elephant flows is small \cite{univmon2016, elastic2018, zhou2018cold}. The number of flows with flow size changes is also small, otherwise there is serious problem which is easy to find \cite{lossradar2016}.
%
2) Middle priority. The frequency of mice flow ($\mathit{3}$) is less important. They can be used to partially estimation flow size distribution and entropy. These information can be compactly compressed due to the similarity of frequencies.
%
3) Low priority. The gray part, \ie, ($\mathit{4}$ minus $\mathit{5}$), which represents the IDs of normal mice flows without packet losses, is the least important, as none of existing measurement tasks need their IDs.
%
Simultaneously, the gray part is also the most memory-expensive part, because most flows are mice flows in practice as many literature pointed out \cite{univmon2016, elastic2018, zhou2018cold, ???}.

%yt comment
\begin{comment}
The number of large flows only takes up a small portion due to the skewness, and thus ($\mathit{1,2}$) only cost small memory; The flows with packet loss ($\mathit{5}$) only takes up a extremely tiny portion\footnote{Otherwise the problem is serious and easy to find \cite{lossradar2016}}; For small flows, compared to precisely recording their 104-bit IDs ($\mathit{4}$), approximately recording their small sizes ($\mathit{3}$) costs much less memory.
%
In summary, our observation is that the gray part is the most memory-expensive one but of the least importance.
%
Based on our observation, our design philosophy is to \textit{discard the worthless normal mice flow IDs (gray part), exactly measure the flows with packet losses ($\mathit{5}$), and estimate the other parts with tolerable error}.
%60是观察，系统基于观察，然后写philosophy，然后
%写细节怎么样

Toward the design goal, we design our system, namely \textbf{\systemname{}}, which is full of thrifty design choices in every part and every step.
Firstly, to separate $\mathit{1,2}$ and $\mathit{3,4}$, we design and use a flow classifier to identify mice and elephant flows.
The classifier is efficient that it can also estimate $\mathit{4}$ and a portion of $\mathit{2}$ with no additional overhead.
Then we use our key technique called \textbf{explicit-implicit} to set and distinguish the measurement strategy of elephant and mice flows, so as to achieve the best efficiency.
For elephant flows, we encode all IDs and flow sizes with explicit strategy, whose memory overhead should be close to the total amount of information in $\mathit{1}$ and the rest portion of $\mathit{2}$.
For mice flows, the challenge is that we cannot discard any flow, because any flow may have lost packets and we cannot identify it before all packets are inserted. In this case, the input is massive with a large amount of flows, but the output that we need is only the small amount of flows with packet loss ($\mathit{5}$).
%
We need an efficient implicit strategy to find $\mathit{5}$ and its memory overhead should be close to $\mathit{5}$, instead of all mice flows $\mathit{3,4}$.
%
\end{comment}

\bbb{Key idea I: Tri-Classification.} We propose to a tri-classification architecture to store the flow information with three parts: Part1) $<ID, frequency>$ of elephant flows; Part2) $<ID, frequency>$ of flows with frequency changes; Part3) shared frequencies of mice flows.
%
Our tri-classification just discards the ID of mice flows which is the most unimportant and memory consuming part.
%
Specifically, we borrow the idea of Cold filter which classifies the flows into two kinds.
%
Differently, we use TowerSketch to classify flows into three kinds: 1) design two error-less data structure to record Part1 and Part2 respectively; 2) approximately record Part3 in TowerSketch; and 3) discard ID of mice flows.
%
In one word, discarding low-priority information contributes a lot to approaching the design goal of using memory size less than $min{m_A, m_B}$.



\bbb{Key idea II: Fermat Sketching.} Classic error-less encoding is to use hash tables, which cannot achieve constant speed due to hash collisions. State-of-the-art solutions (\eg, Lossradar, FlowRadar) improves Invertable Bloom filters \cite{ibf???}, suffering from large memory overhead and complicated\wyh{??why?} operations because one flow could appear many times.
%
Differently, we leverage the Fermat's little theorem to significantly improve memory efficiency and simplify insertion operations (Section ??).
We furture improve efficiency by \textbf{rehash} (Section ??), substraction-modulo operation (Section ??), error-correction (Section ??).
Fermat Sketching further improves memory efficiency, and enable our solution reach the design goal.

%2) We achieve 20\% better memory efficiency by designing a verification without additional memory overhead, namely \textbf{rehash}; \textbf{really new???????}
%3) For hardware friendliness, we leverage the idea of modulo operation to address the overflow of registers and the self-erasure caused by XOR operation used in prior work \cite{lossradar2016}.
%4) We propose a new online query method and offline error correction strategy.

Further, for any given network, we propose a network-wide deployment strategy that only needs edge switches to support \systemname{} deployment to provide one-big-switch \cite{kang2013optimizing} abstraction. We propose and address the frequency changes with/no multicase and broadcase problem for the first time.



We build a testbed with 10 switches and 8 end-hosts connected with 40Gbe links in a FatTree topology. Our testbed includes all the above techniques and the following the following characteristics: 1) Zero-error over losses, 2) High memory efficiency, 3) Hardware friendly, and 4) supporting both online and offline query.
We implement ?? measurement tasks, and implement our algorithms in Tofino switches and ns-2.
%
Our experimental results 1) show that \systemname{} significantly improves the memory efficiency compared to prior art, 2) verify the correctness of the implementation of \systemname{} in P4 \cite{bosshart2014p4} and our network-wide deployment strategy, and 3) demonstrate that \systemname{} can measure the network traffic at 10-ms level time scale.



\begin{comment}
To meet the requirement of \textbf{explicit-implicit} in data plane, we devise a novel data structure called \sketchname{} with the following characteristics: 1) Zero-error over losses, 2) High memory efficiency, 3) Hardware friendly, and 4) supporting both online and offline query.
Our design benefits a lot from Invertible Bloom Lookup Table (IBLT) \cite{goodrich2011invertibleIBLT}, but we make novel contributions: 
1) To make IBLT support loss detection, we design the elastic operations, including subtraction, resizing, and merging.
2) We achieve 20\% better memory efficiency by designing a verification without additional memory overhead, namely \textbf{rehash};
3) For hardware friendliness, we leverage the idea of modulo operation to address the overflow of registers and the self-erasure caused by XOR operation used in prior work \cite{lossradar2016}.
4) We propose a new online query method and offline error correction strategy.

% Next, we devise the deployment strategy and implement \systemname{} in P4.
% With the design of \systemname{} and \sketchname{}, we then propose the deployment strategy and P4 \cite{bosshart2014p4} implementation to enable \systemname{} to function as a practical measurement system in a single switch.
%
%
Further, for any given network, we propose a network-wide deployment strategy that only needs edge switches to support \systemname{} deployment to provide one-big-switch \cite{kang2013optimizing} abstraction.
%
%Next, we propose the implementation of \systemname{} in P4. \cite{bosshart2014p4}.
%
We evaluate \systemname{} with various CPU simulation experiments and a testbed environment with 10 switches and 8 end-hosts connected with 40Gbe links in a FatTree topology.
%
Our experimental results 1) show that \systemname{} significantly improves the memory efficiency compared to prior art, 2) verify the correctness of the implementation of \systemname{} in P4 \cite{bosshart2014p4} and our network-wide deployment strategy, and 3) demonstrate that \systemname{} can measure the network traffic at 10-ms level time scale.
%
\end{comment}

%yt comment
\begin{comment}


% %para2
% Aiming at the optimization goal, we propose a system, namely \textbf{\systemname{}}.
% %The key technique of system is ex-im coding.
% The key technique of \systemname{} is called \textbf{explicit-implicit encode-decode}.  
% % 我们通过大小流过滤器分离大流和小流。对于条数众多的小流，使用极高压缩率（比大流高100倍）“隐式”地编码ID，其ID在丢包发生时可以被还原，其他时间不一定。虽然失去了还原所有小流ID的能力，但是节省了10倍的存储。实现了轻量性; 对条数较少的大流，使用“显式”的编码-解码方案记录完整ID和频数，其ID与频数任何时候均可还原，总开销可控且轻量。
% To distinguish $\mathit{1}$ and $\mathit{3}$, we first distinguish large flows and small flows through a flow classifier (\eg Cold filter \cite{zhou2018cold}.
% %
% Meanwhile, the flow classifier records all of $\mathit{4}$ and part of $\mathit{2}$ incidentally.
% %para3
% For a small number of large flows, we adopt the \textbf{explicit} encode-decode strategy to record their IDs ($\mathit{1}$) and extra sizes that cannot be recorded in the flow classifier (the rest part of ($\mathit{2}$).
% %
% For a large number of small flows, we adopt the \textbf{implicit} encode-decode strategy to record only the IDs and number of lost packets of the small flows experiencing packet losses, so as to discarding all of $\mathit{3}$ except $\mathit{5}$.

%为了支持显示隐式编码，我们需要一类数据结构。理想情况下他应该具有以下特性：1）提供无错的ID以及频数的查询；2）高效的内存利用率，当用于显示编码时，只需要O(F)的空间，当用于隐式编码时，只需要O(丢包流的大小）3）硬件友好，插入代价，仅需要少量的常数次哈希及访存（eg,3)就可以达到最高的内存利用率，支持并行插入。4）查询：既支持实时在线查询也支持解码后的精确查询
% To support \textbf{explicit-implicit encode-decode} as the encoder in data plane, we need a kind of data structures that ideally possessing the following characteristics:
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=0pt,partopsep=0pt]
    
%     \item \textit{Zero-error ID query}
    
%     \item\textit{High memory efficiency:}
    
%     \item\textit{Hardware friendly:}
    
%     \item\textit{Online and offline query:}
    
% \end{itemize} 
% %para4
% %为了满足这些特性，我们设计了sketch，他的key novelty包含两点:1)设计一种无内存开销的解码校验方法，rehash；2）是利用取模操作同时解决了寄存器溢出以及XOR操作的自消除问题；3）我们设计了sketch的弹性操作，包括他的resize，合并，相消操作，使其首次支持流级别的丢包查询。
% To satisfy these characteristics, we propose a novel sketch, namely \sketchname{}.
% %
% Its key novelties include: 
% 1) we design a verification method without memory overhead in decode process, namely \textbf{rehash};
% 2) leveraging modulo operation, we simultaneously address the overflow of registers and self-erasure problem caused by XOR operation used in prior work \cite{lossradar2016}, making it hardware friendly and memory efficiency;
% 3) we design the elastic operations of \sketchname{}, including resizing, merge, subtraction, making it support explicit-implicit encode-decode.

%
% %
% With the design of \systemname{} and \sketchname{}, we then propose the deployment strategy and P4 \cite{bosshart2014p4} implementation to enable \systemname{} to function as a practical measurement system in a single switch.
% %
% Further, we extend \systemname{} to a more realistic network-wide application scenario.
% %
% For any given network, we propose a deployment strategy that only needs edge switches to support \systemname{} deployment to provide one-big-switch \cite{kang2013optimizing} abstraction.

% We evaluate \systemname{} with various CPU simulation experiments and a testbed environment with 10 switches and 8 end-hosts connected with 40Gbe links in a FatTree topology.
% %
% Our experimental results 1) show that \systemname{} significantly improves the memory efficiency compared to prior arts, 2) verify the correctness of the implementation of \systemname{} in P4 and our network-wide deployment strategy, and 3) demonstrate that \systemname{} can measure the network traffic at 10-ms level time scale.
% %



























% \begin{figure}[t!]
%     \setlength{\abovecaptionskip}{0.15cm}
%     \setlength{\belowcaptionskip}{0cm}
%     \prefig
%     \centering  
%     \includegraphics[width=0.84\linewidth]{figure/algfiggure/FermatIntroArc.jpg}
%     \vspace{0.2cm}
%     \caption{Design philosophy of \sketchname{}.}
%     \label{intro:philo}
%     \postfig
% \end{figure}

% \subsection{Background and Motivation}
% %网络测量对很多网络成功的网络操作很重要
% Network measurement is indispensable to successful network operations, including traffic engineering \cite{?}, congestion control \cite{hpcc?}, network accounting and billing \cite{?}, anomaly detection \cite{?}, load balancing \cite{?}, \etc{}.
% %
% Recently, Sketches, a kind of probabilistic data structures, have been widely used to perform flow-level network measurements \cite{??}, and the vast majority of them focus on measurement tasks associated with flow sizes. 
% %
% %根据flow size，有三种任务受到广泛的关注：估计每流的flow size，汇报flow size 大的流，汇报flow size 在相邻节点异常变化的流,\ie,packet losses
% Of these tasks, based on different application-level metrics of interest, three have grabbed widespread attention: 1) flow size estimation \cite{?}; 2) heavy hitters \cite{?}; 3) packet loss detection \cite{?}.

\end{comment}

%yt comment
\begin{comment}
\subsection{Background and Motivation}
%网络测量重要性，引出sketch。
Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{hpcc?}, network accounting and billing \cite{?}, anomaly detection \cite{zhang2013adaptive}, load balancing \cite{?}, \etc{}.
%现有sketch在容许误差的任务上做得很好
Recently, sketching algorithms (and sketch-based systems), which can provide high-accuracy approximate statistics at a high throughput under tight memory limitations, become one of the most promising solutions for error-tolerant measurement tasks that allow limited amount of estimation error, including flow size estimation \cite{?}, heavy hitter detection \cite{?}, entropy estimation \cite{?}, and more \cite{?}.

%现有sketch的误差导致它们无法精确检测丢包。
However, the estimation error of existing sketch prevents it from 
% existing measurement tasks requiring zero-error measurement are not well addressed. 
%
The primary one is the loss detection for network fault diagnosis: By comparing the change of exact flow sizes between nearby forwarding nodes, loss detection aims at finding the abnormal flows with packet losses, which could be incurred by switch faults, misconfiguration, or more \cite{flowradar2016}.
%误差容忍的sketch在解决这个问题的时候会表现非常差，因为估计的不准确导致被认为存在丢包
\wyh{This task requires zero-error measurement instead of existing sketches with errors, because we cannot distinguish whether the change of the estimated flow size is caused by the packet loss or errors from the sketch itself.
}
%是不是把2123删了 是 ok
%\ykc{For existing sketches that provide approximate estimation, the estimation error is not concentrated in a few flows, but widely spread in every flow.
%
%For two nearby forwarding nodes, when adopting different hash functions, the flow size estimation for every flow may differ between the two nodes, and thus any flow could be identified as experiencing losses even no packet is lost at all.
%To address loss detection
To address loss detection, a straightforward solution is to achieve zero-error measurement.
%
However, the dilemma between accuracy, memory, and throughput stops us.
%我们希望实现一个起到"无误差"功能的"带误差"测量系统。 
Instead, our key insight is that zero-error measurement is not necessary to a great extent: sketches can still provide approximate estimation for error-tolerant tasks, but should provide zero-error measurement for flow size change to support loss detection.
%, as long as the sketch with errors can detect packet losses with no error, because detecting packet losses is the primary function of zero-error measurement as we know.


\subsection{Limitations of Prior Art and Our Goal}

Although prior measurement efforts have made great progresses, they cannot support both error-tolerant tasks and the loss detection with high throughput and limited memory.
%
\ykc{Based on the whether there is error in the measurement, We divide prior solutions into two kinds: 1) exact solutions and 2) approximate solutions.}
%
The first kind is the exact solutions, including FlowRadar \cite{flowradar2016}, Flowtable \cite{?}.
%
\ykc{These solutions provide zero-error measurement for all tasks.}
%
However, their memory overhead is proportional to the number of flows, which is unpractical considering the great traffic volume and the limited on-board memory (xx MB memory for FlowRadar on P4 supports xx flows, but xx flows required).
%
The second kind is the approximate solutions, including NitroSketch, Elastic Sketch \cite{?}, and UnivMon.
%
\ykc{These solutions provide accurate estimation for error-tolerant tasks with high memory efficiency and throughput, and thus cannot well handle the loss detection.}
%
Our design goal is to overcome the shortcomings of prior solutions and inherit their strengths: A measurement system that addresses both error-tolerant tasks and the loss detection with high memory efficiency and throughput.

\end{comment}

%yt comment
\begin{comment}
% %
% Although prior sketch-based solutions have made great contributions, they cannot support all the above tasks with high accuracy under limited memory.
% %
% FlowRadar, a solution designed for merchant silicon, support all the above tasks by encoding and decoding the IDs and sizes of all flows with zero error.
% %
% However, its memory overhead is proportional to the number of flows, which is unacceptable and unpractical considering the rapidly growing traffic volume and the limited on-board memory.
% %
% Other state-of-the-art sketches, including NitroSketch, Elastic Sketch \cite{?}, and UnivMon, can provide accurate flow size estimation with high memory efficiency.
% %
% However, they do not record IDs of small flows, and thus cannot support packet loss detection of small flows.
% %
% %
% Our design goal is to overcome the shortcomings of prior solutions, designing a measurement system that supports all the three tasks with high memory efficiency.
% %现有算法在有限内存下无法在大流量场景高精度support上述任务
% %
% %现有算法分为两类：一类支持上述任务但开销巨大（flowradar)，有限的交换机内存难以支持大规模的流量
% %一类开销小但不支持上述任务：elastic，丢掉了小流id，无法检测丢包小流的ID。
% %我们的设计目标是克服现有方法的缺陷，设计一个内存高效并且同时支持以上所有任务的测量系统。



%para1
% %针对我们的设计目标，我们首先对（需要记录的？？？）信息进行了分析。
% Towards our design goal, we first analyze all the information in the network traffic that benefits the target tasks.
% %如图所示，根据流大小(large or small flows) 和信息类型(ID or frequency)，我们将信息分为四类。
% As shown in Figure \ref{inro:philo}, based on flow sizes (large or small flows) and information types (ID or flow sizes), we We divide all the information into four categories.
% %从重要性角度考虑（支持测量任务的能力），124全部信息是较为重要的，3中的少部分信息是重要的（丢包小流的ID 5).
% From the viewpoint of importance, \ie, how can the information benefit the target tasks, $\mathit{1}$, $\mathit{2}$, $\mathit{4}$, and a small amount of $\mathit{3}$ (the IDs of small flows experiencing packet losses) are relatively important.
% %从资源开销角度考虑，由于扭曲的数据分布，大流条数较少，因此12占用的资源较少；相比于精确记录完整的13-byte ID，近似记录小流频数的开销小得多（2-4 bit per flow in experiments)。3占据了绝大多数资源。
% From the viewpoint of memory overhead, considering the skewness in the network traffic \cite{?}, the number of large flows takes up only a tiny portion, and thus $\mathit{1}$ and $\mathit{2}$ only occupy a small amount of memory; For small flows, compared to precisely recording their 104-bit IDs ($\mathit{3}$), approximately recording their small sizes ($\mathit{4}$) occupy much less memory.
% %根据CAIDA上的实验，3占据了多少资源
% According to our experiment in well-known CAIDA dataset, $\mathit{3}$ occupies almost xx\% memory.
% %In summary， 3的开销最大但重要性最低，\textbf{是我们需要优化的主要对象。}
% In summary, our observation is that $\mathit{3}$ occupies most of the memory, but offers least benefits ($\mathit{5}$) to the target tasks.
% %
% Therefore, \textit{how to discard the worthless information of $\mathit{3}$ without involving $\mathit{5}$ is the main optimization goal of this paper}.
% %
% %现有第一类工作如flowradar记录了1234，因此开销巨大
% %FlowRadar records all of $\mathit{1}$, $\mathit{2}$, $\mathit{3}$, and $\mathit{4}$, and thus needs high memory overhead.
% %第二类工作例如elastic完全舍弃了3，因此缺失了检测小流丢包的重要功能。
% %Other solutions, such as Elastic Sketch, completely discard $\mathit{3}$, and thus cannot support loss detection of small flows.

\end{comment}

==> NSDI2023/newintro.tex <==
Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}
%
Recently, sketches, a kind of probabilistic data structures, have been widely used to support network flow-size-based measurements tasks \cite{?}.
%
Based on the intents of network operators, flow-size-based measurement tasks could be divided into two kinds. 
%

%wyh: vantage point感觉有点奇怪？有人用过这个表达？
The first kind of measurement tasks focus on measuring network traffic at a fixed vantage point, including flow size estimation \cite{ribeiro2006fisher}, heavy hitter detection \cite{bandi2007fast}, and more \cite{kumar2004data, lall2006data,zhao2007data}.
%
These tasks require only approximate statistics of flow sizes, as small error in flow sizes only slightly degrades their accuracy.
%
Typical sketches for these tasks include Elastic, and UnivMon.
%because the measurement results .%??

The second kind of measurement tasks focus on measuring the anomalies in the transmission of network traffic, and the primary one is packet loss detection, \ie, detecting the flows whose sizes shrink in a given network/link.
%
In contrast, these tasks require exact statistics of the change of flow sizes, because we cannot distinguish whether the change is due to the packet loss or the estimation error from the sketch itself.
%
Typical sketches for these tasks include LossRadar.

An ideal measurement should support both two kinds of measurement tasks simultaneously, and a naive solution is to build one sketch for the first kind of tasks, and build another sketch for the second kind of tasks.
%
Suppose the memory overhead of the first sketch is $A$, and that of the second sketch is $B$.
%
The naive solution support both kinds of tasks with memory of $(A+B)$, while our design goal is to only use memory less than $min\{A, B\}$.


==> NSDI2023/singledevice.tex <==
%system是设计出来支持flow sketching 和loss detection。
%我们简述他的workflow

%loss detection requirement:我们不能丢弃任何ID信息
%flow sketching requirement: 能够还原任何大流ID；能够估计全流频数
%Resource requirement:



==> SIGCOMM23/intro.tex <==
\presec 
\section{Introduction} 
\postsec

%网络测量很重要,流级别测量逐渐成为工业界的共识
Network measurement provides critical statistics for various network operations, such as traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, and failure troubleshooting \cite{handigol2014know,netbouncer2019}.
% %
In earlier years, sampling-based solutions \cite{everflow2015,netflow2004,sflow2001,csamp2008} were widely accepted in network measurement thanks to their simplicity and ease of use.
%
More recently, emerging sketch-based solutions \cite{elastic2018,zhang2021cocosketch,nitrosketch2019,sketchlearn2018} have become more promising than sampling-based ones, as they are designed to approach the ultimate goal of network measurement \cite{univmon2016,beaucoup2020,zheng2022flymon}: to support more tasks and achieve higher accuracy with less memory.


Network measurement tasks can be mainly classified into two kinds.
%
The first kind focuses on frequency accumulation tasks that are error-tolerate, including flow size estimation \cite{cmsketch}, heavy-hitter detection \cite{sivaraman2017heavy}, heavy-change detection \cite{schweller2004reversible}, \etc.
%
The second kind focuses on frequency difference tasks that should be zero-error, and the most representative one is packet loss detection \cite{lossradar2016}.


Existing sketch-based solutions can be mainly classified into three categories according to supported tasks:
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]


    
    \item \textit{1) Solutions for frequency accumulation tasks:}
    Typical solutions include UnivMon \cite{univmon2016}, Hashpipe \cite{sivaraman2017heavy}, Sketchlearn \cite{sketchlearn2018}, ElasticSketch \cite{elastic2018}, and more.
    %
    Their memory overhead are typically sub-linear to the number of flows as they embrace hash collisions and select the estimation with least collisions to minimize error.
    %
    
    \item \textit{2) Solutions for frequency difference tasks:}
    Typical solutions include LossRadar \cite{lossradar2016}, and its memory overhead is linear to the number of lost packets.
    %
    \item \textit{3) Solutions for both kinds of tasks:}
    These solutions support both kinds of tasks by recording exact IDs and sizes of all flows, including FlowRadar \cite{flowradar2016}, Counter Braids \cite{lu2008counter}, and more.
    %
    Therefore, their memory overhead are linear to the number of flows.
\end{itemize}






Among all flow-level measurement tasks, packet loss detection and heavy-hitter detection attract the most attention, which we call two \textit{key tasks}.
%
However, the two key tasks are seldom considered and supported simultaneously in one solution.
%
One reason behind is that solutions designed for packet loss detection and solutions designed for heavy-hitter detection usually differ significantly in data structures and operations.
%and therefore most solutions only support \ykc{either one}.
%但是在一个practical的network，两类任务都是要检测的。
%However, both tasks are required in a real-world scenario.

However, in practice, the two key tasks are often required at the same time, and there are only limited resources for measurement in programmable switches.
%我们需要构建一个灵活的/flexible，完备的，高效的/efficicent测量系统，可以调和这两种测量任务.
%
Therefore, the \textit{first requirement} for a practical measurement system is versatile to support the two key tasks with high accuracy using limited resources, where limited resources refer to sub-linear space complexity.
%

Based on the first requirement, the \textit{second requirement} is to pay attention to different key tasks for different network states.
% Based on the first requirement, further, the system should have different measurement attention for different network states.
% Based on the first requirement, a practical system further requires the attention to different tasks as the network state changes.
% %
% Based on the first requirement, a practical system further requires the attention on different tasks to change according to the network state.
% Based on the first requirement, a practical system further requires automatically shifting its attention between the above two tasks as network condition changes.
% Based on the first requirement, a practical system should pay different amount of attention to different tasks under different network conditions.
% Based on the required two tasks, a practical system requires shifting its attention between the above two tasks as network condition changes.
% Based on the first requirement of both tasks, a practical system requires shifting its attention between the two tasks as network condition changes.
%
% The network condition frequently changes, placing different demands on the resources for packet loss detection and heavy-hitter detection over time.
When the network state is healthy and there are only few packet losses in the network, the system should pay more attention (\eg, allocate more memory) to heavy-hitter detection.
%
When the network state is ill and there are lots of packet losses in the network, the system should pay more attention to packet loss detection, especially for those flows which experience a great number of packet losses.

% The network condition frequently changes, placing different resource demands on packet loss detection and heavy-hitter detection.
% %
% Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
% %
% Therefore, the second requirement for a practical measurement system is to self-adapt to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%加变色龙 shift focus attention 关键词。

% Meeting the above two requirement is not enough.
% %
% For example, we use a great amount resource. can meet ...
% Third...
% Besides from above two requirements, our third requirement is the high resource efficiency, \ie, high accuracy under limited resources. 
% leverage the limited resources to provide high accuracy results as much as possible
% The measurement system should leverage the limited resources to provide high accuracy results as much as possible.
% , To avoid occupying the resources for main network functions,
% In summary, it is desired to design a \ykc{comprehensive/universal/generic/versatile/multi-function}, self-adaptive, and efficient measurement system.
In summary, it is desired to design a practical measurement system with the following requirements: \textbf{[R$_{1.1}$]} \textit{versatility requirement}: supporting both packet loss detection and heavy-hitter detection simultaneously; \textbf{[R$_{1.2}$]} \textit{efficiency requirement}: achieving high accuracy with sub-linear space complexity; \textbf{[R$_{2}$]} \textit{attention requirement:} paying attention to different key tasks for different network states.

% %这样的测量系统需要三点：1）支持两类任务；2）运行时自动地调整内存以适应网络状况的变化 3）accurate。
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]

%     \item \textbf{[R1]} \textit{Comprehensiveness requirement.}
    
%     \item \textbf{[R2]} \textit{Self-adaptation requirement:}
%     The network condition inevitably changes as time elapses, placing different demands on the resources required for packet loss detection and heavy-hitter detection at different time.
%     %
%     Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
%     %
%     Therefore, the system is desired to be self-adaptive to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%     % first allocating appropriate resources for the packet loss detection to guarantee its accuracy, and then allocating the remaining resources for \ykc{other tasks}.
    
%     \item \textbf{[R3]} \textit{Efficiency requirement:}
%     \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
%     %
%     Therefore, the system is desired to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.
%     %, so as to avoid limiting the main network functions running on switches.
%     % However, it records all the IDs and frequencies of flows in a zero-error manner, and thus requires unacceptable memory overhead.
%     %
% \end{itemize}
% % Besides the above two requirements, we find the efficiency is also a key requirement of the practical measurement system.
% %
% \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
% %
% Therefore, the third requirement for a practical measurement system is to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.


% %
% In addition, the system should also be self-adaptive, and memory efficient.




% Therefore, it is desired to design a \ykc{comprehensive/universal/generic/versatile/multi-function}, self-adaptive, and efficient measurement system that meets the following three \ykc{corresponding} requirements:
% %
% %这样的测量系统需要三点：1）支持两类任务；2）运行时自动地调整内存以适应网络状况的变化 3）accurate。
% \begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]

%     \item \textbf{[R1]} \textit{Comprehensiveness requirement:}
%     Both packet loss detection and heavy-hitter detection greatly benefit the smooth functioning/running of the network.
%     %
%     For example, packet loss detection benefits diagnosis of network failures \cite{007-2018} and service-level agreement (SLA) delivery \cite{netseer2020};
%     %
%     heavy-hitter detection benefits load balancing \cite{curtis2011devoflow,al2010hedera}, DDoS attack detection \cite{lakhina2004characterization}, and traffic engineering \cite{benson2011microte}. 
%     %
%     Therefore, the system is desired to be comprehensive, supporting both tasks simultaneously.
%     %尽管相比正常任务，异常任务更能反应应用质量以及网络状况，也因此有助于诊断网络故障，正常任务所提供的信息往往也是许多网络功能不可或缺的，例如TE，LB，counting。因此，系统被期望同时支持两类任务
    
%     \item \textbf{[R2]} \textit{Self-adaptation requirement:}
%     The network condition inevitably changes as time elapses, placing different demands on the resources required for packet loss detection and heavy-hitter detection at different time.
%     %
%     Of these two tasks, packet loss detection is considered as more important because it directly characterizes application performance and user experience.
%     %
%     Therefore, the system is desired to be self-adaptive to real-time network condition at run-time in the following manner: first adjusting the resources for accurate packet loss detection according to the changes of network condition, and then allocating the remaining resources to heavy-hitter detection.
%     % first allocating appropriate resources for the packet loss detection to guarantee its accuracy, and then allocating the remaining resources for \ykc{other tasks}.
    
%     \item \textbf{[R3]} \textit{Efficiency requirement:}
%     \ykc{The most fundamental function of the network is to transmit the packets from source hosts to destination hosts, which consumes a large amount of various resources.}
%     %
%     Therefore, the system is desired to be efficient, achieving high accuracy while only consuming resources that are sub-linear with the number of flows, including memory, bandwidth, \etc{}, so as to avoid limiting the main network functions.
%     %, so as to avoid limiting the main network functions running on switches.
%     % However, it records all the IDs and frequencies of flows in a zero-error manner, and thus requires unacceptable memory overhead.
%     %
% \end{itemize}
% The system should meet the following three requirements: \textbf{[R1]}, supports both anomaly and normal tasks; \textbf{[R2]}, automatically adapts to the change real-time network condition; \textbf{[R3]}, consumes only a small amount of memory/bandwidth.
% %
% First, the system should support both anomaly and normal tasks simultaneously, considering that both provide \ykc{critical statistics of interest for different applications}.%表现出应用的需要。
%考虑到交换机极其有限的资源，我们应该尽可能最大化给定的内存的利用率。当网络状况良好，丢包数量少时，我们应该最小化用于检测丢包的资源，将资源尽可能用于支持普通任务。
%Considering the 10MB-level memory in switches, typically there is only a small portion of memory 
%Second, the system should automatically adapt to the real-time network condition, considering that the network condition is changeable and places different demands on the resources/memory required for different measurement tasks at different time.
%the dynamic network condition places different demands on the memory required for the packet loss detection at different time.
%

%
%
% When the network condition is fine and only a few flows experience packet losses, which we call victim flows, the system should minimize the memory for packet loss detection, and allocate the remaining memory for other tasks.
% %
% When the network condition is poor and the given memory cannot capture all the victim flows, the system should first capture the most valuable victim flows with most of the memory, which could be victim flows with large frequency or user-specified \wyh{high-priority} flows, and we call these flows \textit{heavy-losses}.
%

%

%当网络很恶劣的时候，已有资源无法检测all-loss，我们应该主要检测最重要的丢包（heavy-loss），丢包的大流或者用户指定的高优先级流，用最有限的memory记录最有价值的信息。
%
%总而言之，我们想要一个能同时支持两类任务，自适应网络状态，且始终最大化资源利用率和支持最重要任务的测量系统。

%1.2
% 1.1 采样算法
% 1.2 sketch 算法。
% 1.3 measurement system
% 提出了很多sketch，most只能做一类，数据结构上的特点：对sketch，error changes smoothly with memory change， Lossradar直接降为0
% %
% 还有一些versatile sketch UNivmon，Elastic,FLyMon,Beaucoup，LightGuardian支持4-10没有touch丢包的问题，不好直接扩展，唯一一个两类都做的是flowradar，不满足r2，以及r3。
%Although researchers and engineers have proposed various solutions for network measurement, none of them meets the above three requirements simultaneously.
% %
%根据测量目标，我们将现有工作分为三类，我们分别讨论其中的代表工作是否满足上述三个要求。
Existing solutions can be mainly classified into three categories according to supported measurement tasks:
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]


    
    \item \textit{1) Solutions for packet loss detection:}
    Typical solutions including LossRadar \cite{lossradar2016} based on Invertible Bloom filter \cite{eppstein2011s}, NetSight \cite{handigol2014know} based on in-band network telemetry (INT), Netseer \cite{netseer2020} based on the advanced features of programmable switches, and more.
    %
    These solutions fail to meet \textbf{[R$_{1.1}$]} because they do not handle heavy-hitter detection.
    %
    
    \item \textit{2) Solutions for heavy-hitter detection:}
    These solutions are usually based on sketches, including HashPipe \cite{sivaraman2017heavy}, UnivMon \cite{univmon2016}, ElasticSketch \cite{elastic2018}, BeauCoup \cite{beaucoup2020}, and more.
    %
    %
    These solutions fail to meet \textbf{[R$_{1.1}$]} because they do not handle heavy-hitter detection.
    \item \textit{3) Solutions for both tasks:}
    These solutions support both tasks by recording exact IDs of all flows, including FlowRadar \cite{flowradar2016}, OmniMon \cite{omnimon2020}, Counter Braids \cite{lu2008counter}, and more.
    However, recording exact IDs of all flows requires memory/bandwidth overhead linear with the number of flows.
    %
    Therefore, these solutions fail to meet \textbf{[R$_{1.2}$]}.
\end{itemize}

%In summary, no existing solution meets the three requirements.%做不了的本质原因是异构性，这导致A+B也不行
%现有算法做不了，除了第三类，前两类不能解决，flowradar这类需要所有的ID和counter，总space的开销超过了完美哈希表所需要的空间，linear space complexity，我们追求sublinear，其中一种是A+B，A+B可以做到sublinear不同构
In summary, the first two categories of solutions cannot meet \textbf{[R$_{1.1}$]} due to their limited measurement capabilities, and the third category of solutions cannot meet \textbf{[R$_{1.2}$]} due to their linear space complexities.
%
A naive solution meeting both \textbf{[R$_{1.1}$]} and \textbf{[R$_{1.2}$]} is to combine the first two categories of solutions: choosing one solution in each category to detect heavy-hitters (HHs for short) and packet losses, respectively.
%
% For example, the solution uses LossRadar for packet loss detection and uses Elastic Sketch for heavy-hitter detection.
%这个问题很challenge
%提r1 r2的全称
However, such a combination fails to achieve \textbf{[R$_{2}$]} on programmable switches. 
%
The reason behind is that the data structures and operations of different categories of solutions usually differ significantly\footnote{For example, LossRadar \cite{lossradar2016} records the IDs and existences of packets using XOR operation and addition, while HashPipe \cite{sivaraman2017heavy} records the IDs and sizes of flows using comparison, substitution, and addition.},
% \footnote{To support packet loss detection that requires zero-error estimation of flow size changes across switches, the first category of sketching algorithms chooses to eliminate hash collisions through decoding.
% %
% In contrast, to support heavy-hitter detection tolerates limited error, the second category of sketching algorithms chooses to embrace hash collisions and select the estimation with least collisions to minimize error.
% %
% Therefore, the data structures of the two categories of sketching algorithms are inherently heterogeneous.
% %
% The first category cannot support query before decoding, while the second category supports direct query;
% %
% As memory increases, the error of the first category sharply decreases around a sharp threshold, while the error of the second category decreases smoothly.}
and therefore the solutions in different categories can only utilize their resources allocated at compile time, which prohibits flexible allocation of memory resources between packet loss detection and heavy-hitter detection.
%
Therefore, the naive solution cannot pay attention to different key tasks for different network states.
%
%一类加法和替换，异或加法，没有替换，误差的角度一类平滑变化，一类有threshold，directly
%第一类拥抱冲突，选择冲突最弱的估计值，第二类通过复杂的解码消除冲突。这第一类支持直接查询，误差平滑变化，第二类不支持直接查询，误差有sharp threshold, sharply changes,这导致他们的数据结构有本质的不同。
%

% and thus different solutions cannot share the resources at run-time when the resources required for different measurement tasks change.

% However, the data structures of the two solutions for combination are \ykc{usually} heterogeneous, and thus they can hardly share memory with each other to adapt to real-time network condition.

% Towards the desired measurement system, a straightforward solution is to combine solutions for packet loss detection and solutions for heavy-hitter detection, so as to meet \textbf{[R1]} and \textbf{[R3]} simultaneously.
% %


%
%\ykc{To address this issue}, we design \systemname{}.%满足三个要求，做其他测量任务，实现了一个testbed，优化精度。
%

%key idea
In this paper, we design \systemname{}, which meets all the above requirements simultaneously.
%
Besides the two key tasks, \ie, packet loss detection and heavy-hitter detection, \systemname{} can support five common measurement tasks. 
%
Compared to the state-of-the-art solutions, for packet loss detection, \systemname{} reduces the memory overhead from proportional to the number of all flows (FlowRadar) or lost packets (LossRadar), to proportional to the number of flows experiencing packet losses, which we call \textit{victim flows}; 
%t
for heavy-hitter detection and the other five tasks, \systemname{} achieves at least comparable accuracy.
%
%We further build a prototype to verify the efficiency and the capability to self-adapt to real-time network condition of \systemname{}.
Our \systemname{} has a key design and a key technique as follows.


%Shift and focus the attention
The key design of \systemname{} is to shift measurement attention as network state changes, which is just like the process of the chameleons changing their skin coloration, through two dimensions of dynamics:
1) dynamically allocating memory between the two key tasks; 2) dynamically monitoring the flows of importance.
%
First, \systemname{} monitors the network state and allocates memory between the two key tasks accordingly.
%
When the network state is healthy and only a few packet losses occur in the network, \systemname{} pays most attention to and allocates most of the memory for heavy-hitter detection.
%
As the network state degrades and packet losses increase, \systemname{} gradually shifts measurement attention to and allocates more and more memory for packet loss detection.
%
Second, \systemname{} ranks the flows according to their importance, and selects those of most importance to monitor.
% For packet loss detection, 
When the network state is ill and there are too many victim flows in the network, \systemname{} selects those flows experiencing many packet losses (called \textit{heavy-losses}, HLs for short) to monitor, instead of monitoring all victim flows.
%

%写一个总结串一下这个过程。
%
Overall, when the network state continuously degrades from the healthy state to the ill state, \systemname{} runs as follows.
%
%
1) As the number of victim flows increases, \systemname{} leverages the first dimension of dynamic: gradually shifting measurement attention to and allocating more and more memory for packet loss detection;
%
2) When the victim flows are too many to monitor, \systemname{} leverages the second dimension of dynamic: focusing measurement attention on HLs while monitoring a small portion of other packet losses (named \textit{light-losses}, LLs for short) through sampling.

% Based on the number of victim flows in the network, we classify the network state into three levels, each of which is represented by one color widely used in traffic lights, \ie, green, yellow and red.
% %
% When the network state is at green level, there are only rare packet losses in network.
% %
% While it is not trivial to identify heavy-losses during monitoring, our observation is that large flows are more likely to become heavy-losses, because they can lose more packets and should lose more packets for the same network state compared to small flows.
% % %
% because small flows cannot lose too many packets due to their limited flow sizes.

% Therefore, \systemname{} selects those large victim flows to monitor to approximate the monitoring of heavy-losses.
%
% 
% For such network state, \systemname{} pays most attention to and allocates most of the memory for heavy-hitter detection, and only reserves a small amount of memory for packet-loss detection to handle the potential small burst of packet losses.
% %
% As the network state degrades and packet losses increase, the network state transitions to yellow level when the reserved memory cannot monitor all the victim flows.
% %
% For such network state, \systemname{} gradually shifts measurement attention to and allocates more and more memory for packet loss detection.
% %
% As the network state further degrades and packet losses further increase, the network state transitions to red level when \systemname{} cannot allocate more memory for packet loss detection and fails to monitor all the victim flows.
% %
% For such network state, \systemname{} gradually pays most measurement attention to and allocates most of the memory for packet loss detection, so as to monitor all the heavy-losses and a portion of light-losses.
%Similarly, for heavy-hitter detection, \systemname{} selects the largest flows to monitor when the allocated memory cannot monitor all the flows.


% %The key technique is our system is to leverage Fermat's Little Theorem theorem to devise a generic and compact data structure to support heavy hitters and packet losses simultaneously.
To realize the key design, \systemname{} incorporates a key technique, leveraging Fermat's little theorem\footnote{Fermat's little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$.} to devise a flexible data structure, namely \textit{\sketchname{}}.
%
The data structure of \sketchname{} is made of many same units.
%
\sketchname{} is dividable, additive, and subtractive, supporting packet loss detection and heavy hitter detection simultaneously.
%
%By partitioning \sketchname{} into three parts, and using each of them to support heavy-loss detection or heavy-hitter detection, \systemname{} can flexibly move the partition points to shift attention and allocate memory between the  two key tasks as network state changes.
%
By dividing \sketchname{} into three parts to detect HLs, LLs, and HHs, \systemname{} can flexibly move the division points to shift attention and allocate memory between the two key tasks as network state changes.
%
%When \systemname{} cannot monitor all victim flows, \systemname{} further partitions the part that supports packet loss detection into two parts, so as to monitor heavy-losses and light-losses separately.
%
For each incoming packet, We further use a flow classifier (TowerSketch \cite{yang2021sketchint}) to determine which of the three parts to insert.
%
For packet loss detection, owing to Fermat's little theorem, \sketchname{} only requires memory proportional to the number of victim flows. 
%
Differently, the state-of-the-art solutions require memory proportional to the number of all flows (FlowRadar) or lost packets (LossRadar).
%
%

Thanks to the visibility to per-flow size provided by Towersketch, \systemname{} can support five other common measurement tasks, including flow size estimation, heavy-change detection, flow size distribution estimation, entropy estimation, and cardinality estimation.
%
We have fully implemented a \systemname{} prototype on a testbed with a Fat-tree topology composed of 10 Tofino switches and 8 end-hosts.
%
We conduct extensive experiments and the results show that \systemname{} supports both kinds of tasks with low memory/bandwidth overhead, and more importantly, it can automatically shift measurement attention as network state changes at run-time.
%
We have released all related source codes at Github\footnote{\url{https://github.com/ChameleMoncode/ChameleMon}}.
%我们用一个分流器去决定每一个数据包应该进入三个部分中的哪一个部分。

%记录频数信息，做common tasks

% To further identify heavy-hitters and heavy-losses that are selected to monitor, \systemname{} deploys a TowerSketch \cite{yang2021sketchint} before \sketchname{}es.
%

% %
% By querying flow sizes, \systemname{} can easily identify selected flows for heavy-hitter detection using a threshold, but still has no visibility to heavy-losses that experience most severe packet losses.
%数据结构 同时支持两个   一套机制数据结构一分为二 切分点来回漂移  可任意切分 灵活切分 一部分做hh，一部分HL，切分点运行时可以自动漂移。
%可切分可合并可组合  可加可减   灵活flexible 
%


%设计一套机制，将数据结构一分为几，支持多种任务

%when the network state is excellent and there is almost no victims flows in the network, the allocated memory cannot measure all the flows and we measure those heavy flows 
%
% \sketchname{} can support both packet loss detection and heavy-hitter detection with homogeneous data structures.
% The homogeneity facilitates \systemname{} to flexibly adjust the memory size of \sketchname{} for supporting each task by simply changing its available range of index, enabling dynamic memory allocation between the two tasks at run-time.
% %
% \sketchname{} significantly reduces the memory overhead for packet loss detection from being proportional to number of flows (FlowRadar) or lost packets (LossRadar) to being proportional to number of victim flows, so as to achieve low memory/bandwidth overhead.
% %

%
% Then, \systemname{} allocates the memory for each task according to its number of selected measurement objects.
%

%
%In practice, \systemname{} always reserves a portion of memory for heavy-hitter detection to maintain minimal support for it.
%系统的key idea是通过两方面的动态调整来自动适应实时网络状态: 1) 动态地为不同地测量任务选择最有价值地测量目标 2)根据选择的目标动态地为不同测量任务分配内存
%
%这两个动态性依次作用以完成自适应
%
%首先，系统感知到需要测量的总目标的数量以及分布，包括全部流的ID以及其进入网络时频数，以及丢包流的ID以及其在网络中丢失的包数。
%
%第二，系统根据目标的重要性排序，对于流内部来说，越大越重要，对于丢包流来说，也是越大越重要，正常来说，所有的丢包流都比正常流重要。其中有一部分大流是特殊的，因为我们想始终维持对一部分大流的可见性。
%
%第三依据排序，系统根据已有的资源，利用阈值选定top-k需要测量的目标。
%第四，依据选定的测量目标向对应的任务分配内存。
%
%
%基于总内存的限制，我们选择
% The key idea of \systemname{} to adapt 
% %在runtime随着网络状态好坏的变化runtime动态自动分配给heavy-hitter和packet loss detection.
% %这个有什么好处，需要什么技术。
% The key idea of \systemname{} is to dynamically allocate memory for each task at run-time as network condition changes, which is just like the process of the chameleons changing their skin coloration.

% first sense the real-time network condition, and then properly allocate the memory for different measurement tasks based on the sensed condition, which is just like the process of the chameleons changing their skin coloration.
% %
% Based on the three \ykc{primary} colors, we coarsely classify the network condition into three states.
% %
% The first state is \textit{green}, that the network condition is excellent and the packet losses are rare\wyh{/nearly-zero}.
% %
% Under green network condition, \systemname{} uses most of the memory to support \ykc{normal} tasks with high accuracy, while reserving a fixed small amount of memory to handle the potential small burst of packet losses.
% %
% As the network condition degrades, when the reserved small memory cannot record all the flows experiencing packet losses, which we call \textit{victim flows}, it transits to the second state, \ie, \textit{yellow}.
% %
% Under yellow network condition, \systemname{} uses more than the reserved small memory to handle packet losses.
% %
% As the network condition further degrades, \systemname{} allocates more and more memory for packet loss detection until there is no more available memory, and then the network condition transits to the third state, \ie, \textit{red}.
% %
% Under red network condition, \systemname{} cannot record all the victim flows even with the maximum available memory, and thus \systemname{} shifts to record the victim flows with high priorities, which could be flows with relatively large frequency or user-specified flows, and we call these flows \textit{heavy-losses}.
%当丢包少的时候，我们用大部分的内存支持高精度的正常测量，保留少量丢包内存来应对突发的少量丢包情况。当丢包部分发现情况恶化，就扩大丢包部分的存储，保证丢包的测量，减少正常测量的资源分配，直到正常测量被压缩到最小。如果网络情况进一步恶化，对丢包部分进行进一步切分，通过阈值筛选重要的丢包流，并采样部分不重要的丢包流进行记录。通过流分布分析丢包流分布，划定heavy loss和light loss，检测出所有的heavy loss，对light loss进行采样汇报。保证测量系统在各种状态下能够用最少量的资源关注最关键的信息。

%上述设计从宏观角度上通过动态资源分配来接近设计目标，但是即使资源分配弹性合理，如果的memory efficiency不够高，仍然无法达成design goal。
%to address the challenge， 我们设计了 一个同构的sketch，他能同时支持两类任务，并且将首要关注的丢包测量开销从O包个数降低成了O丢包流。
%上述设计从宏观角度上通过动态资源分配来接近设计目标，which motivates us to design a data structures that supports both tasks, 但另一个关键问题是数据结构的memory efficiency必须足够令人满意。丢包的理想方案是xxx。。。批判loss radar，说费马 flow level开销小。同时费马还能被用于flow level支持正常任务，适用于前述框架，开销也很小。
%  
% \bbb{\systemname{} meets three technical challenges and addresses each of them.}
%
%key tech 利用费马小定理解决了。。。。
%

%

%
% The key design of \sketchname{} is to leverage Fermat's Little Theorem\footnote{Fermat's little theorem states that if $p$ is a prime, then for any integer $a$ that is indivisible by $p$, we have $a^{p-1} \equiv 1 \mod{p}$.} and modular operations to overcome the counter overflows when Invertible Bloom Lookup Table \cite{goodrich2011invertibleIBLT} (IBLT) is used to recording multiple duplicate keys (\eg, <flow ID, frequency> doublet) while preserving additivity and subtractablity.
%


%
% \sketchname{} supports both tasks with internally homogeneous data structures, so as to enable dynamic memory allocation between them.
%
% \sketchname{} can achieve low memory/bandwidth overhead, because it significantly reduces the overhead for packet loss detection from proportional to number of flows (FlowRadar) or lost packets (LossRadar) to proportional to number of victim flows.
%
% \sketchname{} reduces the memory overhead for packet loss detection from proportional to number of flows (FlowRadar) or lost packets (LossRadar) to proportional to number of victim flows, so as to achieve low memory/bandwidth overhead.
%
%The second key challenge is how to handle red network condition by heavy-losses.
% The second key challenge is to identify heavy-losses under red network condition.
% %
% To address this challenge, \systemname{} deploys a simple and accurate TowerSketch \cite{yang2021sketchint} before \sketchname{}es to support online frequency query, so as to identify heavy-losses.
% %
% Considering IDs of small non-victim flows are redundant statistics for most tasks, \systemname{} uses TowerSketch to identify small flows to further reduce the memory overhead for normal tasks. 
% %

% The \textbf{second} key challenge is to identify the selected measurement objects.
% %
% To address this challenge, we propose a threshold-based identification method.
% %
% \systemname{} deploys a TowerSketch \cite{yang2021sketchint} to support online flow size query.
% %
% By querying flow sizes, \systemname{} can easily identify selected flows for heavy-hitter detection using a threshold, but still has no visibility to heavy-losses that experience most severe packet losses.
% %
% Our observation is that only large flows can become heavy-losses, because they can lose more packets and should lose more packets for the same network state compared to small flows.
% %
% Based on the observation, \systemname{} identifies heavy-losses using another threshold.
% %
% The threshold is zero when all victim flows can be measured, and gradually increases as the network state further degrades and \systemname{} must select victim flows to measure. 
% %
% In addition, with the help of TowerSketch, \systemname{} can support five more typical measurement tasks, including flow size estimation, heavy-change detection, flow size distribution estimation, entropy estimation, and cardinality estimation.
% The challenge is easy to address under green or yellow network condition as \systemname{} can record all the victim flows. 
% However, under red network condition, \systemname{} can only record heavy-losses, and thus loses the crucial visibility to the number and flow size distribution of victim flows.
% %
% Without such visibility, \systemname{} cannot shift to record all the victim flows even if the network condition is already yellow.
% % While it might be easy under green or yellow network condition as \systemname{} can record all the victim flows, under red network condition, \systemname{} can only record heavy-losses, and thus loses visibility to the number and flow size distribution of victim flows.
% %
% Therefore, under red network condition, \systemname{} reserves a small amount of memory to record a portion of low-priority victim flows (called \textit{light-losses}) through sampling, so as to complement the visibility.
% To address this challenge under red network condition, \systemname{} reserves a small amount of memory to record a portion of the victim flows with low priorities through sampling, which we call \textit{light-losses}.
%
% By synthesizing the sampled light-losses and all the heavy-losses, \systemname{} then can still has an unbiased visibility to the number and flow size distribution of victim flows even under red network condition.

%我们需要能够同时支持两类task的solution，两部分的结构需要是同构/相同的，以支持dynamic memory allocation between different measurement tasks
%challenge 2
% 绝对的低开销。 极端情况丢包很多，lossradar等开销和丢包个数正比的方案不可用。
%
%为了实现这个想法，系统需要支持dynamic memory allocation between different measurement tasks。
%为了解决这个issue，我们设计了一个同时支持两类task的solution，两部分的结构需要是同构/相同的
%2.一套精确感知网络状态的方案。
% We split the overall flow-level statistics along two dimensions as illustrated in Figure \ref{?}.
% %
% Among them, the desired statistics for supporting high-priority tasks are the IDs and frequency changes of all victim flows, while that for supporting low-priority tasks are the IDs of large flows and the frequencies of all flows.
% %
% To record the above statistics, the minimum required memory should be the sum of two parts: 1) a frequency part that is sublinear or linear to the number of flows considering that most of the required flow frequencies can be approximate; 2) an ID part that is linear to the number of large flows and victim flows considering that the required flows IDs must be exact. 
% %
% However, existing sketches can hardly support packet loss detection with memory overhead proportional to the number of victim flows.
% %
% To address this issue, we propose \sketchname{}, the key innovation of \systemname{}.
% %
% \sketchname{} leverages Fermat's little theorem and modular operations to overcome the counter overflows when IBLT is used to record duplicate keys, and preserves the additivity and subtractibility of IBLT.
% %
% In this way 
% If unfortunately the network condition degrades to a point where the given memory cannot record all the victim flows, we decide to record at the heavy-losses, while samples and records a small portion of light-losses for comprehensively sensing the real-time network condition.
% %
% In summary, their are at most 
% Towards supporting both kinds of tasks and achieving lightweight, our first design choice is to design a memory-efficient \systemname{} data plane that can record almost only the desired flow statistics at any network condition.

%
%The key innovation of \systemname{}
%
% The key innovation of \systemname{} is a novel sketch of the second kind, namely \sketchname{}.
% %
% \sketchname{} supports both high-priority and low-priority tasks to facilitate the dynamic memory allocation for adaptation to real-time network condition.
% %
% Compared to FlowRadar, \sketchname{} reduces the memory overhead required for packet loss detection from proportional to the number of flows to proportional to the number of victim flows.
% % %
% To further reduce the memory overhead required for low-priority tasks to achieve lightweight, we find the IDs of normal small flows are redundant, and deploys a sketch of the first kind before \sketchname{} to identify large flows.
% %
% \bbb{\sketchname{} design:}

%



%核心思想，设计一个同时支持一类任务和二类任务的sketch，以方便内存的动态共享。
%
% The key innovation of \systemname{} is to design a novel sketch, namely \sketchname{}.
% %
% %和flowradar类似，sketch可以支持两种任务，但相比flowradar在支持高优先级丢包检测时将开销从和流数成正比降低到了和丢包数成正比
% \sketchname{} can be flexibly divided into any number parts, each of which can support both high-priority and low-priority tasks independently, so as to facilitate the dynamic memory allocation for adaptation to real-time network condition.
% %
% Further, we deploy a flow classifier before 
% %

% Network measurement provides critical statistics for both network operators and various network functions, including traffic engineering \cite{benson2011microte,feldmann2001deriving}, congestion control \cite{li2019hpcc}, network accounting and billing \cite{cusketch}, anomaly detection \cite{zhang2013adaptive,mai2006sampled,estan2004building,duffield2003estimating}, failure troubleshooting \cite{handigol2014know,netbouncer2019}, \etc{}.
% %
% \ykc{Recently, with the increasing importance of user experience, measuring at flow level gradually becomes industrial consensus.}


% At a high level, flow-level measurement tasks can be classified into two kinds: 1) \sn{} tasks that measure flow statistics in one network node, including flow sizes\footnote{We use the terms flow sizes and flow frequencies interchangeably.}, heavy-hitters, flow size distribution, \etc{}; 2) \cn{} tasks that measure the changes of flow frequnecies across many network nodes, including packet loss detection.
% %自然，我们想要一个能支持两类任务的低开销测量能力。
% Naturally, we want measurement capabilities that supports the above two kinds of tasks simultaneously with minimum memory/bandwidth overhead, so as to avoid limiting the main network functions running on network nodes.
% %

% From the perspective of information volume, the minimum required information for supporting the first kind of tasks consists of the exact flow IDs of large flows and the approximate frequency of each flow, while that for supporting the second kind of tasks consists of the exact IDs and frequencies changes of the flows that experience packet losses, which we call \textit{victim flows} for convenience.
% %
% To record the above information, the minimum required memory should be the sum of two parts: 1) a frequency part that is sublinear or linear to the number of flows considering that most of the required flow frequencies can be approximate; 2) an ID part that is linear to the number of large flows and victim flows considering that the required flows IDs must be exact. 
% %
% We regard the memory overhead that meet the above two criteria as near-optimal, and one of our design goal is to support both kinds of tasks with near-optimal memory overhead.

% %
% With the rapid growth of bandwidth and relative stop growth of memory, while the given memory could be larger than the near-optimal memory overhead in most cases, so as to accurately measure the network, when the network condition quickly degrades and the number of victim flows drastically increases, memory overhead exceeds the limited memory, memory wastage, accuracy drop.
% %
% Therefore, The second design goal is to elastically adapt to network condition, record the most valuable information without memory wastage.
% %
% Achieving all the design goals is challenging: 1) no prior work achieves; 2) ??

==> SOSP21/Abstract.tex <==
\presec
\begin{abstract}
\postsec
%
As data center networks have grown rapidly in both size and complexity, self-driving networking has become the future direction for data center network management; however, industrial grade solutions have not emerged.
%
Some pioneer work has been done towards the ultimate goal of self-driving networks; however, they are either not scalable or not generally applicable.
%
Towards the ultimate goal of self-driving networking, we build a system that can fast and accurately monitor packet losses, detect anomalies, pinpoint root causes, and find emergent response solutions.
%
For network anomaly detection, we propose a fast, accurate, and light-weight sketch based packet loss monitoring algorithm, leveraging the Fermat's little theorem for handling register overflows and de-duplicate lost packets.
%
For root cause localization, we propose a fast machine learning scheme that pinpoints root causes with high accuracy.
%
For emergency response, we propose different response strategies for anomalies with different levels.
%
%Experimental results show that within tens of microseconds, the system can accurately pinpoint network faults that lead to packet losses, and then automatically calculate an emergency response plan for mitigating these network faults.
\end{abstract}

==> SOSP21/Analysismodule.tex <==
\presec
\section{Diagnosing Root Causes of Packet Losses}\postsec
After the monitoring component decodes the paired \sketchnamees{} and captures the victim flows in the last period, the diagnosis component pinpoints corresponding root cause of packet losses.
%
In this section, we first propose a general ML-based method to identify classes of packet losses without visibility to packet forwarding logic. 
Second, with the identified class, if we can go deeper into packet forwarding logic, we propose another method based on error codes to further pinpoint the root causes, and improve the accuracy of our ML-based method.
Third, we discuss the ability of \systemname{} to diagnose packet losses under different settings. 
%Third, we propose a path tracing method working in \systemname{} to help diagnose the root causes and the following re-configuration.
% \sout{to diagnose them}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[]
\caption{Classes and root causes of packet losses, and the packet losses that \systemname{} can diagnose. LR refers to LossRadar's placement, and FD refers to \systemname{}'s placement in Section \ref{sketchplace}. \checkmark means the root cause can be pinpointed, and $\circ$ means the class can be identified.}
\vspace{0.3cm}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\label{pkt:loss}
Class                                                                           & Root cause                & ML (LR)                   & ML (FD)                   & ML+EC (LR)                & ML+EC (FD)                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Forwarding\\ Blackhole\end{tabular}} & Forwarding table mismatch & $\circ$                   & $\circ$                   & \checkmark & \checkmark \\ \cline{2-6} 
                                                                                & ACL rule drop             & $\circ$                   & $\circ$                   & \checkmark & \checkmark \\ \hline
\multirow{2}{*}{Random Drop}                                                    & Swicth ASIC failure       & $\circ$                   & \checkmark & $\circ$                   & \checkmark \\ \cline{2-6} 
                                                                                & Bent Fiber                & $\circ$                   & \checkmark & $\circ$                   & \checkmark \\ \hline
Forwarding Loop                                                                 & TTL=0                   & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
Congestion                                                                      & Unexpected traffic volume & \checkmark & \checkmark & \checkmark & \checkmark \\ \hline
\end{tabular}
\end{table*}

\presec
\subsection{Diagnosing using Machine Learning}
\label{sec:ana:ml}


\subsubsection{Motivation to Use Machine Learning} \postsec

%
As shown in Table \ref{pkt:loss}, there are mainly four classes and six root causes of packet losses. \textit{We exclude link failure from the table because all the packets are lost in the link, which is a significant characteristic for diagnosis.}
%
In general, when the monitoring component is deployed in commodity switches and software switches, the packet forwarding logic is usually fixed, and invisible to the deployed monitoring component.
%
In this case, it is difficult to pinpoint root causes, because different root causes of the same class may look like the same.
For example, forwarding table mismatch and ACL rule drop show no difference. 
%
Therefore, we focus on identifying classes of packet losses. 
To achieve this, the state-of-the-art LossRadar analyzes the patterns of the lost packets, such as 5-tuple, IP\_ID, TTL, timestamp, TCP flags, \etc{}
%
However, the diagnosis component cannot obtain packet-level information used by LossRadar, it can only obtain the victim flow IDs and the numbers of lost packets after decoding.
%
Note that all the sum counters of a \sketchname{} make up a Count-Min sketch \cite{cmsketch}, so the central controller can also get several frequency estimators of each victim flow\footnote{For \sketchnamees{} decoded in switches, the frequency estimators can also be transmitted to the central controller.}.
%
After a thorough study of the four classes of packet losses, we find different class will lead to different numerical relationship between the frequency of the flow and the number of the lost packets. Motivated by this, we choose to use machine learning to train a classifier to identify the classes.
%

\presec
\subsubsection{Identifying Loss Classes} \postsec

In this section, we elaborate on our insights about how the classes of packet losses are identified.

\bbb{Forwarding blackhole:}
%
%The forwarding blackhole caused by forwarding table mismatch or ACL rule will drop all packets belonging to a flow.
A forwarding blackhole will drop all packets belonging to a flow.
%
In this case, each packet sent from the TCP sender will time out, resulting in the TCP congestion window rapidly reduced to 1.
%
After that, TCP sender will send one packet after every RTO (Retransmission Timeout).
%
Therefore, the packet losses caused by forwarding blackhole has the following characteristics:
%
the number of lost packets is almost the same as the frequency estimator, and the number of lost packets in each monitoring period is almost the same (\ie, the ratio of monitoring period to RTO\footnote{In DCTCP, the RTO is set to 10ms by default.}) except for the first period.

\bbb{Forwarding loop:}
%
A forwarding loop will also cause all packets of a flow to be lost, resulting in the TCP congestion window becoming 1.
%
Therefore, the number of lost packets in each monitoring period is almost the same.
%
There is a significant difference between packet losses caused by loop and packet losses caused by blackhole: each lost packet passes through the switches in the loop many times.
%
Therefore, the packet losses caused by loop has the following significant characteristic: 
%
the ratio of the frequency estimator to the number of lost packet is similar to the number of times a packet passes through the switch (\ie, the ratio of the initial TTL to the loop length).

\bbb{Congestion \& Random drop: }
%
For the packet losses caused by congestion or random drop, the number of lost packets belonging to one flow in each monitoring period is no longer a fixed value.
%
Both of them will cause a portion of packets to be dropped, which makes it difficult to distinguish them from each other in terms of packet losses ratio.
%
However, previous work \cite{yang2018empowering} pointed out that larger network traffic will make the difference of several frequency estimators of a flow greater, which makes it possible to identify these classes.


\presec
\subsubsection{Classifier Training} \postsec
In this section, we present the workflow in classifier training: 1) feature selection; 2) training data collection; 3) classifier model decision.

\bbb{Feature selection.}
Based on the above insights, we propose to use the following features to represent a flow-level packet loss event:
%
The features include data of several consecutive monitoring periods that start from the earliest period in which packet losses are detected.
%
The data of each monitoring period includes: 
%
1) the number of lost packets; 
%
2) the estimated proportion of packet loss, \ie, the proportion of the number of lost packets to the smallest frequency estimator;
%
3) the difference of frequency estimator, \ie, the ratio of the second smallest (the third smallest, ..., the largest) frequency estimator to the smallest frequency estimator.
%
Using more monitoring periods to generate features can achieve higher accuracy, but the cost is that it takes longer time to obtain the results (\S \ref{sec:exp:ml}).
%
Operators of \systemname{} need to make a trade-off between the \textit{accuracy} and \textit{timeliness}.

\bbb{Training data collection.}
The diagnosis component needs labeled dataset to train the classifier. With the deployment of our monitoring component, the packet losses are collectable. However, the classes of packet losses are invisible.
%
Therefore, we can only collect a large amount of unlabeled data with features described above.
To label the data, we inject a small number of trigger flows\footnote{the destination IP of these flows are set to 0.0.0.0, so as to avoid any possible conflict with rules in switches.} into the network, and configure the switches to make these flows experience different classes of packet losses. After the packet losses of these trigger flows are detected, we can collect a small amount of pre-labeled data.
%
Then, we cluster the unlabeled data into multiple groups using the most widely-used clustering algorithm DBSCAN \cite{ester1996density}. 
%
We keep adjusting the parameters of DBSCAN until more than 90\% of the pre-labeled data in each group belong to one class. 
Finally, for each group, we label all the unlabeled data in it as the major class.
%If we can configure the switches, an option to improve the accuracy of label is to sample lost packets. We adopt xxx?? as our cluster algorithm. 

\bbb{Model decision.}
With the labeled data, we can train the classifier. 
%
Making a trade-off between accuracy and computation efficiency, we choose the multi-layer perceptron \cite{pal1992multilayer} with two hidden layers as the classification model, and use cross-entropy as the loss function.
%
In order to ensure that the classifier can adapt to the varying network traffic, we collect training data and train the classifier periodically.



%



% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\presec
\subsection{Diagnosing using Programmable Switches}
\postsec
\label{sec:p4}
When the monitoring component is deployed in the programmable data plane, we can dig deeper into the packet forwarding logic, and further pinpoint the root causes. 
There are three kinds of root causes that are visible to the packet forwarding logic: 1) forwarding table mismatch, which means no rule in the forwarding table matches the packet; 2) ACL rule drop, which means an rule in the ACL table matches the packet; 3) TTL=$0$.
The first two root causes will lead to forwarding blackholes, and the third one suggests the packet is trapped in a forwarding loop.
% 
To record the root causes, we assign a 2-bit error code (EC) to each kind of root cause, and reserve $0$ to indicate that there is no explicit root cause for packet losses. 
%
For each incoming packet. we concatenate its 5-tuple and the error code, and insert the result of concatenation into \sketchnamees{}. 
%
In this way, we can directly pinpoint the root causes of packet losses after decoding.
%
Further, because part of the unlabeled training data can be labeled, the accuracy of the classifier improves.   

\presec
\subsection{Diagnosis Ability under Different Settings}
\postsec
The ability of \systemname{} is determined by the placement strategy and whether error code is available. As shown in Table \ref{pkt:loss}, \systemname{} with only ML-based method cannot distinguish forwarding table mismatch from ACL rule drop because they show no difference; \systemname{} with LossRadar's placement cannot distinguish switch ASIC failure from bent fiber, because it cannot distinguish intra-switch/inter-switch packet losses.

 


==> SOSP21/Conclusion.tex <==
\vspace{-0.1cm}
\presec \section{Conclusions} \postsec
\vspace{-0.2cm}

%
In this paper, we make four key contributions.
%
First, for monitoring, we propose a fast, accurate, and light-weight sketch based algorithm for monitoring the number of lost packets.
%
The significance of this algorithm is that it is both scalable and generally applicable, which makes self-driving networking possible for industry deployment.
%
Second, for diagnosis, we propose a fast machine learning scheme that pinpoints root cause with high accuracy.
%
Third, for response, we propose different response strategies for anomalies with different levels.
%
Fourth, We implemented our packet loss monitoring scheme, root cause localization scheme, and emergency response scheme, and deployed them on a testbed environment.

==> SOSP21/Experiments.tex <==
\presec
\section{Experimental Results}
\postsec
% Our experiment focuses on the following four key issues.
We conduct extensive experiments on a testbed, and focus on the following three key issues.
%
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=1pt,partopsep=1pt]
    \item \bbb{Compared to the existing solutions, how much bandwidth/memory/time can \sketchname{} save?}
    
    We conduct several simple simulation experiments for comparison. 
    %
    We implement \sketchname{}, LossRadar, and FlowRadar in C++, and use the DCTCP workload to simulate packet loss and compare the decoding success rate and processing speed of these algorithms under different conditions.
    %
    % flow size estimation, flow size distribution estimation, entropy estimation, cardinality estimation, delay distribution estimation, last arrival time estimation, and maximum packet interval estimation.
    
    
    \item \bbb{Under real data center traffic distribution, how much precision and recall can our machine learning model achieve?}
    
    We simulate four different classes of packet loss in our system prototype, evaluate the accuracy of the machine learning classifier, and test the performance of the model about the precision and recall.
    
    \item \bbb{When network anomalies occur, how fast and effectively can our system respond to them?}
    
    We evaluate the performance of the recovery of \systemname{} by generating uneven ECMP and link failures in our system prototype.
    
\end{itemize}

% \reder{
% We conduct the experiments using the following metrics: \textbf{ARE}, \textbf{RR}, \textbf{PR}, \textbf{$F_1$ Score}, \textbf{RE}, and \textbf{WMRE}. 
% We explain the details of these metrics in Appendix \ref{sec:met}.
% }



\presec
\subsection{Monitoring Solution Comparisons}
\postsec







\bbb{Experimental setting.}
We conduct simulation experiments using the widely-used traffic distribution DCTCP \cite{dctcp}. 
We conduct the experiments under two settings: 1) 1000 flows totally, where $10\%$ flows drop $5\%$ packets, and 2) 10000 flows totally, where $1\%$ flows drop $100\%$ packets. 
In both settings we use 32-bit flow IDs and 32-bit counters.

\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Setting 1.]{
        \begin{minipage}[b]{0.225\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/accuracy0.pdf}
            \label{fig:sketch:setting1}
            \vspace{-0.2in}
        \end{minipage}
    }
    \subfigure[Setting 2.]{
        \begin{minipage}[b]{0.225\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/accuracy1.pdf}
            \label{fig:sketch:setting2}
            \vspace{-0.2in}
        \end{minipage}
    }
\caption{Decode Success Rate.}
\label{fig:sketch:setting}
\end{figure}
\vspace{-0.2in}

\bbb{Decode success rate \textit{v.s.} memory usage (Figure~\ref{fig:sketch:setting}).}
We compare the decode success rate of our \sketchname{}, FlowRadar \cite{flowradar2016}, and LossRadar \cite{lossradar2016} under different memory usage. 
The experimental results demonstrate that in the first setting, our \sketchname{} can achieve $99\%$ decode success rate using no more than 10KB memory, which is one order of magnitude less than FlowRadar and two orders of magnitude less than LossRadar. 
In the second setting, Fermat also achieves several orders of magnitude lower than FlowRadar and LossRadar. 


\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Insertion Speed.]{
        \begin{minipage}[b]{0.225\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/insert-speed.pdf}
            \label{fig:speed:insert}
            \vspace{-0.2in}
        \end{minipage}
    }
    \subfigure[Decoding Speed.]{
        \begin{minipage}[b]{0.225\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/decode-speed.pdf}
            \label{fig:speed:decode}
            \vspace{-0.2in}
        \end{minipage}
    }

\caption{Processing Speed of the Sketches.}
\postfig
\label{fig:speed}
\end{figure}


\bbb{Processing speed (Figure~\ref{fig:speed}).} 
We compare the insertion speed and the decode time of the three solutions. 
The experimental results show that our \sketchname{} achieves similar insertion speed compared with FlowRadar and LossRadar. 
And the decoding time of \sketchname{} is several orders of magnitude smaller than FlowRadar and LossRadar. 

% We can see that the processing speed of our Fermat sketch significantly outperforms FlowRadar and LossRadar. 















\presec
\subsection{Diagnosing with Machine Learning}
\postsec
\label{sec:exp:ml}

We manually simulate four scenarios of packet losses.
%
1) Congestion: We generate traffic under 90\% link utilization.
%
2) Forwarding Blackhole: We configure the routing table on one ToR switch to drop 20\% flows.
% We make 20\% of the flows lose their routing table entries on a ToR switch.
% We drop on one ToR switch routing table entries related to 20% flows 
%
3) Forwarding Loop: We make 20\% of the flows forward between four switches until TTL becomes 0.
%
4) Random drop: We make 10\% of the packets randomly dropped on a ToR switch.
%
We collect 8954 traces of congestion, 1293 traces of blackhole, 683 traces of loop, and 6080 traces of random drop.

\begin{comment}
\begin{table}[h!]
\setlength{\abovecaptionskip}{0.0cm}
\setlength{\belowcaptionskip}{-0.0cm}
\begin{tabular}{|c|c|}
\hline
\textbf{Root cause} & \textbf{\# Traces} \\ \hline 
Congestion & 8954 \\ \hline
Forwarding Blackhole & 1293 \\ \hline
Forwarding Loop & 683 \\ \hline
Random drop & 6080 \\ \hline
\end{tabular}
\vspace{0.3cm}
\caption{The number of traces of each type of root cause.}
\vspace{-0.5cm}
\label{exp:traces}
\end{table}
\end{comment}

For each type of traces, we use 80\% of them as the training set, and expand it to 8000 data through sampling;
%
We use the remaining 20\% as the validation set, and expand it to 2000 data through sampling.
%
We train 200 epochs.


\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Top-1 accuracy.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/top1accuracy.pdf}
            \label{fig:ml:top1}
            \vspace{-0.26in}
        \end{minipage}
    }
    \subfigure[Recall \& Precision.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/recall&precision.pdf}
            \label{fig:ml:r&p}
            \vspace{-0.26in}
        \end{minipage}
    }
\vspace{0.2cm}
\caption{Top-1 accuracy, Recall, and Precision.}
\postfig
\label{fig:ml:acc}
\end{figure}


\bbb{Top-1 Accuracy v.s. \# monitoring periods (Figure \ref{fig:ml:top1}).}
%
We find that using data from more monitoring periods to generate features helps to improve classification accuracy.
%
We vary the number of the monitoring period used to generate features from one monitoring period to ten consecutive monitoring periods. 
%
As shown in Figure \ref{fig:ml:top1}, although using only one monitoring period has the highest timeliness, it can only achieve 89\% accuracy.
%
One the contrary, using more than 5 monitoring periods will increase the diagnostic latency, but it can achieve nearly 95\% accuracy.

\bbb{Recall \& Precision (Figure \ref{fig:ml:r&p}).}
%
As shown in Figure \ref{fig:ml:r&p}, the MLP (multi-layer perceptron) model can diagnose the forwarding blackhole and the forwarding loop with nearly 100\% recall and precision.
%
For congestion and random drop, the diagnostic accuracy is relatively low, but there are still 88\% and 95\% recall, and 94\% and 88\% precision, respectively.



\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Congestion.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/RRvsPR1.pdf}
            \label{fig:ml:pr1}
            \vspace{-0.2in}
        \end{minipage}
    }
    \subfigure[Forwarding blackhole.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/RRvsPR2.pdf}
            \label{fig:ml:pr2}
            \vspace{-0.2in}
        \end{minipage}
    }
    \subfigure[Forwarding Loop.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/RRvsPR3.pdf}
            \label{fig:ml:pr1}
            \vspace{-0.2in}
        \end{minipage}
    }
    \subfigure[Random drop.]{
        \begin{minipage}[b]{0.22\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/RRvsPR4.pdf}
            \label{fig:ml:pr2}
            \vspace{-0.2in}
        \end{minipage}
    }
\vspace{0.2cm}
\caption{Recall v.s. Presicion.}
\label{fig:ml:pr}
\vspace{-0.3cm}
\end{figure}

\bbb{Recall v.s. Precision (Figure \ref{fig:ml:pr}).}
%
In addition to utilizing a multi-classifier to diagnose all the root causes of packet loss, we can also use multiple two-classifier to diagnose each root cause separately.
%
Although the use of multiple machine learning models will make the diagnosis process complicated, it can bring higher accuracy.
%
At the same time, using two-classifier, we can change the classifier threshold to adjust the relationship between precision and recall, so as to avoid too many false positives or false negatives.
%
As shown in Figure \ref{fig:ml:pr}, the two-classifiers of the four root causes can achieve PR AUC (Precision-Recall Area Under Curve) of 0.986, 0.999, 0.999, and 0.981, respectively.


\vspace{-0.1cm}
\presec
\subsection{Responding to Network Anomalies}
\postsec

In this section, we show how \systemname{} can respond to anomalies on a real testbed.
%
We take responding to uneven ECMP (low-risk) and responding to link failures (medium-risk) as case studies.


\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Packet per second w/o \systemname{}.]{
        \begin{minipage}[b]{0.44\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/Kpps_2.pdf}
            \label{fig:ecmp:1}
            \vspace{-0.3in}
        \end{minipage}
    }
    \vspace{-0.15cm}
    \subfigure[\# lost packets w/o \systemname{}.]{
        \begin{minipage}[b]{0.44\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/LostPac_2.pdf}
            \label{fig:ecmp:2}
            \vspace{-0.3in}
        \end{minipage}
    }
    \vspace{-0.15cm}
    \subfigure[Packet per second w/ \systemname{}.]{
        \begin{minipage}[b]{0.44\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/Kpps_1.pdf}
            \label{fig:ecmp:3}
            \vspace{-0.3in}
        \end{minipage}
    }
    \vspace{-0.15cm}
    \subfigure[\# lost packets w/ \systemname{}.]{
        \begin{minipage}[b]{0.44\textwidth}
            \centering
            \includegraphics[width=\textwidth]{lzr/pics/exp/LostPac_1.pdf}
            \label{fig:ecmp:4}
            \vspace{-0.3in}
        \end{minipage}
    }
\vspace{0.1cm}
\caption{Responding to uneven ECMP.}
\postfig
\label{fig:test:ecmp}
\end{figure}

\bbb{Responding to uneven ECMP.}
%
We maintain two pairs of clients and servers, and generate 30Gbps traffic between each pair of clients and servers.
%
All flows enter a common ToR switch from one of the two ports, and use ECMP to choose one of the two outgoing links.
%
Ideally, ECMP will distribute the incoming flows into two links equally, so there will be no congestion.
%
We manually create an uneven ECMP, where all flows go through one link.
%
As shown in Figure \ref{fig:ecmp:1} and \ref{fig:ecmp:2}, only one link has traffic, and the packet loss caused by congestion always occurs.
%
We run \systemname{} to respond to this anomaly.
%
As shown in Figure \ref{fig:ecmp:3} and \ref{fig:ecmp:4}, \systemname{} detects the anomaly within 60ms, and then re-configures the forwarding table to direct half of victim flows to another idle link.
%
The experimental results show that the packet loss is eliminated after 20ms, and the load of two links is maintained at about 2:1, \ie, 30Gbps (450Kpps):15Gbps (225Kpps).
%
With the establishment of new TCP connections, once the load of a link reaches 40Gbps (around 4s, 12s, and 22s), the packet loss caused by congestion will appear, and \systemname{} will re-configure the forwarding table to quickly eliminate the packet loss and stabilize the link load.
 
\begin{figure}[h!]
\setlength{\abovecaptionskip}{-0.15cm}
\setlength{\belowcaptionskip}{-0.0cm}
\centering
    \subfigure[Packet per second w/ \systemname{}.]{
        \begin{minipage}[b]{0.44\textwidth}
            \includegraphics[width=\textwidth]{lzr/pics/exp/re3.pdf}
            \label{fig:test:link1}
            \vspace{-0.3in}
        \end{minipage}
    }
\vspace{0.2cm}
\caption{Responding to link failures.}
\postfig
\label{fig:test:link}
\end{figure}

\bbb{Responding to link failures.}
%
We maintain two pairs of clients and servers, and generate 10Gbps (150Kpps) traffic between each pair of clients and servers.
%
As shown in Figure \ref{fig:test:link1}, at the beginning, all flows are evenly distributed on the two outgoing links of a ToR switch.
%
We manually shut down one of the links around 20s.
%
The experimental results show that \systemname{} detect the anomaly and redirect the victim flows to the active link within 30ms.

==> SOSP21/Implementation.tex <==
\presec
\section{Prototype Implementation}
\postsec

In this section, we present the important details of our system prototype. We mainly focus on the implementation detail of the monitoring component in data plane as it is not well discussed before.


\subsection{Topology}

As the topology shown in Figure \ref{pic:overview}, we implement our system prototype on a testbed consists of 10 Tofino 32D switches and 8 servers connected with 40Gbe links in a FatTree topology. An additional server linked with a certain edge switch works as the central controller.


\presec
\subsection{Monitoring Component in Data Plane}
\postsec

\label{sec:impl}
% \presec
% \subsubsection{P4 Implementation}
% \postsec

We briefly describe the implementation of \sketchname{} in data plane of Tofino switches. 
%We first present the workflow, and then introduce the important operations and components in data plane.
For more implementation details, please refer to Appendix \ref{app:de}.

\bbb{Workflow.}
At a high level, each incoming packet goes through five stages.
First, the packet is inserted to the downstream \sketchname{} corresponding to its ingress port in the inter-switch path, which is dominated by the upstream switch, with the AM-PM timestamp recorded in one unused bit in IPV4 protocol. 
Second, each incoming packet obtains a 1-bit AM-PM timestamp from switch, records it in the IPV4 protocol, and selects its egress port. 
Third, the packet is inserted to the upstream \sketchname{} corresponding to its selected egress port in the intra-switch path with the AM-PM timestamp.
Fourth, the traffic manager switches it to the egress port.
Fifth, the packet is inserted to the downstream \sketchname{} corresponding to its egress port in the intra-switch path with the AM-PM timestamp. %Note that the inserted \sketchname{} is also the upstream \sketchname{} in the inter-switch path.

\bbb{AM-PM timestamp.}
The timestamp is stored in a register, and the control plane flips it every time the latest monitoring period ends.

\bbb{Buckets in \sketchnamees{}.}
\textit{To save resources, we omit the second modulo counter and the ID verification.}
To record the 5-tuples, a bucket in an ideal \sketchname{} should contains a 105-bit modulo counter. 
%
The reason why the counter is expected to be 105-bit instead of 104-bit is that \sketchname{} uses a modulo operation, so recording a complete 104-bit 5-tuple requires a 105-bit prime. 
%
However, because Tofino supports up to 32-bit counters, the modulo counter cannot be directly built in Tofino.  
%
To store a 104-bit 5-tuple, we divide it into multiple 32-bit counters. 
%
Because Tofino supports up to 32-bit signed constant in stateful ALU (SALU), the largest prime we can use is 31-bit. 
%
Therefore, a 32-bit counter in \sketchname{} can store at most a 30-bit fragment of a 104-bit 5 tuple, and we need four 32-bit counters to store the 5-tuples. 
%
As a result, each bucket of \sketchname{} consists of 5 counters: four 32-bit modulo counters and a 32-bit sum counter.
%

\bbb{Division of 5-tuple.}
To place the 5-tuple in four 32-bit counters, we divide each of the IP source address, the IP destination address, and the concatenation of the source port and destination port into two fragments: a 2-bit fragment and a 30-bit fragment. 
%
Then, we concatenate three truncated 2-bit fragments, and the 8-bit protocol to get a 14-bit new ID. 
%
The 5-tuple is finally divided into three 30-bit fragments, and one 14-bit fragment. The rest 16 bits can be used as error codes (\S \ref{sec:p4}) to provide root causes of packet losses, or fingerprint to improve decoding accuracy.   

\bbb{Building \sketchnamees{} with registers.}
We use registers to build \sketchnamees{}.
Ideally, each port will has its corresponding individual \sketchname{}es. 
%
In Tofino, a packet can only access a register once with SALU. For each bucket array in a \sketchname{}, each incoming packet access five counters in a hashed bucket. 
Therefore, each bucket array requires five registers to store its five counter arrays individually.
Since each time a packet will be inserted into only one \sketchname{}, the five register can be extended to store one \sketchname{} per port.
%
%However, the number of registers in Tofino is limited, and thus we must merge the registers that can be merged. 
%
%Obviously, registers for different ports that correspond to the same counter arrays in the buckets can be merged.
%
%After merging the registers,   
Suppose there are $n_p$ ports in total, considering the 1-bit AM-PM timestamp $t$, the counter in the $i$-th bucket of the $p$-th port with timestamp $t$ is indexed by $t+2\times i \times n_p+2 \times p$.


\bbb{Inserting 5-tuple into \sketchnamees{}.}
We use SALU to perform the insertion. As each time we only insert one packet, the modulo operation can be substituted by an addition operation or a subtraction operation after a comparison, which is naturally supported by SALU.  



%\bbb{Largest capacity of detection.}
%In existing Tofino switches, the Map RAM which can be used to build registers is 6MB in each stage. 
%Due to the memory limitation, for each pipeline with 16 ports, the largest register built as a part of \sketchname{} has 32768 buckets. As discussed in Section \ref{sec:algo:math}, the array number is set to 3 to achieve the most memory efficient. When the monitoring period is set to 10$ms$, the pipeline can totally detect at most $\frac{32768/2}{1.22}\approx13430$ victim flows every 10$ms$. When all the 16 ports are in use, each port can detect at most $\frac{13430}{16}\approx840$ victim flows every 10$ms$.

\bbb{Parameter settings.}
We build a light monitoring component with about 7\% SRAM resources.
For each \sketchname{}, we set the number of arrays to 2, and the number of buckets to 512. That is to say, in our topology where each switch uses 4 ports, the number of counter in each register is set to $512\times2\times4\times2=4096$.
\vspace{-0.5cm}
\begin{table} [h!]
\centering\caption{\small H/W resources used in Tofino.
%{\color{reviewC}The total memory usage of our P4Switch is the product of the baseline usage and the additional usage.}
}
\vspace{0.1cm}
{\centering
\small
\begin{tabular}{|l|r| r|c|}
\hline
\textbf{Resource} & \textbf{Usage} & \textbf{Percentage}\\ \hline
Match Crossbar & 312 & 20.31\% \\ % 474 & 5.9\% \\  % 502
Map RAM & 60 & 10.42\% \\
SRAM & 66 & 6.88\% \\ %288 & 12.5\% \\ %324
TCAM & 0 & 0\% \\  %102 & 0\% \\  %102
VLIW Action & 16 & 4.17\% \\ %145 & 5.5\% \\ %153
Hash Bits & 594 & 11.90\% \\ %1605 & 2.3\% \\ %1642
Stateful ALU & 30 & 62.50\% \\ \hline %4 & 75\% \\ %7
%Packet Header Vector &  %277 & 0.36\% \\ \hline %4877
\end{tabular}
}

\vspace{-0.3cm}
\label{tab:overhead}
\end{table}


\bbb{Resources occupation:}
As shown in Table \ref{tab:overhead}, the monitoring component consumes SALU most, achieving 62.5\%. This is because \sketchnamees{} needs SALU to access registers. Although \systemname{} indeed consumes lots of resources, LossRadar must consume more because it additionally records per-packet information such as IP\_ID, timestamp, TCP flags, \etc{} Further, with the appearance of Tofino II switches, we believe the resource usage will be much more acceptable in the coming future.

\begin{comment}
\presec
\subsection{Collection Strategies}
\postsec

In this section, we briefly describe our implementation of two collection strategies.


\bbb{Fast strategy:}
In this strategy, the control plane program only consists of the part of timestamp flipping. The interval that timestamp flipping is set to 10$ms$. A packet sender implemented in DPDK running on the central controller periodically sends 8192 tailored packets every 10$ms$ to carry \sketchnamees{} of all switches from data plane to the central controller. 

\bbb{Time synchronization:} Both these two strategies require time synchronization. To meet this, we implement Huygens \cite{geng2018exploiting} in all switches and the central controller, achieving 10$\mu$s-accuracy time synchronization. 

\end{comment}

==> SOSP21/Measurementmodule.tex <==
\presec
\section{Monitoring Packet Loss}
\postsec
\label{sec:algo}


The monitoring component is expected to achieve full coverage of network with low overhead in a timely manner.
In this section, we present the design of our monitoring component. 
%First, we propose \sketchname{}, the key innovation of this paper. Then, we discuss the placement of \sketchnamees{}, the collection of \sketchnamees{} and the decoding of \sketchnamees{}. 

\presec
\subsection{The \sketchname{} Algorithm}
\postsec

\bbb{Motivation:}
A satisfactory monitoring component is with low overhead, including three aspects: 1) Storage complexity: low memory consumption in switches; 2) Communication complexity: low bandwidth overhead in transmission; 3) Computation complexity: fast processing speed in decoding. 
The three complexities of the state-of-the-art LossRadar are linear to the number of lost packets.
To achieve a much lower complexity, it is desired to devise a light algorithm whose complexities are linear to the number of flows suffering packet losses, which are called \textit{victim flows}, rather than the number of lost packets.

% Therefore, it is desired to devise a light and neat data structure able to detect each victim flow suffering packet loss and the number of its lost packets with O(victim flows) memory overhead. 
% To meet these requirements, we need a light and neat data structure able to detect each victim flow suffering packet loss and the number of its lost packets with O(victim flows) memory overhead. 

% For scalability, both the computation and communication overhead of our monitoring component  should be small enough. 
% Also, the monitoring component should save memory consumption as the memory resources of the forwarding device are scarce.

% In our experiment, when a congestion happens, within 10 microseconds, there are 1xxx lost packets and 30 flows suffering packet loss. During 10 microseconds, a typical central controller an only receive and process 100 lost packet IDs or flow IDs.



% To well support the self-driving, the monitoring component should be general and low overhead. The generality requires the monitoring component to be easy to deploy on various platforms. The low overhead includes three aspects: 1) low memory consumption in network device; 2) low bandwidth overhead in transmission; 3) fast processing speed in diagnosis. 
% To meet these requirements, we need a light and neat data structure able to detect each victim flow suffering packet loss and the number of its lost packets with O(victim flows) memory overhead. 
% At first glance, Invertible Bloom filter (IBF) \cite{goodrich2011invertibleIBLT} adopting addition operation (not XOR operation) seems like a feasible choice. For each path, by placing a pair of IBFs upstream and downstream, and encoding/inserting each passing packet into the corresponding IBF, we can then subtract and decode the IBFs to detect the victim flows. 
% %Suppose no packets are generated in a path, we place IBF both upstream and downstream and encode the same traffic into them with flow ID (\eg, 5-tuple). The decoding result of the subtraction of the downstream IBF from the upstream IBF is the victim flows. 
% %
% However, IBF suffers from a fatal flaw: the counter used in IBF must be large enough to contain the sum of ID of the items hashed into itself. 
% % However, IBF suffers from a fatal flaw: the counter used in IBF must be large enough to contain the sum of ID of the items hashed into itself. 
% This flaw leads to not only memory-inefficiency, but also deployment difficulty in hardware, especially in programmable data plane. 
% To address this issue, we design a novel data structure which reduces the requirement of counters to the optimal size, 
% the maximum size of the ID and the frequency while maintaining the ability to detect victim flows with O(victim flows) memory overhead.

\bbb{Key idea:}
Our key idea is to leverage Fermat’s little theorem for insertion, addressing the problem of overflows of counters to achieve memory-efficiency.
%
Fermat’s little theorem states that for any prime p and any integer a, we have $a^{p-1} \equiv 1 \mod{p}$. We use this theorem and the modulo operation to reduce the memory needed for storing the ID sum of packets.



\bbb{Data Structure:} 
As shown in Figure~\ref{algopic:insertion}, \sketchname{} consists of $d$ bucket arrays $\mathcal{B}_1, \cdots, \mathcal{B}_d$, each of which has $m$ buckets.  
Each bucket array $\mathcal{B}_i$ is associated with a hash function $h_i(\cdot)$ that maps each incoming packet into one bucket in it. 
Each bucket has three counters: \textbf{1)} one \textit{sum counter} recording the number of packets mapped into the bucket. \textbf{2)} two \textit{modulo counter}s recording the remainders of the sum value of flow IDs \footnote{In this paper, flow ID refers to the 5-tuple.} divided by two different primes $p_1$ and $p_2$, where $p_2$ is greater than any ID and $p_1$ is smaller than $p_2$.
All counters of all buckets are initialized to zero. 

\bbb{Insertion/Encoding:} 
To insert a packet of flow $f$, we first calculate the $d$ hash functions to get the \textit{$d$ mapped buckets} of flow $f$: $\mathcal{B}_1[h_1(f)], \cdots, \mathcal{B}_d[h_d(f)]$. 
For each mapped bucket $\mathcal{B}_i[h_i(f)]$, we update it as follows: 
First, we increment its \textit{sum counter} $\mathcal{B}_i^{sum}[h_i(f)]$ by one. 
Next, we update its first \textit{modulo counter} as
$\mathcal{B}_i^{mod_1}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_1}[h_i(f)] + f \right) \mod{p_1}$, and update its second \textit{modulo counter} as $\mathcal{B}_i^{mod_2}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_2}[h_i(f)] + f \right) \mod{p_2}$. 


\bbb{\textit{Example:}}
As shown in Figure~\ref{algopic:insertion}, to insert a new packet of flow $f = 24$, we calculate the two hash functions to get the two mapped buckets of $f$, \ie{}, $\mathcal{B}_1[2]$ and $\mathcal{B}_2[3]$. 
Then we increment the \textit{sum counters} of the two mapped buckets by one. 
Next, we update the \textit{modulo counters} of the two mapped buckets. 
For example, we update $\mathcal{B}_1^{mod_1}$ to $\left( \mathcal{B}_1^{mod_1} + f \right) \mod{p_1} = \left( 4 + 24  \right) \mod{11} = 6$, and we update $\mathcal{B}_1^{mod_2}$ to $\left( \mathcal{B}_1^{mod_2} + f \right) \mod{p_2} = \left( 4 + 24 \right) \mod{13} = 2$. 

\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.84\linewidth]{lzr/pics/Fermat-Insertion.pdf}
    \vspace{0.2cm}
    \caption{Insertion example of \sketchname{}.}
    \label{algopic:insertion}
    \postfig
\end{figure}

\bbb{Subtraction:}
The subtraction operation takes a pair of \sketchnamees{}. 
We just perform the subtraction operation for each pair of sum counters, and perform the modulo subtraction operation for each pair of modulo counters.

\bbb{Deletion:} 
Deletion is the just the reverse process of insertion. 
Specifically, to delete a packet of flow $f$, we first get its $d$ mapped buckets by calculating hash functions. 
Then, for each mapped bucket $\mathcal{B}_i[h_i(f)]$, we subtract one from its \textit{sum counter} $\mathcal{B}_i^{sum}[h_i(f)]$, and update its two \textit{modulo counter}s as $\mathcal{B}_i^{mod_1}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_1}[h_i(f)] - f \right) \mod{p_1}$ and $\mathcal{B}_i^{mod_2}[h_i(f)] \gets \left( \mathcal{B}_i^{mod_2}[h_i(f)] - f \right) \mod{p_2}$. 





\bbb{Decoding:}
The decoding procedure of \sketchname{} has two steps: 
First, we look for buckets that include just one flow (we call these buckets \textit{pure buckets} and call the flows inside them as \textit{pure flows}). 
Second, for each pure bucket, we delete the flow recorded in it from our \sketchname{}. 
We repeat these two steps until all buckets are empty (successful decoding) or no bucket is pure (failed decoding). 
Next, we explain the details of the two steps. 

\bbb{1) Looking for pure buckets:} 
We repeatedly check all buckets in \sketchname{}. 
For each bucket $\mathcal{B}_i[t]$, we propose two methods to check whether it is pure: 
The first method is called \textbf{ID verification}: 
We just suppose $\mathcal{B}_i[t]$ is pure and try to get the flow ID recorded in it. 
Specifically, we calculate $f_1^{\prime} = \left( \mathcal{B}_i^{mod_1}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_1-2} \right) \mod{p_1}$ and $f_2^{\prime} = \left( \mathcal{B}_i^{mod_2}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_2-2} \right) \mod{p_2}$. 
Then we check whether $f_1^{\prime}$ is equal to $(f_2^{\prime} \mod{} p_1)$. 
If not, $\mathcal{B}_i[t]$ is definitely not a pure bucket. 
If so, let $f^{\prime} = f_2^{\prime}$, and we continue to perform the second method.
The second method is called \textbf{Rehashing verification}: 
We calculate the $i^{th}$ hash function to get the $i^{th}$ mapped bucket of $f^{\prime}$, \ie{}, we calculate $h_i(f^{\prime})$. 
Then we check whether $h_i(f^{\prime})$ is equal to $t$. 
If not, $\mathcal{B}_i[t]$ cannot be pure. 
If so, we think $\mathcal{B}_i[t]$ is a pure bucket. 
Note that the checking procedure has false positive error but no false negative error, \ie{}, we may consider some bucket as a pure bucket whereas it is actually not pure. 
% Our experimental results show that this false positive rate is small and tunable ($\S$~\ref{?}). 

\bbb{2) Deleting pure flows:} 
After finding a pure bucket $\mathcal{B}_i[t]$, we insert the flow inside it (\ie{}, flow $f^{\prime}$) and its corresponding size $\mathcal{B}_i^{sum}[t]$ into a list. 
Then we delete $f^{\prime}$ from our \sketchname{} by repeating the deletion operation $\mathcal{B}_i^{sum}[t]$ times. 





\begin{figure}[t!]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.84\linewidth]{lzr/pics/Fermat-Decoding.pdf}
    \vspace{0.2cm}
    \caption{Decoding example of \sketchname{}.}
    \label{algopic:decoding}
    \postfig
\end{figure}



\bbb{\textit{Example:}}
As shown in Figure~\ref{algopic:decoding}, to decode \sketchname{}, we first check all buckets to look for pure buckets. 
For bucket $\mathcal{B}_2[1]$, after \textit{ID verification} and \textit{Rehashing verification}, we consider it as a pure bucket. 
Then we delete the pure flow inside $\mathcal{B}_2[1]$ from our \sketchname{}. 
Specifically, we first locate the two mapped buckets $\mathcal{B}_1[2]$ and $\mathcal{B}_2[1]$, and then subtract $f^{\prime}$ from the two buckets. 



\bbb{Discussion:}
We have two verification methods in decoding, but they are not necessary in some cases. When the storage/transmission/computation overhead is critical and a little higher probability of decoding failure is tolerable, we can omit the second modulo counter and the ID verification. From our strict proof and experimental result in \label{sec:algo:math}, a \sketchname{} with one modulo counter and rehashing verification can achieve a similar small probability of failed decoding as the original \sketchname{}.




% Specifically, we 


% \textbf{1)} ID verification; \textbf{2)} Rehashing verification. 
% For the ID verification, we just suppose $\mathcal{B}_i[t]$ is pure and try to get the flow ID recorded in it. 
% Specifically, we calculate $f_1 = \left( \mathcal{B}_i^{mod_1}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_1-2} \right) \mod{p_1}$ and $f_2 = \left( \mathcal{B}_i^{mod_2}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_2-2} \right) \mod{p_2}$. 


% We propose two methods to check whether a bucket is pure. 




% Next, for each pure bucket $\mathcal{B}_i[t]$, we first calculate the flow stored in it by $f =  \left( \mathcal{B}_i^{sum}[t] \times \left( \mathcal{B}_i^{sum}[t] \right)^{p_1-2} \right) \mod{p_1}$. 
% we calculate the hash functions to get its other $d$ mapped buckets. 
% Then 

% \bbb{Check pure:}


% In \sketchname{}, a bucket can store multiple flows. 
% We call the bucket that include just one flow as \textit{pure bucket}.  




% Each bucket consists of 1)a pair of 33-bit \textit{SumID} fields, \ie $SumID_{A}$ and $SumID_{B}$, to record the modulo $\mathcal{ID}$ sum of its hosting items; 
% and (2) a \textit{counter} field to record the total frequency of its hosting items. 
% Besides, we designate the largest pair of twin primes that is less than $2^{33}$, $p_a$ and $p_b$, to the two \textit{SumID} fields of \sketchname{} so that $SumID_{A} \in \mathbb{Z}_{p_a}$ and $SumID_{B} \in \mathbb{Z}_{p_b}$ for each bucket. 
% % $counter \in \mathbb{Z}_{2^{32}}$
% For each incoming item $e$, or $\mathcal{\langle ID, F \rangle}$, \sketchname{} first calculates $h_1(\mathcal{ID})$, $h_2(\mathcal{ID})$,..., $h_k(\mathcal{ID})$ to get its $k$ hashed buckets, and then inserts $e$ to bucket $h_1(\mathcal{ID})$ in $A_1$, bucket $h_2(\mathcal{ID})$ in $A_2$, and so on. 
% Figure. \ref{fig:algo:insert} illustrates the data structure of \sketchname{} for the case of $m=3$ and $k=3$. 




\presec
\subsection{Placing \sketchnamees{}}
\postsec
\label{sec:algo:encode}
Placing a pair of \sketchnamees{} can detect the victim flows in the path between them. With proper placement strategy, the monitoring component can achieve full coverage of the network, capturing victim flows with accurate location information.
 


 
\presec
\subsubsection{Where to Place \sketchnamees{}}
\postsec
\label{sketchplace}
A systematic placement strategy of \sketchnamees{} provides the ability to pinpoint where the flows lose their packets, \ie, in which switch or which link the loss happens.
% An important requirement for the placement of \sketchnamees{} is the ability to pinpoint where the flows lose their packets, \ie, in which device or which link the loss happens.

\bbb{LossRadar's placement.}
LossRadar \cite{lossradar2016} divides the network into individual long paths.
Each path starts just after the stage in the upstream switch that selects the egress port, and ends before the stage in the downstream switch that selects the egress port. 
% LossRadar \cite{lossradar2016} divides the network into individual paths, each of which starts just after the upstream switch selects the output port and ends where the downstream switch selects the output port. 
%
For each path, LossRadar places an upstream meter at its beginning and a downstream meter at its end. 
For example, in Figure \ref{algopic:placement}, Switch C is an upstream switch and Switch D is a downstream switch. The path starts from the upstream meter to the downstream meter. 

\bbb{LossRadar's shortcoming.}
Similar to LossRadar, our monitoring component can also place \sketchnamees{} as LossRadar.
However, this placement suffers two shortcomings. First, as LossRadar has no visibility to further location information, it can hardly distinguish intra-switch/inter-switch packet losses. 
%Though LossRadar has root cause analyzer, for example, it can hardly distinguish intra-switch packet loss caused by random drop specific to one port or inter-switch packet loss caused by bent fiber, because these two types of loss show no difference in LossRadar. 
%
Second, the paths start at ToR (Top of Rack) switches and end at end-hosts are not well considered. For these paths, because there are only upstream meters, all the victim flows in these paths cannot be detected.

\bbb{\systemname{}'s placement.}
We propose our placement strategy that overcomes these shortcomings by placing additional \sketchnamees{} to further divide the long paths in LossRadar. As shown in Figure \ref{algopic:placement}, to avoid these two shortcomings, for each path, our monitoring component further divides each long path into two short intra-switch/inter-switch paths from the position after the egress queue, and additionally places \sketchname{} at the boundary. The additional \sketchname{} is considered as the downstream \sketchname{} of the intra-switch path, and the upstream \sketchname{} of the inter-switch path simultaneously.
In this way, the victim flows in intra-switch/inter-switch paths can be explicitly located. Besides, the operators can at least detect intra-switch victim flows in the edge paths, and further detect inter-switch victim flows by placing \sketchname{} in end-hosts.
At a cost, this placement consumes an additional switch resources.
In the deployment, we choose placement strategies flexibly based on the remaining resources.
In this paper, we default to this placement strategy.
\presec
\subsubsection{AM-PM \sketchname{}}
\postsec

To ensure the correctness of detection, for each pair of \sketchnamees{}, they should be collected after the last packet inserted into the upstream \sketchname{} is inserted into the downstream \sketchname{}. 

\bbb{AM-PM timestamp.}
To guarantee this, we choose to divide the traffic into continuous monitoring periods.
%
We leverage a timestamp flipping method similar to Alternate Marking Performance Measurement (AM-PM) \cite{am-pm}. 
%
Each switch maintains and periodically flips a 1-bit AM-PM timestamp just after the ingress ports, and attaches the AM-PM timestamp to each incoming packet.
With the AM-PM timestamp, each switch \textit{``dominates''} a group of paths that upstream \sketchnamees{} in these paths are in the switch. That is to say, traffic passing through a group of paths is divided into continuous and alternating AM and PM equal-sized monitoring periods by the flipping timestamp in the corresponding switch. 
%According to when the traffic arrives at ingress ports, the traffic is divided into different monitoring intervals with different upstream timestamps, and the upstream timestamp is assigned to each incoming packet.
%
Each \sketchname{} is also equally divided into an AM part (AM \sketchname{}) and a PM part (PM \sketchname{}) for packets in AM periods (with AM timestamps) and PM periods (with PM timestamps), respectively. 

\begin{figure}[h!]
    \setlength{\abovecaptionskip}{0cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=1.0\linewidth]{lzr/pics/Fermat_switch.pdf}
    \vspace{-0.2cm}
    \caption{Placement of \sketchnamees{}.}
    \label{algopic:placement}
    \postfig
\end{figure}


\bbb{Distinguishing monitoring period.}
To insert each packet into corresponding part of \sketchname{}, we need to correctly distinguish which monitoring period the packet resides in.
%
For each intra-switch path, it is easy to distinguish because the AM-PM timestamp can be easily attached to and transmitted with the packet in the same switch.
%
However, for each inter-switch path, its downstream \sketchname{} placed in another switch has no visibility to the AM-PM timestamp in the upstream switch. 
%
Therefore, we need a communication mechanism for timestamp transmission across switches. Similar to LossRadar, we achieve this by storing the attached AM-PM timestamp in one of the unused bits of IPv4 protocol. 
%
In this way, downstream \sketchname{} in inter-switch path can also correctly distinguish the monitoring period of each packet and insert it into the corresponding part. 
%no priority queue

\presec
\subsection{Collecting \sketchnamees{}}
\postsec
\label{sec:algo:trans}


For each path, to detect the victim flows in the latest monitoring period, the corresponding AM/PM \sketchnamees{} should be collected periodically. In this section, we focus on two parts: 1) when to correctly collect \sketchnamees{}; 2) how to quickly collect \sketchnamees{}.

\presec
\subsubsection{When to Collect \sketchnamees{}}
\postsec
To guarantee the correctness of detection, for each path, each pair of AM/PM \sketchnamees{} should be collected after the traffic with AM/PM timestamps has passed through the path totally, and before the next AM/PM monitoring period starts. 
%
Considering the situation that the switch is severely congested, after a monitoring period ends, the additional waiting time for its traffic to totally pass through the path is up to $2ms$ \cite{kannan2019precise}. 
This requires 1) the predefined waiting time must be longer than $2ms$; 2) the monitoring period must be at least longer than the additional waiting time. Therefore, in order to provide enough time for decoding, diagnosis, and response, we consider 10$\sim$20$ms$ as the most fine-grained scale for monitoring period to achieve both correctness and timeliness. 


\presec
\subsubsection{How to Quickly Collect \sketchnamees{}}
\postsec
%Take switches with data plane and control plane as example. %Considering a switch $S$ and the paths controlled by its AM-PM timestamp, because the control plane of switch $S$ naturally has visibility to its timestamp, it can easily determine when to start fetching \sketchnamees{} of these intra-switch/inter-switch paths.
%However, the specific strategy to fetch \sketchnamees{} is architecture-dependent, and we describe strategies for software switches and programmable switches below.
%
When a switch $S$ determines to collect \sketchnamees{}, \textit{it only focus on the paths that it dominates.}
It needs to fetch \sketchnamees{} in the intra-switch paths from its data plane, and downstream \sketchnamees{} in the inter-switch paths from the data planes of its downstream switches.
%
Because it is naturally fast to fetch \sketchnamees{} from the data plane of software switch, we focus on how to fetch \sketchnamees{} from the data plane of programmable switch at a fast speed.

\bbb{Slow strawman solution.}
With interfaces (\eg, BFRT API in Tofino switch) for communication between control plane and data plane provided by vendors, in the strawman solution, for switch $S$, its control plane directly fetches \sketchnamees{} in the intra-switch paths from the data plane. Note that we just fetch downstream \sketchnamees{} here because their paired upstream \sketchnamees{} are essentially downstream \sketchnamees{} in the intra-switch paths. To further fetch downstream \sketchnamees{} in the inter-switch paths from the data planes of downstream switches, the control plane communicates with downstream switches, and inform their control planes of fetching corresponding \sketchnamees{} from their data planes. 
However, this solution suffers from the extremely limited rate of accessing registers from the data plane through provided interfaces (about 500K 32-bit entries per second). Therefore, this solution can hardly achieve 10$ms$-level monitoring.
%

\bbb{Fast INT-like strategy:}
To speed up the collection process, we propose another INT-like \cite{kim2015band} strategy to fully utilize programmable data plane.
%
For switch $S$, to collect \sketchnamees{} in the intra-switch paths, instead of accessing registers through the provided interface, we use tailored packets to piggyback \sketchnamees{} from the data plane. 
%
To save the CPU resources required for packet generation, the control plane just inject one trigger packet into the data plane, and leverage the switch mirror component to generate all needed tailored packets.
%
Every time a tailored packet passes through the switch pipeline, it piggybacks and clears a bucket of each array of each \sketchname{}.
%
To further minimize the cost of packet receiving, we leverage the recirculate port to recirculate the tailored packets multiple times, so as to pack the piggybacked buckets to jumbo frames.
%
Note that the recirculation does not result in any tailored packet loss. That is because the tailored packets only occupy the recirculate port and CPU PCIE port, which are usually at low utilization or idle. 
%
To fetch downstream \sketchnamees{} in the inter-switch paths from the data planes of downstream switches, switch $S$ informs each downstream switch, and piggybacks the downstream \sketchnamees{} as described above.
%
Leveraging the high-speed data plane, the strategy can support 10-$ms$ level monitoring period.

\presec
\subsection{Decoding \sketchnamees{}}
\postsec
\label{sec:decode}
After collecting a pair of \sketchnamees{}, the monitoring component decodes them to detect the victim flows. As there are lots of available compute resources (switch CPUs and central controller) in the network, we focus on where to execute decoding. 

\bbb{Distributed decoding manner.}
To minimize the burden on the central controller, we propose a distributed decoding manner. If a switch CPU utilization is less than a predefined threshold, the tailored packets that piggyback \sketchname{}es in its dominated paths will be transmitted to the switch. Otherwise, they will be transmitted to the central controller.
%
After receiving the tailored packets, the receiver reconstructs \sketchnamees{} and executes decoding.
%
After decoding, no matter where the decoding is executed, the decoding results will be transmitted to the central controller as the input of the diagnosis component. 
%
Note that a programmable switch establishes and maintains persistent TCP connections through in-band network with other switches and the central controller. As a result, all \sketchnamees{} and decoding results can be completely and reliably transmitted to the central controller. These connections will be directed to the highest priority queue in switches, so as to achieve the fastest collection.
%field $\mathbb{Z}_p$, where $p$ is the prime used in \sketchnamees{}, 



\presec
\subsection{Mathematical Analysis}
\postsec
\label{sec:algo:math}




\begin{theorem}
For a given number of loss flows $F$, \aname{} encodes each packet in $O(d)$ time, and finds all $F$ flows with at least $1-O(F^{2-d})$ probability, which consumes $O(F)$ space and communication overhead and $O(d F)$ time overhead.
\end{theorem}

\begin{proof}

Suppose the verification of the pure bucket is correct every time, the decode procedure is the same as finding a 2-core of a random hypergraph. Specifically, each bucket of \aname{} can be regarded as a point, and each flow can be regarded as a super edge connecting $d$ random points. A \aname{} can be considered as a random graph.
A 2-core of a graph is a sub-graph that all vertices have degree at least 2. If a 2-core exists, \aname{} cannot decode all loss flows completely. Otherwise, suppose all verifications are correct, \aname{} can decode all flows. The probability of a 2-core exists has been well studied. Existing results \cite{molloy2004pure} show that when the graph size (number of buckets) is grater than $(c_d+\epsilon)F$, the 2-core does not exist with probability $1-O(F^{2-d})$, in which condition we can decode all flows. 
\begin{align}
    c_d\approx c_d^*=\frac{\ln(d)+\ln(\ln(d))}{d(1-\frac{1}{d\ln(d)})^{d-1}}.
\end{align}
When $d=3$ or $4$, we have $c_3^*=1.22, c_4^*=1.29$. The space and communication complexity is $O(F)$.





When considering the verification with errors, the probability of successful decode keeps in a same level as that of verification without error. The failure probability of rehashing verification is $\frac{1}{m}<\frac{d}{F}$, and that of ID verification is $\frac{1}{min(p_1, p_2)}$. There are at most $2F d$ different values need to be verified. By Chenoff bound, there is no more than $t=4d^2$ error with probability $1-O(e^{-F})$, which probability can be considered as $100\%$.
$t=4d^2$ is a constant relative to $F$. These $t$ errors can be considered as a case that $d*t$ random buckets are poisoned, which means these buckets cannot be used for decoding. Existing work \cite{molloy2004pure, rink2013mixed, goodrich2011invertibleIBLT} shows that the probability of decode failure incurred by poisoned bucket is of the same order as the probability that all the mapped buckets of a flow are poisoned, which is $F(\frac{dt}{F})^d=o(F^{2-d})$. If we additionally use ID verification, the probability of decode failure is $\frac{o(F^{2-d})}{min(p_1, p_2)}$, which is an ignorable probability.
Our simulation results (See Figure \ref{math:successpr} and \ref{math:decoderato}) also prof our theory results. Therefore, the probability of finding all $F$ flows is at least $1-O(F^{2-d})$, with $O(F)$ space and communication overhead. As there is only constant number of errors $t$, \aname{} can decode all flows with $O(d F)$ time complexity.
\end{proof}


\begin{figure}[h!]
    \setlength{\abovecaptionskip}{-0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.7\linewidth]{lzr/pics/math/decode_success_rate.pdf}
    \vspace{0.2cm}
    \caption{The probability of decoding all loss flows reaches $100\%$ sharply when the total number of buckets is $1.23$ times more than the number of loss flows, where \textit{``ID-V''} means using the technique of ID Verification. ($d=3$)}
    \label{math:successpr}
    \postfig
\end{figure}


\begin{figure}[h!]
    \setlength{\abovecaptionskip}{-0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.7\linewidth]{lzr/pics/math/ratio_of_decoded_flows.pdf}
    \vspace{0.2cm}
    \caption{The average ratio of the decoded flows among all loss flows reaches $100\%$ sharply, where \textit{``ID-V''} means using the technique of ID Verification. ($d=3$)
    }
    \label{math:decoderato}
    \postfig
    \vspace{0.3cm}
\end{figure}

Compare with the state-of-the-art algorithm of finding the differences, Invertible Bloom Lookup Tables (IBLT) \cite{goodrich2011invertibleIBLT}, we reduce the memory and communication overhead by $m\log_2(m)$ bits, and achieves a new function of aggregating the attributes of the same key.

==> SOSP21/Overview.tex <==
\presec
\section{Overview} \postsec
\label{sec:Overview}


\presec
\subsection{Design Challenge}
\postsec

% \bbb{1) Timeliness:}
% %
% The quality of self-healing system depends on timeliness, because the loss caused by device failures and rule misconfigurations increases significantly with time.
% %
% The whole process from monitoring network status to giving reconfigurations must be completed in time.
% %
% The millisecond level is the consensus of most current works \cite{...}.

% \bbb{2) Reliability: }
% %
% The self-healing system cannot miss any anomalies that have occurred.
% %
% Specifically, it can not report a network component (\eg, queue, link) with packet loss as healthy.
% %
% It should be able to report all flows with packet loss, or at least all network components with packet loss in a monitoring period.

% \bbb{3) Versatility: }
% %
% The self-healing system needs to analyze a variety of packet loss causes, including intra-device packet loss and inter-device packet loss.
% %
% Besides, the system should be able to allow operators to easily add (or modify, delete) a new cause of packet loss.


% \bbb{4) Modularity: }

% As discussed above, a self-driving network should consists of three parts: monitoring, analysis, and recovery. In \systemname, as shown in Figure \ref{??}, we design a module for each part. 

% \bbb{Measurement module:}
% The monitoring module is designed for monitoring the major cause of NPAs: packet drops. It consists of an encoding agent in data plane, a delivering agent in control plane, and a decoding agent in remote collector. Leveraging sketches, the encoding agent encodes the flow-level information of each incoming packet(\eg, 5-tuple) in programmable switches. The delivering agent periodically accesses the sketches from the data plane and delivers them to the remote collector. After receiving the sketches, the decoding agent decodes them to capture the flow-level packet drops in every measurement epoch. 

% \bbb{Analysis module:}
% The analysis module is designed for classify the packet drops. A trained machine learning model.

% \bbb{Recovery module:}
% The recovery module is designed for recovering the network from network anomalies. 


\presec
\subsection{Design Overview}
\postsec

\bbb{
1) Encode per-flow traffic statistic with \sketchname.
}

\bbb{
2) Deliver \sketchname to the global controller and decode the FPLs.
}

\bbb{
3) Analyze the cause of FPLs with machine learning models.
}

%When the network falls into NPAs caused by packet drops, the monitoring module first detects where  work of the three modules, this system successfully realize self-driving. 

==> SOSP21/Overview2.tex <==
\presec \section{\systemname{} Overview} \postsec
%
The overview of our system \systemname{} is shown in Figure \ref{pic:overview}.
%
\systemname{} deploys multiple pairs of our \sketchnamees{} inside and between the switches, to monitor the flow-level packet losses in the key forwarding point.
%
Each switch in the data center network communicates with the central controller periodically to transmit all the internal \sketchnamees{} to the central controller after each monitoring period.
%
The central controller decodes the flow-level packet loss events in key forwarding points according to the corresponding paired \sketchnamees{}, and diagnoses the root cause of packet losses through trained machine learning models.
%
Finally, the controller calculates emergent response plans for mitigating the identified network faults.

\begin{figure}[htbp!]
    \setlength{\abovecaptionskip}{0cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.995\linewidth]{lzr/pics/Fermat_workflow.pdf}
    \vspace{-0.2cm}
    \caption{\systemname{} Overview.}
    \label{pic:overview}
    \postfig
\end{figure}

%%
\noindent
\textbf{Monitoring.}
%
Our \systemname{} monitors packet loss events in the key forwarding point (such as physical links, and switch queues) by deploying a pair of \sketchnamees{} on the upstream and downstream of this point.
%
The sketch on each forwarding point records all the packets that pass through the point.
%
Thus, for each packet from a source to a destination, if it is dropped at some point along the way, then this packet must be recorded only at all the upstream points from the source to the dropping point, and must not be recorded at all the downstream points from the dropping point to the destination; if this packet is not dropped, then it must be recorded at all sketches deployed along the path from the source to the destination.
%
\systemname{} deployed at the central controller periodically collects all these \sketchnamees{}.
%
To identify all the packets that may get lost at a switch or a link, \systemname{} ``subtracts'' the downstream \sketchname{} from the upstream \sketchname{}, and decodes the result to obtain the set of all packets lost at this point.

%%
\noindent
\textbf{Diagnosis.}
%
\systemname{} uses a general machine learning classification model without visibility to packet processing logic to diagnose the root causes of packet losses.
%
Our machine learning model uses the values of several corresponding counters in upstream and downstream \sketchnamees{}, and the number of lost packets to represent a flow.
%two types of features to represent a flow: common features and device specific features.
%
%The common features include the values of several corresponding counters in upstream and downstream \sketchnamees{}, and the number of dropped packets.
%
%Device specific features include packet inter-arrival time distribution, packet queuing delay distribution, bandwidth utilization, forwarding capacity utilization, \etc
With a large amount of unlabeled data of packet loss events as input, \systemname{} injects trigger flows into the network, and configure the switches to make the flows experience different classes of packet losses to collect precious pre-labeled data.
%
\systemname{} clusters all the data into multiple groups. For each group, \systemname{} labels data in it as the major class to generate labeled training data.
%
To ensure that the classifier can adapt to the varying network traffic, \systemname{} collects training data and trains the classifier periodically.
%
\systemname{} can use the data of one monitoring period to diagnose the root causes to achieve the highest timeliness, and can also use the data of several continuous monitoring periods to achieve higher accuracy.
%


%%
\noindent
\textbf{Response.}
%
\systemname{} formulates the re-configuration strategies of switches, according to the different root causes of packet losses.
%
\systemname{} evaluates the risk of the re-configuration strategies, according to the scope of switches and flows affected by the re-configuration strategies.
%
For low-risk strategies, \systemname{} automatically performs re-configurations, monitors the results of performance optimization, and rolls back the configuration once the results do not meet the expectation;
%
For medium-risk strategies, \systemname{} requests the permission of the operators before performing re-configuration.
%
For high-risk strategies, \systemname{} only notifies operators of flows suffering packet losses and corresponding root causes. 

==> SOSP21/Recoverymodule.tex <==
\presec
\section{Responding to Network Anomalies}
\postsec
\label{sec:rec}


To respond to network anomalies, the response component formulates re-configuration strategies according to different root causes of packet losses, and then classify them into different risk-levels. 
%
For strategies of different risk-levels, the response component executes them in different working modes.  
%
In this section, we first describe each risk-level and its corresponding working mode in \systemname{}.
%
Then, we detail the reasons for the classification, and the re-configuration strategies for each root cause.
%
\textit{Note that all the re-configuration strategies are based on a premise that the network topology is known to \systemname{}. The central controller informs the switches of the re-configuration strategies over persistent TCP connections.}

\presec
% \subsection{Low-risk Strategies}
\subsection{Strategies for Low-Risk Anomalies}
\postsec

For low-risk strategies, \systemname{} executes them silently. Low-risk strategies include strategies for forwarding loop, forwarding table mismatch, and congestion caused by uneven ECMP. We consider these strategies as low-risk because they are per-flow response. That is to say, in these strategies, each rule re-configured in the forwarding table only affects a flow.




\presec
\subsubsection{Forwarding Loop}
\postsec
Due to the high packet processing speed of switches, a looped flow usually generates a burst, leading to severe congestion. Not only the flow itself, but also other flows passing through the loop suffer serious packet loss and throughput drop. Therefore, we need to quickly eliminate the loop. 

\bbb{Strategy.}
Leveraging the path tracing method mentioned in Appendix \ref{sec:ana:pt}, for each flow $f$ trapped in forwarding loop, we can quickly locate its path and forwarding loop. Then, we select the switch closest to the destination end-host in the forwarding loop, and re-configure its forwarding table to redirect $f$ to the switch closest to the destination end-host in the network.

\bbb{Rollback.}
We need to rollback because we may misjudge the root cause. We adopt a naive strategy, that if the re-configuration cannot work, we quickly withdraw it and report it to the operator.


\presec
\subsubsection{Forwarding Table Mismatch}
\postsec
When forwarding table mismatch happens on a certain flow, it will be dropped and suffer serious throughput drop. Therefore, we need to quickly direct this flow to its destination end-host.

\bbb{Strategy.}
For each flow $f$ dropped by table lookup miss in a certain switch, we re-configure its forwarding table to redirect $f$ to the switch closest to the destination end-host in the network. 

\bbb{Rollback.}
The same as that in loop.

 
\presec
\subsubsection{Congestion Incurred by Uneven ECMP}
\postsec
ECMP is a widely used routing strategy for load balance in data centers. However, ECMP performs badly when the traffic is extremely skewed to the hash function used in ECMP, leading to load imbalance and serious congestion. Therefore, we need to rearrange the traffic to avoid congestion.

\bbb{Strategy.}
Our strategy is to redirect the flows with packet loss in the latest monitoring period to the idle links. For each optional link, we coarsely estimate the traffic volume directed to it by summing the sum counters of \sketchname{}. For the link with less traffic volume, we re-configure the forwarding table to redirect part of flows to it. In this way, we avoid congestion and reduce the number of packets loss. 

\bbb{Rollback.}
After executing the re-configuration, if traffic becomes more uneven in the following several periods, \systemname{} realizes the packet loss is caused by a sudden burst, and then withdraw the re-configuration.

\presec
\subsection{Strategies for Medium-Risk Anomalies}
\postsec
For medium-risk strategies, \systemname{} requests the permission of operators before execution.
Medium-risk strategies include strategies for link failure, switch ASIC failure, and bent fiber. We consider these strategies as medium-risk because they are per-link response. That is to say, in these strategies, each rule re-configured in the forwarding table affects all the flows directed to a certain link.

\bbb{Common strategy.}
There is a common strategy as it is a per-link anomaly, and all the traffic should be directed away from the abnormal link. To achieve this, we re-configure the forwarding tables of the affected switches to ensure that no flows will be directed to the abnormal link. 


\presec
\subsection{Strategies for High-Risk Anomalies}
\postsec
For high-risk strategies, \systemname{} only notifies the operators of flows suffering packet loss and corresponding root causes.
High-risk strategies include strategies for ACL rule drop. We consider these strategies as high risk because ACL rule is related to network security, even asset safety. Therefore, we consider \systemname{} should have no permission to access ACL rules, let alone re-configure them. 

\presec
\subsection{Discussion}
\postsec
The response component can work well with the diagnosis component which only relies on ML-based method. Although the diagnosis component can hardly distinguish forwarding table mismatch from ACL rule drop, it just needs to regard all blackholes as caused by forwarding table mismatch.
In this way, the blackhole caused by forwarding table mismatch can be re-configured, and the blackhole caused by ACL rule drop is never affected.


%First

%Suppose the remote controller understands the topology of the network well. Once the analysis module determines that there is a link failure, the recovery module sends some packets to the affected switches to reconfigure the flow table to ensure that no flows will be directed to the failed link. For example, as shown in Figure \ref{?}, once link ? is failed, the controller notifies switch ? to redirect its flows. 

%However, the link failure may be recovered after replacing the questioned fiber with a new one, and our system should redirect the traffic to this link at that time. This requires our system to continuously sense the condition of the failed link. Therefore, after a link is regarded as failed, its upstream switch generates and sends a probing flow to the failed link in each measurement epoch. Therefore, once the link failure is recovered, the probing flow will not be dropped. At that time, the 
%controller sends packets to withdraw the reconfiguration of flow table.





%Network operators need to carefully update the forwarding table. However, update error is unavoidable, and the recovery module need to recover them as fast as possible.

%\presec
%\section{Recovery agent}
%After the analyzer module determine the type of packet drops, if the type can be recovered by the recovery agent, then the analyzer module informs the recovery agent 
%\postsec



==> SOSP21/intro.tex <==

\presec
\section{Introduction} \postsec
\label{sec:intro}
%1、自动驾驶目标
%2、现状-要求太高
%3、我们的理念，生病的时候再调整 practical。我们以丢包为例，打通自动驾驶，做出原型系统。

%软件定义网络和网络管理复杂性的关系？
%实时测量信息分析系统？相关工作？
%网络测量不是针对特定模块的问题导向的，对吗？

\subsection{Background and Motivation}

%什么是自动驾驶网络
With the increasing network scale and user requirements for network, various modules for high-performance network have emerged, \eg, better BGP models, optimized TCP protocol, and high performance devices \cite{P4}.
However, these individually developed modules make it challenge for operators to understand the actual situation in network.
Therefore, it is desirable to design a self-driving (SD) network \cite{jennifer} that can automatically manage itself.
% to achieve ideal performance. 
Instead of closed-form models of individual protocols or offline anomaly detection on traces, an ideal SD network relies on real-time large-scale data analysis and learning. 
An SD network has three key components: 1) A high-sensitive \textbf{measurement} system reporting large-scale network statues in real time; 2) A clever \textbf{analysis} system finding the defect of the network (\eg, a congestion in the future, a packet loss); and 3) A reliable \textbf{control} system fixing the defect of the network. 
Instead of let each network module work independently, the self-driving network can make every part of the network deeply cooperate with each other. 


%现有的自动驾驶发展的挑战
%挑战A———隔离
%现有的自动驾驶工作基本只针对某些小任务进行研究，没有贯通测量、分析、决策三个关键部分的系统工作。
%1、测量盲目地提供服务。网络测量的研究丰富多样，但基本都是作为一个独立部分（decoupled）进行研究，以求以低代价提供尽可能丰富的信息。我们了解到，在大规模网络中，每时每刻产生大量的测量信息，但有效有益的测量信息往往无法高效反馈给网络的各个成份来帮助他们更好地工作。这是由于测量信息不是任务导向的，不能针对后续部分的需求个性化地提供测量信息。
%2、分析决策部分无力利用测量信息。
%2.1 测量提供的信息量大，分析难这是度高，很难进行实时的分析和报告。
%2.2 此外，在各个协议设计的时候，并没有专门的设计来处理“外部”的网络环境信息
%2.3 有很多现有的工具可以针对一定的网络配置进行分析，但是很大缺陷在于无法做到实时针对真实流量进行调整。
%在当前情况下，测量、分析、决策三部分没有被打通。
%挑战B——实时性
% 实时性要求大量测量信息被收集，实时地分析，转换为对应的诊断和策略。

There are two key problems in existing SD network development: 1) sightless measurement system and 2) weak analyser.
First, lack of co-design with the analysis and decision part, existing measurement works focus on provide rich and timely information at low cost. This has led to difficulties and inefficiencies in the development of the analysis and decision part. 
We learned from our cooperation that in a large-scale network, the measurement system keeps reporting a large amount of measurement information. But most information is useless. These overmuch information largely increases the latency of key information feedback (....). Also, analyzing large amounts of data and finding out key information is time consuming.
% leading to untimely control and incurring performance and reliability losses. 
% interferes with key information, which greatly increases the burden on the analysis part. 
% At the same time, these overmuch information increases the latency of key information feedback, leading to untimely control and incurring performance and reliability losses. 
Second, the analyzer does not have the ability to analyze a large amount of information and make a decision in a short time (\eg{}, a few milliseconds).
% ....
% However, the existing network can neither send a large amount of information to the controller in a short period of time, nor does the controller have the ability to quickly analyze this information.
% We have learned from our partner cloud service vendors that traditional measurement and alarm information is huge and complex, which is not convenient for rapid analysis and decision.
% Therefore, it is quite difficult to design a controller for SD network.


%本文动机——打通 测量、分析、决策，实现一个最基本的自动驾驶网络。一个最基本的自动驾驶网络应该拥有“实时自愈”功能——遇到异常的时候，能够自动地修复自己。拥有实时自愈功能的网络已经可以称为一个半自动驾驶网络。本文选择以实时自愈的半自动驾驶网络为目标进行研究。网络故障的直接表现是丢包，通过丢包的测量+丢包原因分析+丢包故障恢复可以实现一个简单的半自动驾驶网络。
Instead of a true self driving network, our goal is a half self driving network--- a real-time self-healing (RTSH) network which can automatically repair itself when it encounters an abnormality. This is a half self-driving network, because it can also automatically manage itself but only adjust the network when an anomaly occurs. Network abnormalities directly lead to packet loss. Based on the packet loss, we implement three key parts of SD network: packet loss measurement, packet loss cause analysis, and packet loss failure recovery. 

There are three reasons why we set this goal. 
First, it address the two key problems of self driving network and helps build a true self driving network in the future. The RTSH network is similar to SD network. They have similar key components (\ie, measurement, analysis, and decision), common high requirements for automation and timeliness. A SD network can be built based on a RTSH network. 
Second, it is an achievable goal. An abnormal oriented goal reduces the burden of real-time large-scale data analysis and condition diagnosis, because we know that there must be some abnormalities in somewhere. 
Third, it is valuable in practice. Fast and automatic recovery of network abnormalities can better ensure the quality of service. 

% From this we have achieved a simple half self driving network. It addresses the above two key challenges at a smaller scale --- when a packet loss occurs. 

%为什么选择实时自愈的自动驾驶有效且可行？
%1、可行。
%2、应用有益：网络异常是影响网络性能的核心问题，有效面对网络的核心关切——性能和可靠性。
%2、研究方式可行：这样的工作意义在于打通了自动驾驶系统，可以为自动驾驶系统进一步地扩大任务范围奠定基础。

\subsection{Our Proposed Solution}

%我们设计了一种新算法来实时鲁棒地监测异常，相比于其他算法有何优势。
The real-time self-healing network requires the measurement component to provide information as quickly and accurately as possible to reduce the analysis delay and shorten the self-healing period, but existing measurement work is not satisfactory enough.
The state-of-the art packet loss detection scheme occupies a space linearly related to the number of abnormal packets. 
For small amount of packet loss, it is an efficient scheme. 
However, in many cases, a large amount of packet loss may occur (such as rule configuration errors, congestion). At this time, current solution cannot efficiently feedback the network situation, and it relies on other approaches to analyze the cause of a large number of packet loss. We believe the shortcoming of robustness is that the detection granularity is too small. It will be better to use a packet loss detection algorithm whose cost is linearly related to the number of abnormal flows. In this way, when a flow loses many packets, it will not take up too much resources.
In this regard, we designed a scheme whose cost is satisfactory --- linearly related to the number of abnormal flows. It has millisecond measurement delay and high robustness. Its low space and communication cost make a fast global diagnosis become possible.


%我们有多种use cases包括。。
Benefit from timely global information, we can perform accurate abnormal diagnosis and self-healing. Through machine learning, we can perform fast and accurate real-time abnormal diagnosis and error recovery based on various information collected by programmable switches.
For the following three typical anomalies, we can quickly discover and heal ourselves. 
1) Link failure, 
2) Congestion, and
3) Rule misconfiguration.
% Link failure:
%  原因：光纤出现问题，全部数据包丢失。
% 问题特征：在最近的测量周期内下游的fermatsketch没有获得频数数量的增加
% 恢复方案：分析器根据全局视图分析受到链路故障影响的流和交换机，向受到影响交换机发送修复包，对受到影响的流进行配置，将他们改到另一条链路上。然后举个例子。

% Load imblance:
% 应用环境：使用ecmp分配流量的情况 
% 原因：ecmp 哈希不均匀，导致一条链路出现严重丢包。
% 问题特征：在最近的测量周期内检测到大量的拥塞丢包
% 恢复方案：local 版本：检测丢包超过一定阈值的流，分析器发送恢复包到丢包的交换机，将这些丢包严重的流改路到另一条不拥塞的链路。
% global版本：还在设计

% flow table misconfiguration：
% 原因：因为表项配置错误，出现了不应该出现的丢包
% 问题特征：检测到ttl为0的丢包与acl丢包
% 恢复方案：获取最近更新流表的交换机与流表中最近更新的内容。将因为acl丢包和ttl为0丢包（加错误码）且与最近更新的流表内容匹配的流筛选出来，发到最近更新流表的交换机进行第二次判断，如果确实和更新的流表匹配，就恢复最近更新的流表。


%我们能做到怎样的自愈效果？延迟？


\subsection{Key Contributions}
\begin{itemize}[leftmargin=*,parsep=0pt,itemsep=0pt,topsep=2pt,partopsep=2pt]
    \item We design a real-time self-healing (RTSH) network system which lays the foundation for the self driving network.
    \item We design fermat table algorithm to detect abnormalities timely and accurately.
    \item We implement a RTSH network prototype and make it open-source.
\end{itemize}

















% The first reason is that it is easier to adjust the network when anomaly occurs, because we know that there must be something abnormal. 

% can measure the packet drops, analysis the potential defects in the network, and make corrective decisions in real time.

%The self-driving network is a network system that run automatically with specified high-level policy. 

==> SOSP21/introV2.tex <==



% 问题：Fault Detection and Root Cause Localization in Datacenter Networks
% 方法：
% 1. 方法本质：A Machine Learning Approach to
% 2. 方法属性： An Online Algorithm 

% memory, transmission, wire speed

% Wire-speed Fault Detection and Root Cause Localization in Large Scale Datacenter Networks

% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要Fault Detection and Root Cause Localization？参考前人论文

% P2: A Fault Detection and Root Cause Localization solution需要满足什么条件？
% 检测和定位
% 1) high performance：低延迟 高精度(每次丢包都发现)
% 2) coverage 错误类型多 精确定位位置
% 3) Scalability：low bandwidth consumption    低计算（分析）
% 4) generality： 低存储 低计算（测量） 高模块（不需要打破pipeline逻辑） 平台多样 
% 2. Limitations of Prior Art
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？
%     2.1 State-based solution
%         suffer from unnecessary monitoring overhead 或 低精度
%         a Host-based 延迟高（refer to lossradar） 低精度（会漏报报，缺少准确位置）
%         b Packet telemetry 要求可编程交换机、且逐包测量汇聚信息开销大(refer to netseer)。 
%         c Common Statistic in Switch 针对任何流（相对于丢包流）信息进行测量 flowradar +（netseer里Network statistics collection），测量开销大，不满足 d 低存储开销。难以同时做到低延迟和高精度 
%     2.2 Event-based solution
%         netseer 利用可编程交换机直接得到错误码，汇聚事件，只能解决functional的丢包。不能同时满足generality和coverage
%         lossradar 可以探测丢失的包，但是丢包数量过多的时候不可用。不能同时满足high performance和coverage
% 3. Propposed Approach
% P1：方法核心思路是什么？大概怎么工作？
%     利用一种新型的flow level loss的数据结构来探测丢包。两类丢包分别怎么处理。
% P2: 你的方法为什么满足所有条件？
%     a 结构小，可以频繁地进行传输
%     b 大规模部署（定位准确） 线速统计每个包（不漏报）
%     c 基于丢包发现，而非错误码，降低对可编程的依赖。且支持设备异常时的丢包发现。 结构小，规模扩大的时候开销不明显
%     d 结构小，带宽占用、存储开销少
% 4. Technical Challenges and Solutions（一般3-4个）
% P1: Wire-speed Fault Detection难题和方案
% P2：Root Cause Localization问题和方案
% 5. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）

% Paragraph: 第一句话概况全段，余下都是解释





% 恢复
% 1、全自动 静默 ECMP congestion 
% 2、半自动？ routing     silent drop     
% 3、手动 ACL 


% Towards Self-Driving Network Monitoring, Diagnosis, and Repair
% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% P2: 在自动驾驶中需要Practical deployment， ”准确和及时的Global view of the network with low cost: measurement方法需要快速、轻量, 准确“很重要。
% 2. Limitations of Prior Art
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？
% 3. Propposed Approach（多于三段）
% 
% P1: 方法核心思路是什么？大概怎么工作？idea   
% P2: Sketch方法的优点：满足前面measurement条件
% P3: Diagnosis优点
% P4: System实现以及难点（优点）
% 怎么实现十毫秒
% 4. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）



% Towards Self-Driving Network Monitoring, Diagnosis, and Repair
% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% P2  相关工作的问题，两类  一些专注于某部分 一些只有方法论
% P3: 在自动驾驶中需要Practical deployment， ”准确和及时的Global view of the network with low cost: measurement方法需要快速、轻量, 准确“很重要。 
% 3. Propposed Approach（多于三段）
% P1: 方法核心思路是什么？大概怎么工作？idea    丢包驱动故障实现自动驾驶 
% P2: Sketch方法的优点：满足前面measurement条件
% P3: Diagnosis优点
% P4: System实现以及难点（优点）
% 怎么实现十毫秒
% 4. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）


\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% \textit{Para1: Explain why data center networks need Self-Driving.}\\
Recently, data center networks have grown rapidly in scale \cite{?} and have incorporated more new components, \eg, programmable devices \cite{P4}, better BGP models, and optimized TCP protocol. However, these make it challenge for operators to understand and menage the network.
Therefore, a network that can automatically manage itself, called self-driving network, is considered to be an ideal goal of network management \cite{jennifer}.
%自动驾驶三部分
The workflow of self-driving network consists of three parts, monitoring, diagnosis, and repair.
The monitor part measurements the network and provides a network statues for the diagnosis part, \eg, packet loss, congestion and link utilization.
The diagnosis part localize the root cause of any anomaly and report it to the repair part, which diagnosis must be reliable to prevent the wrong repair plan. 
The repair part makes a repair plan based on the diagnosis, and decide whether to adjust the network based on the preset settings.

%自动驾驶的思路
% Instead of traditional approaches including closed-form analysis of individual protocols and offline anomaly detection on traces, one reasonable approach of self-driving network relies on real-time global view and learning-based controllers to perform management.
% The monitor part provides a real-time global view of the network statues for the diagnosis part, which view can reduce the misdiagnosis due to lack of global statues and minimize the loss due to not being discovered in time.




% P2: 在自动驾驶中，”准确和及时的Global view of the network with low cost: measurement方法需要快速、轻量, 准确“很重要。并且需要Practical deployment.
% 
A practical self-driving system that provides fast response, accurate diagnosis, and helpful recovery plan, requires a strong monitor providing timely and clear global view.
The monitor should report every anomaly very quickly to minimize the impact. 
The anomaly statistics should be adequate enough for accurate diagnosis and recovery planning, but not incur too much transmission for networks or computation overhead for the diagnosis part.
In deployment, the self-driving system should be scalable for large number of devices and be general for various platforms, including programmable hardware devices, commodity servers, and dedicated hardware like middleboxes.


% There are four requirements for a packet loss localization solution: high performance, coverage, scalability, and generality.
% (1) high performance. It can locate every unwanted packet loss very quickly (in a few microseconds) to reduce the impact.
% (2) coverage. It can locate most kinds of losses due to different reasons that happened in most devices.
% (3) scalability. It can be deployed in a large-scale data-center network consists of thousands of switches. To reduce additional congestion and the computation overhead of the central analyzer, the solution can only report a limited amount of information to the central analyzer.
% (4) generality. It can be deployed in various platforms, including programmable hardware devices, commodity servers, and dedicated hardware like middleboxes, which require the solution to be memory efficient, computation efficient, and highly modular.
% In programmable hardware devices (\eg, P4 switches and ASIC), the solution should be with small storage consumption (\eg, less than 100KB, 10\%? storage resources in a Tofino switch).
% In software platforms based on commodity servers, the solution should be efficient in computation and memory.
% In dedicated hardware, the solution should be highly modular without relying on other's functions (\eg, the error code).

\subsection{Limitations of Prior Art}
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？
At present, there is no self-driving system and existing monitoring schemes are not satisfactory for self-driving network.
Among exiting monitoring schemes, only event-based solutions, which only focus on the flows with abnormal events rather than all flows, may meet our requirement. Because non event-based solutions, including probe \cite{?}, the statistic of all flows \cite{?}, and in-band telemetry solutions \cite{?}, cannot achieve high timeliness and clearness due to their unnecessary overhead generated by healthy flows.
The state-of-the-art event-based solutions are NetSeer \cite{iga2003dynamical} and LossRadar \cite{li2016lossradar}. 
NetSeer summarizes abnormal events reported by the programmable switches efficiently, but cannot achieve good generality of platforms without relying on active reporting from the programmable switch. 
LossRadar achieves good generality in deployment, but both its transmission overhead and computation overhead in diagnosis are linearly increasing with the number of loss packets, which becomes intolerable when serious and wide anomaly happens.

% loss radar netseer
\subsection{Proposed Approach}

% P1: 方法核心思路是什么？大概怎么工作？idea
Our key idea is to leverage a self-driving system by a proper monitor scheme designed according to the requirements of the diagnosis and the recovery part.
The diagnosis and recovery part requires a timely and clear view, and the view should cover all components of the networks. We design a novel sketch algorithm as our monitor scheme, which is in the right position in the trade-off of monitoring timeliness and reporting clarity.
Based on the monitor, our controller, which diagnosis and recovery the network, can locate the root cause of anomalies and make a practical recovery plan.

% P2: Sketch方法的优点：满足前面measurement条件
The superiority of our monitor lies in its active telemetry of flow events. Our monitor performs active telemetry that can detect anomalies by a sketch module without relying on the device to actively report anomalies. Therefore out monitor can achieve good generality of different platforms. In addition, the storage and transmission overhead incurred by the monitor is linearly related to the number of abnormal flows, which is a suitable granularity that can provide sufficient monitoring information without causing excessive burden on the network.

% P3: Diagnosis and Repair优点
Our diagnosis system based on machine learning model can accurately classify the root causes of anomalies, and our recovery system will automatically generate corresponding recovery plans for the operators. 
Our accurate diagnosis performance benefits from both the high-quality data from the monitor and the significant advancement of machine learning technology. 
Our machine learning model can easily incorporate new input features from monitor and new causes of anomalies. Also, the model is highly modular that can be improved and be replaced in the future easily without disturbing other parts of the system.
Our recovery system classifies different anomalies into different risk levels, generates recovery plans, and brings the operator the option of configuring automatic self-driving recovery.

% P4: System实现以及难点（优点）
A key challenge in our system is to design a satisfactory monitor scheme that can capture abnormal flows efficiently. 
Among all network anomalies, packet loss is the most serious and most widespread type of anomaly. 
Take the packet loss as an example, the problem is to find the flow with packet loss.
In many cases, the device cannot actively report packet loss, such as middlebox anomaly, malfunction of the data plan??, we must actively discover the flow with packet loss through algorithms.
The problem becomes finding the flow with packet loss through comparing two traffic streams pass through different locations to find the difference.

An existing solution Invertible Bloom Filter (IBF) can find the lost packets by comparing two traffic streams, but its overhead is linearly increasing with the packet number. We design a new data structure called \aname{} inspired by IBF.
\aname{} has gained a more powerful function that can de-duplicate lost packets to accurately report abnormal flows, and \aname{} uses less hash computation and occupies less bandwidth. The key technique of \aname{} is to leverage Fermat’s little theorem to handle the register overflows and de-duplicate lost packets.

%  packet-drop-driving?

% claim....
% In this paper, we build a system prototype of self-driving network.
% ...


% Key idea 1: why we can build the first self-driving networks..  
% 1. serious problem, packet drop cause problems.. activate system.
% compared with exisitng, small problem, active work.. packet-drop-driving
% many other problem, we will address it in the future work.
% 2. measurement light... small for packet drop. memory/bandwith usage, dignosize 联动起来

% key idea 2
% fermat table的keyidea... XOR same key appear twice, none. Fermat addition...
% no need for carry in.

% How we disgnoize and recovery repair..
% ...

% Our sytem advangages, challenges, .10ms...
% ...key design... test-bed, ns-2, C++ ...

% practical deployement..
% Self-driving too ideal.. 
% Our key idea is active telemetry of flow event. 
\subsection{Summary of Experimental Results}
% P1: 如何试验，结果如何（列最好结果）
....



==> SOSP21/introV3.tex <==
\presec 
\section{Introduction} 
\postsec


\subsection{Background and Motivation}
\postsec
%%
As data center networks have grown rapidly in both size and complexity, managing such networks has been a difficult task that involves a great deal of manual effort.
%
Although the concept of self-driving networking has been proposed \cite{feamster2017andJennifer}, industrial grade solutions have not emerged.
%
A self-driving networking solution should consist of three components for performance monitoring, fault diagnosis, and emergency response, respectively.
%
The performance monitoring component measures network metrics that represent the status of a network, such as packet loss, congestion, and link utilization, and detect network anomalies.
%
The monitoring component needs to be both scalable and generally applicable.
%
For scalability, for example, for a packet loss based network monitor, its communication and computation complexity need to be scalable with the number of lost packets.
%
For applicability, a network monitor should work for different types of switches.
%
Given a network anomaly, the fault diagnosis component localizes the root cause.
%
Given a root cause, the emergency response component calculates a remedy solution that can address the detected anomaly, such as changing the routing path for a flow so that an abnormal path can be avoided.

\subsection{Limitations of Prior Art}
%%
Some pioneer work has been done towards the ultimate goal of self-driving networks; however, they are either not scalable or not generally applicable.
%
LossRadar \cite{lossradar2016} captures each packet loss individually in a data center network.
%
Although LossRadar can be deployed on different types of switches, its transmission and computation overhead increases linearly with the number of lost packets, which is not scalable and thus difficult to be deployed in industry as a network anomaly may cause a large number of lost packets.
%
NetSeer \cite{netseer2020} is an in-data-plane monitor that aggregates abnormal flow events in a data plane and locates the root cause of an anomaly.
%
Although NetSeer is scalable with the number of lost packets, it can only be deployed on programmable P4 switches.

\begin{table*} [!ht]
\begin{center}
\caption{Comparison with the state-of-the-arts. In this table, $\Delta F$ refers to the number of flows with packet losses, $\Delta P$ refers to the number of packets with packet losses, $F$ refers to the number of flows, and BM refers to P4 behavior model \cite{p4behaviormodel}.}
\vspace{0.3cm}
\label{table:compare}
\begin{tabular}{|c|c|c|c|c|}
\hline

\textbf{Characteristics}&\textbf{FermatDriver}&\textbf{LossRadar}&\textbf{FlowRadar}&\textbf{NetSeer}\\
\hline
Computation/Communication complexities& $O(\Delta F)$& $O(\Delta P)$& $O(F)$ & $O(\Delta P \sim \Delta F)$\\
\hline
Independence on programmable switch & \checkmark& \checkmark& \checkmark & $\times$\\
\hline
Implementation in Tofino switch& \checkmark& BM& BM & \checkmark\\
\hline
\end{tabular}
\vspace{-0.2in}
\end{center}
\end{table*}



\presub \subsection{Proposed Approach} \postsub
%
Towards the ultimate goal of self-driving networking, we build a system called \emph{FermatDriver}, which can fast and accurately monitor packet losses, detect anomalies, pinpoint root causes, and find urgent response solutions.
%
For network anomaly detection, we propose a fast, accurate, and light-weight sketch based algorithm, called \sketchname{}, for monitoring the number of lost packets, and our algorithm works for different types of switches, no matter they are programmable or not.
%
We focus on packet losses because most network anomalies (no matter caused by switch hardware, software, configuration, or protocols) experience packet losses.
%
The key novelty of our packet loss monitoring algorithm is on designing a new sketch data structure based on the Fermat's little theorem for handling register overflows and de-duplicate lost packets.
%
For root cause localization, we propose a fast machine learning scheme that can pinpoint root cause with high accuracy.
%
For emergency response, we propose different response strategies for anomalies with different levels.

%%
Our packet loss monitoring algorithm is both scalable and generally applicable.
%
For scalability, the computation and communication complexities of our algorithm are both $O(\Delta F)$, where $\Delta F$ is the number of flows with packet losses.
%
In contrast, the computation and communication complexities of the state-of-the-art packet loss monitoring algorithm, LossRadar \cite{lossradar2016}, is $O(\Delta P)$, where $\Delta P$ is the number of lost packets.
%
Note that $\Delta F$ is typically orders of magnitude smaller than $\Delta P$ as one flow may have many lost packets.
%
For applicability, our algorithm can be deployed on both programmable and non-programmable switches.

%%
We implemented our packet loss monitoring scheme, root cause localization scheme, and emergency response scheme, and deployed them on a testbed environment with 10 switches and 8 end-hosts connected with 40Gbe links in a FatTree topology.
%
%
Our experimental results show that within tens of milliseconds, the system can accurately monitor packet losses, pinpoint network faults that lead to packet losses, and automatically calculate an emergency response plan for mitigating these network faults.
%
All related codes will be open-sourced anonymously\footnote{\url{https://github.com/FermatDriver/FermatDriver}}.

==> SOSP21/introV3old.tex <==



% 问题：Fault Detection and Root Cause Localization in Datacenter Networks
% 方法：
% 1. 方法本质：A Machine Learning Approach to
% 2. 方法属性： An Online Algorithm 

% memory, transmission, wire speed

% Wire-speed Fault Detection and Root Cause Localization in Large Scale Datacenter Networks

% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要Fault Detection and Root Cause Localization？参考前人论文

% P2: A Fault Detection and Root Cause Localization solution需要满足什么条件？
% 检测和定位
% 1) high performance：低延迟 高精度(每次丢包都发现)
% 2) coverage 错误类型多 精确定位位置
% 3) Scalability：low bandwidth consumption    低计算（分析）
% 4) generality： 低存储 低计算（测量） 高模块（不需要打破pipeline逻辑） 平台多样 
% 2. Limitations of Prior Art
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？
%     2.1 State-based solution
%         suffer from unnecessary monitoring overhead 或 低精度
%         a Host-based 延迟高（refer to lossradar） 低精度（会漏报报，缺少准确位置）
%         b Packet telemetry 要求可编程交换机、且逐包测量汇聚信息开销大(refer to netseer)。 
%         c Common Statistic in Switch 针对任何流（相对于丢包流）信息进行测量 flowradar +（netseer里Network statistics collection），测量开销大，不满足 d 低存储开销。难以同时做到低延迟和高精度 
%     2.2 Event-based solution
%         netseer 利用可编程交换机直接得到错误码，汇聚事件，只能解决functional的丢包。不能同时满足generality和coverage
%         lossradar 可以探测丢失的包，但是丢包数量过多的时候不可用。不能同时满足high performance和coverage
% 3. Propposed Approach
% P1：方法核心思路是什么？大概怎么工作？
%     利用一种新型的flow level loss的数据结构来探测丢包。两类丢包分别怎么处理。
% P2: 你的方法为什么满足所有条件？
%     a 结构小，可以频繁地进行传输
%     b 大规模部署（定位准确） 线速统计每个包（不漏报）
%     c 基于丢包发现，而非错误码，降低对可编程的依赖。且支持设备异常时的丢包发现。 结构小，规模扩大的时候开销不明显
%     d 结构小，带宽占用、存储开销少
% 4. Technical Challenges and Solutions（一般3-4个）
% P1: Wire-speed Fault Detection难题和方案
% P2：Root Cause Localization问题和方案
% 5. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）

% Paragraph: 第一句话概况全段，余下都是解释





% 恢复
% 1、全自动 静默 ECMP congestion 
% 2、半自动？ routing     silent drop     
% 3、手动 ACL 


% Towards Self-Driving Network Monitoring, Diagnosis, and Repair
% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% P2: 在自动驾驶中需要Practical deployment， ”准确和及时的Global view of the network with low cost: measurement方法需要快速、轻量, 准确“很重要。
% 2. Limitations of Prior Art
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？
% 3. Propposed Approach（多于三段）
% 
% P1: 方法核心思路是什么？大概怎么工作？idea   
% P2: Sketch方法的优点：满足前面measurement条件
% P3: Diagnosis优点
% P4: System实现以及难点（优点）
% 怎么实现十毫秒
% 4. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）



% Towards Self-Driving Network Monitoring, Diagnosis, and Repair
% Introduction:
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% P2  相关工作的问题，两类  一些专注于某部分 一些只有方法论
% P3: 在自动驾驶中需要Practical deployment， ”准确和及时的Global view of the network with low cost: measurement方法需要快速、轻量, 准确“很重要。 
% 2. Propposed Approach（多于三段）
% P1: 方法核心思路是什么？大概怎么工作？idea    丢包驱动故障实现自动驾驶 
% P2: Sketch方法的优点：满足前面measurement条件
% P3: Diagnosis优点
% P4: System实现以及难点（优点）
% 怎么实现十毫秒
% 4. Summary of Experimental Results
% P1: 如何试验，结果如何（列最好结果）


\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}
% 1. Background and Motivation
% P1: 为什么Datacenter Networks需要自动驾驶？Datacenter Networks自动驾驶主要三个部分，三部分功能。
% \textit{Para1: Explain why data center networks need Self-Driving.}\\
As data center networks have grown rapidly in both size and complexity, managing such networks has been a difficult task that involves a great deal of manual effort.
%
Although the concept of self-driving networks has been proposed \cite{feamster2017andJennifer}, industrial grade solutions, which can unify themonitoring, diagnosis, and repair, have not emerged.
%


scale and have incorporated more new components, \eg, programmable devices \cite{bosshart2014p4}, better BGP models \cite{abhashkumar2021running}, and optimized TCP protocol \cite{mukerjee2020adapting}. However, these make it challenge for operators to understand and manage the network.
Therefore, a network that can automatically manage itself, called self-driving network, is considered to be an ideal goal of network management \cite{feamster2017andJennifer}.
The workflow of self-driving network consists of three layers, monitoring, diagnosis, and repair.
The monitor layer measures the network and provides a network statues for the diagnosis layer, \eg, packet loss, congestion, and link utilization.
The diagnosis layer localizes the root cause of any anomaly and reports it to the repair layer.
% which diagnosis must be reliable to prevent the wrong repair plan. 
The repair layer makes a repair plan based on the diagnosis, and decides whether to adjust the network based on the preset settings. 
Based on the three layer, a self-driving system can provide timely monitoring, accurate diagnosis, and helpful repair plan.


% 
To the best of our knowledge, there is no practical self-driving system. Existing works related to self-driving can be classified into two types. 
%
The first type stays at conceptual level \cite{??}.
%种子
The seminiar work is done by Nick and Jennifer, and they propose the concept and principle of self-driving network and discuss its characteristic and feasibility for the first time \cite{feamster2017andJennifer}.
%
The second type only focuses on specific layers of self-driving networks \cite{...}. %监测+诊断
% Some existing works focus on specific layers of self-driving networks, such as monitoring and diagnosis. 
% Most exiting monitoring schemes are not practical for the self-driving network because they cannot capture all network anomalies timely.
% In the monitor layer, most exiting schemes are not
% practical for the self-driving network because they cannot capture all network anomalies with both high timeliness and clearness.
% Only event-based monitor, which only focuses on the flows with abnormal events rather than all flows, can achieve high timeliness and clearness, because they avoid unnecessary overhead of monitoring healthy flows.
Two typical works are LossRadar \cite{lossradar2016} and NetSeer \cite{netseer2020}. 
%
LossRadar is general for various devices, but both its transmission overhead and computation overhead in diagnosis are linearly increasing with the number of loss packets, which becomes intolerable when serious and wide anomaly happens.
%
NetSeer summarizes anomalies reported by making full use of the programmability of P4 switches, but is inapplicable for data centers in which some switches are not programmable.
Further, these two systems do not implement the repair layer.
%but cannot achieve good generality of platforms without active reporting from the programmable switch. 
%
% NetSeer cannot achieve good generality of platforms because it relies on active reporting from the programmable switch. LossRadar has high transmission overhead and computation overhead that are linearly increasing with the number of loss packets, which becomes intolerable when serious and wide anomaly happens.
%诊断监测没有连接
% Exiting diagnosis tools are offline analysis tools based on network topology and configurations \cite{liu2018automatic, ???}. 
% After that, some work focuses on specific tasks in self-driving networks, such as intent-based policy configuration \cite{jacobs2018refining}, preventing Denial-of-service attacks \cite{demoulin2018automated}, and others \cite{kalmbach2018empowering}. 


As shown in Figure \ref{intro:layers}, existing works about self-driving networks focus on and extend the ability, scalability, and functions of one or two of the three layers. 
%One possible reason is that it is much more challenging to simultaneously design and implement all three layers.
One possible reason is that an elegant design and implementation of any one of the three layer is already very challenging.
The ideal goal is to build a well-established system with all three layers, and can automatically repair any network problems quickly.
%
To approach the ideal goal, the design goal of this paper aims to build a system prototype with all three layers, and can automatically repair some typical network problems quickly. No existing work achieves this design goal.


\begin{comment}
% A practical self-driving system should provide fast response to anomalies, accurate diagnosis, and helpful repair plan on various network devices.
A practical self-driving system should provide fast response, accurate diagnosis, and helpful repair plan on various network devices.
% , requiring a strong monitor providing timely and clear global view.
Specifically, the system should respond to every anomaly very quickly to minimize the impact. 
The anomaly statistics provided by monitor should be adequate enough for accurate diagnosis and repair planning, but not incur too much transmission for networks or computation overhead for the diagnosis layer.
In deployment, the self-driving system should be scalable for large number of devices and be general for various platforms, including programmable hardware devices, commodity servers, and dedicated hardware like middle boxes.
\end{comment}



% There are four requirements for a packet loss localization solution: high performance, coverage, scalability, and generality.
% (1) high performance. It can locate every unwanted packet loss very quickly (in a few microseconds) to reduce the impact.
% (2) coverage. It can locate most kinds of losses due to different reasons that happened in most devices.
% (3) scalability. It can be deployed in a large-scale data-center network consists of thousands of switches. To reduce additional congestion and the computation overhead of the central analyzer, the solution can only report a limited amount of information to the central analyzer.
% (4) generality. It can be deployed in various platforms, including programmable hardware devices, commodity servers, and dedicated hardware like middleboxes, which require the solution to be memory efficient, computation efficient, and highly modular.
% In programmable hardware devices (\eg, P4 switches and ASIC), the solution should be with small storage consumption (\eg, less than 100KB, 10\%? storage resources in a Tofino switch).
% In software platforms based on commodity servers, the solution should be efficient in computation and memory.
% In dedicated hardware, the solution should be highly modular without relying on other's functions (\eg, the error code).

% \subsection{Limitations of Prior Art}
% P1：前人solution都不能全部满足这些条件： 前人方法分几类，每一类怎么工作，为什么这一类不能满足条件？

\begin{figure}[t]
    \setlength{\abovecaptionskip}{0.15cm}
    \setlength{\belowcaptionskip}{0cm}
    \prefig
    \centering  
    \includegraphics[width=0.995\linewidth]{wuyuhan/intro_graph1.pdf}
    \caption{Methodology for designing self-driving system.}
    \label{intro:layers}
    \postfig
\end{figure}

% loss radar netseer
\presub
\subsection{Proposed Approach} \postsub


% P1: 方法核心思路是什么？大概怎么工作？idea
Towards the above design goal, we manage to build a system which can automatically repair those network problems that lead to packet loss.
We choose these problem because most network problems are closely related to the packet loss \cite{netseer2020}.
% Our methodology is that we devise a backbone self-driving system with all three layers which can be extended to various complex situations.
% We start from a backbone system fixing the packet loss, which is the most common anomaly in the network, to build a 
In our system, we carefully design each of the three layers.
% We devise a complete self-driving system consists of monitoring, diagnosis, and repair.
The first and most critical step is to design a light and effective monitoring layer, because the subsequent two layers deeply rely on the monitor.
%搜一下deeply rely on
% The diagnosis and repair layer requires the monitor to report timely and clear packet loss information.
%monitor这块主流方法是sketch，最好的是lossradar，不够efficient，所以我们提出了新的sketch
We propose a novel algorithm leveraging Fermat's little theorem, which can monitor packet loss fast and accurately and is general for various platforms.
% Based on the monitor, our controller, which diagnosis and repair the network, can locate the root cause of anomalies and make a practical repair plan.
In the diagnosis layer, we devise a machine learning model that is accurate and general for various input features and output results.
In the repair layer, we classify the network problems into different risk levels and provide corresponding repair plan.



% P2: Sketch方法的优点：满足前面measurement条件
The key technical depth of our system lies in the design of the monitoring layer. 
For the monitor layer, sketches, a type of probabilistic algorithm, have been widely acknowledged as the most promising solution.
The state-of-the-art sketch for packet loss is LossRadar \cite{lossradar2016}.
It leverage Invertible Bloom Filters \cite{?IBT} to detect packet loss.
LossRadar can find the lost packets by comparing two traffic streams, and its space complexity is $O(p)$, where $p$ is the number of lost packets. 
The key operation of LossRadar is the XOR operation of packet IDs, where the ID of each packet is different.
% As a flow have many packets, it uses a Bloom filter to distinguish the packets of the same flow.
% de-duplicate the packets of the same flow.
In practice, some network problems incurred by misconfigurations often lead to the loss of many packets, but these packets often belongs to one or a few flows.
It is desired to have an algorithm whose space complexity is $O(N)$ to reduce the overhead of transmission and storage, where $N$ is the number of flows with packet loss. 
% Therefore, we propose a new data structure called \aname{}, which leverages the Fermat's little theorem.
% Our \aname{} replaces the XOR operation with Fermat addition operation (See details in Section \ref{?}).
Therefore, we propose a new data structure called \aname{}, which leverages the Fermat's little theorem to 
% Our \aname{} replaces the XOR operation with Fermat addition operation (See details in Section \ref{?}).
gains a more powerful function that can de-duplicate lost packets to accurately report flows, and \aname{} uses less hash computation and occupies less bandwidth. 
% The key technique of \aname{} is to leverage Fermat’s little theorem to handle the register overflows and de-duplicate lost packets.
% its active telemetry of flow events. 
% Our monitor performs active telemetry that can detect anomalies by a sketch module without relying on the device to actively report anomalies.
% Therefore out monitor can achieve good generality of different platforms. 
% In addition, the storage and transmission overhead incurred by the monitor is linearly related to the number of abnormal flows, which is a suitable granularity that can provide sufficient monitoring information without causing excessive burden on the network. 
% The key challenge is to design a satisfactory monitor scheme that can capture abnormal flows efficiently. 
% In many cases, the device cannot explicitly report packet loss, such as in commodity switches or black-box middleboxes, we must actively discover the flow with packet loss through algorithms.
% The problem becomes finding the flow with packet loss through comparing two traffic streams pass through different locations to find the difference.
% An existing solution LossRadar \cite{lossradar2016} can find the lost packets by comparing two traffic streams, but its overhead is linearly increasing with the packet number. We design a new data structure called \aname{} inspired by IBF.
% \aname{} has gained a more powerful function that can de-duplicate lost packets to accurately report abnormal flows, and \aname{} uses less hash computation and occupies less bandwidth. The key technique of \aname{} is to leverage Fermat’s little theorem to handle the register overflows and de-duplicate lost packets.


% P3: Diagnosis and Repair优点
Our diagnosis system based on machine learning model can accurately classify the root causes of anomalies, and our repair system will automatically generate corresponding repair plans for the operators. 
Our accurate diagnosis performance benefits from both the high-quality data from the monitor and the significant advancement of machine learning technology. 
Our machine learning model can easily incorporate new input features from monitor and new causes of anomalies. Also, the model is highly modular that can be improved and be replaced in the future easily without disturbing other layers of the system.
Our repair system classifies different anomalies into different risk levels, generates repair plans, and brings the operator the option of configuring automatic self-driving repair.


% P4: System实现以及难点（优点）
We fully devise all layers of a self-driving system driven by packet loss events, and implement it based on programmable switches and servers. To our knowledge, it is the first self-driving network system. Within tens of microseconds, the system can accurately diagnosis 10 kinds of anomalies leading to packet loss, and then automatically fix the network or send a repair plan to the operators. Our system design is general for deployment in various platforms and can be extended to many more anomalies.
%10ms，实验环境，具体任务，我们将在未来扩展更多任务。

%  packet-drop-driving?
% claim....
% In this paper, we build a system prototype of self-driving network.
% ...


% Key idea 1: why we can build the first self-driving networks..  
% 1. serious problem, packet drop cause problems.. activate system.
% compared with exisitng, small problem, active work.. packet-drop-driving
% many other problem, we will address it in the future work.
% 2. measurement light... small for packet drop. memory/bandwith usage, dignosize 联动起来

% key idea 2
% fermat table的keyidea... XOR same key appear twice, none. Fermat addition...
% no need for carry in.

% How we disgnoize and repair repair..
% ...

% Our sytem advangages, challenges, .10ms...
% ...key design... test-bed, ns-2, C++ ...

% practical deployement..
% Self-driving too ideal.. 
% Our key idea is active telemetry of flow event. 
% \subsection{Summary of Experimental Results}
% P1: 如何试验，结果如何（列最好结果）
% ....



==> SOSP21/related.tex <==
\presec
\section{Background and Related Work} \postsec
\label{sec:relatedworks}

%sub1：现有自动驾驶的特点
%sub2：现有的工作做某一部分。
\presec
\subsection{Self-Driving Networks } \postsec
% To wyh: 既然related work放在后面，应该不用介绍self-driving network，应该在intro里就有了？


Self-driving network includes two key components: 1) interpretation from high-level policy to concrete measurement and control scheme; 2) real-time monitoring, analysis and control realization.
Due to the difficulty of establishing a full automatic self-driving network, recent works are associated to only part of the self-driving network system. 

% 不想引workshop，质量太低
Few works actually try to solve the problem of generating measurement and control operations with high-level specification.
However, some are closely related to this field.
Marple\cite{marple} and its corresponding hardware design bridges the network performance queries and switch programs. 
Sonata\cite{sonata} provides a telemetry system with flexible interfaces for a wide range of telemetry tasks.
Unfortunately, in the above-mentioned works the high-level policy should first be expressed in detail with the language or interfaces before translating to a concrete measurement scheme.

real-time monitoring, analysis and control is essential for self-driving network to run.
One popular way to make these functions fast is to apply these in the data plane, especially programmable switches.
Plenty of works concentrate on how to store and operate data structures on programmable switches\cite{univmon, beaucoup, elastic}.
We make effort to deploy fermatSketch in programmable switches to provide real-time measurement.


\presec
\subsection{Packet Drop} \postsec



% Why we need self-driving network? 随着物联网、5G时代的到来，网络规模变得愈发庞大。各种新型应用，如VR，对网络提出了前所未有的实时性、稳定性要求。在此情况下，网络管理变得愈发重要且困难。随着人工智能技术的蓬勃发展，人们不禁要问：是否能构建自动驾驶网络——一种实时地which measure, analyze, and run themselves的网络。

%What's self-driving network?
%The self-driving network is a network system that can run itself independently--- automatically adjust itself to achieve high performance, sufficient reliability and low additive cost.
%Specifically, it has three key components: 1) A high sensitive measurement reporting network statues in real time; 2) A clever analysis system finding the defect of the network; and 3) A reliable decision-making system fixing the defect of the network. A perfect/ideal self-driving network was not built in a day. We focus on a real-time self-correcting network, an infant self-driving network, that can measure the packet drops, analysis the potential defects in the network, and make corrective decisions in real time.

%The self-driving network is a network system that run automatically with specified high-level policy. 

%然而，要想实现这一宏大的目标，需要一代网络工作者的不懈努力。
%\subsection{Measurements for SD Network}


%In this section, we mainly introduce the following four kinds of existing monitoring tools. As shown in Table \ref{??}, compared with our \systemname{}, existing monitoring tools either cannot report exact location information of packet drops, or cannot handle all flow-level drop with limited memory in switches. Our \systemname{} is designed to handle these requirements simultaneously.
%Due to their limitations, we design \systemname{} to meet them simultaneously




%\bbb{End-host-based Solutions}
%These solutions send probe packets into network or analyze the performance of transport layer to capture and analyze packet drops in end-hosts. Typical end-host-based solutions include Pingmesh \ref{???}, Trumpet \ref{??}, 007 \ref{??}, and more \ref{??}. Specifically, 007 sends carefully crafted traceroute packets to find the path of flows suffering packet drops. Based on these paths, 007 adapts a voting scheme to locate the most problematic link. However, because of the lack of insight into switches, end-host-based cannot pinpoint exactly where a packet is dropped every time.


%\bbb{Mirroring Solutions}
%These solutions mirror packets to control plane in switches or remote controller. Typical end-host-based solutions include EverFlow \ref{??}, Netseer \ref{??}. The state-of-the-art Netseer leverage programmable switches to mirror packets dropped in programmable switches to control plane......??? 


%\bbb{Sketching-based Solutions}
%These solutions build counters in switches to detect packet drop by collecting flow-level or packet-level information. Typical sketching-based solutions include SNMP \ref{??}, Flowradar \ref{??}, Lossradar \ref{??}, Omnimon \ref {??}. Flowradar captures flow-level packet drops by leveraging bloom filter \ref{?}, invertible bloom filter \ref{?} and CM sketch simultaneously. The memory usage of Flowradar is proportional to the number of flows. Its successor Lossradar captures per-packet drop in invertible bloom filter with the memory usage proportional to the number of dropped packets. Omnimon ....
%However, existing solutions either drill down to packet-level drop, which is over-monitored because existing drop modes never consider the sequence number of packets, or provide fine-grained flow-level drop measurement with the memory usage proportional to the total number of flows in the measurement epoch, which is unacceptable in large-scale network under the strict constraint of extremely limited memory in switches.


%\subsection{Analysis and Decisions in SD Network}

% 目前，在特定任务上，已经有部分工作推动网络自动化的发展，但还没有一个完整的自动驾驶系统。“On Analyzing Self-Driven Networking: A Systems Thinking Approach”和“Empowering Self-Driving Networks”给出了许多关于自动驾驶的思考。Refining Network Intents for Self-Driving Networks 使用意图驱动模型生成网络配置，Automatic Life Cycle Management of Network Configurations实现了自动化的网络配置管理。
%Automatically Repairing Network Control Planes Using an Abstract Representation实现了自动化的控制面配置修复，但是实时性较差。









%\presec
%\subsection{Requirements on Packet Drop Detection} \postsec
We list four key requirements on packet drop detection as follows. 


%\bbb{Fast detection to minimize the impact on network}
Packet drop may occur for various reasons in data center.
 However, TCP regards all kinds of drops as signal of congestion, and it will degrade the throughput to mitigate the congestion. Therefore, a few packet drops unrelated to congestion may seriously degrade the throughput, hurt the performance of application, and thus cause service level violations \ref{??}. To address this issue, we need to capture packet drops as fast as possible, guaranteeing the performance of network operations and application by fast recovery. 

%\bbb{Persistent monitoring to detect all packet drops} 
Packet drop can happen at any time. As discussed above, missing a few packet drops may lead to slow recovery and a period of SLA violation. Therefore 

%\bbb{Flow-level packet drop detection:}    


%\bbb{Locating where and why packet drops}


% \presec
% \subsection{Existing Monitoring Tools} \postsec   

% In this section, we mainly introduce the following four kinds of existing monitoring tools. As shown in Table \ref{??}, compared with our \systemname{}, existing monitoring tools either cannot report exact location information of packet drops, or cannot handle all flow-level drop with limited memory in switches. Our \systemname{} is designed to handle these requirements simultaneously.
% %Due to their limitations, we design \systemname{} to meet them simultaneously




% \bbb{End-host-based Solutions}
% These solutions send probe packets into network or analyze the performance of transport layer to capture and analyze packet drops in end-hosts. Typical end-host-based solutions include Pingmesh \ref{???}, Trumpet \ref{??}, 007 \ref{??}, and more \ref{??}. Specifically, 007 sends carefully crafted traceroute packets to find the path of flows suffering packet drops. Based on these paths, 007 adapts a voting scheme to locate the most problematic link. However, because of the lack of insight into switches, end-host-based cannot pinpoint exactly where a packet is dropped every time.


% \bbb{Mirroring Solutions}
% These solutions mirror packets to control plane in switches or remote controller. Typical end-host-based solutions include EverFlow \ref{??}, Netseer \ref{??}. The state-of-the-art Netseer leverage programmable switches to mirror packets dropped in programmable switches to control plane......??? 


% \bbb{Sketching-based Solutions}
% These solutions build counters in switches to detect packet drop by collecting flow-level or packet-level information. Typical sketching-based solutions include SNMP \ref{??}, Flowradar \ref{??}, Lossradar \ref{??}, Omnimon \ref {??}. Flowradar captures flow-level packet drops by leveraging bloom filter \ref{?}, invertible bloom filter \ref{?} and CM sketch simultaneously. The memory usage of Flowradar is proportional to the number of flows. Its successor Lossradar captures per-packet drop in invertible bloom filter with the memory usage proportional to the number of dropped packets. Omnimon ....
% However, existing solutions either drill down to packet-level drop, which is over-monitored because existing drop modes never consider the sequence number of packets, or provide fine-grained flow-level drop measurement with the memory usage proportional to the total number of flows in the measurement epoch, which is unacceptable in large-scale network under the strict constraint of extremely limited memory in switches.


==> SOSP21/relatedv2.tex <==

\presec
\section{Related Work} \postsec
\label{sec:relatedworks}



\subsection{Self-driving Network}
\postsec
The concept of self-driving networking was proposed by Nick and Jennifer \cite{feamster2017andJennifer}. 
A self-driving network should learn to drive itself by making real-time and closed-loop decisions.
However, the industrial grade solutions have not emerged.
Due to the difficulty of establishing a full automatic self-driving network, recent works are associated to only part of the self-driving network systems \cite{narayana2017language,sonata2018,kalmbach2018empowering,liu2018automatic,jacobs2018refining,demoulin2018automated}.
% Marple\cite{marple} and its corresponding hardware design bridges the network performance queries and switch programs. 
% Sonata\cite{sonata} provides a telemetry system with flexible interfaces for a wide range of telemetry tasks.
% The real-time monitoring, analysis and control is essential for self-driving network to run.
% One popular way to make these functions fast is to apply these in the data plane, especially programmable switches.
% Plenty of works concentrate on how to store and operate data structures on programmable switches\cite{univmon, beaucoup, elastic}.
% We make effort to deploy fermatSketch in programmable switches to provide real-time measurement.


%sub1：现有自动驾驶的特点
%sub2：现有的工作做某一部分。
% \presec
% \subsection{Self-Driving Networks } \postsec
% To wyh: 既然related work放在后面，应该不用介绍self-driving network，应该在intro里就有了？


%What's self-driving network?


% The self-driving network is a network system that can run itself independently, which consists of three key components: 
% \textbf{1)} A high sensitive measurement module to report network status in real time; 
% \textbf{2)} A clever analysis modulo to quickly and accurately find the reasons of network failures; 
% and \textbf{3)} A reliable control modulo to fix network problems with low risk. 
% To the best of our knowledge, \sysname{} is the first true self-driving network. 
% Thus, in the related work section, we mainly focus on how existing systems implement the three key components of the self-driving network. 


\presec
\subsection{Network Measurement Solutions} \postsec

Existing network measurement systems can be roughly divided into four categories: mirroring/sampling solutions, sketch-based solutions, end-host solutions, and programmable switch assisted solutions.
%
As shown in Table \ref{table:compare}, compared with the state-of-the-art solutions that can achieve full coverage of packet losses, only our algorithm achieves $O(\Delta F)$ complexity without dependence on programmable switches, where $\Delta F$ is the number of flows with packet losses.
%

\bbb{Mirroring/sampling solutions.} These solutions mirror or selectively mirror packets to control plane in switches or a central controller. 
Typical mirroring solutions include Planck \cite{planck2014}, PacketHistory \cite{packethistory2014}, and EverFlow \cite{everflow2015}. 
However, these solutions usually incur significant overhead to transmit and process all mirrored packets. 
Thus, many solutions first sample network traffic and then mirror the sampled packets to the central controller. 
Typical sampling solutions include NetFlow \cite{netflow2004}, sFlow \cite{sflow2001}, OpenSketch \cite{opensketch2013}, and more \cite{snmp,duffield2001trajectory,csamp2008,sekar2010revisiting,flexam2013,opensample2014,li2019large}. 
All the above solutions cannot capture all packet losses.
%

\bbb{Sketch-based solutions.} These solutions build compact data structures in switches and compress fine-grained packet-level information into them. 
Typical sketch-based solutions include Flowradar \cite{flowradar2016}, Lossradar \cite{lossradar2016}, OmniMon \cite {omnimon2020}, Beaucoup \cite{beaucoup2020}, and more \cite{cmsketch,cusketch,countsketch,univmon2016,sketchlearn2018,elastic2018,nitrosketch2019}. 
However, existing sketches are unable to capture all packet losses at low computation and communication complexities. Therefore, their implementation in switches is strictly limited due to the scarce SRAM resources. To address this issue, we propose \systemname{}.
%

\bbb{End-host solutions.} These solutions monitor the network by either actively sending tailored probing packets into the network and acquiring network status according to responses \cite{pingmesh2015,dhamdhere2018inferring,netbouncer2019}, or analyzing the performance of the protocol stack or I/O interface to infer network status \cite{trumpet2016,arzani2016taking,007-2018,simon2019,confluo2019,zeno2019}. 
% Typical solutions include Netbouncer \cite{?}, Pingmesh \cite{?}, Trumpet \cite{?}, and more \cite{?}. 
However, as the bottom-layer link status or switch status are invisible to these solutions, it is hard for them to pinpoint the abnormal link or switch where packet losses happen. 
%

\bbb{Programmable switch assisted solutions.} These solutions offload the monitoring process into the powerful programmable switches. 
Typical solutions include NetSeer \cite{netseer2020}, PacketScope \cite{packetscope2020}, Sonata \cite{sonata2018}, and more \cite{flowradar2016,lossradar2016,narayana2017language,sonchack2018scaling,sonchack2018turboflow}. 
However, these solutions lose generality due to the dependence on programmable switches. 



% these systems
% are not designed with the goal of comprehensively monitoring
% network events, such as inter-switch packet drops that are timeconsuming
% to locate with existing tools. Thus, they cannot

% Unfortunately, none of the above solutions are the perfect choice for a self-driving network. 
% The common flaw of existing measurement solution is that they cannot 
% Their common flaw is that they cannot report packet loss information in various situations at low cost. 
% For instance, NetSeer \cite{zhou2020flownetseer} and LossRadar \cite{li2016lossradar} report packet-level packet loss information, which reports too much information when a large amount of packet loss occurs, resulting in high latency and increasing the burden on the analyzer. FlowRadar \cite{li2016flowradar} needs to store each flow information on the switch, which takes up too much resources.











% Typical solutions of this kind include Pingmesh \cite{???}, Trumpet \cite{??}, 007 \cite{??}, and more \cite{??}. 
% Specifically, 007 sends carefully crafted traceroute packets to find the path of flows suffering packet drops. Based on these paths, 007 adapts a voting scheme to locate the most problematic link. However, because of the lack of insight into switches, end-host-based cannot pinpoint where a packet is dropped every time. 





% to detect packet drop by collecting flow-level or packet-level information. Typical sketch-based solutions include SNMP \cite{??}, Flowradar \cite{??}, Lossradar \cite{??}, and Omnimon \cite {??}. 



% The measurement part collects global information and becomes a basis for analysis and decision-making for network self-healing. 
% There are many existing measurement tasks, and we focus on measurement solutions related to packet loss. 
% Existing measurement systems can be roughly divided into three categories: mirroring-based solutions, sketch-based solutions, and end-host solutions. 

% \textbf{End-host solutions} either send probe packets into network or analyze the performance of transport layer to capture and analyze packet drops in end-hosts. 
% Typical solutions of this kind include Pingmesh \cite{???}, Trumpet \cite{??}, 007 \cite{??}, and more \cite{??}. 
% Specifically, 007 sends carefully crafted traceroute packets to find the path of flows suffering packet drops. Based on these paths, 007 adapts a voting scheme to locate the most problematic link. However, because of the lack of insight into switches, end-host-based cannot pinpoint where a packet is dropped every time. 
% %
% \textbf{Mirroring-based solutions} mirror packets to control plane in switches or remote controller. 
% Typical solutions include EverFlow \cite{??} and Netseer \cite{??}. 
% The state-of-the-art Netseer leverage programmable switches to mirror packets dropped in programmable switches to control plane......??? 
% %
% \textbf{Sketch-based solutions} build counters in switches to detect packet drop by collecting flow-level or packet-level information. Typical sketch-based solutions include SNMP \cite{??}, Flowradar \cite{??}, Lossradar \cite{??}, and Omnimon \cite {??}. 
% Flowradar captures flow-level packet drops by leveraging a bloom filter \cite{?}, an invertible bloom filter (IBLT) \cite{?} and a CM sketch simultaneously. 
% However, The memory usage of Flowradar is proportional to the number of flows. Its successor Lossradar captures per-packet drop in invertible bloom filter with the memory usage proportional to the number of dropped packets.
% However, existing solutions either drill down to packet-level drop, which is over-monitored because existing drop modes never consider the sequence number of packets, or provide fine-grained flow-level drop measurement with the memory usage proportional to the total number of flows in the measurement epoch, which is unacceptable in large-scale network under the strict constraint of extremely limited memory in switches.

\presec
\subsection{Machine Learning in Networking Systems}
\postsec

Thanks to the strong ability to fit complex distribution for prediction, ML methods have been extensively used in recent network systems to address various problems, including resource management \cite{rusek2019unveiling,zhang2019nfv}, traffic control \cite{auto2018,deep2019}, and more \cite{mao2017neural,yeo2018neural,mao2019learning}.
%DBSCAN \cite{ester1996density} is one of the most widely-used and the most cited clustering algorithms.
%Deep Neural Networks (DNNs) have demonstrated a significant improvement over traditional heuristic methods in analyzing network status and providing failure diagnosis \cite{deeplearning,multilayer1993}. 
%\systemname{} builds a small and lightweight DNN model to analyze the root causes of packet losses. 




 



% The analyzer analyzes the network conditions and provides problem diagnosis. 
% Network diagnostic work includes. 

% The network controller adjusts the state of the network and repairs the network.


==> TongYang/abstract.tex <==
\begin{abstract}


In this paper, we propose a guess, namely Exponential Twin Prime Guess, and verify it from 1 to $2^{64}$.

Based on this guess, we propose a new data structure, namely Twin Prime Table, TPT for short.
%
%
%invertible bloom lookup table
Essentially, TPT is a kind of hash table.
%
Different from conventional hash table suffering from memory consuming and hash collisions, TPT always achieve constant insert speed and memory efficiency.
%
The overhead of TPT is that it needs decoding before querying, and could incur decoding failures. To address the problem of Decoding failures, we proposed several method, namely ...,


%
The key novelty of TPT lies in two aspects: 1) it is based on our proposed guess; 2) it uses the well known Fermat theorem.
%
In theory, we propose a set of field theory to prove the correctness and rationale of TPT.
%
We insist TPT is really general, and apply TPT to ??? fields, including constant hash tables, packet loss detection, multi-set conciliation, stream Information Statistic, \textit{etc}.
For each application, our experimental results show that TPT significantly outperforms the state-of-the-art.
%
We open sourced all related code at Github without identify information.
%
\end{abstract}

==> TongYang/algorithm.tex <==
\presec
\section{Algorithm} \postsec
\label{sec:intro}

\subsection{Rationale}

%\yt{yt: use mathcal for symbols.}
% In this paper, $\mathcal{ID}$ is defined as a 32-bit positive integer, and the frequency $\mathcal{F}$ is defined as a signed integer. 
% We define the Cartesian product of an $\mathcal{ID}$ and a frequency $\mathcal{F}$ (\ie $\mathcal{\langle ID, F \rangle}$) as an item to be inserted, which is denoted by $e$. 
In this paper, we assume each item consists of a 32-bit unsigned integer $\mathcal{ID}$ and a signed integer frequency $\mathcal{F}$, which is denoted by ``$e$" or ``$\mathcal{\langle ID, F \rangle}$".  

1. Fermat's little theorem



Fermat's little theorem states that for any prime $p$ and any integer $a$, we have $a^p\equiv a\pmod p$.
We use this theorem and the modulo operation to reduce the memory needed for storing the ID sum of items.


2. First Hardy-Littlewood conjecture

First Hardy-Littlewood conjecture gives an estimation of the distribution of twin primes. 
It implies that although twin primes become more and more sparse as the number grows, their total number is infinite. 
Based on this conjecture, the number of twin primes in binary exponential range $[2^r, 2^{r+1}]$ is about $2C_2\frac{2^r}{(r+1)^2}$, where $C_2$ is a constant. 
This conjecture guarantees that enough twin primes could be found and applied to \aname{}. 

% The well known twin prime guess says that the number of twin primes are infinite.

% We propose an enhanced guess as follows.

% The twin prime is evenly distributed in binary exponential ranges.


% Binary exponential range refers to a range starting from $2^n$ to $2^{n+1}$, where $n (n>0)$ is an integer.

% Although the number of primes becomes more and more sparse with the increase of the number, the distribution of twin prime number is even/universal in terms of binary exponential ranges.


% Although we cannot prove it currently, we believe it is right.
% We have write C program to verify its correctness from $2$ to $2^{64}$. The source code is available at Github \cite{opensource}.


3. Verify the buckets without hashing

We propose \textit{Twin-ID Verification} and \textit{Overlap Verification} to check whether a bucket host just one item (called \textbf{pure bucket}). 
These two verification operations do not need hash calculation, which significantly reduce the decoding time. 

% \ljz{We propose using overlapping to verify the validity instead of using hashing, which saves the time for hash calculation.}


\input{lzr/algorithm_DataStructure_lzr.tex}


% \subsection{Data Structure}

% Our data structure is an array of $m$ buckets, where each bucket is used to store three fields: idA, idB, counter.
% \sout{Our data structure is an array of $m$ buckets, where each bucket is used to store three fields: ID, twin ID, counter.}
% We designate a pair of twin primes $pa$ and $pb$ for idA and idB. 
% The array has $k$ hash functions $h_1(.)...h_k(.)$. These hash functions map an ID to $k$ hashed buckets.
% \wyh{domain of the hash function is ID. write in mathematical}
% %The array has $k$ hash functions: $h_1(.)...h_k(.)$.


% \bbb{Fermat Operation:}
% We propose two kinds of Fermat operations, namely Fermat plus and Fermat subtract, on the idA and idB fields. The operations on the twin IDs are based on modular arithmetic. To add $IDA_i$ into the idA field with a frequency of $V_i$ by the Fermat plus, we compute as follows:
% \begin{equation*}idA=(idA+IDA_i\cdot V_i)\%pa\end{equation*}
% \begin{comment}
% Furthermore, if $V_i$ is 1, we compute as follows to remove the modulo operation, which is time-consuming: 
% \begin{equation*}
% \begin{aligned}
%     &idA=idA+IDA_i\\
%     &if~idA\geq pa~is~True:\\
%     &~~~~idA=idA-pa
% \end{aligned}    
% \end{equation*}
% \end{comment}
% The Fermat subtract is an inverse operation of the Fermat plus. Similarly, to subtract $IDA_i$ from the idA field with a frequency of $V_i$ by the Fermat subtract, we compute as follows:
% \begin{equation*}idA=(idA-IDA_i\cdot V_i)\%pa\end{equation*}
% %需要额外说明负数取余运算
% The modulo operation for a negative number varies among different programming languages. For example, in C++ we have $(-7)\%3=-1$.
% We define the modulo operation for a negative number as follows: if $r=a\%d$ where a is a negative integer and d is a positive integer, then we have $a=qd+r$ where q is a integer and $0\leq r<d$.


% \bbb{Initialization}. Initially, all the fields of every bucket in the array are set to zero/null.

% \bbb{Insert.}\wyh{constant time?} To insert a key-value pair $<ID_i, V_i>$, we calculate $k$ hash functions and get $k$ buckets, which are called $k$ hashed buckets in this paper.
% \ljz{We also divide the $ID_i$ into two parts, namely $IDA_i$ and $IDB_i$, which will be described later.}
% \ljz{We increment the count field by $V_i$, and perform the Fermat Plus to add $IDA_i$ and $IDB_i$ with a frequency of $V_i$ into the idA and idB fields respectively.}
% \sout{If the bucket is empty, we set the ID field to $ID_i$, increment the count field from 0 to 1. The twin ID is calculated by our proposed Fermat plus, which is illustrated as follows.}



% \bbb{ID Division.}%或ID Encode, ID transformation... //ID Division and ID Verification
% We divide $ID_i$ into $IDA_i$ and $IDB_i$ and store them in the idA and idB field respectively. $IDA_i$ is the higher r-bit of $ID_i$ and $IDB_i$ is calculated by XORing the lower r-bit of $ID_i$ and a mask number $m$, where $r$ and $m$ is given in advance.
% The number r determines the overlapped bits between $IDA_i$ and $IDB_i$. For example, if $ID_i$ is 32-bit long and $r$ equals 24, then $IDA_i$ and $IDB_i$ both have 8 overlapped bits.
% The number $m$ contributes to the verification of the validity of $ID_i$. In our implementation, $m$ consists of 1 and 0 arranged alternately in binary, and for $r=24$, the number $m$ is 0xaaaaaa.


% \bbb{Delete.} The delete operation is just the reverse process of insert operation.
% To delete a key-value $<ID_i, V_i>$, similar to the insert, we calculate hashing and get $k$ hashed buckets, for each of these buckets, we perform the Fermat substract operation as stated above instead of Fermat plus.


% \bbb{Decode.} 
% Some buckets may contain multiple items, and we can not directly retrieve the items stored in these buckets. Buckets with only one item hashed into it are called \textit{pure buckets}, and it stores the original information about the items.
% We use two techniques to check whether a bucket is a pure bucket. 
% 1) rehash.\wyh{detail}
% 2) overlapped check.\wyh{detail}
% We retrieve the items in these pure buckets, and delete them from all their hashed buckets, which may transform some buckets into pure buckets. By repeat this process, we can decode the sketch with a high probability.
% The process has a hidden error recovery function. If we mistake a bucket for a pure bucket in early process and delete it, we could recover this mistake in later process with high probability. \wyh{prove this with experiment}
% %关键概念加斜线？

% % 解压过程对数据结构是破坏性的，解压完后bucket中会是空的（之后修改）
% \bbb{Query.}
% After decoding, each bucket only stores one key value pair.
% To query a key $ID_i$, we calculate hash functions and get the $k$ hashed buckets to find $ID_i$.
% If found, we report the corresponding value; otherwise, we report query failed.
% %只有在这个格子只有一个元素的情况下才能成功

% \bbb{Example.} Below we use examples to show how the insert/delete/decode operation is performed in our hash table.
% 1) insert\&delete;
% 2) decode;


% \begin{figure}
%     \prefig
%     \includegraphics[width=0.98\linewidth]{wuyuhan/algo_graph1.pdf}
%     \vspace{-0.1in}
%     \vspace{-0.05in}
%     \caption{\footnotesize{An example of insertion. The size of the structure is $4$ and the number of hash functions is $2$. To insert a key-value pair $<15, 2>$, we select two buckets by hash and add the pair into each bucket. When adding $<10, 2>$ to a position, we divide the $ID=15$ into $IDA$ and $IDB$. For simplicity, we assume the $IDA$ to be $10$ and we only illustrate how to update $IDA$. As shown in the figure, we add the product of the $IDA$ and the value(\ie, $10*2=20$) to the idA and add the value $2$ to the counter.\wyh{make $??_i$ consistent}}}
%     \label{fig:algo:v2:universal_insert}
    
% \end{figure}
% %待修改，图中packet 改item。


% \begin{figure}
%     \prefig
%     \includegraphics[width=0.98\linewidth]{wuyuhan/algo_graph2.pdf}
%     \vspace{-0.1in}
%     \vspace{-0.05in}
%     \caption{\footnotesize{ decode}}
%     \label{fig:algo:v2:universal_decode}
    
% \end{figure}




==> TongYang/application.tex <==
\presec
\section{Applications} \postsec
\label{sec:app}
In this section, we apply \aname{} to three different applications: constant hash tables, packet loss detection and set reconciliation. We give detailed descriptions and solutions for each application.

\input{lzr/application_lzr.tex}

%\presec
%\subsection{Constant Hash Tables} \postsec
%\label{sec:const:hash}
%\bbb{Problem Statement:}
%\bbb{Data Structure:}
%\bbb{Solutions:}



%\presec
%\subsection{Packet Loss Detection} \postsec
%\label{sec:loss}
%\bbb{Problem Statement:}
%\bbb{Data Structure:}
%\bbb{Solutions:}



\input{ljz/application-set_reconciliation.tex}






\presec
\subsection{Membership Filter} \postsec
\label{sec:stream}
\bbb{Problem Statement:}
Given an element $e$, the membership filter decides whether element $e$ is in a set $S$ with small probability of false positive.

\bbb{Data Structure:}
We build a \aname{} for membership queries. \aname{} records the fingerprints of elements instead of the whole IDs.

\bbb{Solutions:}
All elements in $S$ are inserted into \aname{}. To query an element $e$, we decode \aname{} and check the $k$ hashed buckets of $e$.
If a pure bucket containing $e$ is found, \aname{} returns positive.



==> TongYang/conclusion.tex <==
\presec
\section{Conclusion} \postsec
\label{sec:conclusion}

In this paper, we propose a guess, namely Twin Prime Even Guess, and verify it from 1 to $2^{64}$.
Based on this guess, we propose a new data structure, namely Twin Prime Table, TPT for short.
%
Essentially, TPT is a kind of hash table.
%
Different from convential hash table suffering from memory consuming and hash collisions, TPT always achieve constant insert speed and memory efficiency.
%
The overhead of TPT is that it needs decoding before querying, and could incur decoding failures. To address the problem of Decoding failures, we proposed several method, namely ...,
%
The key novelty of TPT lies in two aspects: 1) it is based on our proposed guess; 2) it uses the well known Fermat theorem.
%
In theory, we propose a set of field theory to prove the correctness and rationale of TPT.
%
We insist TPT is really general, and apply TPT to ??? fields, including constant hash tables, multi-set conciliation, memorization of streaming data, packet loss detection, \textit{etc}.
For each application, our experimental results show that TPT significantly outperforms state-of-the-art.
%
We open sourced all related code at Github \cite{opensource} without identify information.






==> TongYang/intro.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}
%1、自动驾驶目标
%2、现状-要求太高
%3、我们的理念，生病的时候再调整 practical。我们以丢包为例，打通自动驾驶，做出原型系统。


\subsection{Background and Motivation}

Hash table is one of the most classic data structures in computer science, and has been widely used in various fields, such as 
%存储系统
data bases \cite{shapiro1986join,williams2007graph}, caches \cite{laarman2010boosting,metreveli2012cphash},
%数据挖掘等
data mining \cite{shafer1996sprint,chen1998efficient,nanopoulos2000finding,parthasarathy2001parallel}, machine learning\cite{jain2009online,vijayanarasimhan2014large,tang2017exploration}, NLP \cite{bohnet2010very,goyal2011approximate}, computer vision \cite{chum2007scalable,chum2008near,wang2010semi}, autonomous vehicles \cite{lacaze1998path,pereira2012integrated,wang2017pedestrian},
%网络
network monitoring \cite{song2005fast,estan2004building}, intrusion detection \cite{paxson1999bro,schuehler2003architecture}, IP lookups \cite{waldvogel1997scalable,dharmapurikar2003longest}, packet classification \cite{srinivasan1999packet,xu2013high}, IP traceback \cite{snoeren2002single,xiang2008flexible,al2006novel}, multicast \cite{huang1998enabling,ratnasamy2001application}, 
%
cloud computing \cite{hwang2010trusted,crago2011heterogeneous},
P2P networks \cite{stoica2001chord,ratnasamy2001scalable}, sensor networks \cite{ratnasamy2002ght,ratnasamy2003data}, overlay networks \cite{aberer2004gridvine,baumgart2007oversim}, data center networks\cite{al2010hedera,lu2009cafe,cao2013per},
%
computer languages \cite{van1995python,flanagan2006javascript}.



% % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\begin{comment}
databases:
Join processing in database systems with large main memories
Graph Database Indexing Using Structured Graph Decomposition 

data mining：
SPRINT: A scalable parallel classifier for data mining
Efficient data mining for path traversal patterns
Finding generalized path patterns for web log data mining
Parallel data mining for association rules on shared-memory systems

network monitoring:
Fast hash table lookup using extended bloom filter: an aid to network processing
Building a better NetFlow

intrusion detection:
Bro: A System for Detecting Network Intruders in Real-Time
Architecture for a hardware based, TCP/IP content scanning system

IP lookup：
Scalable High Speed IP Routing Lookups
Longest Prefix Matching Using Bloom Filters

packet classification:
Packet classification using tuple space search
High-throughput and memory-efficient multimatch packet classification based on distributed and pipelined hash tables

caches:%multi-core processor caches:
CPHASH: A Cache-Partitioned Hash Table
Boosting multi-core reachability performance with shared hash tables

computer languages:
Python reference manual
JavaScript: the definitive guide

P2P networks:
Chord: A scalable peer-to-peer lookup service for internet applications
A Scalable Content-Addressable Network

sensor networks:
GHT: a geographic hash table for data-centric storage
Data-centric storage in sensornets with GHT, a geographic hash table

overlay networks:
Gridvine: Building internet-scale semantic overlay networks
OverSim: A Flexible Overlay Network Simulation Framework

data center networks：
Hedera: dynamic flow scheduling for data center networks
CAFE: a configurable packet forwarding engine for data center networks
Per-packet load-balanced, low-latency routing for clos-based data center networks

IP traceback:
Single-Packet IP Traceback
Flexible deterministic packet marking: An ip traceback system to find the real source of attacks
Novel hybrid schemes employing packet marking and logging for IP traceback

multicast：
Application-level multicast using content-addressable networks
Enabling large-scale simulations: selective abstraction approach to the study of multicast protocols

cloud computing:
Trusted Cloud Computing with Secure Resources and Data Coloring
Heterogeneous cloud computing

machine learning:
Online metric learning and fast similarity search
Large-scale live active learning: Training object detectors with crawled data and crowds
Exploration: A study of count-based exploration for deep reinforcement learning

NLP:
Very high accuracy and fast dependency parsing is not a contradiction
Approximate scalable bounded space sketch for large data nlp

computer vision:
Scalable near identical image and shot detection
Near duplicate image detection: min-hash and tf-idf weighting
Semi-supervised hashing for scalable image retrieval

autonomous vehicles:
Path planning for autonomous vehicles driving over rough terrain
An integrated architecture for autonomous vehicles simulation
Pedestrian recognition and tracking using 3D LiDAR for autonomous vehicle

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
web caching, name based networks, cellular networks, queue management, regular expression matching, content distribution networks
\end{comment}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % %


%Conventional hash tables have two main advantages: O(1) insert time and O(1) query time, where O(1) is in average.
%O(1)需要修改， large memory usage不一定。如果99%装载率，每次插入平均探查100次，时间也是O(1)
Conventional hash tables have two main advantages: O(1) insert time and O(1) query time in average.
Its overhead is large memory usage, \ie, memory inefficiency.
The key shortcoming of hash table is hash collision, which makes the insert and query speed very slow in the worst cases.
%
If there is no hash collision, the insert and query speed will be fast and constant in the worst cases.
%
Perfect hash tables \cite{....} can achieve no collision at the cost of not supporting update.
%

\ykc{The invertible Bloom lookup table(IBLT) \cite{} is designed to achieve fast and stable O(1) insertion time and deletion time at the cost of an indispensable decoding before query. The IBLT has two insertion strategies: inserting by XOR operation or inserting by simple addition. 
Both insertion strategies have their strengths and weaknesses. If the IBLT choose to insert by XOR operation, it gets faster insertion and deletion speed and becomes more memory-efficient. 
As a result, it can not support the storage of multiset as the frequency information is never kept. 
If the IBLT choose to insert by simple addition, it can support the storage of multiset. 
As a result, it is not so fast as XOR operation, and its memory usage is much larger because each counter should be large enough to store the items hashed into itself.

The design goal of this paper is to combine the strengths and discard the weaknesses of the two insertion strategies of IBLT, targeting at a new kind of hash table, which can achieve fast and constant insertion/deletion speed, memory efficiency, and the storage of multiset. 
The only overhead is that we need to decode all items before query. After the decoding, we can query at fast and constant speed.}

\begin{comment}


This paper targets at a new kind of hash table, which can achieve fast and constant insertion/deletion speed, and memory efficiency. 
The overhead is that we need to decode all items before query. After that, we can query at fast and constant speed.

\ljz{
add some introduction (and shortcomings) of invertible bloom filters here?%invertible bloom lookup table

insert by xor: cannot deal with frequency

insert by addition: waste memories, the storing bits should be larger than the sum of id bits and frequency bits.
}


Our hash table is based on the following three key techniques: 1) we propose a new mathematical guess, namely twin prime guess; 2) we leverage Fermat theorem to address the problem of overflows of counters; 3) we propose a new verification method to verify the decoded item.
%1)删掉？
%3)是否要更详细说明取代指纹校验

Our propose hash table can be applied in many applications, and we have applied it to four different applications: 
1) constant hash tables; 
2) packet loss detection;
3) set reconciliation;
4) membership filter
%4) stream information statistic.
\end{comment}


\subsection{Our proposed Solutions}
\ykc{In this paper, we propose the \aname{}, a new kind of hash table achieving stable O(1) insertion/deletion time, memory-efficiency, and supporting storage of multiset. Compared to the IBLT, Our key idea is to leverage Fermat's little theorem for insertion, addressing the problem of overflows of counters to achieve memory-efficiency.}

TPT consists of multiple rows of buckets, and each incoming item will be mapped and inserted into one bucket of each row by pairwise-independent hash functions. 

%先介绍IBF/IBLT
\ljz{\aname{} overcomes the two short comings of traditional IBF/IBLT(?)}

For all items that are mapped into the same buckets, we use a counter to record the sum of frequencies and another counter to record ID sums, which is the sum of multiplications of each item's ID and frequency.
%the sum of IDs multiplied by their frequencies.
%怪怪的？modular operations定义不明
All operations are modular operations.
\ykc{Each time the counter recording ID sums is about to overflow, (need correction)we modulo the counter to a predefined large prime number, $p$. To reduce the memories for storing the ID sums, we choose the smallest prime above all IDs as $p$. }
%To reduce the memories for storing the ID sums, we choose the smallest prime above all IDs as the modulus for operations over ID sums. 
%To decode the TPT, we utilize Fermat's little theorem to recover the stored IDs. 
%Let $p$ be the chosen modulus for storing IDs. 
%If a bucket only holds one item $id$ with frequency $f$, then it stores $idsum=(id*f)\%p$ and $f$. We can recover the original $id$: $id=(idsum*f^{p-2})\%p$.

Before queries, we need to decode the TPT to handle the hash collisions and retrieve all inserted items. 
To decode the TPT, we utilize Fermat's little theorem to recover the stored IDs. 
%Let $p$ be the chosen modulus for storing IDs. 
Buckets that store multiple items cannot provide any information directly.
If a bucket only holds one item $id$ with frequency $f$, then it stores $idsum=(id*f)\%p$ and $f$. We can recover the original $id$: $id=(idsum*f^{p-2})\%p$.

Therefore, we first look for the buckets that stores only one item, called pure buckets. For each item in pure buckets, we retrieve and delete the item from all buckets that it is mapped into. After deletion, new pure buckets may appear. By repeating this procedure, we can retrieve all items with high probability.

\ykc{However, since a bucket only records the frequency and the ID sum, we can judge whether a bucket is a pure bucket by an unreliable method, namely \textbf{rehashing verification}. 
In rehashing verification, we first recover the item $id$ in the bucket and them determine whether it will b hashed to the bucket. 
If so, we regard this bucket as a pure bucket and continue the decoding. 
The main shortcoming of rehashing verification is not reliable enough. If a bucket is misjudged as a pure bucket, the decoding may completely fail.
To address this issue, we introduce the second verification method, namely \textbf{overlap verification}. We separate the counter recording ID sum to two counters. When inserting an incoming item, the ID is separate to two parts with a common overlap. For example, we can divide a 32-bit ID to two IDs. One ID is the first 24 bits of the 32-bit ID, and the other ID is the last 24 bits of the 32-bit ID. The two ID has a 16-bit overlap. Then, we insert the two IDs to two counters respectively. 
When decoding,  }

\ljz{experimental results here}


\subsection{Key Contributions}

This paper makes the following key contributions: 

1) We propose a new hash table, namely twin prime hash table. It is based on our proposed twin prime guess and Fermat theorem. 

2) We use field theory to prove the completeness of our hash table in theory.


3) We apply the hash table to four different applications, and conducted extensive experiments, and results show that our hash table significantly outperforms existing solutions.



==> TongYang/relatedworks.tex <==
\presec
\section{Background and Related Work} \postsec
\label{sec:relatedworks}

%In this section, we first describe multiset and data streams, and then illustrate three applications that we will apply TPT to.

\presub
\subsection{Constant Hash Tables}



\wyh{Should we define the constant hash table? Add Cuckoo hashing?
The hash table is a well-known data structure that is used for maintaining a set $S$ consisting of Key-Value pairs.
It supports the insertion, deletion, and lookup of Key-Value pairs. 
A constant hash table can complete the insertion and the deletion in constant time in the worst case.
Typical constant hash table includes the Cuckoo hashing.}

The hash table is an ubiquitous data structure in computer science. 
It is used for maintaining a set $S$ consisting of Key-Value pairs under insertion and deletion. 

FlowRadar\cite{li2016flowradar} records all flow IDs and flow sizes in a Bloom filter and an Invertible Bloom Lookup Table (IBLT) \cite{goodrich2011invertible}. Aiming at memory usage reduction, the authors propose a solution of network-wide decoding. 
The goal of TPT is to reduce memory usage and improve the insertion speed at the same time.



\presub
\subsection{Packet Loss detection}\postsub

LossRadar\cite{li2016lossradar} records the xorSum of the immutable header fields that can uniquely identify a packet and the count of packets in the Bloom filter. The authors propose a new loss detection solution that can capture all types of losses that happen at anywhere timely and identify individual lost packets while keeping the overhead low. However, compared with TPT, the overhead is much higher.


Our TPT uses less memory than LossRadar in both packet-level and flow-level packet loss detection while batch success rate is the same. Also, under different data skewness, TPT can achieve the same batch success rate as Lossradar while using less memory. More over, the insertion speed of TPT is almost the same as that of LossRadar. 



\presub
\subsection{Multiset Reconciliation} \postsub

%multiset定义太长了。
%Multiset is a modification of the conception of a class of sets that allow for multiple instances for each of elements.
\begin{comment}
To characterize a multiset, some parameters must be determined.

\bbb{Definition 1:} let $x$ be an element of multiset $A$, then the multiplicity of $x$ records the number of instances for $x$ in $A$, denoted by $A(x)$. 

\bbb{Definition 2:} the root set of $A$ named $A*$ is defined as $A*=\{x\in A|m_{A}(x)\textgreater0\}$.

With the two above definitions, we can accurately characterize a multiset by its root set and the multiplicities of all its elements, which means that every multiset $A$ can be represented as a set of pairs, \textit{i.e.}, $A=\{\langle x_{1} ,m_{A} (x_{1})\rangle,~\langle x_{2},m_{A}(x_{2})\rangle,...,~\langle x_{i},m_{A}(x_{i})\rangle,...\}$.

For instance, $A=\{\langle x_{1},1\rangle,~\langle x_{2},2\rangle,~\langle x_{3},3\rangle\}$ denotes $\{x_{1},~x_{2},~x_{2},~x_{3},~x_{3},~x_{3}\}$.
\end{comment}

\wyh{intro to this problem and some notations.}

Multiset is a class of sets that allow for multiple instances for each element.
Multiset Reconciliation is the process of ensuring that two sets become the same.
There are lots of methods for reconciliation of single set \cite{eppstein2011s,...}. However, few methods are proposed for multisets.
Up to now, there are only two efficient multi-set reconciliation methods named as Invertible Counting Bloom Filter (ICBF)\cite {luo2017efficient} and Trie\cite{luo2018near}.

ICBF records all flow IDs and flow size in a Bloom filter, and solve the different items by subtracting ICBF from each other. To enhance the performance, the authors use mode value instead of min value in Bloom filter as the number of elements. However, it can hardly solve all the different items, and the communication overhead is $O(n)$, where $n$ \wyh{??check} is the number of distinct items in the union of the two sets.

Trie records all flow IDs and flow size in a compressed Trie, and solves the different items by subtracting Trie from each other. With the help of the fingerprint, it can solve all the different items with very high probability. However, the communication overhead is also $O(n)$.

To the best of our knowledge, our TPT is the first work that can solve all the different items with very high probability while the communication overhead is only $O(d)$, where $d$ is the number of distinct different items.



\presub
\subsection{Membership Filter} \postsub
A membership filter is to answer whether an item belongs to a set. 
These filters compact a given set into a tiny filter with tolerable false positives, which means that they may mistakenly judge an item not in the set as belonging to the set.
% These filters have very small space to record the membership of large sets at the cost of small possibility of false positive, which means that they may mistakenly judge an item not in a set as belonging to the set.

The Bloom filter (BF) is one of the most widely used membership filters, which uses an array of bits to record the membership information. Each item is hashed into several bits, and BF judges the item is in the set when all hashed bits are set to 1. While the insertion of an item sets all hashed bits into 1, BF can not support deletion by just setting all hashed bits into 0, because these bits may also be hashed into by other items.
Counting Bloom Filter uses an array of counters instead of bits, so that it supports deletion of items by just decreasing these counters by 1. However, it takes much more space than BF, which makes it impractical in many situations.
%quotient filter

Cuckoo Filter takes advantage of Cuckoo Hashing to implement membership filters. A Cuckoo Filter uses two arrays of buckets to record the fingerprint of an item, and each bucket may contain several items. Each item is hashed into two buckets of each array, respectively. To insert an item into the Cuckoo Filter, the algorithm first checks whether these two buckets have empty space, and if there is any, insert the item into the empty space. If there is no space for hosting a new item, the algorithm randomly replaces it with an victim item in these two buckets, and kicks out the victim to its alternative bucket to make room for the new item. The victim item may replace another item in its hash bucket of the another array, and this process may repeat several times, until there is room for the victim item. If the repeat time reaches a threshold, the insertion fails and we believe the Cuckoo Filter is full.
To allow the items to locate their alternative buckets by their fingerprints, Cuckoo Filter use one hash function $h(\cdot)$ to hash an item $f$ to its first bucket: $h(f)$ , and get the second bucket by its fingerprint $fp$ and XOR operation: $h(f)\oplus h(fp)$. For an item recorded in one of the buckets, the alternative bucket index is the hash of the fingerprint XORing the index of the original bucket.

%A membership filter is to xxx.
%Bloom filter
%cuckoo filter
%quotient filter?
%.....



==> TongYang/theory.tex <==
\presec
\section{Mathematical Proofs} \postsec
\label{sec:math}
In this section, we first introduce the well-known Fermat's little theorem and explain how it supports our \aname{}.
Then we propose Twin Prime Guess. % and describe how it supports our algorithm.
Last, we propose the concept of Fermat Group. %, which is a 框架？
Finally, we demonstrate the formulas about set reconciliation.





\presec
\subsection{Fermat's little theorem} \postsec
\label{sec:fermat}

Fermat's little theorem states that for any prime number $p$ and any integer $a$, we have $a^p\equiv a\pmod p$. Furthermore, if $a$ is not divisible by $p$, then we have $a^{p-1}\equiv 1\pmod p$. The theorem was first stated by Pierre de Fermat in 1640, and various proofs of it were proposed\cite{euler1761theoremata,golomb1956combinatorial,iga2003dynamical} from then on.

\begin{theorem}
Given a pure bucket with its $SumID_{A}$, $SumID_{B}$ and $counter$, we have
\begin{equation*}ID_A=(SumID_{A}\cdot counter^{p_a - 2})\%p_a\end{equation*}
and
\begin{equation*}ID_B=(SumID_{B}\cdot counter^{p_b - 2})\%p_b\end{equation*}
where $p_a$ and $p_b$ are the pair of twin primes for each bucket. 
%we can restore the original item $id$.
\end{theorem}

\begin{proof}
We only prove the first equation, because the second equation can be proved in the same way.
Recall that a pure bucket only stores one item, so we have:
$$SumID_{A}=(ID_A\cdot counter)\%p_a$$
According to the rules of modulo operations and Fermat's little theorem, we have:
\begin{equation*}
\begin{aligned}
&~(SumID_{A}\cdot counter^{p_a-2})\%p_a\\
=&~(ID_A\cdot counert^{p_a-1})\%pa\\
=&~((ID_A\%p_a)\cdot (counter^{p_a-1}\%p_a))\%p_a\\
=&~ID_A\%p_a=ID_A
\end{aligned}
\end{equation*}
Thus the theorem holds.
\end{proof}



\input{lzr/mathproof_hardyConjecture.tex}

% \presec
% \subsection{Twin Prime Guess} \postsec
% \label{sec:twin}
% % Twin Prime Conjecture
% We propose an guess as follows.
% The twin prime is universally distributed in binary exponential ranges.
% Binary exponential range refers to a range starting from $2^n$ to $2^{n+1}$, where $n (n>0)$ is an integer.
% Although the number of primes becomes more and more sparse with the increase of the number, the distribution of twin prime number is universal in terms of binary exponential ranges.

% Hardy and Littlewood\cite{hardy1923some} gives an accurate estimation of the density of twin primes. It states as follows:
% For large values of n, we have
% \begin{equation*}
%     \pi_2(n)=2C_2\frac{n}{log^2(n)}
% \end{equation*}
% where $\pi_2(n)$ is the number of twin primes smaller than $n$, and $C_2$ is the twin prime constant:
% \begin{equation*}
%     C_2=\prod_{p\geq 3}(\frac{p(p-2)}{(p-1)^2})=0.66016...
% \end{equation*}

% For a binary exponential range starting from $2^n$ to $2^{n+1}$, the number of twin primes $B_2(n)$ is:
% \begin{equation*}
%     B_2(n)=2^{n+1}\frac{C_2}{log^{2}2}(\frac{2}{(n+1)^2}-\frac{1}{n^2})
% \end{equation*}


\begin{comment}
The well known twin prime guess says that the number of twin primes are infinite.
We propose an enhanced guess as follows.
The twin prime is evenly distributed in binary exponential ranges.
Binary exponential range refers to a range staring from $2^n$ to $2^{n+1}$, where $n (n>0)$ is an integer.
Although the number of primes becomes more and more sparse with the increase of the number, the distribution of twin prime number is even/universal in terms of binary exponential ranges.
Although we cannot prove it currently, we believe it is right.
We have write C program to verify its correctness from $2$ to $2^{64}$. The source code is available at Github \cite{opensource}.
\end{comment}




\input{lzr/mathproof_fermatGroup.tex}

% \presec
% \subsection{Fermat group} \postsec
% \label{sec:field}
% A Fermat vector contains three fields: $SumID_{A}$, $SumID_{B}$ and $counter$. $SumID_{A}$ and $SumID_{B}$ record the weighted sum of the $ID$ and its frequency $F$, and $counter$ record the cumulative sum of the frequency $F$. 
% We use $S_{ida}$, $S_{idb}$ and $S_{count}$ to denote the sets that comprises all possible values in $ida$, $idb$ and $count$ respectively.
% To distinguish the operations in these sets from the basic operations of arithmetic, we let "$+_S$" denotes the operation of addition in $S_{ida}$, $S_{idb}$ and $S_{count}$, and let "$\cdot_S$" denotes the operations of multiplication in $S_{ida}$ and $S_{idb}$.
% %对加法和乘法做定义
% Both addition and multiplication are modular versions of basic addition and multiplication in arithmetic. Generally, we have $a+_S b=(a+b)\% m$ and $a\cdot_S b=(a\cdot b)\% m$, where m is the modulus of the set. The modulus is $pa$ for $ida$, $pb$ for $idb$, and $2^r$ for a r-bit counter $count$.

% We use $S_{fermat}$ to denote the set of all Fermat vectors:
% \begin{equation*}
%     S_{fermat}=\{<a, b, c>|a\in S_{ida}\wedge b\in S_{idb}\wedge c\in S_{count}\}
% \end{equation*}
% We also define the addition in $S_{fermat}$ as follows: for any $V_1=<a_1, b_1, c_1>, V_2=<a_2, b_2, c_2>$ in $S_{fermat}$, we have
% \begin{equation*}
%     V_1+V_2=<a_1+_S a_2, b_1+_S b_2, c_1+_S c_2>
% \end{equation*}

% In this paper, the word field has two meanings. Generally, we use field to represent a counter that storing numbers.
% In mathematics, a field is a set with specific rules of mathematical operations like addition and multiplication.

% \begin{theorem}
% $S_{count}$ is an abelian group.
% \end{theorem}

% \begin{proof}
% A abelian group is a set with an operation that satisfies the group axioms: 1) Closure; 2) Associativity; 3) Commutativity; 4) Identity element; 5) Inverse element.
% %考虑引用一下与群定义有关的论文
% Suppose that $count$ is a r-bit counter, then we have $S_{count}=\{a|0\leq a<2^r\wedge a\in Z\}$.
% We prove that $S_{count}$ and its operation "$+_S$" satisfy each of these axioms.

% \bbb{Closure:}
% For all $a$, $b$ in $S_{count}$, we have
% \begin{equation*}
%     a+_S b=(a+b)\%2^r
% \end{equation*}
% which is also in $S_{count}$.

% \bbb{Associativity:}
% For all $a$, $b$ and $c$ in $S_{count}$, we have
% \begin{equation*}\begin{aligned}
%     (a+_S b)+_S c =&((a+b)\%2^r)+c)\%2^r\\
%     =&(a+(b+c)\%2^r))\%2^r\\
%     =&a+_S (b+_S c)
% \end{aligned}\end{equation*}

% \bbb{Commutativity:}
% For all $a$, $b$ in $S_{count}$, we have
% \begin{equation*}
%     a+_S b=b+_S a
% \end{equation*}

% \bbb{Identity element:}
% %There exists an element e in G such that, for every element a in G, the equation e • a = a • e = a holds. Such an element is unique (see below), and thus one speaks of the identity element.
% $S_{count}$ has an unique identity element, 0, such that, for all $a$ in $S_{count}$, we have:
% \begin{equation*}
%     0+_S a=(0+a)\%2^r=a=(a+0)\%2^r=a+_S 0
% \end{equation*}

% \bbb{Inverse element:}
% %For each a in G, there exists an element b in G, commonly denoted a−1 (or −a, if the operation is denoted "+"), such that a • b = b • a = e, where e is the identity element.
% All elements in $S_{count}$ have a inverse element such that they add up to the identity element. For 0, the inverse element is itself. For all other elements $a$ in $S_{count}$, the inverse element is $2^r-a$.

% In conclusion, $S_{count}$ is an abelian group.

% \end{proof}



% \begin{theorem}
% $S_{ida}$ and $S_{idb}$ are fields.
% \end{theorem}

% \begin{proof}
% We only prove that $ida$ is a field.

% A field is a set with two operations that satisfies the field axioms: 1) Closure; 2) Associativity; 3) Commutativity; 4) Distributivity of multiplication over addition; 5)Identity element; 6) Inverse element.
% We prove that $S_{ida}$ and its operation "$+_S$", "$\cdot_S$" satisfy each of these axioms.

% \bbb{Closure:}
% For all $a$, $b$ in $S_{ida}$, we have
% \begin{equation*}\begin{aligned}
%     a+_S b=&(a+b)\%pa\\
%     a\cdot_S b=&(a\cdot b)\%pa
% \end{aligned}\end{equation*}
% which are also in $S_{ida}$.

% \bbb{Associativity:}
% For all $a, b$ and $c$ in $S_{ida}$, we have
% \begin{equation*}\begin{aligned}
%     (a+_S b)+_S c =&a+_S (b+_S c)\\
%     (a\cdot_S b)\cdot_S c =&a\cdot_S (b\cdot_S c)
% %(a+_S b)+_S c =&((a+b)\%2^r)+c)\%2^r\\
% %=&(a+(b+c)\%2^r))\%2^r\\
% %=&a+_S (b+_S c)
% \end{aligned}\end{equation*}

% \bbb{Commutativity:}
% For all $a$, $b$ in $S_{ida}$, we have
% \begin{equation*}\begin{aligned}
%     a+_S b=&b+_S a\\
%     a\cdot_S b=&b\cdot_S a
% \end{aligned}\end{equation*}

% \bbb{Distributivity of multiplication over addition:}
% %a · (b + c) = (a · b) + (a · c).
% For all $a, b$ and $c$ in $S_{ida}$, we have
% \begin{equation*}\begin{aligned}
%     a\cdot_S (b+_S c)=&a\cdot ((b+c)\%pa)\%pa\\
%     =&(a\cdot b\%pa+a\cdot c\%pa)\%pa\\
%     =&(a\cdot_S b)+_S(a\cdot_S c)
% \end{aligned}\end{equation*}

% \bbb{Identity element:}
% $S_{ida}$ has an identity element for addition, 0, and an identity element for multiplication, 1, such that, for all $a$ in $S_{ida}$, we have:
% \begin{equation*}\begin{aligned}
%     &0+_S a=(0+a)\%pa=a=(a+0)\%pa=a+_S 0\\
%     &1\cdot_S a=(1\cdot a)\%pa=a=(a\cdot 1)\%pa=a\cdot_S 1
% \end{aligned}\end{equation*}

% \bbb{Inverse element:}
% %Additive inverses: for every a in F, there exists an element in F, denoted −a, called the additive inverse of a, such that a + (−a) = 0.
% %Multiplicative inverses: for every a ≠ 0 in F, there exists an element in F, denoted by a−1 or 1/a, called the multiplicative inverse of a, such that a · a−1 = 1.

% All elements in $S_{ida}$ have a inverse element for addition such that they add up to the additive identity element, 0. For 0, the inverse element is itself. For all other elements $a$ in $S_{count}$, the inverse element is $2^r-a$.

% All elements in $S_{ida}$ other than 0 have a inverse element for multiplication such that their product is the multiplicative identity element, 1. For an element $a$ in $S_{ida}$ other than 0, the inverse element is $a^{pa-2}\%pa$ according to Fermat’s little theorem.

% In conclusion, $S_{ida}$ is a field.
% \end{proof}




% \begin{theorem}
% $S_{fermat}$ is a group.
% \end{theorem}

% \begin{proof}
% Each vector field in the Fermat vector is a group over addition, thus $S_{fermat}$ and its addition also satisfies the group axioms.
% In a word, $S_{fermat}$ is a group.
% \end{proof}

% By the definition of addition we can define the subtraction of $S_{fermat}$: to subtract a Fermat vector is to add its inverse element.
% For $V_1=<a_1, b_1, c_1>, V_2=<a_2, b_2, c_2>$, we have
% \begin{equation*}\begin{aligned}
% &V_1-V_2=<\!(a_1-a_2+pa)\%pa,\\
% &(b_1-b_2+pb)\%pb, (c_1-c_2+2^r)\%2^r\!>
% \end{aligned}\end{equation*}
% %    V_1-V_2=<a_1, b_1, c_1>-<a_2, b_2, c_2>\\
% %    =&<a_1, b_1, c_1>+<(pa-a_2)\%pa, (pb-b_2)\%pb, (2^r-c_2)\%2^r>\\
% %    =&<(a_1-a_2+pa)\%pa, (b_1-b_2+pb)\%pb, (c_1-c_2+2^r)\%2^r>
% where pa, pb are the primes for $ida$ and $idb$, and r is the length of $count$.


% \begin{comment}
% 1.	费马向量
% 一个费马向量包含三个域：ID、指纹、计数器。ID是元素的标识符，占用空间a比特，指纹是通过一个哈希函数F(.)计算出的指纹，占用空间b比特，计数器是一个累加值。
% 2.	费马加法。
% 给定两个费马向量<ID_1, F_1, C_1>和<ID_2, F_2, C_2>，找出费马质数P_a和P_b，费马加法的结果是<(ID_1+ID_2)%P_a，(F_1+F_2)%P_b，C_1+C_2>。
% 3.	费马减法。
% 给定两个费马向量<ID_1, F_1, C_1>和<ID_2, F_2, C_2>，找出费马质数P_a和P_b，费马减法的结果是<(ID_1-ID_2)%P_a，(F_1-F_2)%P_b，C_1-C_2>。
% \end{comment}








\presec
\subsection{Set reconciliation} \postsec
\label{sec:reconcile}
In set reconciliation, we need to first communicate the lower bit of the counter (a sum sketch) to estimate the size of the set difference.

\begin{theorem}
Let $M1$ and $M2$ be the multi-set with $d$ different item ids,
and let $S$ be the sum sketch established by $M1$ and $M2$ with $k\cdot c$ counters and $r$ bits in each counter, where $k$ is the number of hash functions and $c$ is the number of counters covered by each hash function.
After communicating the sum sketch (inserting each item in $M1$ into $S$ and then deleting each item in $M2$ from $S$),
if there are $e_i$ zero counters covered by the $ith$ hash function ($1\leq i\leq k$),
then the expectation of the set difference's size $d=\frac{1}{k}\sum_{i=1}^k\log_{1-\frac{1}{c}}\frac{2^r\cdot \frac{e_i}{c}-1}{2^r-1}$.
\end{theorem}

\begin{comment}
假设sum sketch中每个哈希函数对应空间的长度为c（即总长c * hash数），这个空间中相同的个数为e，实际上对应位置没有差异元素的个数为e0，sum sketch中每个counter位数为r，差异元素数量为d，则：
每个位置没有差异元素的概率 p = ((c-1)/c)^d
没有差异元素的位置个数期望 e0 = mp = c*(1-1/c)^d
差异元素数 d = log(1-1/c, e0/c)
由于counter的位数是r，因此某个位置存在差异元素，但是其sum sketch中的值相同的概率为1/2^r（假设counter的值是随机的）
则e = e0 + (c-e0)/2^r
e0 = (2^r * e - c)/(2^r - 1)
即d = log(1-1/c, (2^r * e/c - 1)/(2^r - 1))
可考虑根据多个哈希各自算出对应的d再取平均，也可考虑先对e取平均
\end{comment}

\begin{proof}
We first consider the counters covered by one certain hash function. Suppose the size of set difference $d$ is known, then the probability of each counter being empty is $(1-\frac{1}{c})^d$, and the expectation number of empty counters (\ie no items of set difference are hashed into these counters) $e'$ have
\begin{equation}e'=c(1-\frac{1}{c})^d\label{eq:empty_counter}\end{equation}
Empty counters must be zero counters, but some non-empty counters may overflow to zero. We assume that the value of a non-empty counter is uniformly distributed among its domain, so the probability of a non-empty counter having the zero value is $\frac{1}{2^r}$.
Thus we have the relation between the number of empty counters $e'$ and the number of zero counters $e$:
\begin{equation}e=e'+\frac{c-e'}{2^r}\label{eq:zero_counter}\end{equation}
Combining (\ref{eq:empty_counter}) and (\ref{eq:zero_counter}) we have
\begin{equation*}d=\log_{1-\frac{1}{c}}\frac{2^r\cdot \frac{e}{c}-1}{2^r-1}\end{equation*}
% 考虑多个hash function的情况
Estimations from each hash functions form a group of independent random events, so we have 
\begin{equation*}d=\frac{1}{k}\sum_{i=1}^k\log_{1-\frac{1}{c}}\frac{2^r\cdot \frac{e_i}{c}-1}{2^r-1}\end{equation*}
Thus the theorem holds.
\end{proof}





==> YKC/experiments.tex <==
\presub
\section{Experimental Results}\postsub


\begin{comment}

\begin{figure}
    \prefig
    \includegraphics[width=0.49\linewidth]{figure/set_reconciliation/sharp_threshold-crop.pdf}
    \includegraphics[width=0.49\linewidth]{figure/set_reconciliation/caida_difference-crop.pdf}
    \vspace{-0.1in}
    \vspace{-0.05in}
    \caption{\footnotesize{Applying the straw-man solution}}
    \label{fig:algo:v2:universal}
    
    % \vspace{-0.1in}
    % \vspace{-0.1in}
    % \vspace{-0.1in}
\end{figure}

\begin{figure}[H]
	\centering
	
	\begin{subfigure}{.24\textwidth}
        \centering
        \includegraphics[width=\textwidth]{wuyuhan/exp2.pdf}
        \vspace{-0.30in}
        \caption{\footnotesize{FPR \textit{vs.} Packet Age.}}
        	\label{figure_exp_BF_pos}
        \end{subfigure}
	%
	\begin{subfigure}{.24\textwidth}
        \centering
		\includegraphics[width=\textwidth]{wuyuhan/exp2.pdf}
        \vspace{-0.30in}
        \caption{\footnotesize{FPR \textit{vs.} \# of Hash Functions.}}
        	\label{figure_exp_BF_hash}
        \end{subfigure}	
	%
	\vspace{-0.05in}
    \caption{\footnotesize{Parameters of \algonameBF.}}
	\label{figure_para_of_BloomFilter}
% 	\vspace{-0.12in}
\end{figure}

\end{comment}

\input{figure/hash_table/hash_table_size.tex}
\input{figure/packet_loss/packet_loss.tex}


% \subsection{Experimental Setup} 
\bbb{Platform:}
We run the programs on the server with 20-core CPUs and 104GB total system memory.
% 以下描述要大改(不然就是抄袭了)
%We implement our algorithm in C++. The programs are run on the server with dual 6-core CPUs(24 threads, Intel Xeon CPU E5-2620 @2.00 GHz), which have 64GB total system memory. To test the accuracy in each task vs. the memory of our data structure, we vary the total memory from 0.4MB to 0.8MB, half of which is occupied by the heavy part. And to test the accuracy vs. the data skewness, 0.4MB of the memory is used to build our data structure and 0.2MB of the data structure is used to build the heavy part. We compare our algorithm with Elastic and CM in the experiments of different tasks.

\bbb{Datasets:}
We use three kinds of datasets to measure the algorithms. CAIDA\cite{caida.org} is an anonymized IP trace collected from high-speed monitors on backbone links. WebDocs\cite{fimi} is a collection of web html documents built by crawling web pages and generating items from these collected documents. Synthetic datasets are generated according to Zipf\cite{Powers1998Applications} distribution and comprise 11 datasets with different distribution skewness ranging from 0.0 to 3.0(a step of 0.3).

\bbb{Evaluation metrics:}
%待添加
Decode Success Rate: The probability of decoding all the items.

Insertion Speed: Million of insertions per second (Mips). %We used Million of insertions per second (Mips) to measure the insertion speed. 
%batch success rate, packet success rate

Batch success rate: The probability of decoding all the items in a batch for packet loss.

Packet success rate: The proportion of successfully decoded lost packets to all lost packets.


\subsection{Hash Table}

\bbb{Sketch size (Figure~\ref{fig:hash_table:size}):}
%dump success rate意思是什么？
%flowradar 用decode success rate来表示全部解出的概率，我们考虑也用这个
The results show that \aname{} requires smaller size than \flowradar{} to achieve 99\% 用decode success rate in all datasets. It is also found that the decode success rate of \aname{} and \flowradar{} are not affected by data skewness.

\input{figure/hash_table/hash_table_suc.tex}

\bbb{Success rate in different sizes (Figure~\ref{fig:hash_table:suc}):}
The results show that compared to \flowradar{}, \aname{} requires significantly smaller size to achieve the same 用decode success rate.


\input{figure/hash_table/hash_table_mips.tex}
%mips的图可能不用加上caption，因为测速度的方法不重要，用任何手段（插入多少packet）测到的速度应该是完全一样的

\bbb{Insertion speed (Figure~\ref{fig:hash_table:mips}):}
%We used Million of insertions per second (Mips) to measure the insertion speed. 
The results show that the insertion speed of \aname{} is obviously faster than that of \trie{}, \flowradar{} and \icbf{}, and it is about the same as that of \lossradar{}.





\subsection{Packet Loss Detection}

\bbb{Success rate in different sizes (Figure~\ref{fig:packet_loss}):}
We find that in both packet-level and flow-level packet loss detection, \aname{} requires smaller size than \lossradar{} to achieve the same batch success rate and packet success rate. 
%batch success rate and packet success rate需要解释（考虑加在metrics里）
In flow-level packet loss detection, \lossradar{} needs dozens of times more memory to achieve the same success rate than that of \aname{}. This is because \lossradar{} cannot capture huge packet losses in the same flow, while \aname{} can capture them with very little memory. In flow-level packet loss detection of WebDocs, the packet success rate of \lossradar{} is about 60\% when the batch success rate reaches 99\%, because WebDocs contains a few very big flows that take up a large part of lost packets.

\input{figure/packet_loss/packet_loss_zipf.tex}

\bbb{Memory under different data skewnesses (Figure~\ref{fig:packet_loss:zipf}):}
We find that \aname{} requires smaller size than \lossradar{} to achieve 99\% batch success rate in all datasets. In the dataset with a skewness of zero, the size of \aname{} needed is 16.02\% lower than that of \lossradar{}. As the skewness increases, the size of \aname{} declines while the size of \lossradar{} remains the same. When the skewness reaches 3, the size of \aname{} needed becomes 66.32\% lower than that of \lossradar{}.









\subsection{Set reconciliation}

In this section, we conduct experiments on multi-set reconciliation, comparing \aname{} with two existing methods named \icbf{} and \trie{}. We use authentic datasets and synthetic datasets to comprehensively evaluate the performance of multi-set reconciliation from three aspects: decode success rate, communication overhead and time consumption of decoding.
%sharp htreshold考虑换一个词

\input{figure/set_reconciliation/set_reconciliation.tex}

\subsubsection{Decode success rate} 

First, we show that there is a sharp threshold in \aname{}.

\bbb{Decode success rate vs. buckets per difference (Figure~\ref{fig:reconcile:st}):} In this experiment, we test the decode success rate against buckets per difference on two authentic datasets. We use different number of differences and varies the size of our sketch to test the decode success rate while the total flow number keeps unchanged. The experimental results show that there is a sharp threshold of buckets per difference for the decode success rate at around 1.22. 
As the buckets per difference increases, the decode success rate grows.
When buckets per difference is not around the threshold, the decode success rate grows at a slow pace, and when buckets per difference is passing the threshold, the decode success rate grows rapidly.
%when (buckets per dif) is above the threshold, the decode success rate almost equals to one.
We also find that, the larger the number of differences is, the sharper the threshold is.
%But the threshold is at least 1.22? because of (three hashes??).(which is used to test)

\subsubsection{Communication overhead} 

Second, we show that the communication overhead of \aname{} is far less than \icbf{} and \trie{}, because the communication overhead of \aname{} is O(d), while the communication overhead of both \icbf{} and \trie{} is O(n).

\bbb{Communication overhead vs. proportion of differences (Figure~\ref{fig:reconcile:CO}):}
In this experiment, we vary the proportion of differences from zero to five percent, and test the communication overhead on two authentic datasets with 20000 flows.
The experimental results show that the communication overhead of \aname{} is far less than \icbf and \trie.
%As \icbf{} can hardly solve all items, we test the communication overhead when \icbf{} solves 99\% of all items.%For other two algorithms, we test the communication overhead when all items are solved.
%keep the ratio of items that can be solved at 0.99 after communication to test the communication overhead,
When the proportion of differences varies, the communication overhead of \aname{} increases almost linearly, while the communication overhead of \icbf{} and \trie{} keeps nearly constant, and is far more than that of \aname{}.

\subsubsection{Time consumption of decoding} 

Finally, we show the time consumption of decoding of \aname{} with SIMD acceleration, \aname{} without SIMD acceleration, \icbf{} and \trie{}.

\bbb{Time consumption vs. proportion of differences (Figure~\ref{fig:reconcile:dif}):}
In this experiment, we test the time consumption when the proportion of differences varies from zero to five percent on two authentic datasets.
%As \icbf{} can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption, and we use 20000 flows as data. 
The experimental results show that the time consumption of \aname{} with SIMD acceleration is far less than the others.
When the proportion of differences varies, the time consumption of \aname{} with SIMD acceleration, \aname{} without acceleration and \trie{} increases almost linearly, while the the time consumption of \icbf{}  keeps nearly constant.

\bbb{Time consumption vs. flow number (Figure~\ref{fig:reconcile:flow}):}
In this experiment, we test the time consumption as the flow number varies from 10000 to 100000 on two authentic datasets while the ratio of difference keeps at five percent.
The experimental results show that the time consumption of \aname{} with SIMD acceleration is far less than the others.
%As \icbf{} can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption. 
When the flow number varies, the time consumption of all structures increases almost linearly.

\bbb{Time consumption vs. data skewness) (Figure~\ref{fig:reconcile:zipf}:}
In this experiment, we test the time consumption as the data skewness varies from 0 to 3 on synthetic datasets while the ratio of difference keeps at five percent.
%As \icbf{} can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption, and we use 20000 flows as data. 
The experimental results show that the time consumption of \aname{} with SIMD acceleration is far less than the others.
When the data skewness varies, the time consumption of all structures oscillates at different constants.
%(which is used to test, in what condition(solve item 99))




==> figure/full_measurement/full_measurement.tex <==
\begin{figure*}[!htbp]
	\centering
	\subfigure[flow size ARE]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/FS_ARE.pdf}
        \postsubfig
        \label{fig:flow size estimation(heavy)}
        \end{minipage}
    }
        \subfigure[flow size AAE]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/FS_AAE.pdf}
        \postsubfig
        \label{fig:flow size estimation(heavy)}
        \end{minipage}
    }
        \subfigure[heavy hitter F1 score]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/HH_F1.pdf.pdf}
        \postsubfig
        \label{fig:heavy hitter detection}
        \end{minipage}
    }
        \subfigure[heavy change F1 score]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/HC_F1.pdf.pdf}
        \postsubfig
        \label{fig:heavy change detection}
        \end{minipage}
    }
        \subfigure[flow size distribution WMRE]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/FSD_WMRE.pdf.pdf}
        \postsubfig
        \label{fig:flow size distribution estimation}
        \end{minipage}
    }
        \subfigure[entropy RE]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/ENTR_RE.pdf.pdf}
        \postsubfig
        \label{fig:entropy estimation}
        \end{minipage}
    }
        \subfigure[cardinality RE]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/full_measurement/CARD_RE.pdf.pdf}
        \postsubfig
        \label{fig:cardinality estimation}
        \end{minipage}
    }
    \caption{
    }
    \label{fig:evluation on 6 measurement tasks}
% 	\vspace{-0.12in}
\end{figure*}

==> figure/hash_table/hash_table_mips.tex <==
\begin{figure}[h!]
	\centering
    \prefig
    \includegraphics[width=0.25\textwidth]{figure/hash_table/Insertion_Mips.pdf}
    \postfig
    \vspace{-0.1in}
    \caption{
        We read 1000000 flows from CAIDA dataset, and insert them to the sketches to measure the insert Mips.
    }
    \label{fig:hash_table:mips}
\end{figure}

==> figure/hash_table/hash_table_size.tex <==
\begin{figure*}[!htbp]
	\centering
	\subfigure[CAIDA]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/hash_table/sketch_size_caida.pdf}
        \postsubfig
        \label{fig:hash_table:size_caida}
        \end{minipage}
    }
	\subfigure[WebDocs]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/hash_table/sketch_size_webpage.pdf}
        \postsubfig
    	\label{fig:hash_table:size_webdocs}
        \end{minipage}
    }
	\subfigure[Zipf]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/hash_table/sketch_size_zipf.pdf}
        \postsubfig
        \label{fig:hash_table:size_zipf}
        \end{minipage}
    }
    \caption{
        In CAIDA and WebDocs experiments, we change the number of inserted flows to measure the minimum size of the two sketches under the condition that dump success rate is over $99\%$.
        In Zipf experiment, we insert 4000 flows to the sketches, and measure the minimum size of the sketches when dump success rate is over $99\%$.
    }
    \label{fig:hash_table:size}
% 	\vspace{-0.12in}
\end{figure*}

==> figure/hash_table/hash_table_suc.tex <==
\begin{figure}[h!]
	\centering
	\subfigure[CAIDA]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/hash_table/success_rate_caida.pdf}
        \postsubfig
        \label{fig:hash_table:suc_caida}
        \end{minipage}
    }
    \subfigure[WebDocs]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/hash_table/success_rate_webpage.pdf}
        \postsubfig
        \label{fig:hash_table:suc_webdocs}
        \end{minipage}
    }
    \vspace{-0.1in}
    \caption{
        We insert 1000 flows from CAIDA and WebDocs datasets to the sketches, and change the size of the sketches to measure the dump success rate. 
    }
    \label{fig:hash_table:suc}
\end{figure}

==> figure/packet_loss/packet_loss.tex <==
\begin{figure*}[!htbp]
	\centering
	\subfigure[Packet-level(CAIDA)]{
	\begin{minipage}[b]{0.243\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/packet_loss/packetLossCAIDA-crop.pdf}
        \postsubfig
        \label{fig:packet_loss:p_caida}
        \end{minipage}
    }
	\subfigure[Packet-level(WebDocs)]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/packet_loss/packetLossWebPage-crop.pdf}
        \postsubfig
    	\label{fig:packet_loss:p_webdocs}
        \end{minipage}
    }
	\subfigure[Flow-level(CAIDA)]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/packet_loss/flowLossCAIDA-crop.pdf}
        \postsubfig
        \label{fig:packet_loss:f_caida}
        \end{minipage}
    }
	\subfigure[Flow-level(WebDocs)]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/packet_loss/flowLossWebPage-crop.pdf}
        \postsubfig
        \label{fig:packet_loss:f_webdocs}
        \end{minipage}
    }
    \caption{
        In packet-level experiments, we read 2000000 packets and simulate packet loss situations by discarding each packet with probability of $0.06\%$.
        In flow-level experiments, we read 1000000 packets and simulate packet loss situations by discarding each flow with probability of $1\%$.
        We experiment two kinds of success rates: 1) Packet success means that a lost packet is captured by the algorithm; 2) Batch success means that every packet in one batch is captured by the algorithm.
    }
    \label{fig:packet_loss}
% 	\vspace{-0.12in}
\end{figure*}



==> figure/packet_loss/packet_loss_zipf.tex <==
\begin{figure}[h!]
	\centering
    \prefig
    \includegraphics[width=0.25\textwidth]{figure/packet_loss/packetLossZipf-crop.pdf}
    \postfig
    \vspace{-0.1in}
    \caption{
        We read 2000000 items and simulate packet loss situations by discarding  each packet with probability of $0.06\%$. We use binary search to find the minimal size for the data structure to achieve batch success rate of 99\%.
    }
    \label{fig:packet_loss:zipf}
\end{figure}


==> figure/set_reconciliation/set_reconciliation.tex <==
\begin{figure}[h!]
	\centering
	\subfigure[CAIDA]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/st_caida-crop.pdf}
        \postsubfig
        \label{fig:hash_table:suc_caida1}
        \end{minipage}
    }
    \subfigure[WebDocs]{
	\begin{minipage}[b]{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/st_web-crop.pdf}
        \postsubfig
        \label{fig:hash_table:suc_webdocs1}
        \end{minipage}
    }
    \vspace{-0.1in}
    \caption{
       Sharp thresholds.
    }
    \label{fig:reconcile:st}
\end{figure}

\begin{figure}[h!]
	\centering
\subfigure[CAIDA Communication cost]{
	\begin{minipage}[b]{0.213\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/caidaco-crop.pdf}
        \postsubfig
        \label{fig:reconcile:caidaco}
        \end{minipage}
    }
	\subfigure[WebDocs Communication cost]{
	\begin{minipage}[b]{0.213\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/webco-crop.pdf}
        \postsubfig
        \label{fig:reconcile:webco}
        \end{minipage}
    }
    	
   \caption{
        Communication cost
    }
    \label{fig:reconcile:CO}
% 	\vspace{-0.12in}
\end{figure}







\begin{figure}[h!]
	\centering
\subfigure[CAIDA difference]{
	\begin{minipage}[b]{0.213\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/caidadif-crop.pdf}
        \postsubfig
        \label{fig:reconcile:caidadif}
        \end{minipage}
    }
	\subfigure[WebDocs difference]{
	\begin{minipage}[b]{0.213\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/webdif-crop.pdf}
        \postsubfig
        \label{fig:reconcile:webdif}
        \end{minipage}
    }
    	
   \caption{
        Time consumption
    }
    \label{fig:reconcile:dif}
% 	\vspace{-0.12in}
\end{figure}


\begin{figure}[h!]
	\centering
	\subfigure[CAIDA flownum]{
	\begin{minipage}[b]{0.223\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/caidaflow-crop.pdf}
        \postsubfig
        \label{fig:reconcile:caidaflow}
        \end{minipage}
    }
	\subfigure[WebDocs flownum]{
	\begin{minipage}[b]{0.223\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figure/set_reconciliation/webflow-crop.pdf}
        \postsubfig
    	\label{fig:reconcile:webflow}
        \end{minipage}
    }
	
    \caption{
        Time consumption
    }
    \label{fig:reconcile:flow}
% 	\vspace{-0.12in}
\end{figure}


\begin{figure}[h!]
	\centering
    \prefig
    \includegraphics[width=0.25\textwidth]{figure/set_reconciliation/zipf-crop.pdf}
    \postfig
    \vspace{-0.1in}
    \caption{
       data skewness
    }
    \label{fig:reconcile:zipf}
  
\end{figure}





==> ljz/evaluation.tex <==
\input{figure/hash_table/hash_table_size.tex}
\input{figure/packet_loss/packet_loss.tex}


% \subsection{Experimental Setup} 
\bbb{Platform:}
We run the programs on the server with 20-core CPUs and 104GB total system memory.
% 以下描述要大改(不然就是抄袭了)
%We implement our algorithm in C++. The programs are run on the server with dual 6-core CPUs(24 threads, Intel Xeon CPU E5-2620 @2.00 GHz), which have 64GB total system memory. To test the accuracy in each task vs. the memory of our data structure, we vary the total memory from 0.4MB to 0.8MB, half of which is occupied by the heavy part. And to test the accuracy vs. the data skewness, 0.4MB of the memory is used to build our data structure and 0.2MB of the data structure is used to build the heavy part. We compare our algorithm with Elastic and CM in the experiments of different tasks.

\bbb{Datasets:}
We use three kinds of datasets to measure the algorithms. CAIDA\cite{caida.org} is an anonymized IP trace collected from high-speed monitors on backbone links. WebDocs\cite{fimi} is a collection of web html documents built by crawling web pages and generating items from these collected documents. Synthetic datasets are generated according to Zipf\cite{Powers1998Applications} distribution and comprise 11 datasets with different distribution skewness ranging from 0.0 to 3.0(a step of 0.3).







\subsection{Hash Table}

\bbb{Sketch size (Figure~\ref{fig:hash_table:size}):}
The results show that \aname{} requires smaller size than \flowradar{} to achieve 99\% dump success rate in all datasets. It is also found that the dump success rate of \aname{} and \flowradar{} are not affected by data skewness.

\input{figure/hash_table/hash_table_suc.tex}

\bbb{Success rate in different sizes (Figure~\ref{fig:hash_table:suc}):}
The results show that compared to \flowradar{}, \aname{} requires significantly smaller size to achieve the same dump success rate.


\input{figure/hash_table/hash_table_mips.tex}
%mips的图可能不用加上caption，因为测速度的方法不重要，用任何手段（插入多少packet）测到的速度应该是完全一样的

\bbb{Insertion speed (Figure~\ref{fig:hash_table:mips}):}
We used Million of insertions per second (Mips) to measure the insertion speed. The results show that the insertion speed of \aname{} is about the same as \lossradar{}, which is obviously faster than  \trie{}, \flowradar{} and \icbf{}.





\subsection{Packet Loss Detection}

\bbb{Success rate in different sizes (Figure~\ref{fig:packet_loss}):}
We find that in both packet-level and flow-level packet loss detection, \aname{} requires smaller size than \lossradar{} to achieve the same batch success rates and packet success rates. In flow-level packet loss detection, \lossradar{} needs dozens of times more memories to achieve the same success rate than that of \aname{}. This is because \lossradar{} cannot capture huge packet losses in the same flow, while \aname{} can capture them with very few memories. In flow-level packet loss detection of WebDocs, the packet success rate is about 60\% while the batch success rate reaches 99\%, because WebDocs contains a few very big flows that take up a large part of lost packets.

\input{figure/packet_loss/packet_loss_zipf.tex}

\bbb{Memory under different data skewnesses (Figure~\ref{fig:packet_loss:zipf}):}
We find that \aname{} acquires smaller size than \lossradar{} to achieve 99\% batch success rates in all datasets. In the dataset with a skewness of zero, the size of \aname{} needed is 16.02\% slower than that of \lossradar{}. As the skewness increases, the size of \aname{} declines while the size of \lossradar{} remains the same. When the skewness reaches 3, the size of \aname{} needed becomes 66.32\% slower than that of \lossradar{}.









\subsection{Set reconciliation}
In this section, we conduct experiments on multi-set reconciliation, compared TPT with the two existing methods, named ICBF and TRIE. We use authentic datasets and synthetic datasets to comprehensively evaluate the performance of multi-set reconciliation from three aspects: sharp threshold, communication overhead and time consumption of decoding.

\input{figure/set_reconciliation/set_reconciliation.tex}

\subsubsection{Sharp threshold} 
\\First, we show that a sharp threshold is in TPT.
\\\textbf{Successful decoding rate vs. ??(buckets per dif) (Figure~\ref{fig:reconcile:st}):} The experiment results show that there is a sharp threshold of (buckets per dif) for the success rate of decoding at around 1.22. In this experiment, we test the success rate against (buckets per dif) of (different difference) on two authentic datasets. We use different size of differece to test the success rate while the total flow number keep in constant. As (buckets per dif) increases, when (buckets per dif) is below the threshold, the success rate nearly equals to zero, when (buckets per dif) is passing the threshold, the success rate rapidly raising, when (buckets per dif) is above the threshold, the success rate almost equals to one. The larger (buckets per dif) is, the sharper the threshold is. But the threshold is at least 1.22? because of (three hashes??).(which is used to test)
\subsubsection{Communication overhead} 
\\Second, we show that the communication overhead of TPT is far less than ICBF and TRIE, because the communication overhead of TPT is O(d), while the communication overhead of both ICBF and TRIE is O(n).
\\\textbf{Communication overhead vs. ??(Ratio of difference) (Figure~\ref{fig:reconcile:CO}):}  The experiment results show the communication overhead of TPT is far less than ICBF and TRIE. In this experiment, We test the communication overhead when (the ratio of difference) varies from zero to five percent on two authentic datasets.As ICBF can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the communication overhead, and we use 20000 flows as data. When the (ratio of difference) varies, the communication overhead of TPT increases almost linearly, while the communication overhead of TRIE and ICBF nearly keeps in constant, far more than that of TPT.
\subsubsection{Time consumption of decoding} 
\\Finally, we show the time consumption of decoding of TPT with SIMD acceleration, TPT without SIMD acceleration, ICBF and TRIE.
\\\textbf{Time consumption vs. ??(Ratio of difference) (Figure~\ref{fig:reconcile:dif}):} The experiment results show the time consumption of TPT with SIMD acceleration is far less than the others. In this experiment, we test the Time consumption when (the ratio of difference) varies from zero to five percent on two authentic datasets. As ICBF can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption, and we use 20000 flows as data. When the (ratio of difference) varies, the time consumption of TPT SIMD, TPT and TRIE increases almost linearly, while the the time consumption of ICBF nearly keeps constant.
\\\textbf{Time consumption vs. ??(Flow number) (Figure~\ref{fig:reconcile:flow}):} The experiment results show the time consumption of TPT with SIMD acceleration is far less than the others. In this experiment, we test the Time consumption when (Flow number) varies from 10000 to 100000 on two authentic datasets while the ratio of difference keeps in constant at five percent. As ICBF can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption. When the (flow number) varies, the time consumption of all structures increases almost linearly.
\\\textbf{Time consumption vs. ??(Data skewness) (Figure~\ref{fig:reconcile:zipf}:} The experiment results show the time consumption of TPT with SIMD acceleration is far less than the others. In this experiment, we test the Time consumption when (Data skewness) varies from 0 to 3 on  synthetic datasets while the ratio of difference keeps in constant at five percent. As ICBF can hardly make all items solved, we (establish?) structures to keep the ratio of items that can be solved at 0.99 after communication to test the time consumption, and we use 20000 flows as data. When the (Data skewness) varies, the time consumption of all structures oscillates at different constants.(which is used to test, in what condition(solve item 99))




==> ljz/reconciliation.tex <==
\presec
\section{Multiset reconciliation} \postsec
\label{sec:setcon}
%多重集合协调、云存储同步

In this section, we discuss how to apply \aname{} to multiset reconciliation.

\presec
\subsection{Problem Statement} \postsec
%\bbb{Problem Statement:}
Given two multi-sets $S_1$ and $S_2$ located in two remote servers $u_1$ and $u_2$ which have the same elements with the same frequencies in majority.
However, in these two multi-sets, some elements may have different frequencies, and some elements may only appear in one of these multi-sets.
We call these two kinds of elements the differences between the two multi-sets.
%
The problem consists in finding the differences between the multi-sets with as low communication overhead as possible between two servers.

%\bbb{Data Structure:}
\presec
\subsection{Data Structure} \postsec
Before building a \aname{} in each server, we should first estimate the size of differences between the multi-sets and then decide the size of \aname{} accordingly. We build a large sum sketch in each server that only consists of the lower bits of the count fields in the \aname{}. Same items in each server will be mapped into the same buckets of sketches. 
After we estimate the size of differences, we build a \aname{} in each server with the same hash functions in the sum sketches. All sketches use the same hash functions.

%\bbb{Solutions:}
\presec
\subsection{Solutions} \postsec
First, both servers build a sum sketch and insert all elements into it. Because each bucket of the sum sketch is only the lower bits of the count fields, the sum sketch is very small.
Then $u_1$ sends its sum sketch to $u_2$ and $u_2$ subtracts the corresponding buckets in the sketches.
After subtraction, if a bucket holds a number that is not zero, then there must be some differences in all items that are mapped into this bucket.
If a bucket holds a zero number, then there are two possibilities: 1) items mapped into this bucket are identical in each server; 2) there are small chances that items mapped into this bucket in each server are not identical.
$u_2$ count the quantity of all zero buckets to evaluate the size of differences, and decide the size of \aname{} accordingly. 
\ljz{how to decide the size of \aname{} accordingly.}
$u_2$ builds a \aname{} and send it to $u_1$, and then $u_1$ subtract and decode the sketches to get the different items.

%\bbb{Improvements:}
\presec
\subsection{Improvements} \postsec
We take following methods to reduce the communication overhead between the servers.
We let the hash functions for the \aname{} be based on the sum sketch. Suppose that the sizes for the sum sketch and \aname{} are $k*c_s$ and $k*c_t$ respectively, where $k$ is the number of hash functions and $c_s$ and $c_t$ are the numbers of counters covered by each hash function in the sum sketch or \aname{}. 
\ljz{how to compress}



\presub
\subsection{Optimization} \postsub
%\subsection{Optimization \uppercase\expandafter{\romannumeral2}- Error Recovery} \postsub

In decoding operation, an error occurs when we mistake a non-pure bucket for a pure one and delete the false item in it from its other $k-1$ hashed buckets. 
We provide an \textit{Error Recovery} mechanism by slightly modifying the deletion process in decoding operation.
%We can slightly modify the deletion process in decoding operation to endow our \aname{} an \textit{Error Recovery} mechanism. 

Suppose bucket $b_0$ has been judged as a pure bucket, and we are about to delete its item $e^{(b_0)}$ from the $k-1$ hashed buckets. 
In the deletion process, whenever we meet a processed pure bucket $b_1$, we check whether it is the additive inverse of bucket $b_0$, \ie check whether $(SumID_{A}^{(b_0)} + SumID_{A}^{(b_1)})\%p_a = 0$, $(SumID_{B}^{(b_0)} + SumID_{B}^{(b_1)})\%p_b = 0$ and $counter^{(b_0)} + counter^{(b_1)} = 0$ are all true. 

If the check result is positive, we think we once mistook the non-pure bucket $b_1$ for a pure bucket, and deleted the false item $e^{(b_1)}$ from its $k-1$ buckets, one of which is bucket $b_0$. 
To fix our previous mistake, we remove the processed pure mark of $b_1$ and continue the deletion process. 
When the deletion process is over, we set all fields of bucket $b_0$ to zero/null instead of mark $b_0$ as a processed pure bucket. 
This way, after these, bucket $b_0$ will become empty and bucket $b_1$ will return to its previous state. 
We have successfully recovered a misjudge error. 
% This incorrect deletion process adds the additive inverse of $e^{(m_1)}$ into bucket $m_0$. When bucket $m_0$ becomes a \textit{pure bucket} afterwards, its reduced item $e^{(m_0)}$ will be $-e^{(m_1)}$, and now the hidden error is exposed. 

%If the check result is positive, we conjecture an error once occurred when processing the incorrectly presumed \textit{pure bucket} $m_1$. That is, we once mistook the \textit{non-pure bucket} $m_1$ for a \textit{pure bucket}, and deleted the item $e^{(m_1)}$ from its other $k-1$ buckets, one of which is bucket $m_0$. This incorrect deletion process adds the additive inverse of $e^{(m_1)}$ into bucket $m_0$. When bucket $m_0$ becomes a \textit{pure bucket} afterwards, its reduced item $e^{(m_0)}$ will be $-e^{(m_1)}$, and now the hidden error is exposed. 

% In this case, the deletion process is modified to add item $-e^{(m_0)}$, i.e. $e^{(m_1)}$, to all the hashed buckets of $e^{(m_0)}$ except bucket $m_1$. And the \textit{processed pure bucket} mark of bucket $m_1$ is removed to indicate bucket $m_1$ is actually a \textit{non-pure bucket}. After this process, bucket $m_0$ will become an empty bucket, and bucket $m_1$ will return to its previous state. So far, we have successfully recovered a previous error. 

On the other hand, if the check result is negative, we think the decoding operation fails and report decoding failure. 
Actually this case shows up very rarely. 

\lzr{experimental results about mistake recovery rate...}

==> lzr/algorithm.tex <==
\presec
\section{Algorithm} \postsec
\label{sec:alg}
%Section 3、多重集合算法、校验、哈希表、filter

In this section, we explain the basic algorithm of \aname{}. We first discuss the rationale, then we explain the data structure and operations, last we provide two optimizations for \aname{}.

\subsection{Rationale}

\yt{yt: use mathcal for symbols.}
% In this paper, $\mathcal{ID}$ is defined as a 32-bit positive integer, and the frequency $\mathcal{F}$ is defined as a signed integer. 
% We define the Cartesian product of an $\mathcal{ID}$ and a frequency $\mathcal{F}$ (\ie $\mathcal{\langle ID, F \rangle}$) as an item to be inserted, which is denoted by $e$. 
In this paper, we assume each item consists of a 32-bit unsigned integer $\mathcal{ID}$ and a signed integer frequency $\mathcal{F}$, which is denoted by ``$e$" or ``$\mathcal{\langle ID, F \rangle}$".  

1. Fermat's little theorem


Fermat's little theorem states that for any prime $p$ and any integer $a$, we have $a^p\equiv a\pmod p$.
We use this theorem and the modulo operation to reduce the memory needed for storing the ID sum of items.


2. First Hardy-Littlewood conjecture

First Hardy-Littlewood conjecture gives an estimation of the distribution of twin primes. 
It implies that although twin primes become more and more sparse as the number grows, their total number is infinite. 
Based on this conjecture, the number of twin primes in binary exponential range $[2^r, 2^{r+1}]$ is about $2C_2\frac{2^r}{(r+1)^2}$, where $C_2$ is a constant. 
This conjecture guarantees that enough twin primes could be found and applied to \aname{}. 

% The well known twin prime guess says that the number of twin primes are infinite.

% We propose an enhanced guess as follows.

% The twin prime is evenly distributed in binary exponential ranges.


% Binary exponential range refers to a range starting from $2^n$ to $2^{n+1}$, where $n (n>0)$ is an integer.

% Although the number of primes becomes more and more sparse with the increase of the number, the distribution of twin prime number is even/universal in terms of binary exponential ranges.


% Although we cannot prove it currently, we believe it is right.
% We have write C program to verify its correctness from $2$ to $2^{64}$. The source code is available at Github \cite{opensource}.


3. Verify the buckets without hashing

We propose \textit{Twin-ID Verification} and \textit{Overlap Verification} to check whether a bucket host just one item (called \textbf{pure bucket}). 
These two verification operations do not need hash calculation, which significantly reduce the decoding time. 

% \ljz{We propose using overlapping to verify the validity instead of using hashing, which saves the time for hash calculation.}




\subsection{Data Structure}

% In this paper, $ID$ is defined as a 32-bit positive integer, and the frequency $F$ is defined as a 32-bit integer. The Cartesian product of an $ID$ and a frequency $F$, i.e. $<ID, F>$, is defined as an item, which is denoted by the sign $e$. 
% %From now on, we assume item $e_i$ is equivalent to $<ID_i, F_i>$. 
%From now on, we assume item $e_i$ is equivalent to $<ID_i, F_i>$. 
\aname{} consists of $k$ arrays, $A_1$, $A_2$,..., $A_k$. 
Each array $A_i$ has $m$ buckets and a hash function $h_i:\mathcal{ID}\mapsto \{ 0,...,m-1 \}$ that maps the $\mathcal{ID}$ of an incoming item to one of the $m$ buckets. 
%and $k$ hash functions $h_1,h_2,...h_k:\mathcal{ID}\mapsto \{ 0,...,m-1 \}$. 
Each bucket consists of (1) a pair of 33-bit \textit{SumID} fields, \ie $SumID_{A}$ and $SumID_{B}$, to record the modulo $\mathcal{ID}$ sum of its hosting items; 
and (2) a \textit{counter} field to record the total frequency of its hosting items. 
Besides, we designate the largest pair of twin primes that is less than $2^{33}$, $p_a$ and $p_b$, to the two \textit{SumID} fields of \aname{} so that $SumID_{A} \in \mathbb{Z}_{p_a}$ and $SumID_{B} \in \mathbb{Z}_{p_b}$ for each bucket. 
% $counter \in \mathbb{Z}_{2^{32}}$
For each incoming item $e$, or $\mathcal{\langle ID, F \rangle}$, \aname{} first calculates $h_1(\mathcal{ID})$, $h_2(\mathcal{ID})$,..., $h_k(\mathcal{ID})$ to get its $k$ hashed buckets, and then inserts $e$ to bucket $h_1(\mathcal{ID})$ in $A_1$, bucket $h_2(\mathcal{ID})$ in $A_2$, and so on. 
Figure. \ref{fig:algo:insert} illustrates the data structure of \aname{} for the case of $m=3$ and $k=3$. 



\presub
\subsection{Fermat Operations}\postsub

To better explain the design principles of \aname{}, we introduce three Fermat operations: 1) Fermat addition, 2) Fermat subtraction, and 3) Fermat reduction. 
%On the ID sum field, we introduce Fermat addition and Fermat subtraction that are based on modular arithmetic. 

\noindent\textbf{(1) Fermat addition} is used to insert an item to the \textit{SumID} field of a bucket.
Specifically, to add $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$ to a $SumID$ field accompanied with a prime $p$, we compute as follows: 
\begin{equation*}SumID=(SumID+\mathcal{ID}_i\cdot \mathcal{F}_i)\%p\end{equation*}

%%% 还要不要加？
% \begin{comment}
% Furthermore, if $V_i$ is 1, we compute as follows to remove the modulo operation, which is time-consuming: 
% \begin{equation*}
% \begin{aligned}
%     &idA=idA+IDA_i\\
%     &if~idA\geq pa~is~True:\\
%     &~~~~idA=idA-pa
% \end{aligned}    
                       % \end{equation*}
% \end{comment}

\noindent\textbf{(2) Fermat subtraction}, the inverse operation of Fermat addition, is used to delete an item from the \textit{SumID} field.
Similarly, to subtract $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$ from a $SumID$ field accompanied with a prime $p$, we compute as follows:
\begin{equation*}SumID=(SumID- \mathcal{ID}_i\cdot \mathcal{F}_i)\%p\end{equation*}

Note that the result of the modulo operation on a negative integer varies among different programming languages. For instance, in C++ we have $(-7)\%3=-1$. 
In order to keep the \textit{SumID} field always non-negative, we particularly specify the modulo operation for a negative integer as: For a negative integer $a$ and a positive integer $d$, the modulo result of $r=a\%d$ should satisfy $0\leq r<d$ and $a=q \cdot d+r$ where $q$ is an integer.

\noindent\textbf{(3) Fermat reduction} operation is used to derive the real $\mathcal{ID}$ from a \textit{SumID} field of a bucket that hosts only one item.
%\textit{pure bucket}, 
%which is based on Fermat's little theorem. 
This operation is based on Fermat's little theorem. 
When the counter field is positive, the reduced value is defined as: 
\begin{equation*} 
\mathcal{ID} ^{\prime} = (SumID\cdot counter^{p-2})\%p
\end{equation*}
When the counter field is negative, the reduced value is: 
\begin{equation*} 
\mathcal{ID} ^{\prime} = ((p - SumID) \cdot (-counter)^{p-2})\%p
\end{equation*}
The reduced value is what we want only if the bucket hosts exactly one item. For a bucket hosting multiple items, Fermat reduction operation will return a false $\mathcal{ID}$. 

\presub
\subsection{TPT Operations}\postsub

\bbb{Initialization.} 
To start with, all fields of all buckets are initialized to zero/null. 
We find the largest pair of twin primes that is less than $2^{33}$, $p_a$ and $p_b$, for \aname{}, so that $SumID_{A} \in \mathbb{Z}_{p_a}$ and $SumID_{B} \in \mathbb{Z}_{p_b}$ for each bucket. 

\bbb{Insertion.} To insert an item $e_i$, or $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$, we first calculate the $k$ hash functions $h_1(\mathcal{ID}_i),...,h_k(\mathcal{ID}_i)$ to get its $k$ hashed buckets. 
Then the counter fields of the $k$ hashed buckets are incremented by $\mathcal{F}_i$, and the Fermat addition is performed to add $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$ to the two \textit{SumID} fields of the $k$ hashed buckets respectively.

The insertion operation is illustrated in Figure. \ref{fig:algo:insert} for the case of a \aname{} with $m=3$ and $k=3$. Before the insertion operation, an item $\langle 4,1 \rangle$ already exists in the \aname{}. 

\bbb{Deletion.} Deletion is the reverse operation of insertion. To delete an item $e_i$, or $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$, we subtract $\mathcal{F}_i$ from the counter fields of its $k$ hashed buckets, and perform the Fermat subtraction operation to subtract $\langle \mathcal{ID}_i, \mathcal{F}_i \rangle$ from the two \textit{SumID} fields of its $k$ hashed buckets respectively.

% For a bucket $m_0$, we first exploit the Fermat reduction operation to get its two unjustified IDs: $ID_{A}^{\prime (m_0)}$ and $ID_{B}^{\prime (m_0)}$.
% In order to check whether bucket $m_0$ is a \textit{pure bucket}, we first propose the \bbb{Twin-ID Verification} test, which is to compare the two unjustified IDs. 
% And if $ID_{A}^{\prime (m_0)} \neq ID_{B}^{\prime (m_0)}$, bucket $m_0$ cannot be a \textit{pure bucket}. Otherwise, suppose that $ID_{A}^{\prime (m_0)} = ID_{B}^{\prime (m_0)} = ID^{\prime (m_0)}$. 
% The \bbb{Rehashing} test is proposed to check this bucket further. That is, we calculate the $k$ hash values $h_1(ID^{\prime (m_0)}),...,h_k(ID^{\prime (m_0)})$ and compare them with $m_0$. If $m_0 \in \{ h_1(ID^{\prime (m_0)}),...,h_k(ID^{\prime (m_0)}) \}$, bucket $m_0$ is judged as a \textit{pure bucket}, and if not, it cannot be a \textit{pure bucket}. 

% If bucket $m_0$ passes the two tests above and is judged as a \textit{pure bucket}, we can consider it as storing a real item $e^{(m_0)} = <ID^{\prime (m_0)}, counter^{(m_0)}>$. 

\bbb{Verification.} 
We call a bucket that hosts only one item as \textbf{pure bucket} in the rest of the paper. 
For a pure bucket, we can retrieve its hosting item by Fermat reduction operation. 
However, due to hash collisions, most buckets in \aname{} host multiple items, so we need a method to verify whether a bucket is pure or not. 
% In the rest of the paper, we will call the bucket $m_i$ from array $k_i$ as bucket $m_i$-$k_i$. 
%We call a bucket \textbf{pure bucket} if it only hosts one item. 
%To verify whether bucket $m_0$ from array $k_0$ is pure, we first perform the Fermat reduction operation on its two \textit{Sum\_ID} fields and get two reduced ID: $\mathcal{ID}_{A}^{\prime}$ and $\mathcal{ID}_{B}^{\prime}$. 
%If the two reduced ID are not equal, bucket $m_0$ can not be pure. 
%Otherwise, assume $\mathcal{ID}_{A}^{\prime} = \mathcal{ID}_{B}^{\prime} = \mathcal{ID}^{\prime}$. 
%Then we check whether $h_{k_0}(\mathcal{ID}^{\prime})=m_0$.
%If so, we judge bucket $m_0$ as a pure bucket and can consider it as storing a real item $e^{(m_0)} = \langle \!\mathcal{ID}^{\prime}, counter^{(m_0)}\! \rangle$. 

Now, let's consider the $m_0$-th bucket in array $k_0$ (we call it bucket $b_0$ henceforth). 
We first introduce the \bbb{Twin-ID Verification} test.  
That is, we use the Fermat reduction operation to get the two unjustified IDs of bucket $b_0$, namely $\mathcal{ID}_{A}^{\prime}$ and $\mathcal{ID}_{B}^{\prime}$, and then check whether they are equal. 
If $\mathcal{ID}_{A}^{\prime} \neq \mathcal{ID}_{B}^{\prime}$, bucket $b_0$ cannot be a pure bucket. 
Otherwise, suppose that $\mathcal{ID}_{A}^{\prime} = \mathcal{ID}_{B}^{\prime} = \mathcal{ID}^{\prime}$, 
% there is very high probability that the bucket is a pure bucket.
the \bbb{Rehashing Verification} test is introduced to verify this bucket further. 
That is, we recalculate the hashed value of $\mathcal{ID}^{\prime}$ in array $k_0$ and check whether $h_{k_0}(\mathcal{ID}^{\prime})=m_0$.
If not, this bucket can not be pure. 
If bucket $b_0$ passes the two tests above, it is judged as a pure bucket.
Then we can consider it as storing a real item $e^{(b_0)} = \langle \!\mathcal{ID}^{\prime}, counter^{(b_0)}\! \rangle$. 

The verification operation cannot guarantee that each bucket that we judge as pure is definitely a pure bucket. 
In other words, there exist some false positive errors. 
% For a pure bucket $m_0$, we can perform the Fermat reduction operation on it to get the real item $e^{(m_0)} = \langle \!\mathcal{ID}^{\prime (m_0)}, counter^{(m_0)}\! \rangle$ it hosting.
% For a pure bucket $m_0$, we can consider it as storing a real item $e^{(m_0)} = <\!ID^{\prime (m_0)}, counter^{(m_0)}\!>$. 
% If a bucket $m_0$ only host one item, we call it a \textit{pure bucket} and consider it as storing a real item $e^{(m_0)} = <\!ID^{\prime (m_0)}, counter^{(m_0)}\!>$. 
%Twin-ID test. Rehashing test. Processed pure bucket.
But our experimental results show that the probability of the false positive error is very tiny. 
In fact, we tested the verification operation on two millions buckets, and haven't encountered even one false positive error. 

\begin{figure}
    \prefig
    \includegraphics[width=0.98\linewidth]{lzr/insertion2.pdf}
    \vspace{-0.1in}
    \vspace{-0.05in}
    \caption{Insertion operation of \aname{} with $m=3$ and $k=3$.}
    \label{fig:algo:insert}
    
\end{figure}

\bbb{Decoding.} %Decoding operation starts by searching the $m$ buckets for \textit{pure buckets}. 
%The general idea of Decoding operation is to repeatedly search all buckets for \textit{pure buckets}.
In Decoding operation, we repeatedly search the $k$ arrays for pure buckets using the verification operation described above. % using the  described above.
%For each pure bucket, we partially delete its hosting item so that the item has only one copy in \aname{}. 
%For a bucket $m_0$, we first verify whether it is a \textit{pure bucket}.%, which is explained later.
%For a bucket $m_0$, we first exploit the Fermat reduction operation to get its two unjustified IDs: $ID_{A}^{\prime (m_0)}$ and $ID_{B}^{\prime (m_0)}$. 
%If bucket $m_0$ passes the verification, we judge it as a \textit{pure bucket} and consider it as storing a real item $e^{(m_0)} = <\!ID^{\prime (m_0)}, counter^{(m_0)}\!>$. 
Suppose we have found a pure bucket $b_0$, which is the $m_0$-th bucket from array $k_0$.
Then a deletion process is performed to subtract $b_0$'s hosting item $e^{(b_0)}$ from its other $k-1$ hashed buckets (except bucket $b_0$ itself). 
Note that in this process, we keep the original pure bucket $b_0$ unchanged to ensure its item $e^{(b_0)}$ could be retrieved there later on, which is different from the deletion operation described above. 
After the deletion process, we mark bucket $b_0$ as a \textbf{processed} pure bucket. 
The deletion process may transform some non-pure buckets into pure, and we can repeat the deletion process again on these new pure buckets. 
We keep on searching the $k$ arrays repeatedly and performing the deletion process for each pure bucket, until all pure buckets have been marked as processed and no more pure buckets could be found. 
%After searching process stops, 
In the end, if each bucket is either empty or processed pure, we report decoding success. 
Otherwise, we report decoding failure. 

Due to the false positive error of the verification operation, there are some extra details we need to take into account.
For example, consider we have already finished the deletion process of item $e^{(b_0)}$. Thereafter, if in the deletion process of another item $e^{(b_1)}$, the processed pure bucket $b_0$ is encountered again, this means we must at least mistaken one non-pure bucket among $b_0$ and $b_1$ as a pure bucket. 
%we have mistaken at least one \textit{non-pure bucket} among $m_0$ and $m_1$ as a \textit{pure bucket}.
For now, we just think the Decoding operation fails. % and report decoding failure.
We will introduce an Error Recovery mechanism to handle this case later.
%\lzr{Our experimental results show that the probability of regarding a \textit{non-pure bucket} as a \textit{pure bucket} is very very tiny. 
%}

The decoding operation is illustrated in Figure. \ref{fig:algo:decode}. 
When we find a pure bucket, we perform the deleting process to subtract its hosting item from its other hashed buckets. 
We can clearly see that after a deletion process, more pure buckets appear. 

%the above retrieve more items from these pure buckets. 
%This way, we can get more pure buckets by repeating the operation above. 
%By repeating this process, we can decode the \aname{} with high probability.
%说我们通过重复查询pure bucket和deletion process，我们可以以大概率解码整个sketch
%
%下面这句话有问题，引入overlap应该会让解错概率增加
%Actually, if the \textit{Overlap Verification} test which will be introduced later is adopted, this situation will almost never show up. 
%

%\lzr{experimental results about decode success rate...}

\begin{comment}
For a bucket $m_0$, we first exploit the Fermat reduction operation to get its two unjustified IDs: $ID_{A}^{\prime (m_0)}$ and $ID_{B}^{\prime (m_0)}$. 
In order to check whether bucket $m_0$ is a \textit{pure bucket}, we first propose the \bbb{Twin-ID Verification} test, which is to compare the two unjustified IDs. 
And if $ID_{A}^{\prime (m_0)} \neq ID_{B}^{\prime (m_0)}$, bucket $m_0$ cannot be a \textit{pure bucket}. Otherwise, suppose that $ID_{A}^{\prime (m_0)} = ID_{B}^{\prime (m_0)} = ID^{\prime (m_0)}$. 
The \bbb{Rehashing} test is proposed to check this bucket further. That is, we calculate the $k$ hash values $h_1(ID^{\prime (m_0)}),...,h_k(ID^{\prime (m_0)})$ and compare them with $m_0$. If $m_0 \in \{ h_1(ID^{\prime (m_0)}),...,h_k(ID^{\prime (m_0)}) \}$, bucket $m_0$ is judged as a \textit{pure bucket}, and if not, it cannot be a \textit{pure bucket}. 

If bucket $m_0$ passes the two tests above and is judged as a \textit{pure bucket}, we can consider it as storing a real item $e^{(m_0)} = <\!ID^{\prime (m_0)}, counter^{(m_0)}\!>$. 
Then a deletion process is performed to delete item $e^{(m_0)}$ from its other $k-1$ hashed buckets. In the deletion process, we keep the \textit{pure bucket} $m_0$ unchanged to ensure $e^{(m_0)}$ could be retrieved in bucket $m_0$ later, which is different from the deletion operation described above. 
The deletion process will transform some \textit{non-pure buckets} into \textit{pure buckets}. After the deletion process, we mark bucket $m_0$ as a \textit{processed pure bucket}.

If in the deletion process of item $e^{(m_0)}$, we encounter a \textit{processed pure bucket} $m_1$. This situation indicates we have mistaken at least one \textit{non-pure bucket} of bucket $m_0$ and bucket $m_1$ for a \textit{pure bucket}. For now, we just think the Decoding operation fails and report decoding failure.
\lzr{Our experimental results show that the probability of regarding a \textit{non-pure bucket} as a \textit{pure bucket} is very very tiny. 
}
%下面这句话有问题，引入overlap应该会让解错概率增加
%Actually, if the \textit{Overlap Verification} test which will be introduced later is adopted, this situation will almost never show up. 
We will also propose an \textit{Error Recovery} mechanism to better handle this situation later on.

We keep on searching the $m$ buckets repeatedly and performing the deletion process until all the \textit{pure buckets} have been marked as \textit{processed pure buckets} and no more new \textit{pure buckets} could be found. After the search stops, if each one of the $m$ buckets is either empty bucket or \textit{pure bucket}, we report decoding success. Otherwise, we report decoding failure. 
\end{comment}





\bbb{Query.} 
After a successful decoding operation, all buckets in \aname{} are either empty or processed pure, then we can perform the query operations. 
%The query operation must follow a successful decoding operation, after which all of the non-empty buckets in \aname{} are pure buckets. 
To query $\mathcal{ID}_0$, we first calculate $h_1(\mathcal{ID}_0),...,h_k(\mathcal{ID}_0)$ to get its $k$ hashed buckets. 
%all of the non-empty buckets in \aname{} are processed pure buckets.
We then perform the Fermat reduction operation on the non-empty buckets of those $k$ hashed buckets, and check whether $\mathcal{ID}_0$ equals to a reduced $\mathcal{ID}'$ from one of these buckets.
If we find a bucket whose reduced $\mathcal{ID}'$ just equals to $\mathcal{ID}_0$, we return the counter field of that bucket as the frequency $\mathcal{F}$ of $\mathcal{ID}_0$; Otherwise we think that  $\mathcal{ID}_0$ is not in \aname{}, and return zero.

\begin{figure}
    \prefig
    \includegraphics[width=0.98\linewidth]{lzr/decoding2.pdf}
    \vspace{-0.1in}
    \vspace{-0.05in}
    \caption{Decoding operation of \aname{} with $m=3$ and $k=3$.}
    \label{fig:algo:decode}
\end{figure}

%Then we search them for pure buckets, which are just non-empty bucket in this case. 
%When some non-empty bucket is found, we compare its reduced $\mathcal{ID}'$ with $\mathcal{ID}_0$. 
%If they are equal, we report query success. 

% \bbb{Example.} Below we use examples to illustrate how the \aname{} operations are performed. 

% 1) Insertion \& Deletion

% As is shown in Figure. \ref{fig:algo:insert}, 


% 2) Decoding


% \lzr{figure to show insertion and decoding operations. }

\presub
\subsection{Optimization - Overlap Verification} \postsub
%\subsection{Optimization \uppercase\expandafter{\romannumeral1} - Overlap Verification} \postsub

We find that, in practice, the false positive rate of the verification operation is very tiny. %远小于所需
%As the experimental results show, the false positive rate of the verification operation is very tiny.
Therefore, we consider making a trade-off between verification accuracy and the size of the two \textit{SumID} fields. 
%Therefore, we consider sacrificing a part of verification accuracy to lower the size of the two \textit{SumID} fields. 
By slightly degrading the decode success rate, we can significantly reduce the size of the data structure.
To achieve this, we introduce the \textbf{ID Division} technique, which divides the original 32-bit $\mathcal{ID}$ into two overlapped $r$-bit sub-$\mathcal{ID}$s, namely $\mathcal{ID}_A$ and $\mathcal{ID}_B$. 
Suppose $\mathcal{ID}_A$ is the high-order $r$ bits of an original $\mathcal{ID}$, and $\mathcal{ID}_B$ is the low-order $r$ bits of that $\mathcal{ID}$, \ie $\mathcal{ID}_A = \mathcal{ID}[31:32-r]$, $\mathcal{ID}_B = \mathcal{ID}[r-1:0]$. 
We can see that they have $l=2r-32$ overlapped bits, which are the low-order $l$ bits of $\mathcal{ID}_A$ and the high-order $l$ bits of $\mathcal{ID}_B$. 
Then we change the size of the two \textit{SumID} fields to $r+1$ bits, and let them store the modulo sum of $\mathcal{ID}_A$ and $\mathcal{ID}_B$ respectively, instead of $\mathcal{ID}$.
Accordingly, the twin primes designated to $\mathcal{ID}_A$ and $\mathcal{ID}_B$ should be less than $2^{r+1}$.
%This time, in the initialization stage, we look for the largest pair of twin primes that is less than $2^{r+1}$ instead.
According to the twin prime conjecture, no matter what number $r$ is, there are enough pairs of twin primes for us to choose in the range of $[2^r, 2^{r+1}]$. 
Finally, the Twin-ID Verification test is modified to comparing the overlapped $l$-bit of the two reduced sub-$\mathcal{ID}$s, \ie to check whether $\mathcal{ID}_A^{\prime}[l-1:0] = \mathcal{ID}_B^{\prime}[r-1:r-l]$. 
This modified verification test is called \textbf{Overlap Verification}. 

%To further optimize Overlap Verification, we modify the two sub-$\mathcal{ID}$s before inserting them to their \textit{SumID} fields. 
We do this by XORing a $r$-bit $mask$ with $\mathcal{ID}_B$. 
%We do this by (1) flipping the bit representation of $\mathcal{ID}_A$, and (2) XORing a $r$-bit $mask$ with $\mathcal{ID}_B$. 
Specifically, suppose $\mathcal{ID}_A^{*}$ is the bit reversal of the $r$-bit $\mathcal{ID}_A$, and suppose $\mathcal{ID}_B^{*}$ is the result of the $r$-bit $\mathcal{ID}_B$ XOR a $r$-bit $mask$, \ie $\mathcal{ID}_B^{*} = \mathcal{ID}_B \oplus mask$. 
This time, we let the two \textit{SumID} fields store the modulo sum of $\mathcal{ID}_A^{*}$ and $\mathcal{ID}_B^{*}$ respectively. 
Then the overlap verification naturally becomes to compare the lower $l$ bit of the bit reversal of the reduced $\mathcal{ID}_A^{\prime}$ and the upper $l$ bit of the XOR value of the reduced $\mathcal{ID}_B^{\prime}$ and $mask$. 

Note that there is a trade-off between memory usage and verification accuracy. 
Fewer overlapped bits mean more verification false positive errors, which degrades the decode success rate. 
Figure. \cite{} shows the trade-off between bit overlap and decoding success rate. 
We can see that overlap verification achieves good performance when $l \geq 8$. 
But even when $l < 8$, we can still use the rehashing verification to maintain a high decode success rate. 




% And suppose $\mathcal{ID}_B^{*}$ is the value of the lower r-bit $\mathcal{ID}$ \textbf{xor} a r-bit $mask$, \ie $\mathcal{ID}_B^{*} = \mathcal{ID}_B \oplus mask$. 

% We modify the Insertion \& Deletion operations so that the $SumID_A$ field stores the weighted sum of $ID_A$ and $F$, instead of $ID$ and $F$, and the $SumID_B$ field stores the weighted sum of $ID_B$ and $F$. 

% \lzr{figure to illustrate ID division}

% Then we propose the \bbb{Overlap Verification} test and replace the \textit{Twin-ID Verification} test in Decoding operation with it. In \textit{Overlap Verification} test, the overlapped $l$-bit of the two reduced ID is compared. For instance, consider bucket $m_0$, we compare $ID_{A}^{\prime (m_0)} [l-1:0]$ with $ID_{B}^{\prime (m_0)} [r-1:r-l] \oplus mask$. If the two compared values are not equal, bucket $m_0$ must be a \textit{non-pure bucket}. Otherwise it passes the \textit{Overlap Verification} test and we can continue to perform the \textit{Rehashing} test. 

% In our implementation, $mask$ has a 0-1 alternate pattern in its bits representation. For the case of $r=24$, we have $mask=0xaaaaaa$.

% We can also define $ID_A$ as the reversal of the upper r-bit of $ID$ and slightly modify the \textit{Overlap Verification} test by comparing the reversal of $ID_{A}^{\prime (m_0)} [r-1:r-l]$ with $ID_{B}^{\prime (m_0)} [r-1:r-l] \oplus mask$. 

% \lzr{experimental results to prove the effect of \bbb{Overlap Verification} and the \bbb{mask}?}

% \lzr{flip ID. }


% \bbb{ID Division.}%或ID Encode, ID transformation... //ID Division and ID Verification
% To adjust the ability of Verification and save memory, we introduce the \textit{ID Division} by avoiding inserting same ID to the two \textit{SumID} field.
% We divide $ID_i$ into $IDA_i$ and $IDB_i$ and store them in the idA and idB field respectively. $IDA_i$ is the higher r-bit of $ID_i$ and $IDB_i$ is calculated by XORing the lower r-bit of $ID_i$ and a mask number $m$, where $r$ and $m$ is given in advance.
% The number r determines the overlapped bits between $IDA_i$ and $IDB_i$. For example, if $ID_i$ is 32-bit long and $r$ equals 24, then $IDA_i$ and $IDB_i$ both have 8 overlapped bits.
% The number $m$ contributes to the verification of the validity of $ID_i$. In our implementation, $m$ consists of 1 and 0 arranged alternately in binary, and for $r=24$, the number $m$ is $0xaaaaaa$.


% \bbb{Delete.} The delete operation is just the reverse process of insert operation.
% To delete a key-value $<ID_i, V_i>$, similar to the insert, we calculate hashing and get $k$ hashed buckets, for each of these buckets, we perform the Fermat substract operation as stated above instead of Fermat plus.


% \bbb{Decode.} 
% Some buckets may contain multiple items, and we can not directly retrieve the items stored in these buckets. Buckets with only one item hashed into it are called \textit{pure buckets}, and it stores the original information about the items.
% We use two techniques to check whether a bucket is a pure bucket. 
% 1) rehash.\wyh{detail}
% 2) overlapped check.\wyh{detail}
% We retrieve the items in these pure buckets, and delete them from all their hashed buckets, which may transform some buckets into pure buckets. By repeat this process, we can decode the sketch with a high probability.
% The process has a hidden error recovery function. If we mistake a bucket for a pure bucket in early process and delete it, we could recover this mistake in later process with high probability. \wyh{prove this with experiment}
%关键概念加斜线？

% % 解压过程对数据结构是破坏性的，解压完后bucket中会是空的（之后修改）
% \bbb{Query.}
% After decoding, each bucket only stores one key value pair.
% To query a key $ID_i$, we calculate hash functions and get the $k$ hashed buckets to find $ID_i$.
% If found, we report the corresponding value; otherwise, we report query failed.
% %只有在这个格子只有一个元素的情况下才能成功


\subsection{SIMD accelerating}
We show how to use SIMD accelerating to speed up the decoding of \aname{}.

%#include <immintrin.h>
%void mulModSIMD1(uint64_t *a, uint64_t *b, uint64_t *c, __m512i _p, __m512d _k)
%{
%    __m512i _a = _mm512_loadu_si512((__m512i*)(a));
%    __m512i _b = _mm512_loadu_si512((__m512i*)(b));
%    __m512i _d = _mm512_mullo_epi64(_a, _b);
%    __m512d _d1=_mm512_cvtepi64_pd(_d);
%    __m512d _d2=_mm512_mul_pd(_d1, _k);
%    __m512i _e = _mm512_cvttpd_epi64(_d2); // e = int(float(d)/float(p));
%    __m512i _d3= _mm512_mullo_epi64(_e, _p);
%    __m512i _c = _mm512_sub_epi64(_d, _d3);
%    _mm512_storeu_si512((__m512i*)(c), _c);
%}
%void mulModSIMD2(uint64_t *a,uint64_t *c, __m512i _p, __m512d _k)
%{
%    __m512i _a = _mm512_loadu_si512((__m512i*)(a));
%    __m512d _d1=_mm512_cvtepi64_pd(_a);
%    __m512d _d2=_mm512_mul_pd(_d1, _k);
%     __m512i _e = _mm512_cvttpd_epi64(_d2); // e = int(float(d)/float(p));
%    __m512i _d3= _mm512_mullo_epi64(_e, _p);
%     __m512i _c = _mm512_sub_epi64(_a, _d3);
%    _mm512_storeu_si512((__m512i*)(c), _c);
%}
%void powModBatch(uint64_t *a, uint64_t b, uint64_t *c, uint64_t p)
%{
%    __m512i _p = _mm512_set1_epi64(p);
%    __m512d _k = _mm512_set1_pd(1.0d / p);
%    mulModSIMD2(a, base, _p, _k);
%    while(b)
%    {
%        if(b&1)
%            mulModSIMD1(c, base, c, _p, _k);
%        mulModSIMD1(base, base, base);
%        b>>= 1;
%    }
%}

\subsection{Filter}



\begin{comment}
\presec
\subsection{Constant Hash Tables} \postsec
\label{sec:const:hash}
\bbb{Problem Statement:}
%The hash table is an ubiquitous data structure in computer science. 
%It is used for maintaining a set $S$ under insertion and deletion of elements. 
Given an element $e$, the query operation should return the frequency of element $e$ is in set $S$ at the query time. If the element $e$ is not in Set $S$, the operation returns zero. We define the used hash table as a Constant Hash Table if the elements of set $S$ do not change after the first query operation occurs.

\bbb{Data Structure:}
A \aname{} is built to implement the function of Constant Hash Tables.

\bbb{Solutions:}
For each element $e$ in set $S$, we insert $e$ to a \aname{}. The insertion process is the same as described in Section 3. After the elements in set $S$ are fixed, the \aname{} is decoded.
%这个应该不用特别提出来，或者不用说different。另外第三节部分可能也改成这种解码法
%The decoding process is slightly different from the process described in Section 3 in that this time we does not delete the item from the pure buckets.
To query an element $e$, we check the $k$ hashed buckets of $e$. If a pure bucket containing $e$ is found, we report the count field, which is the frequency of the item.
\end{comment}



==> lzr/mathproof_fermatGroup.tex <==
\presec
\subsection{Fermat group} \postsec
\label{sec:field}
A Fermat vector is defined as the 3-tuple of $SumID_{A}$, $SumID_{B}$ and $counter$. $SumID_{A}$ and $SumID_{B}$ record the weighted sum of $ID$ and its frequency $F$, and $counter$ record the cumulative sum of the frequency $F$. 
We use $\mathbb{Z}_{p_a}$, $\mathbb{Z}_{p_b}$ and $\mathbb{Z}$ to denote the sets of all the possible values of $SumID_{A}$, $SumID_{B}$ and $counter$ respectively. To distinguish our Fermat operations from the basic arithmetic operations, we use $\hat{+}$ and $\hat{\times}$ to denote \textit{Fermat addition} and \textit{Fermat multiplication} over the two $SumID$ fields. Our Fermat operations are the modular versions of the basic arithmetic operations, that is, we have $a \hat{+} b = (a+b)\%p$ and $a \hat{\times} b = (a \times b)\% p$. 

We use $S_{fermat}$ to denote the set of all Fermat vectors:
\begin{equation*}
    S_{fermat}=\{ <a, b, c>|a\in \mathbb{Z}_{p_a} \wedge b\in \mathbb{Z}_{p_a} \wedge c\in \mathbb{Z} \}
\end{equation*}

For any $V_1=<a_1, b_1, c_1>$ and $V_2=<a_2, b_2, c_2>$ in $S_{fermat}$, the addition operation over $S_{fermat}$ is naturally defined as:
\begin{equation*}
    V_1 + V_2 = <a_1 \hat{+} a_2, b_1 \hat{+} b_2, c_1 + c_2>
\end{equation*}

In this paper, the word `field' has two meanings. Generally, we use `field' to represent a variable that can store values. But in our mathematical theorems, the word `field' refers to an algebraic structure over which addition and multiplication operations are well-defined and specific rules are met. 

$\overset{*}{+} \hat{+}$

% To distinguish the operations in these sets from the basic operations of arithmetic, we let "$+_S$" denotes the operation of addition in $S_{ida}$, $S_{idb}$ and $S_{count}$, and let "$\cdot_S$" denotes the operations of multiplication in $S_{ida}$ and $S_{idb}$.
% %对加法和乘法做定义
% Both addition and multiplication are modular versions of basic addition and multiplication in arithmetic. Generally, we have $a+_S b=(a+b)\% m$ and $a\cdot_S b=(a\cdot b)\% m$, where m is the modulus of the set. The modulus is $pa$ for $ida$, $pb$ for $idb$, and $2^r$ for a r-bit counter $count$.

% We use $S_{fermat}$ to denote the set of all Fermat vectors:
% \begin{equation*}
%     S_{fermat}=\{<a, b, c>|a\in S_{ida}\wedge b\in S_{idb}\wedge c\in S_{count}\}
% \end{equation*}
% We also define the addition in $S_{fermat}$ as follows: for any $V_1=<a_1, b_1, c_1>, V_2=<a_2, b_2, c_2>$ in $S_{fermat}$, we have
% \begin{equation*}
%     V_1+V_2=<a_1+_S a_2, b_1+_S b_2, c_1+_S c_2>
% \end{equation*}

In this paper, the word field has two meanings. Generally, we use field to represent a counter that storing numbers.
In mathematics, a field is a set with specific rules of mathematical operations like addition and multiplication.

\begin{theorem}
$S_{count}$ is an abelian group.
\end{theorem}

\begin{proof}
A abelian group is a set with an operation that satisfies the group axioms: 1) Closure; 2) Associativity; 3) Commutativity; 4) Identity element; 5) Inverse element.
%考虑引用一下与群定义有关的论文
Suppose that $count$ is a r-bit counter, then we have $S_{count}=\{a|0\leq a<2^r\wedge a\in Z\}$.
We prove that $S_{count}$ and its operation "$+_S$" satisfy each of these axioms.

\bbb{Closure:}
For all $a$, $b$ in $S_{count}$, we have
\begin{equation*}
    a+_S b=(a+b)\%2^r
\end{equation*}
which is also in $S_{count}$.

\bbb{Associativity:}
For all $a$, $b$ and $c$ in $S_{count}$, we have
\begin{equation*}\begin{aligned}
    (a+_S b)+_S c =&((a+b)\%2^r)+c)\%2^r\\
    =&(a+(b+c)\%2^r))\%2^r\\
    =&a+_S (b+_S c)
\end{aligned}\end{equation*}

\bbb{Commutativity:}
For all $a$, $b$ in $S_{count}$, we have
\begin{equation*}
    a+_S b=b+_S a
\end{equation*}

\bbb{Identity element:}
%There exists an element e in G such that, for every element a in G, the equation e • a = a • e = a holds. Such an element is unique (see below), and thus one speaks of the identity element.
$S_{count}$ has an unique identity element, 0, such that, for all $a$ in $S_{count}$, we have:
\begin{equation*}
    0+_S a=(0+a)\%2^r=a=(a+0)\%2^r=a+_S 0
\end{equation*}

\bbb{Inverse element:}
%For each a in G, there exists an element b in G, commonly denoted a−1 (or −a, if the operation is denoted "+"), such that a • b = b • a = e, where e is the identity element.
All elements in $S_{count}$ have a inverse element such that they add up to the identity element. For 0, the inverse element is itself. For all other elements $a$ in $S_{count}$, the inverse element is $2^r-a$.

In conclusion, $S_{count}$ is an abelian group.

\end{proof}



\begin{theorem}
$S_{ida}$ and $S_{idb}$ are fields.
\end{theorem}

\begin{proof}
We only prove that $ida$ is a field.

A field is a set with two operations that satisfies the field axioms: 1) Closure; 2) Associativity; 3) Commutativity; 4) Distributivity of multiplication over addition; 5)Identity element; 6) Inverse element.
We prove that $S_{ida}$ and its operation "$+_S$", "$\cdot_S$" satisfy each of these axioms.

\bbb{Closure:}
For all $a$, $b$ in $S_{ida}$, we have
\begin{equation*}\begin{aligned}
    a+_S b=&(a+b)\%pa\\
    a\cdot_S b=&(a\cdot b)\%pa
\end{aligned}\end{equation*}
which are also in $S_{ida}$.

\bbb{Associativity:}
For all $a, b$ and $c$ in $S_{ida}$, we have
\begin{equation*}\begin{aligned}
    (a+_S b)+_S c =&a+_S (b+_S c)\\
    (a\cdot_S b)\cdot_S c =&a\cdot_S (b\cdot_S c)
%(a+_S b)+_S c =&((a+b)\%2^r)+c)\%2^r\\
%=&(a+(b+c)\%2^r))\%2^r\\
%=&a+_S (b+_S c)
\end{aligned}\end{equation*}

\bbb{Commutativity:}
For all $a$, $b$ in $S_{ida}$, we have
\begin{equation*}\begin{aligned}
    a+_S b=&b+_S a\\
    a\cdot_S b=&b\cdot_S a
\end{aligned}\end{equation*}

\bbb{Distributivity of multiplication over addition:}
%a · (b + c) = (a · b) + (a · c).
For all $a, b$ and $c$ in $S_{ida}$, we have
\begin{equation*}\begin{aligned}
    a\cdot_S (b+_S c)=&a\cdot ((b+c)\%pa)\%pa\\
    =&(a\cdot b\%pa+a\cdot c\%pa)\%pa\\
    =&(a\cdot_S b)+_S(a\cdot_S c)
\end{aligned}\end{equation*}

\bbb{Identity element:}
$S_{ida}$ has an identity element for addition, 0, and an identity element for multiplication, 1, such that, for all $a$ in $S_{ida}$, we have:
\begin{equation*}\begin{aligned}
    &0+_S a=(0+a)\%pa=a=(a+0)\%pa=a+_S 0\\
    &1\cdot_S a=(1\cdot a)\%pa=a=(a\cdot 1)\%pa=a\cdot_S 1
\end{aligned}\end{equation*}

\bbb{Inverse element:}
%Additive inverses: for every a in F, there exists an element in F, denoted −a, called the additive inverse of a, such that a + (−a) = 0.
%Multiplicative inverses: for every a ≠ 0 in F, there exists an element in F, denoted by a−1 or 1/a, called the multiplicative inverse of a, such that a · a−1 = 1.

All elements in $S_{ida}$ have a inverse element for addition such that they add up to the additive identity element, 0. For 0, the inverse element is itself. For all other elements $a$ in $S_{count}$, the inverse element is $2^r-a$.

All elements in $S_{ida}$ other than 0 have a inverse element for multiplication such that their product is the multiplicative identity element, 1. For an element $a$ in $S_{ida}$ other than 0, the inverse element is $a^{pa-2}\%pa$ according to Fermat’s little theorem.

In conclusion, $S_{ida}$ is a field.
\end{proof}




\begin{theorem}
$S_{fermat}$ is a group.
\end{theorem}

\begin{proof}
Each vector field in the Fermat vector is a group over addition, thus $S_{fermat}$ and its addition also satisfies the group axioms.
In a word, $S_{fermat}$ is a group.
\end{proof}

By the definition of addition we can define the subtraction of $S_{fermat}$: to subtract a Fermat vector is to add its inverse element.
For $V_1=<a_1, b_1, c_1>, V_2=<a_2, b_2, c_2>$, we have
\begin{equation*}\begin{aligned}
&V_1-V_2=<\!(a_1-a_2+pa)\%pa,\\
&(b_1-b_2+pb)\%pb, (c_1-c_2+2^r)\%2^r\!>
\end{aligned}\end{equation*}
%    V_1-V_2=<a_1, b_1, c_1>-<a_2, b_2, c_2>\\
%    =&<a_1, b_1, c_1>+<(pa-a_2)\%pa, (pb-b_2)\%pb, (2^r-c_2)\%2^r>\\
%    =&<(a_1-a_2+pa)\%pa, (b_1-b_2+pb)\%pb, (c_1-c_2+2^r)\%2^r>
where pa, pb are the primes for $ida$ and $idb$, and r is the length of $count$.


\begin{comment}
1.	费马向量
一个费马向量包含三个域：ID、指纹、计数器。ID是元素的标识符，占用空间a比特，指纹是通过一个哈希函数F(.)计算出的指纹，占用空间b比特，计数器是一个累加值。
2.	费马加法。
给定两个费马向量<ID_1, F_1, C_1>和<ID_2, F_2, C_2>，找出费马质数P_a和P_b，费马加法的结果是<(ID_1+ID_2)%P_a，(F_1+F_2)%P_b，C_1+C_2>。
3.	费马减法。
给定两个费马向量<ID_1, F_1, C_1>和<ID_2, F_2, C_2>，找出费马质数P_a和P_b，费马减法的结果是<(ID_1-ID_2)%P_a，(F_1-F_2)%P_b，C_1-C_2>。
\end{comment}



==> lzr/mathproof_hardyConjecture.tex <==
\presec
\subsection{First Hardy-Littlewood conjecture} \postsec
\label{sec:twin}
% Twin Prime Conjecture
% We propose an guess as follows.
% The twin prime is universally distributed in binary exponential ranges.
% Binary exponential range refers to a range starting from $2^n$ to $2^{n+1}$, where $n (n>0)$ is an integer.
% Although the number of primes becomes more and more sparse with the increase of the number, the distribution of twin prime number is universal in terms of binary exponential ranges.

The First Hardy-Littlewood conjecture (named after G. H. Hardy and John Littlewood) \cite{hardy1923some} gives an accurate estimation of the distribution of twin primes. It states as follows:
As integer $n$ becomes very large, we have 
\begin{equation*}
    \pi_2(n) \approx 2C_2 \int_{2}^{n} \frac{\,dx}{(\ln x)^{2}} \approx 2C_2\frac{n}{(\ln n)^{2}}
\end{equation*}
where $\pi_2(n)$ denotes the number of primes $p$ such that $p+2$ is also prime and $p \leq x$. And $C_2$ is the \textit{twin prime constant}:
\begin{equation*}
    C_2=\prod_{prime \ p\geq 3}(\frac{p(p-2)}{(p-1)^2})=0.66016...
\end{equation*}

Based on this, for a binary exponential range starting from $2^r$ to $2^{r+1}$, the number of twin primes $B_2(r)$ is:
\begin{equation*}
    B_2(r) = 2C_2\frac{r+1}{(\ln (r+1))^{2}} - 2C_2\frac{r}{(\ln r)^{2}} \approx 2C_2\frac{2^r}{(r+1)^2}
\end{equation*}

This conjecture guarantees that enough twin primes could be found and assigned to the two $SumID$ fields of \aname{}. It has been confirmed that there are $808,675,888,577,436$ twin prime pairs below $10^{18}$ \cite{Sloane}.



==> lzr/packetloss.tex <==
\presec
\section{Packet Loss Detection} \postsec
%单链路丢包、全网丢包、割点


In this section, we discuss how to apply \aname{} to detect packet loss.
The detection of packet loss is at the core of many modern network protocols. We first describe the detection of packet loss in a single link, which we call link-level packet loss. Then we discuss the detection of packet loss in the whole networks, which we call network-level packet loss.

\presec
\subsection{Link-Level Packet Loss} \postsec

Link-level packet loss occurs between two switches, where a data stream comes from the upstream switch and goes to the downstream switch. We state the problem as follows.

%\bbb{Problem Statement:}
Given a data stream $S$, two users $u_1$ and $u_2$ are located at the top and bottom of the data stream respectively. We denote the set of packets going through the user $u_i$ as $S_i$. The task is to find the lost packets between two users, that is, the elements in set $S_1$ and not in set $S_2$.

%\bbb{Data Structure:}
%\presec
%\subsection{Solutions} \postsec
We build a \aname{} $T_i$ for each user $u_i$. All the packets going through the user $u_i$ are inserted into $T_i$ in the way described in Section \ref{sec:alg}.
%\bbb{Solutions:}
%\presec
%\subsection{Solutions} \postsec
After $T_1$ and $T_2$ are constructed, we subtract the $m$ buckets of $T_2$ from the $m$ buckets of $T_1$ respectively, the resulted \aname{} is denoted as $T_0$.
For the $idA$ and $idB$ fields, we perform Fermat subtraction operation, and for the counter field, we perform ordinary subtraction operation.
Note that $S_2\subseteq S_1$, so the resulted count field must be non-negative.
By performing the subtraction of $T_2$, we delete all packets stored in $T_2$ from $T_1$.
After subtraction, all the lost packets are stored in $T_0$. We finally decode $T_0$ and get all the lost packets.

\bbb{Optimization for Decoding.}
%可以把重叠校验去掉，解码时从频数最低的桶开始解
%可以写理论证明
%可以把相互包含的集合协调从packet loss中抽出来单独写
We can prove that if at least one pure bucket exists, then the nonempty bucket with minimum count field value must be one of them.
Based on this idea, we decode $T_0$ by repeatedly searching for the bucket with minimum count filed value and retrieving the item in this bucket.
As a result, we can stop using the Twin-ID Verification or Overlap Verification, which will save a lot of space for storing the twin-ID.


\presec
\subsection{Network-Level Packet Loss} \postsec
In network-level packet loss, we should 
%如何全网丢包
%在网络中有的交换机属于数据输入，有的交换机属于数据输出。我们建立这两者之间的，可以在最少的交换机上布置sketch以实现丢包测量
%在每条链路的上下游建立sketch，寻找丢包时直接频数相减，如果发现丢包数少，可以将做差后得到的sketch和其他链路上丢包少的做差后得到sketch相加


==> note.tex <==
1、哈希表stream summary。
2、多集合协调。

3、heavy change

问题描述：在两个相邻时间窗口中，包可以看成多重集合，目标是寻找元素频率变化大于delta的元素。
解法：
a、假设每个窗口内能得到 <元素，频数>的信息，把频数的单位模糊化，以delta-1为单位。做两个集合的差集。这样就能找到频数差异大于delta的所有元素。

b、针对a中假设，尝试构造CM sketch？好像也不一定行。

4、寻找延迟大的包。

接收端维护对应时间“0” “1” “2” 的三个费马sketch，对于0 和2 建一个BF。
期望0时间发送的包在1时间到达。
发送端的0和接收端的1算差集求延迟不正常的包。

5、丢包

==> xzc/experiment.tex <==
\presec
\subsection{Evaluation on Tower+\sketchname{}}
\postsec
\label{eval:2}
\bbb{Dataset:}
We use the anonymized IP traces collected in 2018 from CAIDA \cite{caida} as our dataset.
%
We set 5 seconds as a time window, in which exists about 2.3M packets with about 63K flows(using 32-bit srcIP as flow ID).
\bbb{Tasks:}
We use Tower+\sketchname{} to complete 6 measurement tasks which have been extensively studied.
\item\texit{Flow size(FS) estimation:}
We estimate the flow size for each flow ID. In order to analyse performance of different algorithms clearly, we divide all the flows into three groups by flow size. The flows whose size is below 50 are assigned to the small flows group, the flows whose size is between 50 and 250 are assigned to the medium flows group, while the rest flows are assigned to the heavy flows group. We evaluate the performance of flow size estimation of each algorithm on these three groups respectively.
\item\texit{Heavy hitter(HH) detection:}
Heavy hitters, to which previous studies have attached great importance, are the flows whose sizes surpass a predefined threshold. This task required algorithms to report heavy hitters precisely and as many as possible. In our experiment, we set the threshold at 500, which is about $0.02\%$ of the number of total packets within a time window.
\item\texit{Heavy change(HC) detection:}
A flow is reported as a heavy change flow if its flow size changes more than a predefined threshold in two adjacent time windows. Here we set the threshold at 250.
\item\texit{Flow size distribution(FSD) estimation:}
This task is to estimate the distribution of flow sizes.
\item\texit{entropy estimation:}
This task is to estimate the entropy of flow sizes.
\item\texit{Cardinality estimation:}
This task is to estimate the number of flows in a time window.
\bbb{Metrics:}
\item\textit{ARE(Average Relative Error):}
$\frac{1}{n}\sum_{i=1}^{n}\frac{|f_i-\hat{f_i}|}{f_i}$, where $n$ is the number of flows, $f_i$ is the actual flow size and $\hat{f_i}$ is the estimated flow size. We use ARE to evaluate the flow size estimation task.
\item\textit{AAE(Average Absolute Error):}
$\frac{1}{n}\sum+{i=1}^{n}|f_i-\hat{f_i}|$. We use AAE to evaluate the flow size estimation task.
\item\textit{F1 score:}
$\frac{2\times PR\times RR}{PR + RR}$, where $PR$(Precision Rate) represents the ratio of true positives to the total of true positives and false positives while $RR$(Recall Rate) represents the ratio of true true positives to the total of true positives and false negatives. We use F1 score to evaluate the heavy hitter(HH) detection and heavy change(HC) detection tasks.
\item\textit{WMRE(Weighted Mean Relative Error):}
$\frac{\sum_{i=1}^{z}|n_i - \hat{n_i}|}{\sum_{i=1}^{z}(\frac{n_i + \hat{n_i}}{2})}$, where z is the maximum of flow size, while $n_i$ and $\hat{n_i}$ represent the number of true and estimate flows of size i respectively. We use WMRE to evaluate the the flow size distribution(FSD) estimation task.
\item\textit{RE(Relative Error):}
$\frac{|t - e|}{t}$, where $t$ and $e$ respectively represents the true and estimate value. We use RE to evaluate the accuracy of entropy estimation and cardinality estimation tasks.

\bbb{Setup:}
We compare Tower+\sketchname{} with several prior algorithms for six tasks. The details of these algorithms are as below:
\item\textit{Tower+\sketchname{}:} 
We set that a flow will insert to the \sketchname{} part if its reported size in Tower part exceeds 250, which is the threshold of heavy change detection, in order to report all the flow IDs that may matters. We allocate 2500 buckets to the \sketchname{} part which is plenty to make the possibility of decoding successfully high enough. As for the Tower part, we use a 8-bit layer and a 16-bit layer. We use it to complete all the six measurement tasks.
\item\textit{ElasticSketch\cite{elastic2018}:} 
We use the hardware version of ElasticSketch to complete the six tasks. For the heavy part, we use 4 stages, and each stage has 3072 buckets. For the light part, we use a 8-bit layer.
\item\textit{FCMSketch:}
We use the FCM+TopK version of FCMSketch. For the TopK part, we use the same data structure and parameters as the heavy part of ElasticSketch. For the FCM part, we use 16-ary version and set the depth to 2 as recommended. We use it to complete all the six tasks.
\item\textit{UnivMon\cite{univmon2016}}
We use UnivMon to complete HH detection, HC detection, entropy estimation and cardinality estimation. We use 14 levels and each level can record 1000 heavy hitters. 
\item\textit{Hashpipe\cite{sivaraman2017heavy}}
We use Hashpipe to detect heavy hitters. 
\item\textit{CocoSketch\cite{zhang2021cocosketch}}
We use CocoSketch to detect heavy hitters. We use 1 hash function.
\item\textit{CMSketch\cite{cmsketch}}
We use CMSketch to estimate flow sizes. We use 3 hash functions as recommended in \cite{cmsketch}.
\item\textit{CUSketch\cite{cusketch}}
We use 3 hash functions for CUSketch to estimate flow size.
\item\textit{CountSketch with a heap(CountHeap)\cite{countsketch}}
We use 3 hash functions and set the heap capacity to 4096. We use it to detect heavy hitters and heavy changes.
\item\textit{MRAC}
We use MRAC to estimate flow size distribution.

\bbb{Accuracy:}
Figure *** shows the accuracy of algorithms above on six tasks. We test the performance of each algorithm and each task with memory ranges from 200KB to 1000KB.
\textit{Flow size estimation(Figure **):}
We find that Tower+\sketchname{} has a evident lower AAE when comparing to CM, CU, Elastic and FCM.  We analysis ARE on small, medium and heavy flows and find that Tower+\sketchname{} performs well on each group.

\textit{Heavy hitter detection(Figure **):}
We find that Tower+\sketchname{} always achieves above $99.8\%$ F1 score, which is close to HashPipe. When comparing to algorithms that can measure multiple tasks, Tower+\sketchname{} performs much better.
\textit{Heavy change detection(Figure **):}
We find that Tower+\sketchname{} achieves above $99.6\%$ F1 score when using 400KB memory, while the F1 score of the other algorithms is below $99.0\%$ even when using 1000KB memory.
\textit{Flow size distribution(Figure **):}
We find that Tower+\sketchname{} has a lower WMRE than Elastic and FCM, especially when the memory is lager or equal than 800KB, and performs no worse than MRAC.
\textit{Entropy estimation(Figure **):}
We find that Tower+\sketchname{} performs no worse than Elastic and FCM, and much better than UnivMon.
\textit{Cardinality estimation(Figure **):}
We find that Tower+\sketchname{} has the lowest RE, which is at least 10 times lower than the other algorithms.


==> xzc/pseucode.tex <==
%insertion algorithm
\begin{algorithm}[h!]
\renewcommand\baselinestretch{0.9}\selectfont
    \caption{Insertion of Fermat.}
 \label{alg:insert}
 \KwIn{Flow ID $f$}
 \For {$i \in [1, d]$}
 {
     $pos$=H_i($$f$$);\\
     Bucket[$i$][$pos$].ID=(Bucket[$i$][$pos$].ID+$f$)\%PRIME;\\
     Bucket[$i$][$pos$].count++;
 }
\end{algorithm}


%decode algorithm
\begin{algorithm}[h!]
\renewcommand\baselinestretch{0.9}\selectfont
    \caption{FlowDecode}
\label{alg:decode}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{FIsPure}{IsPure}
\SetKwFunction{FDelete}{Delete}
\SetKwFunction{FDecode}{Decode}
\Fn{\FIsPure{$bucket, row, column$}}
{
    $f$=$bucket$.count^{\rm {(PRIME - 2)}}\% \rm{PRIME};\\
    \KwRet column==H_{row}($$f$$);\\
}
~\\
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FDelete{$bucket$, $purebucket$}}
{
    $bucket$.count-=$purebucket$.count;\\
    $bucket$.ID=($bucket$.ID$-purebucket$.ID)\%PRIME;\\
}\\
~\\
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FDecode{}}{
    \tcc{$Candidate$ is a empty queue to take down the buckets which are pure, while $result$ is a map to take down flow IDs and sizes.}
    \For{$\all b \in $\rm Bucket}{
        \If{\FIsPure{b}}{
            $Candidate$.\rm push(b);
        }
    }
    \While{\rm!$Candidate.$\rm empty()}{
    $b$=$Candidate$.front();\\
    $Candidate$.pop();\\
    $result$[$b$.ID]+=$b.$count;\\
    \For{b' \rm mapped by $b.$ID \&\& $b'$!=$b$}{
        \FDelete($b', b$);\\
        \If{\FIsPure{b'}}{
            $Candidate$.push($b'$);
        }
        \FDelete($b, b$);
    }
    }
    \Return{reusult}
}
\end{algorithm}
